Jarvis: Large-scale Server Monitoring with Adaptive Near-data Processing

Rapid detection and mitigation of issues that impact performance and reliability is paramount for large-scale online services. For real-time detection of such issues, datacenter operators use a stream processor and analyze streams of monitoring data collected from servers (referred to as data source nodes) and their hosted services. The timely processing of incoming streams requires the network to transfer massive amounts of data, and significant compute resources to process it. These factors often create bottlenecks for stream analytics. To help overcome these bottlenecks, current monitoring systems employ near-data processing by either computing an optimal query partition based on a cost model or using model-agnostic heuristics. Optimal partitioning is computationally expensive, while model-agnostic heuristics are iterative and search over a large solution space. We combine these approaches by using model-agnostic heuristics to improve the partitioning solution from a model-based heuristic. Moreover, current systems use operator-level partitioning: if a data source does not have sufficient resources to execute an operator on all records, the operator is executed only on the stream processor. Instead, we perform data-level partitioning, i.e., we allow an operator to be executed both on a stream processor and data sources. We implement our algorithm in a system called Jarvis, which enables quick adaptation to dynamic resource conditions. Our evaluation on a diverse set of monitoring workloads suggests that Jarvis converges to a stable query partition within seconds of a change in node resource conditions. Compared to current partitioning strategies, Jarvis handles up to 75% more data sources while improving throughput in resource-constrained scenarios by 1.2-4.4x.

==> Paper.tex <==
% \RequirePackage[2020-02-02]{latexrelease}
% \documentclass[conference]{IEEEtran}
% \input{header}

% % \IEEEoverridecommandlockouts
% % % The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
% \usepackage{cite}
% % \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{comment}

% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% \begin{document}

% \title{Jarvis: Large-scale Server Monitoring with\\ Adaptive Near-data Processing}


% % \author{

% % \IEEEauthorblockN{Atul Sandur} \IEEEauthorblockA{\textit{UIUC}}
% % %\email{gangmuk@unist.ac.kr}
% % \and

% % \IEEEauthorblockN{ChanHo Park} \IEEEauthorblockA{\textit{UNIST}}
% % %\email{}
% % \and

% % \IEEEauthorblockN{Stavros Volos} \IEEEauthorblockA{\textit{Microsoft
% % Research}}
% % %\email{}
% % \and

% % \IEEEauthorblockN{Gul Agha} \IEEEauthorblockA{\textit{UIUC}}
% % %\email{}
% % \and

% % \IEEEauthorblockN{Myeongjae Jeon} \IEEEauthorblockA{\textit{UNIST}}
% % %\email{mjjeon@unist.ac.kr}
% % }

% \author{\IEEEauthorblockN{Atul Sandur\IEEEauthorrefmark{1}, ChanHo Park\IEEEauthorrefmark{2}, Stavros Volos\IEEEauthorrefmark{3}, Gul Agha\IEEEauthorrefmark{1}, Myeongjae Jeon\IEEEauthorrefmark{2}}
% \IEEEauthorblockA{\IEEEauthorrefmark{1}University of Illinois at Urbana-Champaign~~ \IEEEauthorrefmark{3}Microsoft Research~~
% \IEEEauthorrefmark{2}UNIST}}

% % \author{\IEEEauthorblockN{Atul Sandur\IEEEauthorrefmark{1}, ChanHo Park\IEEEauthorrefmark{2}, Stavros Volos\IEEEauthorrefmark{3}, Gul Agha\IEEEauthorrefmark{1}, Myeongjae Jeon\IEEEauthorrefmark{2}}
% % \IEEEauthorblockA{\IEEEauthorrefmark{1}
% % University of Illinois at Urbana-Champaign, Illinois, USA. Emails: \{sandur2,agha\}@illinois.edu\\
% % \IEEEauthorrefmark{2}UNIST, South Korea. Emails: \{pch8286,mjjeon\}@unist.ac.kr\\
% % \IEEEauthorrefmark{3}Microsoft Research, UK. Email: svolos@microsoft.com}}
% %% \author{Anonymous author(s)}

% \maketitle
% % \thispagestyle{plain}
% % \pagestyle{plain}

% \input{sections/abstract}
% \input{sections/introduction}
% \input{sections/background-motivation}
% \input{sections/insight}
% \input{sections/design}
% \input{sections/implementation}
% \input{sections/evaluation}
% \input{sections/related}

% \section{Conclusion}% \& Future Work}
% We presented \ours{}, a fully decentralized data-level query partitioning engine for server monitoring systems. Our analysis using real-world monitoring query workloads suggests that \ours{} substantially improves system throughput while quickly adapting to changes in resource conditions. 
% % \ours{} code is available open source at \url{https://omnia-git.unist.ac.kr/omnia_projects/jarvis/jarvis}.
% % ~\cite{jarvis-code}.
% % \ours{} is open-sourced and available at \url{https://omnia-git.unist.ac.kr/omnia_projects/jarvis/jarvis}.
% % \url{https://doi.org/10.5281/zenodo.5120492}.
% % changes within seconds
 
% \section{Acknowledgements}
% % \small{
% We thank the anonymous reviewers, Ruoyu Sun and Niao He from UIUC for their feedback and comments. This work was supported in part by the National Science Foundation under Grant No. SHF 1617401, and in part by the Laboratory Directed Research and Development program at Sandia National Laboratories, a multi-mission laboratory managed and operated by National Technology and Engineering Solutions of Sandia, LLC, a wholly owned subsidiary of Honeywell International, Inc., for the U.S. Department of Energy’s National Nuclear Security Administration under contract DE-NA0003525, the 2018 Research Fund (1.180079.01) of UNIST(Ulsan National Institute of Science \& Technology), and Samsung Data \& Information Technology Center.
% % }
% %Institute of Information \& Communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2020-0-01336, Artificial Intelligence Graduate School Program (UNIST)).

% % , Karthik Chandrasekaran, Niao He
% % , Kirill Mechitov, Dan Plyukhin, Dipayan Mukherjee and Jeongyoon Eo
% \bibliographystyle{IEEEtran}
% % \bibliographystyle{ACM-Reference-Format}
% % \bibliography{\jobname}
% % \bibliography{references}
% \bibliography{Paper}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{document}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> archive/background-motivation-v1.tex <==
\section{Background \& Motivation}
%\vspace{-0.15cm}
In this section, we describe 
%the monitoring system targeted by our work. We showcase 
challenges in building efficient large-scale monitoring systems and uncover insights for designing such systems by characterizing the resource usage of query operators for a real-world enterprise workload.

\subsection{Monitoring System}
\label{sec:background}
Although numerous useful scenarios correspond to large-scale server monitoring~\cite{helios,deepview,fingerprint}, here we describe two scenarios that guide the design of \ours{}:

\begin{myitemize}
\item \textit{Scenario 1:} Network team deploys Pingmesh~\cite{pingmesh} agents on datacenter nodes to collect  latency data between server pairs. An internal web search team uses Pingmesh to monitor network health of their latency-sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold as determined by the search service SLA.
 
\item \textit{Scenario 2:} A log processing system, Helios~\cite{helios}, enables live debugging of storage analytics services such as Cosmos~\cite{cosmos}. A bug in cluster resource manager leads to service resources being under-provisioned. To temporarily mitigate performance degradation, several TBs of log streams~\cite{helios} are processed quickly to identify impacted tenants. Their latency and CPU/memory utilization data are queried to predict resource needs and make scaling decisions.
\end{myitemize}

Processing in these scenarios requires a diverse set of operations. The first scenario requires processing of periodically generated metrics composed of structured numerical data; queries consist of common computations specific to numerical data, such as filtering and aggregation. On the contrary, the second scenario requires processing of aperiodically generated logs composed of unstructured strings; queries accompany computations for string processing such as parsing, splitting, and search. 

%Moreover, resource usage for these operators is diverse, varies significantly, and  depends on the operator logic and the input data. We consider a common set of operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. 
Moreover, these operations are computationally different and their costs are highly dynamic depending on the input data. To illustrate, let us consider a common set of primitive operators such as Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. Filter (stateless operator) drops uninteresting records by applying the predicates on each record and typically requires little amount of compute resource. Grouping (stateful operator) organizes records by key fields, and hence requires key lookups in hash tables. Join (stateful operator) joins an input stream with a static table on \client{}, which typically requires key lookups on the static table while joining the two inputs into a new output stream.
%which typically requires building a hash table over the static table followed by key lookups for the input stream.
%\footnote{Due to limitations in \client{}-side execution discussed in Section~\ref{sec:jarvis}, we do not consider other complex join operators.} 
Contrary to filter, both grouping and join operators can be quite expensive due to the irregular compute patterns of hash table lookups. Their cost highly depends on the hash table size, which corresponds to the group count and the static table size, respectively. Map operator performs user-defined transformations on the input (e.g., parsing and splitting text logs) and its cost depends on the transformation logic. We present a quantitative analysis of resource usage characteristics of these operators in~\cite{jarvis-extended}. 

\Paragraph{Illustrative example.} For the remaining section, we consider a real-world query on Microsoft's \pingmesh{} trace to highlight challenges in designing large-scale monitoring systems. \pingmesh{} measures network latency for server pairs across the datacenter, by requiring that each server send probe messages to its peer servers in the datacenter. Each probe message generates a 86B record that includes timestamp (8B), source IP address (4B), source cluster ID (4B), destination IP address (4B), destination cluster ID (4B), round trip time in microseconds (us) (4B), and error code (4B). %The round trip time is in microseconds.

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{DAG of stream operations for the query in Listing~\ref{lst:motivating-query}.}
    \label{fig:pipeline_tor}
    \vspace{-0.4cm}
\end{figure}

This rich set of record fields allows exhaustive analyses, such as zoom-in/out latency probes by grouping them across datacenter network hierarchy to identify cluster-, ToR-, spine switch-, and server-level issues  ~\cite{tersecades, pingmesh}. Listing~\ref{lst:motivating-query} describes the implementation of a real-world \pingmesh{} query for latency probing among server pairs. The query is written in a declarative programming model used by popular stream engines, such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming}, which express a query using dataflow operations. 

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}


\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}


A monitoring query can be represented as a directed acyclic graph (DAG) $G = (V,E)$. In a DAG, the vertices V denote stream operations which transform their input records and emit output records to downstream operation, and the edges $E$ denote dataflow dependencies between operations. Subsequently, in Figure~\ref{fig:pipeline_tor}, we show a simple DAG of how data flows between operations for the query in Listing~\ref{lst:motivating-query}.


\subsection{A Case for Adaptive Partitioning in Query Engines}
\label{sec:motivation}

\Paragraph{Hierarchical query engines.} Physical resources involved in the query execution can be seen as a tree structure as shown in Figure~\ref{fig:arch-monitoring-scale}(b), where leaf nodes represent the \client{}s. In each leaf node, fixed amount of compute resources are allocated to facilitate monitoring queries. Such allocation can be done by provisioning a container to isolate the monitoring resources (e.g., 1 or 2 cores and 1 GB RAM) from foreground services. Each \client{} can send data to its parent \server{} node (i.e., intermediate node) and leverage its compute resources for query processing. The intermediate nodes send data to the root \server{} node which completes the query before outputting final result.

\Paragraph{Query partitioning.} 
%Real-world monitoring scenarios exhibit \textit{high traffic volume}~\cite{chi, gandalf, m3}.
%Logs collected from applications can generate up to 971 Gbps~\cite{chi}. Other systems~\cite{gandalf,m3} process up to tens of TB data per day or millions of events every second per monitoring task, straining compute, memory, and network capacities of the monitoring system. 
We corroborate existing real-world monitoring scenarios with \textit{high traffic volume}~\cite{chi, gandalf, m3} by quantifying the volume of data transferred over the network in the \pingmesh{} scenario. Assuming that a datacenter consists of 200K servers and each server probes 20K other servers with a probing interval of 5 seconds ~\cite{pingmesh}, the data generation rate is estimated to be 512.6~Gbps. Similar to~\cite{chi, gandalf, m3}, transferring such high volumes of data would strain network capacity and incur high deployment cost of compute resources in the \server{}.  

As introduced before, query partitioning is an effective approach to alleviate network bottlenecks and reduce deployment cost by pushing a subset of the query's execution closer to the \client{} to leverage available its compute resources. Specifically, given a query DAG with $M$ operations, an operator-level partitioning plan identifies operations that can execute locally on each \client{} and those that require remote execution on the \server{}. This requires a boundary operator $b_i$ to be defined for \client{} $i$ to indicate that operators prior to $b_i$ along with $b_i$ in the topological order of the DAG are executed on \client{} and those after $b_i$ are executed remotely. 
%To illustrate, consider a topologically sorted list of $M$ operators from the query graph $G$ following dataflow dependencies of the query. 
For instance, for a \client{} $i$ with $M=4$ operators, $b_i=3$ implies that the first three operators execute on \client{} and the last operator executes remotely.

\Paragraph{Adaptive query partitioning.} Resource conditions can change dramatically across \client{}s and time due to high variability in the generation of monitoring data \cite{chi,helios} affecting the effectiveness of a query partitioning plan. In our running example, we also observe that data source nodes generate highly variable data rates and distributions as follows:

\begin{myitemize}
\item A subset of servers probe a larger set of peers to cover a wider network range on behalf of other servers in the same ToR switch~\cite{pingmesh}. We measure data rates of network probe messages generated by individual \client{}s, illustrated in  Figure~\ref{fig:data-gen-rate}. The data rates are normalized to the highest one observed among \client{} nodes. Data generation rates exhibit high variability, with 58\% of nodes generating 50\% or lower of the highest data rate we observe.
\item When a subset of servers are being over-loaded, latency profiles of these servers become more variable~\cite{rubik, pegasus}. Hence, each of these data source nodes will generate a unique data footprint, which is quite different than the average data source node that does not encounter any abnormality.
\end{myitemize}

The data variability complicates resource usage characteristics of query operators during query execution. 
%Declarative operators in a pipeline execute in sequence as shown in Figure~\ref{fig:pipeline_tor}. 
The primary reason is that resource demand for an operator in a DAG is affected by its incoming data rate after executing all preceding operators. In Figure~\ref{fig:pipeline_tor}, F operator leads to the first data volume reduction from the input stream. Since erroneous, insignificant records are usually not dominant, the operator happens to drop only a small fraction of records. A majority of records are then to be processed by G+R operator, increasing compute cost for the query. However, if we were to have network issues for inbound or outbound traffic for some servers, generating a large proportion of erroneous data,
%toggle the filtering predicates to perform a zoom-in analysis on a small subset of erroneous data, 
those servers will experience a high degree of data reduction in F operator, thus lowering resource usage of the G+R operator.

As a consequence, when resource conditions change on a \client{} node, a new partitioning plan needs to be identified so that its compute demands meet available resource budget. To initiate refinement, \client{}s periodically inject \emph{refinement watermarks} into the stream (similar to~\cite{trill}) and they
delimit ordered consecutive \emph{refinement epochs} of records. 
%Refinement watermarks are different from the traditional watermark described in data model. 
For brevity, epoch and watermark refer to refinement epoch and refinement watermark respectively in the rest of the paper.

\Paragraph{Computation efficiency of optimal adaptation.} Given the network and compute resources available on \server{}, we seek to maximize the number of \client{}s that can be served. Thus, the optimization goal of query partitioning is to identify the boundary operator $b_i$ for each \client{} $i$, such that the processing load sent to \server{} is minimized, subject to local computation not increasing overall processing time of each data stream, compared to remote execution. This is a NP-hard problem and computationally difficult to solve: we present a formal definition and proof in~\cite{jarvis-extended}.

\begin{figure}[t]
  \centering
    \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
    \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
    \label{fig:data-gen-rate}
    \vspace{-0.4cm}
\end{figure}

\subsection{Insights for Designing Jarvis}
\label{sec:drawbacks}

%We highlight the drawbacks of state-of-the-art approaches in addressing the operator-level partitioning problem as well as uncover insights for designing \ours{}.

%\Paragraph{Drawback 1: Coarse-grained partitioning can significantly
%under-subscribe \client{} node resources.} State-of-the-art monitoring systems~\cite{everflow,
%sonata, dshark} have explored coarse-grained partitioning strategies---i.e., either all records are processed by an operator or none. 
\Paragraph{Data-level query partitioning.}
Operator-level query partitioning could be undesirable when attempting to run a computationally expensive operator like grouping within limited compute resources provided by \client{}, because it could over-subscribe available resources. However, the alternative is for the partitioning mechanism to leave the resource highly underutilized.
To highlight this issue concretely, we execute the query in
Figure~\ref{fig:pipeline_tor} using 80\% of single core operating at 2.4GHz, which reflects
compute constraints on \client{}. The upper part of Figure~\ref{fig:data-partition-explain}
shows the resulting resource usage statistics in detail among the operators. 
Because F operator drops only a small portion of input records, it is not
possible to execute the expensive G+R operator entirely on \client{}. This leads to
under-utilization of the available compute resources and generation of network traffic as high as 22.5 Mbps, which is close to the input rate to the query.

\begin{figure}[t]
\centering

\includegraphics[width=\linewidth]{fig/DataPartitionExplain.pdf}
%\vspace{-0.1in}
\caption{\label{fig:data-partition-explain} Coarse-grained operator-level vs. fine-grained data-level partitioning on \client{} with 80\% CPU budget. G+R requires 80\% CPU to process all output data from F operator.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

On the contrary, extending the operator-level partitioning model to support \datapart{} could significantly improve the utilization of limited compute resources on \client{}.
This fine-grained \datapart{} allows an operator to process a fraction of its input records on \client{} and drain the rest for remote processing. With this approach, as shown in the lower part of Figure~\ref{fig:data-partition-explain}, the operator G+R in the query can process 83\% of its input, resulting in total network traffic of 9.4 Mbps. Note that this traffic amount is 2.4x lower than the traffic generated by the coarser-grained operator-level partitioning strategy.

%\noindent \underline{Insight 1:} \emph{Extending the operator-level partitioning model to support data-level partitioning significantly improves the utilization of limited compute available on \client{} nodes.}



\Paragraph{Drawback 2: Without fast \& accurate adaptation, partitioning approaches cannot keep up with highly dynamic resource conditions on \client{}s.}
The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently the available compute per-query. Given these dynamics, query planners need to compute and execute a new partitioning plan in a timely manner, even in seconds.

While optimal partitioning can be achieved using a query cost model \& centralized planner to leverage global information about available resources~\cite{sonata,ds2,optimal-odp},  it is computationally expensive due to high algorithmic complexity (NP-hard~\cite{jarvis-extended}). Other cost model-based query planners have been explored in literature without considering partitioning under highly variable \client{} resource conditions~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (Section~\ref{sec:RelatedWork}). 
Furthermore, a greedy approach which relies solely on optimizing for a cost model may output an incorrect partitioning decision as the model may not accurately capture complex query execution behavior~\cite{model-free-control-drl}.
% , potentially leading to inaccurate partitioning decisions.  
% Furthermore, it may not be feasible to obtain accurate performance models at runtime.

\noindent \underline{Insight 2:} \emph{A greedy \& embarrassingly parallel heuristic utilizing a combination of cost model-based \& model-agnostic techniques enables fast, accurate and fully decentralized query refinement on each \client{}.}


% Prior work relies on centralized query planners that leverage global information about available resources to solve an expensive optimization function~\cite{sonata} and on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Optimal partitioning is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach for partitioning. Other centralized and decentralized query planners have also explored model-free and model-based approaches but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}). 
%\ours{} investigates a greedy and embarrassingly parallel approach which uses hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}. 
%dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs. 
% \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}
% A greedy and embarrassingly parallel approach utilizing a hybrid performance model-based and model-agnostic technique can enable fast and fully decentralized query refinement on each \client{}, which is accurate, robust and scalable and automatic.

==> archive/background-motivation-v2.tex <==
\section{Background \& Motivation}
%\vspace{-0.15cm}
%In this section, we
%%describe
%%the monitoring system targeted by our work. We showcase
%%challenges in building efficient large-scale monitoring systems and
%uncover insights for designing efficient large-scale monitoring systems by
%characterizing the resource usage of a real-world enterprise workload.

In this section, we explain the background and motivation of our work by
referring to real-world enterprise workloads.

\subsection{Monitoring Systems Overview}
\label{sec:background}

Although numerous useful scenarios correspond to large-scale server monitoring~\cite{helios,deepview,fingerprint}, here we describe two common scenarios that guide the design of \ours{}:

\begin{myitemize}

\newcontent{\item \textit{Scenario 1:} Pingmesh~\cite{pingmesh} agents are deployed to datacenter nodes to collect latency data between servers. A web search team uses Pingmesh to monitor network health of their latency-sensitive service and generate an alert if more than a predefined proportion of nodes (e.g., 1\%) have probe latencies exceeding a threshold (e.g., 5~ms)~\cite{pingmesh}.}
% \item \textit{Scenario 1:} Network team deploys Pingmesh~\cite{pingmesh} agents on datacenter nodes to collect  latency data between server pairs. An internal web search team uses Pingmesh to monitor network health of their latency-sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold as determined by the search service SLA.

\item \textit{Scenario 2:} A log processing system, Helios~\cite{helios},
    enables live debugging of storage analytics services such as
    Cosmos~\cite{cosmos}. A bug in cluster resource manager may lead to service
    resources being under-provisioned. To temporarily mitigate performance
    degradation, several TBs of log streams~\cite{helios} are processed
    quickly to identify impacted tenants. Their latency and CPU/memory
    utilization data are queried to predict resource needs and make scaling
    decisions.
\end{myitemize}

%Processing in these scenarios requires a diverse set of operations.
There scenarios rely on a diverse set of computations. Scenario 1 requires
processing of periodically generated metrics composed of structured numerical
data; queries consist of computations specific to numerical data, such as
filtering and aggregation. On the contrary, Scenario 2 requires processing of
aperiodically generated logs composed of unstructured strings; queries
accompany computations for string processing such as parsing, splitting, and
search.

%Moreover, resource usage for these operators is diverse, varies significantly, and  depends on the operator logic and the input data. We consider a common set of operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}.
%Moreover, these operations are computationally different and their costs are
%highly dynamic depending on the input data.
%To illustrate, let us consider a common set of primitive operators such as
%Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and
%Map(M)~\cite{streamboxhbm,trill,flink}.

Moreover, these computations rely on various primitive operators, which are
computationally different and whose costs are highly dynamic depending on the
input data. For example, filter (F) drops uninteresting records by applying
the predicates on each record and typically requires little amount of compute
resource. Grouping (G) organizes records by key fields and hence requires key
lookups in hash tables. Join (J) joins an input stream with a static table,
which typically requires key lookups on the table while joining the two
inputs into a new output stream~\cite{tersecades}.
%which typically requires building a hash table over the static table followed by key lookups for the input stream.
%\footnote{Due to limitations in \client{}-side execution discussed in Section~\ref{sec:jarvis}, we do not consider other complex join operators.}
Contrary to filter, both grouping and join operators can be expensive due to
the irregular compute patterns of hash table lookups. Their cost highly
depends on the hash table size, which corresponds to the group count and the
static table size, respectively. Map (M) performs user-defined
transformations on the input (e.g., parsing and splitting text logs) and its
cost depends on the transformation logic. We present a quantitative analysis
of resource usage characteristics of these operators
in~\cite{jarvis-extended}.

\Paragraph{Hierarchical query engines.} Physical resources involved in the
monitoring query execution can be viewed as a \emph{tree structure} as shown
in Figure~\ref{fig:arch-monitoring-scale}(b), where leaf nodes represent the
\client{}s and the other nodes represent the \server{}. In each leaf node,
fixed amount of compute resources are allocated to facilitate monitoring
queries. Such allocation must
%can be done by provisioning a container to
isolate the monitoring resources (e.g., 1 or 2 cores and 1 GB RAM) from
foreground services. Each \client{} sends data to its parent (intermediate)
node, where we can leverage compute resources for query processing. The
intermediate nodes relay data to the root \server{} node, which completes the
query and outputs the final result.

\Paragraph{Illustrative example.} We consider a
real-world query on Microsoft's \pingmesh{} trace as an illustrative example to highlight challenges in
designing large-scale monitoring systems. \pingmesh{} measures network
latency for server pairs across the datacenter, by requiring that each server
send probe messages to its peer servers in the datacenter. Each probe message
generates a 86B record that includes timestamp (8B), source IP address (4B),
source cluster ID (4B), destination IP address (4B), destination cluster ID
(4B), round trip time in microseconds (us) (4B), and error code (4B).
%The round trip time is in microseconds.

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{DAG of stream operations for the query in Listing~\ref{lst:motivating-query}.}
    \label{fig:pipeline_tor}
    \vspace{-0.5cm}
\end{figure}

The Pingmesh trace allows exhaustive analyses
%, such as zoom-in/out latency probes
by grouping latency probes across datacenter network hierarchy and
identifying cluster-, ToR-, and server-level issues ~\cite{tersecades,
pingmesh}. Listing~\ref{lst:motivating-query} describes the implementation of
a real-world \pingmesh{} query for latency probing among server pairs. The
query is written in a declarative programming model used by popular stream
engines, such as Flink~\cite{flink} and Spark
Streaming~\cite{sparkstreaming}, which express a query using dataflow
operations.

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}

\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}

%Real-world monitoring scenarios exhibit \textit{high traffic volume}~\cite{chi, gandalf, m3}.
%Logs collected from applications can generate up to 971 Gbps~\cite{chi}. Other systems~\cite{gandalf,m3} process up to tens of TB data per day or millions of events every second per monitoring task, straining compute, memory, and network capacities of the monitoring system.

\subsection{Monitoring pipeline characteristics}
\label{sec:motivation}
\Paragraph{High data volume.} We corroborate existing real-world monitoring scenarios with \textit{high
traffic volume}~\cite{chi, gandalf, m3} by quantifying the volume of data
transferred over the network in the \pingmesh{} scenario. Assuming that a
datacenter consists of 200K servers and each server probes 20K other servers
with a probing interval of 5 seconds ~\cite{pingmesh}, the data generation
rate is estimated to be 512.6~Gbps. Transferring such high volumes of data
would strain network capacity and incur high deployment cost of compute
resources in the \server{}.

\Paragraph{Variability in resource conditions.} \newcontent{An effective approach to consider for alleviating network bottlenecks due to high traffic volumes is to process data closer to the \client{} and reduce its size before network transfer. We refer to the pushing of a subset of the query's execution workload closer to the source as \emph{query partitioning}.

Monitoring queries typically permit incremental data processing and lead to data size reduction. But executing the entire query on each \client{} node is not always feasible given the limited compute allocated for monitoring workloads. Thus, we need to carefully consider the compute-communication tradeoff involved in pushing query operations closer to the \client{}. These decisions need to be made in an online manner to account for changes in the resource conditions on each \client{} node.

High temporal variability in available compute is caused by changing compute demands of the server node's foreground services. E.g., real world traces from large scale web services like Alibaba~\cite{alibaba-bursty-workload}, Wikipedia~\cite{wikipedia-bursty-workload} and ML-based predictive analytics services for speech and vision~\cite{barista-predictive-analytics,mark-ml-inference-atc} show bursty request rates requiring variable compute needs in the order of minutes to meet service SLA. Such variability requires making fast query partitioning decisions at runtime on each \client{}.
Furthermore, input data affects compute demands of monitoring queries which exhibit high temporal (i.e., on each \client{}) and spatial (i.e., across \client{}s) variability. We look at the factors that affect query compute demands:}

% High temporal (i.e., on each \client{}) and spatial (i.e., across \client{}s) variability in resource conditions can be observed in monitoring pipelines.

% generation of monitoring data \cite{chi,helios} affecting the effectiveness of a query partitioning plan. In our running example, we also observe that data source nodes generate highly variable data rates and distributions as follows:
\begin{myitemize}
\item In our illustrative example, a subset of servers probe a larger set of peers to cover a wider network range on behalf of other servers in the same ToR switch~\cite{pingmesh}. We measure data rates of network probe messages generated by individual \client{}s, illustrated in  Figure~\ref{fig:data-gen-rate}. The data rates are normalized to the highest one observed among \client{} nodes. Data generation rates exhibit high variability, with 58\% of nodes generating 50\% or lower of the highest data rate we observe.
\newcontent{
\item Changing input rates for service logs can affect query compute needs. Service failures (e.g., scenario 2 in Section~\ref{sec:background}), can cause impacted analytics services to generate traffic bursts in error log volumes generated by each \client{} node until the failure is mitigated. Real-world systems have observed high variability in log record count across 1 minute windows due to service failures~\cite{chi,data-variable-minutes-dcs,helios}.
\item Changing data distribution can complicate compute usage characteristics. In our running example, network issues can cause temporary spikes in server probe latencies. We observed in \pingmesh{} traces that such spikes range in duration from 40 seconds to 2 minutes.}\todo{confirm} Each query operation's compute demand is affected by the incoming data rate after executing all preceding operations in the query. Figure~\ref{fig:pipeline_tor} shows a directed acyclic graph (DAG) of how data flows between operations for the query in Listing~\ref{lst:motivating-query}. Each query operator executes an operation such as filter, grouping, etc. F operator performs filtering and leads to the first data volume reduction from the input stream. Since erroneous (or high latency) records are usually not dominant, the operator happens to drop only a small fraction of records. A majority of records are then to be processed by G+R operator, increasing compute cost for the query. However, if we were to have network issues for inbound or outbound traffic for some servers, generating a large proportion of erroneous data,
%toggle the filtering predicates to perform a zoom-in analysis on a small subset of erroneous data,
those servers will experience a high degree of data reduction in F operator, thus lowering resource usage of the G+R operator.

\item \sout{When a subset of servers are being over-loaded, latency profiles of these servers become more variable. Hence, each of these data source nodes will generate a unique data footprint, which is quite different than the average data source node that does not encounter any abnormality.}~\cite{rubik, pegasus}
\end{myitemize}

Quick adaptation of our partitioning plans reduces the duration for which queries over/under-subscribe compute resources. On each \client{}, over-subscription can lead to resource interference with foreground services, while under-subscription provides an opportunity to reduce network traffic leaving the node. Given that compute conditions can change in the order of a few minutes, existing works like Sonata~\cite{sonata} which take up to 20 minutes to compute a new partitioning plan become a bottleneck for adaptation. A new partitioning plan needs to be quickly identified so that query compute demands meet available budget. To initiate query refinement and compute a new plan at runtime, \client{}s periodically inject \emph{refinement watermarks} into the stream (similar to~\cite{trill}) and they
delimit ordered consecutive \emph{refinement epochs} of records.
%Refinement watermarks are different from the traditional watermark described in data model.
For brevity, epoch and watermark refer to refinement epoch and refinement watermark respectively in the rest of the paper.

\begin{figure}[t]
\centering

\includegraphics[width=\linewidth]{fig/DataPartitionExplain.pdf}
%\vspace{-0.1in}
\caption{\label{fig:data-partition-explain} Coarse-grained operator-level vs. fine-grained data-level partitioning on \client{} with 80\% CPU budget. G+R requires 80\% CPU to process all output data from F operator.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

\section{Problem definition and insights}
\label{sec:drawbacks}
\newcontent{In this paper, we investigate how to effectively utilize limited and dynamic compute resources available on \client{} nodes, by quickly partitioning query workloads between \client{} and \server{} nodes and reduce network transfer costs for supporting large scale server monitoring pipelines.}

Consider that a monitoring query can be represented as a DAG $G = (V,E)$. In a DAG, the vertices V denote stream operations which transform their input records and emit output records to downstream operation, and the edges $E$ denote dataflow dependencies between operations. Among prior approaches to addressing query partitioning, the operator-level partitioning~\cite{everflow,gigascope,jetstream} is one of the most widely used approaches. Given a query DAG, an operator-level partitioning plan identifies operations that can execute locally on each \client{} and those that require remote execution on the \server{}. This requires a boundary operator to be defined for each \client{} to indicate that all operators prior to the boundary operator (including itself) in the topological order of the DAG are executed on \client{} and those after the boundary operator are executed remotely. In Figure~\ref{fig:pipeline_tor}, if F operator is
designated as a boundary operator, W and F operators would execute on the \client{} to filter out unnecessary data inside the \client{}, effectively reducing the amount of data transferred to the \server{}.

% $b_i$
%To illustrate, consider a topologically sorted list of $M$ operators from the query graph $G$ following dataflow dependencies of the query.
%For instance, for a \client{} with 4 operators, if the boundary operator is 3
%then it implies that the first three operators execute on \client{} and the
%last operator executes remotely.
% $M=4$

%% Given fixed network and compute resources available on \server{}, we seek to maximize the number of \client{}s that can be served to execute a monitoring query in a timely manner. Thus,
%Subsequently, the optimization goal of query partitioning in the context of
%server monitoring ends up identifying the boundary operator for each
%\client{}, such that the processing load sent to \server{} is minimized while
%harnessing the given monitoring resources from the \client{}.
%%The optimization goal of query partitioning is to identify the boundary
%%operator for each \client{}, such that the processing load sent to \server{}
%%is minimized, subject to local computation not increasing overall processing
%%time of each data stream, compared to remote execution.

% This is a NP-hard problem and computationally difficult to solve: we present a formal definition and proof in~\cite{jarvis-extended}.

\begin{figure}[t]
  \centering
    \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
    \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
    \label{fig:data-gen-rate}
    \vspace{-0.5cm}
\end{figure}


\textcolor{blue}{
We formally define the query partitioning problem. Let \textbf{b} represent the boundary operators for a given query, where $b_i$ denotes boundary operator for the $i^{th}$ \client{}. Our optimization problem is as follows:
\begin{align*}
    & \displaystyle \min_{\textbf{b}} \sum_{i=1}^{N_{d}}\sum_{j=1}^{M} c_j x_{ij}\\
    subject\ to,&\\
    & T_{local}(i,b_{i}) <= T_{remote}(i,b_{i})\ \forall b_{i}>0, i\epsilon[1,N_{d}]
\end{align*}
Here $x_{ij}$ indicates if boundary operator of $i^{th}$ \client{} is $j$, $c_j$ is the processing cost on \server{} due to partitioning the query on \client{} at $j^{th}$ operator, $T_{local}(i,b_{i})$ computes the local computation time cost for operators 1 to $b_{i}$ on the $i^{th}$ \client{} node and $T_{remote}(i,b_{i})$ denotes the network transmission time cost of intermediate data from $b_{i}^{th}$ operator to its parent stream processor node along with computation time cost of executing operators $b_{i}+1$ till $M$ on the parent node. We want to incentivize executing operators on \client{} so the partitioning costs are ordered as $c_1>c_2>,...>c_M$. Unfortunately, solving the partitioning problem is extremely challenging.
\begin{theorem}
Query partitioning problem to distribute query operators across \client{} and \server{} nodes, with the objective of maximizing the resource utilization of \client{} nodes without degrading query processing time, is NP-hard.
\end{theorem}
\begin{proof}
The key idea of the proof is that the generalized assignment problem~\cite{gap} can be reduced to a special case of our query partitioning problem in polynomial time. Therefore, if we have an algorithm that can minimize the number of operators sent to the \server{} without sacrificing query processing time, then we can also obtain optimal solution to GAP. Since GAP is NP-hard, our problem is also NP-hard. More details for the proof can be found in~\cite{jarvis-extended}.
\end{proof}
}
\newcontent{
Having established the NP-hardness of query partitioning, we note that in our monitoring system, each \client{} runs an instance of the query on its incoming input stream. Query partitioning involves determining the boundary operator for each query instance. Thus, we need to evaluate $M^{N_{d}}$ possible partitioning solutions, where $N_{d}$ is the number of \client{}s and $M$ is the number of operators per query instance. Given that resource conditions change in the order of minutes (Section~\ref{sec:motivation}), we need to quickly compute a new partitioning plan. Each \server{} node in our setup can receive data from up to 250 \client{}s so the exponential cost in \client{}s would not scale for the large number of \client{}s. Other techniques such as trading off accuracy for reducing network transfer costs using data summaries could be considered but their limitations are highlighted at the end of this section. Thus, to make query partitioning practical in large scale server monitoring pipelines, we investigate the effectiveness of a greedy and embarrassingly parallel partitioning heuristic, which reduces network traffic leaving each \client{}. We postulate that to effectively utilize the limited and dynamic compute on each \client{}, it is critical to make fine-grained, data-level partitioning decisions for query operators at runtime, which can be done using a query cost model-based partitioning approach that relies on online and fine-grained profiling of each operator's compute cost. However, accurate online profiling can be challenging due to limited compute available on \client{}. Thus, iteratively fine-tuning the output of query cost model-based approach, using a feedback-driven technique which is agnostic to the cost model, can significantly improve the performance of our adaptation. Our proposed heuristic is simple, computationally tractable and a reasonable first attempt at addressing the query partitioning problem in large scale server monitoring pipelines. Finally, we build a proof-of-concept system Jarvis, which implements the designed partitioning heuristic in a fully decentralized manner using novel system abstractions called \Proxy{} and \run{}. \ours{} is used to evaluate the practicality and effectiveness of our heuristic in scaling monitoring pipelines. Below, we discuss the insights to design the heuristic used by \ours{}. }

%We highlight the drawbacks of state-of-the-art approaches in addressing the operator-level partitioning problem as well as uncover insights for designing \ours{}.

%\Paragraph{Drawback 1: Coarse-grained partitioning can significantly
%under-subscribe \client{} node resources.} State-of-the-art monitoring systems~\cite{everflow,
%sonata, dshark} have explored coarse-grained partitioning strategies---i.e., either all records are processed by an operator or none.
\Paragraph{Data-level query partitioning.}
Operator-level query partitioning could be undesirable when attempting to run a computationally expensive operator like grouping within limited compute resources provided by \client{}, because it could over-subscribe available resources. However, the alternative is for the partitioning mechanism to leave the resource highly underutilized.
To highlight this issue concretely, we execute the query in
Figure~\ref{fig:pipeline_tor} using 80\% of single core operating at 2.4GHz, which reflects
compute constraints on \client{}. The upper part of Figure~\ref{fig:data-partition-explain}
shows the resulting resource usage statistics in detail among the operators.
Because F operator drops only a small portion of input records, it is not
possible to execute the expensive G+R operator entirely on \client{}. This leads to
under-utilization of the available compute resources and generation of network traffic as high as 22.5 Mbps, which is close to the query input rate.

On the contrary, extending the operator-level partitioning model to support \datapart{} could significantly improve the utilization of limited compute resources on \client{}.
This fine-grained \datapart{} allows an operator to process a fraction of its input records on \client{} and drain the rest for remote processing. With this approach, as shown in the lower part of Figure~\ref{fig:data-partition-explain}, the operator G+R in the query can process 83\% of its input, resulting in total network traffic of 9.4 Mbps. Note that this traffic amount is 2.4x lower than the traffic generated by the coarser-grained operator-level partitioning strategy.

%\noindent \underline{Insight 1:} \emph{Extending the operator-level partitioning model to support data-level partitioning significantly improves the utilization of limited compute available on \client{} nodes.}

\Paragraph{Fast and accurate adaptation enabled by combining cost model-based and model-agnostic techniques.}
% \Paragraph{Fast and effective adaptation mechanism.}
% Partitioning approaches need to keep up with highly dynamic resource conditions on \client{}s.
The requirement for frequent and dynamic query refinement due to high variability in resource conditions calls for a highly efficient refinement approach. In particular, given the aforementioned dynamics, query planners may need to compute and execute a new and effective partitioning plan in a timely manner, even in seconds.

%The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently the available compute per-query. Given these dynamics, query planners need to compute and execute a new partitioning plan in a timely manner, even in seconds.

While optimal partitioning can be achieved using a query cost model and a centralized planner to leverage global information about available resources~\cite{sonata,ds2,optimal-odp},  it is computationally expensive due to high algorithmic complexity (NP-hard~\cite{jarvis-extended}). A cost model-based heuristic is attractive if it can efficiently be solved to obtain a partitioning solution. However, the model may not accurately capture complex query behavior~\cite{model-free-control-drl}. Solely relying on a cost model may lead to inaccurate partitioning. A greedy and embarrassingly parallel heuristic utilizing a combination of cost model-based and model-agnostic techniques enables fast, accurate and fully decentralized query refinement on each \client{}.


% \Paragraph{Drawback 2: Without fast \& accurate adaptation, partitioning approaches cannot keep up with highly dynamic resource conditions on \client{}s.}
% The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently the available compute per-query. Given these dynamics, query planners need to compute and execute a new partitioning plan in a timely manner, even in seconds.

% While optimal partitioning can be achieved using a query cost model \& centralized planner to leverage global information about available resources~\cite{sonata,ds2,optimal-odp},  it is computationally expensive due to high algorithmic complexity (NP-hard~\cite{jarvis-extended}). Other cost model-based query planners have been explored in literature without considering partitioning under highly variable \client{} resource conditions~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (Section~\ref{sec:RelatedWork}).
% Optimizing for a cost model is attractive if it can be solved efficiently for a partitioning decision. However, the model may not accurately capture complex query behavior, in which case solely relying on it leads to inaccurate decisions~\cite{model-free-control-drl}.
% , potentially leading to inaccurate partitioning decisions.
% Furthermore, it may not be feasible to obtain accurate performance models at runtime.

% \noindent \underline{Insight 2:} \emph{A greedy \& embarrassingly parallel heuristic utilizing a combination of cost model-based \& model-agnostic techniques enables fast, accurate and fully decentralized query refinement on each \client{}.}

% Furthermore, a greedy approach which relies solely on optimizing for a cost model may output an incorrect partitioning decision as the model may not accurately capture complex query execution behavior~\cite{model-free-control-drl}.

% Prior work relies on centralized query planners that leverage global information about available resources to solve an expensive optimization function~\cite{sonata} and on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Optimal partitioning is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach for partitioning. Other centralized and decentralized query planners have also explored model-free and model-based approaches but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}).
%\ours{} investigates a greedy and embarrassingly parallel approach which uses hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}.
%dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs.
% \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}
% A greedy and embarrassingly parallel approach utilizing a hybrid performance model-based and model-agnostic technique can enable fast and fully decentralized query refinement on each \client{}, which is accurate, robust and scalable and automatic.

\newcontent{\Paragraph{Can data synposes reduce network traffic?} Data synopsis techniques, such as sampling, histograms, and
sketches~\cite{synopsis-berkeley}, are commonly used to enable scalable
stream analysis by trading off accuracy for
performance~\cite{continuous-sampling-streams, mergeable-summaries}. Despite
their effectiveness and practicality, losing output accuracy may be undesirable for telemetry tasks such as anomaly detection, in which anomalies are hard to predict before they occur~\cite{omnimon}. Data that corresponds to anomalies are typically infrequent, so the lossy output could lead to undetected anomalies and affect server reliability. And false alarms may also require developers to manually review alerts which quickly become a burden when dealing with complex and large scale systems~\cite{thread-alert-fatigue}. Furthermore, debugging scenarios for server misconfigurations and failures such as gray failures~\cite{gray-failure} benefit from having access to per-node statistics at fine-grained timescales, to enable localizing and repairing of problematic server nodes. In Section~\ref{sec:sampling-vs-jarvis}, we compare the effectiveness (i.e., accuracy and network transfer costs) of \ours{} and a state-of-the-art window-based sampling
protocol~\cite{continuous-sampling-streams} using the query in Listing~\ref{lst:motivating-query}. In particular, when network transfer costs between the two approaches are almost at par, sampling misses a number of anomalous data points, resulting in high errors in the final query result.
}

%\subsection{Can we use data synposes?}
%\label{sec:data-summaries}

% Pingmesh query uses threshold-based technique for alerts. Sampling is sensitive to skew and outliers, and requires knowledge of the underlying distribution of values to apply estimators like Horvitz-Thompson (HT)~\todo{cite}. HT cannot be applied to max and min. More recently, Condor~\cite{condor-approx-streams} proposed integrating data synopses into stream processing engines.
% Scenarios which benefit include:
% \begin{myitemize}
% \item Anomaly detection: do not worry about false alarms or undetected anomalies due to measurement error.
% \item performance diagnosis or gray failures?
% \end{myitemize}
% Three types of monitoring queries:
% \begin{myitemize}
% \item Queries processing raw data~\cite{helios,gandalf}.
% \item Queries that can use statistical summaries: Several monitoring pipelines utilize data summaries to reduce the data traffic going to \server{} for processing. Statistics work well if the raw data is well-behaved, i.e., it follows a certain distribution such as Gaussian~\cite{statistics-online-anomaly-detect}.  \todo{Can we show Pingmesh rtt's do not follow any well-known distributions over time? What about non-parametric statistical techniques? Can we compare Jarvis with a statistical technique and show as much data reduction without the burden of configuring parameters and/or introducing false positives/negatives?}.
% \item The summaries can be part of the monitoring query itself. E.g., histogram calculation to summarize the collected data is part of the monitoring query in \dnnlog{} query. Section~\ref{sec:evaluation} shows the benefits of using \ours{} to improve the performance of such queries.
% \end{myitemize}


==> archive/background-motivation-v3.tex <==
\section{Background \& Motivation}
%\section{Background}

%\vspace{-0.15cm}
%In this section, we
%%describe
%%the monitoring system targeted by our work. We showcase
%%challenges in building efficient large-scale monitoring systems and
%uncover insights for designing efficient large-scale monitoring systems by
%characterizing the resource usage of a real-world enterprise workload.

%In this section, we explain the background and motivation of our work by
%referring to real-world enterprise workloads.


\subsection{Monitoring Systems Overview}
\label{sec:background}

Although numerous useful scenarios correspond to large-scale server
monitoring~\cite{helios,deepview,fingerprint}, here we briefly describe two
scenarios that guide the design of \ours{}:

\begin{myitemize}

\newcontent{
\item \textit{Scenario 1:} Network engineers
    deploy Pingmesh~\cite{pingmesh} agents on
    datacenter nodes to collect latency data between node pairs. A web search
    team uses Pingmesh to monitor network health of their latency-sensitive
    service and generate an alert if more than a predefined proportion of
    hosting nodes (e.g., 1\%) have probe latencies exceeding a threshold (e.g.,
    5~ms)~\cite{pingmesh}.} \mj{check Atul}
% \item \textit{Scenario 1:} Network team deploys Pingmesh~\cite{pingmesh} agents on datacenter nodes to collect  latency data between server pairs. An internal web search team uses Pingmesh to monitor network health of their latency-sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold as determined by the search service SLA.

\item \textit{Scenario 2:} A log processing system, Helios~\cite{helios},
    enables live debugging of storage analytics services such as
    Cosmos~\cite{cosmos}. A bug in cluster resource manager may lead to service
    resources being under-provisioned. To temporarily mitigate performance
    degradation, several TBs of log streams~\cite{helios} are processed
    quickly to identify impacted tenants. Their latency and CPU/memory
    utilization data are queried to predict resource needs and make scaling
    decisions.
\end{myitemize}

%Processing in these scenarios requires a diverse set of operations.
There scenarios rely on a diverse set of computations. Scenario 1 requires
processing of periodically generated metrics composed of structured numerical
data; queries consist of computations specific to numerical data, such as
filtering and aggregation. On the contrary, Scenario 2 requires processing of
aperiodically generated logs composed of unstructured strings; queries
accompany computations for string processing such as parsing, splitting, and
search.

%Moreover, resource usage for these operators is diverse, varies significantly, and  depends on the operator logic and the input data. We consider a common set of operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}.
%Moreover, these operations are computationally different and their costs are
%highly dynamic depending on the input data.
%To illustrate, let us consider a common set of primitive operators such as
%Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and
%Map(M)~\cite{streamboxhbm,trill,flink}.

Moreover, these computations rely on various streaming primitives, which are
computationally different and whose costs are highly dynamic depending on the
input data. For example, filter (F) drops uninteresting records by applying
the predicates on each record and typically requires little amount of compute
resource. Grouping (G) organizes records by key fields and hence requires key
lookups in a hash table. Join (J) joins an input stream with a static table,
which requires key lookups on the table while joining the two inputs into an
output stream~\cite{tersecades}.
%which typically requires building a hash table over the static table followed by key lookups for the input stream.
%\footnote{Due to limitations in \client{}-side execution discussed in Section~\ref{sec:jarvis}, we do not consider other complex join operators.}
Contrary to filter, both grouping and join can be expensive due to the
irregular access patterns of hash table lookups. Their cost highly depends on
the hash table size, which corresponds to the group count and the static
table size, respectively. Map (M) performs user-defined transformations on
the input (e.g., parsing and splitting text logs) and its cost depends on the
transformation logic. We present resource usage characteristics of these
primitives in detail in~\cite{jarvis-extended}.

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{DAG of stream operations for the query in Listing~\ref{lst:motivating-query}.}
    \label{fig:pipeline_tor}
    \vspace{-0.5cm}
\end{figure}

\newcontent{
\Paragraph{Programming model.} We adopt a declarative programming
model~\cite{flink, sparkstreaming} to define a monitoring query. By this
programming model, a query can be generally expressed as a directed acyclic
graph (DAG). In a DAG, the vertices denote stream operations which transform
their input records and emit output records to downstream operations, and the
edges denote how data flows between the operations, i.e., dataflow
dependencies. Listing~\ref{lst:motivating-query} shows how programmers can
declaratively describe a real query on the \pingmesh{} data. In
Figure~\ref{fig:pipeline_tor}, we present a simple DAG of how data flows
between operations for the \pingmesh{} query. }

\Paragraph{Hierarchical query engines.} Physical resources involved in the
monitoring query execution can be viewed as a \emph{tree structure} as shown
in Figure~\ref{fig:arch-monitoring-scale}(b) \mj{bring up?}, where leaf nodes
represent the \client{} (i.e., server nodes) and the other nodes represent
the \server{}. Each \client{} node allocates
%a fixed amount of
compute and memory resources (e.g., 1 or 2 cores and 1 GB RAM) to facilitate
monitoring queries. Such allocation of the monitoring resources is done in
isolation without affecting
%can be done by provisioning a container to isolates the monitoring resources from
the resources utilized by foreground services. Each \client{} sends data to
its parent (intermediate) node and can leverage compute resources available
in the node for query processing. The root \server{} node receives data
relayed by all intermediate nodes and completes the query to output the final
result.

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}

\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}

%\Paragraph{Illustrative example.} We consider a
%real-world query on Microsoft's \pingmesh{} trace as an illustrative example to highlight challenges in
%designing large-scale monitoring systems. \pingmesh{} measures network
%latency for server pairs across the datacenter, by requiring that each server
%send probe messages to its peer servers in the datacenter. Each probe message
%generates a 86B record that includes timestamp (8B), source IP address (4B),
%source cluster ID (4B), destination IP address (4B), destination cluster ID
%(4B), round trip time in microseconds (us) (4B), and error code (4B).
%%The round trip time is in microseconds.
%
%The Pingmesh trace allows exhaustive analyses
%%, such as zoom-in/out latency probes
%by grouping latency probes across datacenter network hierarchy and
%identifying cluster-, ToR-, and server-level issues ~\cite{tersecades,
%pingmesh}. Listing~\ref{lst:motivating-query} describes the implementation of
%a real-world \pingmesh{} query for latency probing among server pairs. The
%query is written in a declarative programming model used by popular stream
%engines, such as Flink~\cite{flink} and Spark
%Streaming~\cite{sparkstreaming}, which express a query using dataflow
%operations.
%
%%Real-world monitoring scenarios exhibit \textit{high traffic volume}~\cite{chi, gandalf, m3}.
%%Logs collected from applications can generate up to 971 Gbps~\cite{chi}. Other systems~\cite{gandalf,m3} process up to tens of TB data per day or millions of events every second per monitoring task, straining compute, memory, and network capacities of the monitoring system.


\subsection{Adaptive Query Partitioning in Query Engines}
\label{sec:motivation}

Many existing real-world monitoring scenarios exhibit \textit{high traffic
volume}~\cite{chi, gandalf, m3} due to a large number of \client{}s and
diverse data streams collected for monitoring. We corroborate this by
analyzing the volume of data transferred over the network observed in the
Microsoft's \pingmesh{} trace, which we will use as an illustrative example
in this section. Each record in the trace corresponds to a single probe
message for a server pair. A record is 86B in size, including timestamp (8B),
source IP address (4B), source cluster ID (4B), destination IP address (4B),
destination cluster ID (4B), round trip time in microseconds (us) (4B), and
error code (4B).
%The round trip time is in microseconds.
Now, assuming that a datacenter consists of 200K servers and each server
probes 20K other servers with a probing interval of 5
seconds~\cite{pingmesh}, the data generation rate is estimated to be
512.6~Gbps. Transferring such high volume of data would strain network
capacity and delay the query execution.

%\Paragraph{High data volume.} We corroborate existing real-world monitoring
%scenarios with \textit{high traffic volume}~\cite{chi, gandalf, m3} by
%quantifying the volume of data transferred over the network in the
%\pingmesh{} scenario. Assuming that a datacenter consists of 200K servers and
%each server probes 20K other servers with a probing interval of 5 seconds
%~\cite{pingmesh}, the data generation rate is estimated to be 512.6~Gbps.
%Transferring such high volumes of data would strain network capacity and
%incur high deployment cost of compute resources in the \server{}.

Monitoring queries typically permit data processing that incrementally
reduces the data volume---e.g., Figure~\ref{fig:pipeline_tor} shows that
records are first filtered and then aggregated into a few statistical
numbers. An effective approach to alleviating the network bottleneck is thus
to allow processing data \emph{near the \client{}} and reduce its size before
transmitting over the network. For brevity, we refer to the technique of
offloading a part of query execution near the \client{} as \emph{query
partitioning}. As will be described below, the ability to take partitioning
decisions dynamically and promptly is crucial due to variable resource
conditions.
%, but it is non-trivial to do so effectively.

%\Paragraph{Variability in resource conditions.}
\newcontent{
%An effective
%approach to consider for alleviating network bottlenecks due to high traffic
%volumes is to process data closer to the \client{} and reduce its size before
%network transfer. We refer to the pushing of a subset of the query's
%execution workload closer to the source as \emph{query partitioning}.

%Monitoring queries typically permit incremental data processing and lead to
%data size reduction. But executing the entire query on each \client{} node is
%not always feasible given the limited compute allocated for monitoring
%workloads. Thus, we need to carefully consider the compute-communication
%tradeoff involved in pushing query operations closer to the \client{}. These
%decisions need to be made in an online manner to account for changes in the
%resource conditions on each \client{} node.

\Paragraph{Changing resource availability.} As resource demands of foreground services are
changing dynamically over time, unused compute resources on \client{} nodes
available for monitoring queries exhibit temporal variability. This is a
common characteristic of \client{} nodes as they usually host highly dynamic
workloads. For instance, large-scale web services (e.g., Alibaba and
Wikipedia) and ML inference services are all provisioned to withstand bursty
request loads to meet their SLA targets~\cite{alibaba-bursty-workload,
wikipedia-bursty-workload, barista-predictive-analytics,
mark-ml-inference-atc}. This leads to variable demands on compute resources
changing in the order of minutes by those services. Subsequently, query
partitioning decisions need to be made promptly \emph{at runtime} on
\emph{each \client{}}, to be compatible with dynamic resource conditions
available to exploit on each \client{}.

%High temporal variability in available compute is caused by changing compute
%demands of the server node's foreground services. E.g., real world traces
%from large scale web services like Alibaba~\cite{alibaba-bursty-workload},
%Wikipedia~\cite{wikipedia-bursty-workload} and ML-based predictive analytics
%services for speech and
%vision~\cite{barista-predictive-analytics,mark-ml-inference-atc} show bursty
%request rates requiring variable compute needs in the order of minutes to
%meet service SLA. Such variability requires making fast query partitioning
%decisions at runtime on each \client{}.

\Paragraph{Changing resource needs.} Input rates and data distributions can change over time, significantly impacting query resource needs. Input rates are affected by service failures which can generate traffic bursts in error log volumes on each \client{}, until the failure is mitigated. Several real-world log analytics systems in the datacenter report high temporal variability in record count of log streams, even across 1~minute time windows~\cite{chi, data-variable-minutes-dcs, helios}. 

Anomalous behavior on server nodes can cause monitoring data distributions to change. In our running example, network issues can cause temporary spikes in server probe latencies. Analyzing our \pingmesh{} traces, we observed that such spikes can last in duration from 40 seconds up to a minute. Such spikes complicate query resource usage characteristics. Each query operation's compute demand is affected by the incoming data rate after executing all preceding operations in the query. In Figure~\ref{fig:pipeline_tor}, F operator performs filtering and leads to the first data volume reduction from the input stream. Since erroneous (or high latency) records are usually not dominant, the operator happens to drop only a small fraction of records. A majority of records are then to be processed by G+R operator, increasing compute cost for the query. However, if we were to have network issues for inbound or outbound traffic for some servers, generating a large proportion of erroneous data,
%toggle the filtering predicates to perform a zoom-in analysis on a small subset of erroneous data,
those servers will experience a high degree of data reduction in F operator, thus lowering resource usage of the G+R operator.
% Each query operator executes an operation such as filter, grouping, etc.

Furthermore, data generation rates also vary across \client{} nodes (i.e., spatial variability). We analyzed the \pingmesh{} trace for how data rates for network probe messages generated by individual \client{}s, differ from each other. We observed highly variable data rates, with 58\% of the nodes generating 50\% or lower of the highest rate (details in~\ref{jarvis-extended}). The reason for this is that some servers are configured to probe a larger set of peers to cover a larger network range on behalf of other servers in the same ToR
switch.}

% our target use cases including
% \pingmesh{} queries. To this end, we present in
% Figure~\ref{fig:data-gen-rate} how data rates of network probe messages
% generated by individual \client{}s in our \pingmesh{} trace differ from each
% other. In the figure, the data rates are normalized to the highest one
% observed among \client{} nodes. The data rates are highly variable, with 58\%
% of the nodes generating 50\% or lower of the highest rate. The reason behind
% is primarily due to some servers configured to probe a larger set of peers to
% cover a larger network range on behalf of other servers in the same ToR
% switch. Note that this configuration can be adjusted as network topology is
% being updated.

%by exhibiting both temporal (i.e., on each \client{}) and spatial (i.e.,
%across \client{}s) variabilities, as follows:
%We look at the following factors that affect query compute demands:

% \begin{figure}[t]
%   \centering
%     \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
%     \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
%     \label{fig:data-gen-rate}
%     \vspace{-0.5cm}
% \end{figure}

% }

%% High temporal (i.e., on each \client{}) and spatial (i.e., across \client{}s) variability in resource conditions can be observed in monitoring pipelines.
%
%% generation of monitoring data \cite{chi,helios} affecting the effectiveness of a query partitioning plan. In our running example, we also observe that data source nodes generate highly variable data rates and distributions as follows:
%
%\begin{myitemize}
%\item In our illustrative example, a subset of servers probe a larger set of
%    peers to cover a wider network range on behalf of other servers in the
%    same ToR switch~\cite{pingmesh}. We measure data rates of network probe
%    messages generated by individual \client{}s, illustrated in
%    Figure~\ref{fig:data-gen-rate}. The data rates are normalized to the
%    highest one observed among \client{} nodes. Data generation rates exhibit
%    high variability, with 58\% of nodes generating 50\% or lower of the
%    highest data rate we observe.
%\newcontent{
%\item Changing input rates for service logs can affect query compute needs.
%    Service failures (e.g., scenario 2 in Section~\ref{sec:background}), can
%    cause impacted analytics services to generate traffic bursts in error log
%    volumes generated by each \client{} node until the failure is mitigated.
%    Real-world systems have observed high variability in log record count
%    across 1 minute windows due to service
%    failures~\cite{chi ,data-variable-minutes-dcs, helios}.
%\item Changing data distribution can complicate compute usage
%    characteristics. In our running example, network issues can cause
%    temporary spikes in server probe latencies. We observed in \pingmesh{}
%    traces that such spikes range in duration from 40 seconds to 2
%    minutes.}\todo{confirm} Each query operation's compute demand is affected
%    by the incoming data rate after executing all preceding operations in the
%    query. Figure~\ref{fig:pipeline_tor} shows a directed acyclic graph (DAG)
%    of how data flows between operations for the query in
%    Listing~\ref{lst:motivating-query}. Each query operator executes an
%    operation such as filter, grouping, etc. F operator performs filtering
%    and leads to the first data volume reduction from the input stream. Since
%    erroneous (or high latency) records are usually not dominant, the
%    operator happens to drop only a small fraction of records. A majority of
%    records are then to be processed by G+R operator, increasing compute cost
%    for the query. However, if we were to have network issues for inbound or
%    outbound traffic for some servers, generating a large proportion of
%    erroneous data,
%%toggle the filtering predicates to perform a zoom-in analysis on a small subset of erroneous data,
%
%    those servers will experience a high degree of data reduction in F operator,
%    thus lowering resource usage of the G+R operator.
%
%\item \sout{ When a subset of servers are being over-loaded, latency profiles
%    of these servers become more variable. Hence, each of these data source
%    nodes will generate a unique data footprint, which is quite different
%    than the average data source node that does not encounter any
%    abnormality}~\cite{rubik, pegasus}.
%\end{myitemize}

\Paragraph{Summary.} The ability to quickly adjust query partitioning plans
(i.e., \emph{query refinement}) would reduce the duration for which queries
either over-subscribe or under-subscribe available compute resources. The
over-subscription can lead to an interference with foreground services in
each \client{} node, whereas the under-subscription loses an opportunity to
further reduce network traffic leaving the node. Prior work proposes an ILP
solver for online query refinement, but it is too costly taking up to
20~minutes to compute a new query partitioning plan~\cite{sonata} \mj{should
connect to the next section?}. Therefore, our goal is to develop an approach
which not only completes query refinement at low latency but also effectively
reduces the network traffic given the compute budget on each \client{} node.

%Quick adaptation of our partitioning plans reduces the duration for which
%queries over/under-subscribe compute resources. On each \client{},
%over-subscription can lead to resource interference with foreground services,
%while under-subscription provides an opportunity to reduce network traffic
%leaving the node. Given that compute conditions can change in the order of a
%few minutes, existing works like Sonata~\cite{sonata} which take up to 20
%minutes to compute a new partitioning plan become a bottleneck for
%adaptation. A new partitioning plan needs to be quickly identified so that
%query compute demands meet available budget. To initiate query refinement and
%compute a new plan at runtime, \client{}s periodically inject
%\emph{refinement watermarks} into the stream (similar to~\cite{trill}) and
%they delimit ordered consecutive \emph{refinement epochs} of records.
%%Refinement watermarks are different from the traditional watermark described in data model.
%For brevity, epoch and watermark refer to refinement epoch and refinement
%watermark respectively in the rest of the paper.


==> archive/background.tex <==
\section{Server Monitoring Background}
%\section{Datacenter Monitoring}
%\section{Telemetry Monitoring in Datacenter}
\label{sec:background}
\vspace{-0.15cm}
%This section presents background on datacenter telemetry monitoring with
%example scenarios.

%\subsection{Monitoring Architecture}
%\subsection{Background and Challenges}
%\label{sec:background}

%Troubleshooting, root-cause analysis and remediation of production issues are
%common challenges facing modern, cloud-scale datacenter operators. Monitoring
%infrastructure built to understand and debug availability and performance
%problems in the datacenter~\cite{fingerprint, pingmesh, autoscaling,
%netbouncer, scuba, m3, deepview}, are critical to uphold infrastructure
%uptime and honor customer SLAs with minimum disruption.
% Datacenter telemetry monitoring is indispensable for incident management, troubleshooting, and performance crisis detections in the datacenter~\cite{fingerprint, pingmesh, autoscaling, netbouncer, scuba, m3} that runs numerous important applications such as database systems and web services.
%Such monitoring systems collect and investigate
%performance metrics corresponding to HW, OS, application, runtime
%systems, etc.

% So monitoring can refer to collecting and processing data at hardware level, different layers of the application stack, management services, security, packet-level telemetry from network switches, etc. 
%Monitoring infrastructure for a datacenter is required to report availability and performance problems at low latency to reduce the mean time to fault detection, and at high accuracy to reduce the possibility of false discoveries or faults remaining undetected. To satisfy dual requirements of accuracy and timeliness, existing monitoring systems are built to gain insights from continuous data streams generated across the system stack. In particular, 
Two classes of data that monitoring systems capture are  timestamped measurement data from individual datacenter nodes corresponding to health of hardware, OS, and runtime systems~\cite{pingmesh, deepview, m3}, \emph{and/or} textual logs generated by a specific service which spans a large number of nodes to be hosted~\cite{philly, chi}.
Although numerous useful scenarios correspond to large-scale server monitoring~\cite{helios,deepview,fingerprint}, the design of \ours{} is guided by two scenarios, one for each class of data:
%Requirements for processing the collected monitoring data vary %substantially depending on the use case, data volume and %nature of data processing~\cite{slack-observability}.

\begin{myitemize}
\item \textit{Scenario 1:} Network team deploys PingMesh~\cite{pingmesh} agents on each datacenter node to collect probe latency data between server pairs. An internal Search team uses PingMesh to monitor network health of their latency sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold. The threshold is determined by the search service SLA.
    % Note that we also use this scenario to motivate our work and introduce \ours{} in Sections~\ref{sec:motivation} and~\ref{sec:jarvis}.
    % , to assist in debugging network issues for hosted applications.
\item \textit{Scenario 2:} A log processing system (e.g. Helios~\cite{helios}) enables live debugging of storage analytics services (e.g. Cosmos~\cite{cosmos}). A bug in cluster resource manager leads to service resources being under-provisioned. To temporarily mitigate performance degradation, multiple TBs of log streams~\cite{helios} are processed quickly to identify impacted tenants. Their latency and CPU/memory utilization data are queried to predict resource needs and make scaling decisions.

% The storage team has built a service (such as Cosmos~\cite{cosmos}) to enable users to write analytics jobs on their data. Logs generated by these jobs are processed to generate an alert if the job running times exceed user provided threshold. Users can request additional information like resource utilization extracted from the logs, to debug long running jobs.

    % \item \textit{Scenario 2:} Multiple product teams train ML models to integrate into their products. ML training jobs are run on a shared GPU cluster~\cite{philly,deep-learning-photographs,deep-learning-siri}. Jobs can fail due to many reasons as described in~\cite{philly} so to help prioritize failure categories to debug, job logs are processed to track percentiles for runtime to failure of different failure categories on a dashboard, using histogram-based estimation~\cite{prometheus-estimate-percentile}.~\todo{Need to fix this scenario}
\end{myitemize}

%Consider a large datacenter managed by an enterprise company/cloud provider. The internal monitoring team deploys a sophisticated data processing pipeline to support low latency monitoring needs of teams within the company, as shown in Figure~\ref{fig:arch}. Dashboards are created by users to monitor their services for different scenarios. We focus on the following types of monitoring scenarios in this paper: 
%\begin{myitemize}
%    \item \textit{Scenario 1:} Network team deploys PingMesh~\cite{pingmesh} agents on each datacenter node to collect probe latency data between server pairs. An internal Search team uses PingMesh to monitor network health of their latency sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold. The thresold is determined by the search service SLA.
%    % Note that we also use this scenario to motivate our work and introduce \ours{} in Sections~\ref{sec:motivation} and~\ref{sec:jarvis}.
%    % , to assist in debugging network issues for hosted applications.
%    \item \textit{Scenario 2:} The storage team has built a service (such as~\cite{cosmos}) to enable users to write analytics jobs on their data. Logs generated by these jobs are processed to generate an alert if the job running times exceed user provided threshold. Users can request additional information like resource utilization extracted from the logs, to debug long running jobs. 
%    
%    % \item \textit{Scenario 2:} Multiple product teams train ML models to integrate into their products. ML training jobs are run on a shared GPU cluster~\cite{philly,deep-learning-photographs,deep-learning-siri}. Jobs can fail due to many reasons as described in~\cite{philly} so to help prioritize failure categories to debug, job logs are processed to track percentiles for runtime to failure of different failure categories on a dashboard, using histogram-based estimation~\cite{prometheus-estimate-percentile}.~\todo{Need to fix this scenario}
%\end{myitemize}

In these scenarios, processing of incoming monitoring data requires different types of query operations. The first scenario requires processing of metrics which are structured numeric data and generated periodically; queries on this data consist of operations, such as filtering and aggregation. On the contrary, the second scenario requires processing of logs which are unstructured strings and are generated aperiodically; queries consist of string processing operations, such as parsing, splitting, and search. 

Resource usage for operators is diverse and varies significantly depending on the operator logic and the input data. In this work, we consider widely used operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. These operators are computationally different and their costs are highly dynamic. For example, Filter (stateless operator) drops uninteresting records by applying the predicates on each record and typically operates at a low computational cost. Grouping (stateful operator) organizes records by key fields, and hence requires key lookups (in hash tables). Join (stateful operator) joins an input stream with a static table on \client{}, which typically requires building a hash table over the static table followed by key lookups for the input stream.\footnote{Note that due to limitations of \client{}-side execution discussed in Section~\ref{sec:jarvis}, we do not consider other complex join operators in the paper.} Both grouping and join operators may be expensive due to expensive and irregular compute patterns of hash table lookups. Their cost highly depends on the hash table size, which depends on the group count and the static table size, respectively. Map operator performs user-defined transforms on the input (e.g. parse and split text logs) and their cost depends on the transform logic. Quantitative analysis of the resource usage characteristics can be found elsewhere~\todo{cite}.

% The following summarizes key characteristics of popular operators:

% \begin{myitemize}
% % \item Project(P) operator extracts fields of interest from each record in the input stream
% % \item Map(M) takes an element from the input stream and outputs an element which is result of user-defined transformation.
% \item Filter(F) drops uninteresting records by applying filtering predicates on a set of record fields. It is a stateless operator, so typically operates at a low computational cost.

% \item Grouping(G) organizes records by key fields. In popular hash-based grouping, key lookups and moving of records needs to be done making it an expensive operator that dominates total query execution time~\cite{streamboxhbm}.
% \item Reduction(R) computes aggregate statistics incrementally, requiring only a few variables~\cite{trill}, e.g., sum and count to compute an average. If R aggregates on many records, it achieves enormous data reduction on the input stream.
% \item Join(J) operator combines record fields from one or more data sources within a time window, for those records satisfying a given join predicate. We focus on joins between input stream and a static table on \client{} nodes due to limitations of operators that can be executed on \client{} discussed in Section~\ref{sec:jarvis}.
% Other common operators include project and map operators which extract fields of interest from each input record and apply user-defined transformations on each record, respectively.

% % a join can occur between two streams or a stream and a static table. We focus on joins between input stream and a static table on \client{} nodes, due to limitations of executing operators on \client{} nodes discussed in Section~\ref{sec:jarvis}.
% \end{myitemize}

\begin{comment}
\begin{figure}[t]
\centering
%\subfigure[Filter operator]{\includegraphics[width=1.65in,height=1.3in]{fig/FilterProfileHighInpRate.pdf}}
\subfigure[G+R operator]{\includegraphics[width=1.65in,height=1.3in]{fig/GroupbyProfilePingmeshInpRate.pdf}}
\subfigure[Join operator]{\includegraphics[width=1.65in,height=1.3in]{fig/JoinOperatorProfileNew.pdf}}
%\vspace{-0.1in}
\caption{\label{fig:profile-op} Profiling of query operators.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

% This setup corresponds to running ten monitoring queries with equal sharing of the given single core budget and puts enough stress on the \server{} node.

%To observe how input data distribution causes operators' CPU utilization to
%vary, we profile F, G+R \footnote{Reduction commonly follows grouping to
%apply aggregation functions incrementally per group, so both are often
%combined.} and J operator using our trace on a \server{} node with 4 2.4~GHz
%cores. We configure data input rate to be 26.2~Mbps (10x scaled up) to ease
%our measurements (see \textbf{\pingmesh{}} in Section~\ref{sec:evaluation}
%for details). We then adjust different parameters that affect operator
%resource usage: (1) filtering predicate for F operator to obtain different
%filter-out rates (between 20-80\%), (2) output group counts for G+R operator
%reflecting a range from coarse-grained grouping (e.g., cluster level) to
%fine-grained grouping (e.g., server level) and (3) static table size for J
%operator which is joined with input stream reflecting query to look up ToR
%switch ID for each server IP address in \textbf{\pingmesh{}} dataset, to
%enable network latency analysis at the ToR level. We observed that for a
%range of filter-out rates, F operator requires 17-25\% CPU with low compute
%cost and variance. However, Figure~\ref{fig:profile-op} shows that when the
%number of groups and static table size changes for G+R and J operators
%respectively, CPU usage varies substantially between 50\%-350\%. Notice that
%in the presence of non-uniform data generation rates across \client{} nodes,
%we expect G+R and J operators to have more variable resource demands.

We shed light on resource usage characteristics of query operators by considering the first scenario. In particular, we profile the operators F, G+R,\footnote{Reduction commonly follows grouping to apply aggregation functions incrementally per group, so both are often combined.} and J operators on a real-world \pingmesh{} trace on a \server{} 4-core CPU. We configure the data input rate to 26.2~Mbps (Section~\ref{sec:evaluation} details why we consider this rate) and adjust several parameters that affect operator resource use: (i) filtering predicate for F to obtain different filter-out
rates (between 20-80\%), (ii) output group counts for G+R reflecting
a range of grouping granularity and (ii) the size of static table for J which is joined with input stream.  
% to add ToR switch ID's given server IP addresses to each record (for grouping by ToR ID's). 
We observe that the F operator requires low compute resources (i.e., 17-25\% of the CPU) with low variance  even for such wide range of filter-out rates. On the contrary, as shown in  Figure~\ref{fig:profile-op}, G+R and J operators can be quite expensive with high variance (i.e., 50\%-350\% of the CPU) as they are quite sensitive to the number of groups and table size, respectively.
\end{comment}

==> archive/background_extended.tex <==
\section{Background and Challenges for Large-scale Server Monitoring}
%\section{Datacenter Monitoring}
%\section{Telemetry Monitoring in Datacenter}
\label{sec:background_ext}

%This section presents background on datacenter telemetry monitoring with
%example scenarios.

%\subsection{Monitoring Architecture}
%\subsection{Background and Challenges}
%\label{sec:background}

%Troubleshooting, root-cause analysis and remediation of production issues are
%common challenges facing modern, cloud-scale datacenter operators. Monitoring
%infrastructure built to understand and debug availability and performance
%problems in the datacenter~\cite{fingerprint, pingmesh, autoscaling,
%netbouncer, scuba, m3, deepview}, are critical to uphold infrastructure
%uptime and honor customer SLAs with minimum disruption.
% Datacenter telemetry monitoring is indispensable for incident management, troubleshooting, and performance crisis detections in the datacenter~\cite{fingerprint, pingmesh, autoscaling, netbouncer, scuba, m3} that runs numerous important applications such as database systems and web services.
%Such monitoring systems collect and investigate
%performance metrics corresponding to HW, OS, application, runtime
%systems, etc.

% So monitoring can refer to collecting and processing data at hardware level, different layers of the application stack, management services, security, packet-level telemetry from network switches, etc. 
%Monitoring infrastructure for a datacenter is required to report availability and performance problems at low latency to reduce the mean time to fault detection, and at high accuracy to reduce the possibility of false discoveries or faults remaining undetected. To satisfy dual requirements of accuracy and timeliness, existing monitoring systems are built to gain insights from continuous data streams generated across the system stack. In particular, 
The monitoring systems we target must be able to investigate timestamped measurement data from individual datacenter nodes corresponding to health of hardware, OS, and runtime systems~\cite{pingmesh, deepview, m3}, \emph{and/or} textual logs generated by a specific service which spans a large number of nodes to be hosted~\cite{philly, chi}.
Although numerous useful scenarios correspond to large-scale server monitoring in real world~\cite{helios,deepview,fingerprint}, we introduce the following two monitoring scenarios in an enterprise company that guide the design of \ours{}:
%Requirements for processing the collected monitoring data vary %substantially depending on the use case, data volume and %nature of data processing~\cite{slack-observability}.

\begin{myitemize}
\item \textit{Scenario 1:} Network team deploys PingMesh~\cite{pingmesh} agents on each datacenter node to collect probe latency data between server pairs. An internal Search team uses PingMesh to monitor network health of their latency sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold. The threshold is determined by the search service SLA.
    % Note that we also use this scenario to motivate our work and introduce \ours{} in Sections~\ref{sec:motivation} and~\ref{sec:jarvis}.
    % , to assist in debugging network issues for hosted applications.
\item \textit{Scenario 2:} A log processing system (e.g. Helios~\cite{helios}) enables live debugging of storage analytics services (e.g. Cosmos~\cite{cosmos}). A bug in cluster resource manager leads to service resources being under-provisioned. To temporarily mitigate performance degradation, multiple TBs of log streams~\cite{helios} are processed quickly to identify impacted tenants. Their latency and CPU/memory utilization data are queried to predict resource needs and make scaling decisions.

% The storage team has built a service (such as Cosmos~\cite{cosmos}) to enable users to write analytics jobs on their data. Logs generated by these jobs are processed to generate an alert if the job running times exceed user provided threshold. Users can request additional information like resource utilization extracted from the logs, to debug long running jobs.

    % \item \textit{Scenario 2:} Multiple product teams train ML models to integrate into their products. ML training jobs are run on a shared GPU cluster~\cite{philly,deep-learning-photographs,deep-learning-siri}. Jobs can fail due to many reasons as described in~\cite{philly} so to help prioritize failure categories to debug, job logs are processed to track percentiles for runtime to failure of different failure categories on a dashboard, using histogram-based estimation~\cite{prometheus-estimate-percentile}.~\todo{Need to fix this scenario}
\end{myitemize}

%Consider a large datacenter managed by an enterprise company/cloud provider. The internal monitoring team deploys a sophisticated data processing pipeline to support low latency monitoring needs of teams within the company, as shown in Figure~\ref{fig:arch}. Dashboards are created by users to monitor their services for different scenarios. We focus on the following types of monitoring scenarios in this paper: 
%\begin{myitemize}
%    \item \textit{Scenario 1:} Network team deploys PingMesh~\cite{pingmesh} agents on each datacenter node to collect probe latency data between server pairs. An internal Search team uses PingMesh to monitor network health of their latency sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold. The thresold is determined by the search service SLA.
%    % Note that we also use this scenario to motivate our work and introduce \ours{} in Sections~\ref{sec:motivation} and~\ref{sec:jarvis}.
%    % , to assist in debugging network issues for hosted applications.
%    \item \textit{Scenario 2:} The storage team has built a service (such as~\cite{cosmos}) to enable users to write analytics jobs on their data. Logs generated by these jobs are processed to generate an alert if the job running times exceed user provided threshold. Users can request additional information like resource utilization extracted from the logs, to debug long running jobs. 
%    
%    % \item \textit{Scenario 2:} Multiple product teams train ML models to integrate into their products. ML training jobs are run on a shared GPU cluster~\cite{philly,deep-learning-photographs,deep-learning-siri}. Jobs can fail due to many reasons as described in~\cite{philly} so to help prioritize failure categories to debug, job logs are processed to track percentiles for runtime to failure of different failure categories on a dashboard, using histogram-based estimation~\cite{prometheus-estimate-percentile}.~\todo{Need to fix this scenario}
%\end{myitemize}

The above scenarios require processing different types of monitoring data.
\textit{Scenario 1} requires processing metrics which are structured numeric data
and generated periodically. Queries on this
data consist of operations such as filtering and aggregation.
On the contrary, \textit{Scenario 2} requires processing logs which are unstructured strings
and are generated aperiodically. Queries consist of string processing
operations such as parsing, splitting, search, etc. We observe the following
common challenges facing modern monitoring pipelines in supporting the two
scenarios:
% The need for incorporating such a wide range of telemetry data is also well reflected by our recent conversations with datacenter operators, quoted as follows:

% \emph{``We collect more than 500 performance metrics to comprehensively
% diagnose HW issues across datacenter server, storage, and network. In
% addition, by collecting and analyzing scheduler logs and logs from their
% scheduled jobs, we identify platform issues that affect datacenter
% utilization''}

% \hfill -- A datacenter operator at \samsung{}


% We focus on the challenges in monitoring performance of datacenter applications which requires timely analysis of logs generated by application operations to detect errors~\cite{helios} as well as host-level metrics generated on underlying server nodes to monitor health of resources such as network latency, cpu and disk usage~\cite{pingmesh,deepview}. Such workloads are characterized by high data volume and high variability in data generation rates (details in Section~\ref{sec:background},\ref{sec:motivation}). 


%Among a number of performance metrics, we are primarily interested in the
%metrics for machine-generated, timestamped measurement data, e.g., network
%latency~\cite{pingmesh, tersecades} and HW performance counters~\cite{scuba,
%m3, philly}, which are the most common telemetry to inspect in the
%datacenter. There are typically hundreds of such metrics collected in each
%server.

%Figure~\ref{fig:arch} presents the overall architecture of a telemetry
%monitoring system deployed on a datacenter.
% Once data is generated by datacenter servers (or \emph{data source nodes}), they traverse a sophisticated monitoring pipeline deployed on a datacenter, as shown in Figure~\ref{fig:arch}. 

% \Paragraph{Voluminous data transfer:} Several production monitoring systems report unprecedented volume of data being produced at the \client{}. 
%, limiting the efficiency and
%scalability of monitoring systems~\cite{scuba, ddsketch, m3}.
\Paragraph{Voluminous data transfer:} A monitoring system must process
up to tens of TB data per day or millions of events every second per monitoring
task~\cite{chi, pingmesh, gandalf}, straining compute, memory, and network
capacities of the monitoring system. As an example, we illustrate how costly
data transfer can be for network latency monitoring in \textit{Scenario 1},
assuming a traditional approach where the entire data is aggregated into
\emph{stream processor} to be analyzed. Assume that a datacenter
has 200k servers. Guided by~\cite{pingmesh}, each server may probe 20k other
servers with a probing interval of 5 seconds. Then, the data generation rate
for this system alone is estimated at 512.6~Gbps as a result
of large-scale probing performed by 200K servers. Similarly, logs collected from
applications (as in \textit{Scenario 2}) can generate up to 971
Gbps~\cite{chi}. To keep up with these high data generation rates, stream processors need to employ a large number of compute cores, making it costly to build the monitoring system.
%Scaling to these rates using modern stream processors is
%prohibitively costly due to the lower (2–3 orders of magnitude) processing
%capacity per core~\cite{sparkstreaming,memcached-redis,kafka-benchmark}. 
This
pressing issue suggests that achieving high efficiency and scalability is a
key design challenge for large-scale server monitoring.
%Several real-world monitoring systems report data of the unprecedented volume
%of data to transfer from \client{} nodes to \server{}, limiting the
%efficiency and scalability of monitoring systems~\cite{scuba, ddsketch, m3}.
%To illustrate how costly data transfer is, let us take the network latency
%monitoring scenario as an example. We assume a probing interval of 10 seconds
%as used in~\cite{pingmesh} and a deployment of data collection pipeline on a
%large system with 200K servers. The data generation rate is estimated at
%0.82~TB per second as a result of a large-scale pairwise server probing among
%200K servers.

% \Paragraph{Highly varying data and workload:}
\Paragraph{Highly varying data:} Monitoring input data and their generation
rates vary significantly across different \client{} nodes.
Section~\ref{sec:motivation} describes in detail how metrics data differs
across \client{} nodes. Recent works~\cite{chi,helios} have also described
high variation in ingestion rates for log streams generated in production
monitoring systems. To keep up with high varying data, monitoring pipelines
are equipped with large amount of compute and memory resources, which are
highly distributed across dedicated nodes. To handle processing load from a
large number of \client{} nodes, the \server{} may integrate several levels
of computing nodes. Query optimization techniques need to support the
requirements of highly dynamic workloads in a complex distributed
environment.

% Furthermore, monitoring systems in large enterprises process a massive number of queries everyday, as reported by~\cite{m3}. Monitoring systems make it easy for engineers to express monitoring tasks over data streams of interest. So they can use a programming language they are familiar with, to issue several types of queries including standing queries for long-time monitoring tasks and custom/ad-hoc queries for analyzing time-sensitive data from logs. 


 

% It is reported that  M3 in Uber handles around 2500 queries per second across their metrics~\cite{m3}. 
% In network telemetry, Sonata~\cite{sonata} reports potentially thousands of monitoring queries that need to be executed concurrently.



% \textit{In this paper, we focus on the challenges associated with running continuous monitoring queries on large amounts of numeric or text streaming data being generated from datacenter nodes and being processed in a central \server{}}.



==> archive/cover_letter.tex <==
\begin{center}\Huge
Cover Letter
\end{center}

We thank reviewers once again for their valuable feedback and comments in helping improve the paper. Below, we describe each item for improvement and action item taken by us to address it. New content is in \textcolor{blue}{blue}.


\textbf{==== Reviewer 1 ====}
\begin{myitemize}
\item \Paragraph{O2: How frequently do monitoring workloads change?} 
Addressed by updating Section~\ref{sec:motivation} with specific examples and real-world systems which cause workload variability in order of minutes, along with justifications for why such frequencies are reasonable in server monitoring.
\item \Paragraph{O3: Compare with in-situ processing in MapReduce-like systems.}
We discuss design differences of works in in-situ processing against \ours{} in Section~\ref{sec:RelatedWork}.  
\item \Paragraph{O4: Compatibility with existing query engines.} Addressed in Section~\ref{sec:implementation}.
\item \Paragraph{O5: Compare control proxy with backpressure} Addressed in Section~\ref{sec:architecture}.
\item \Paragraph{O6: Why is Jarvis decentralized?} Addressed in Section~\ref{sec:architecture}.
\item \Paragraph{O7: Exactly-once processing semantics} We briefly describe our current thinking and direction for investigation in Section~\ref{sec:discussion}. Given more time, we intend make more progress in our study of fault tolerance mechanisms of existing stream processing engines.
\end{myitemize}


\textbf{==== Reviewer 2 ====}
\begin{myitemize}
% \todo{There is a bug in sampling algorithm (Algorithm 2) in the paper on continuous sampling from distributed streams that the reviewer referenced. Should we highlight it?}

% \item "Why these works were not discussed in the first place?" \\
% Thank you for all your helpful comments. We had discussed operator scaling and placement papers in Related Works section, mentioning that they are applicable for optimizations on the \server{} side in Jarvis. However, limitations in applying them for on \client{} nodes  were not highlighted so we have fixed that in the revised version. 

\item \Paragraph{O1: Comparison with related work in in-network processing} 
The entire related work section (Section~\ref{sec:RelatedWork}) is new. The section title is made blue to indicate the content is new. We have kept some major works from previous version but removed those that were less relevant due to space constraints. Below we explain how we addressed individual questions: 
\begin{myitemize}
    \item Question: For paper 1 and 4, why is an optimization problem being NP-hard a drawback?
    
    We explain why this would be an issue for our target monitoring systems in Section~\ref{sec:drawbacks}. We refer to this content when discussing papers which solve NP-hard optimization problem.
    \item Question: For paper 3, why can’t one simply run the algorithm, find a list of solutions and then discard those that do not satisfy compute node constraints?
    
    In Related Works Section~\ref{sec:RelatedWork}, we discuss the challenges with enumerating the list of solutions and checking for compute constraints for the algorithms discussed in paper 3. 
    
    \item Question: Why Jarvis’ problem setup is better suited for the studied environment, compared to works in data splitting across replicated operator instances?
    
    Work on load balancing across replicated operator instances is explained in detail in Section~\ref{sec:RelatedWork}. We then highlight our problem characteristics which are not considered by these works and thus, cannot be applied to our target systems. 
\end{myitemize}
\item \Paragraph{O2: Highlight research contributions} We have added content in Section III to highlight contributions and insights.  

\item \Paragraph{O3: Compare Jarvis with data synopses work}\\
We implemented the distributed sampling algorithm~\cite{continuous-sampling-streams} and evaluated its accuracy and savings in network transfer cost, on our query in Listing 1. A summary is provided in Section~\ref{sec:insights} and the analysis is discussed in Section~\ref{sec:evaluation}.  
\end{myitemize}


\textbf{==== Reviewer 3 ====}
\begin{myitemize}
    \item \Paragraph{O1: Consider moving Section II.D to Section III.} We removed the \ours{} insights out of Section II. It now focuses on the monitoring pipeline characteristics and Section III discusses the problem and strategies to address it. 
    \item \Paragraph{O2: Move choice of partitioning granularity and adaptation approach to Section III.} Fixed. We now have section III focusing on the problem definition and \ours{} insights. 
    \item \Paragraph{O3: State limitations and assumptions clearly.} Fixed. We added Section~\ref{sec:limitations} for \ours{} assumptions and limitations.
    \item \Paragraph{O4: Explain what transformations mean in the data partitioning optimization.}. Addressed in Section~\ref{sec:data-partitioning-problem}.
    \item \Paragraph{O5: Rewrite implementation section.}\\
    We added a discussion point about integrating \ours{} with other streaming engines. We also merged two of the implementation issues in the previous paper version (i.e., "Maintaining streaming semantics." and "Merging results at stream processor"). We now have a single point on "Accurate query processing". Due to space constraints, we removed the point on "Probing downstream queues" and moved it to extended paper version. We have also worked on improving language in this section. 
\end{myitemize}

==> archive/design-v1.tex <==
\section{Jarvis system}
\label{sec:jarvis}

% \ours{} allows each query to independently refine its execution for data partitioning without consulting any centralized query planner. 
\ours{} design extends conventional query computation graphs to be compatible with existing query engines that express query execution as a computation graph of stream operators. Since the extension is done after a query compiler constructs the query graph, \ours{} is fully transparent to users. In this section, we discuss \ours{} architecture, its overall design and an algorithm to achieve fast and accurate query refinement.
% programming model

\subsection{High-level Architecture}
\label{sec:architecture}
Figure~\ref{fig:arch-monitoring-scale}(a) shows a user-defined a query that is submitted to \ours{} \manager{}. \Manager{} consists of a Query Optimizer which performs query optimizations similar to those done by state-of-the-art streaming engines~\cite{flink}. %Custom optimizations are also introduced by \ours{} in this component. 
\Manager{} consists of a Resource Manager, which maintains the current list of \client{} and \server{} nodes, along with their network topology in a Resource Directory. Topology information is updated whenever nodes are added, modified, or removed. Query Optimizer uses the node topology to generate an optimized physical plan for each node. Query Deployer generates the executable code corresponding to the physical plan and deploys it on the stream processing engine running on each node. Figure~\ref{fig:arch-monitoring-scale}(b) shows how \manager{} interacts with \client{} and \server{} nodes. Our work in \ours{} focuses on changes to the query plan generation pipeline in Query Optimizer and runtime optimizations after queries are deployed on \client{} and \server{} nodes.
% Figure~\ref{fig:arch-monitoring-scale}(b) shows the high level architecture of the \server{}, \client{} and \manager{} nodes.
% We note that for \client{} and \server{} nodes, intermediate  when the query processing needs exceed available budget on a node, the remaining computation is done in its parent node. 

\begin{figure}
\centering     %%% not \center
\subfigure[]{\label{fig:b}\includegraphics[width=40mm]{fig/QueryManagerArch.pdf}}
\subfigure[]{\label{fig:a}\includegraphics[width=40mm]{fig/JarvisArchExtended.pdf}}
\caption{\label{fig:arch-monitoring-scale} (a) Architecture for \ours{} Query Manager, (b) Architecture for the full monitoring pipeline. SP refers to stream processor and $L_{0}$ to $L_{H}$ refer to the hierarchy levels in a tree topology of height $H$.}
\vspace{-0.7cm}
\end{figure}

To realize \datapart{} and fast query refinement, \ours{} adds two new primitives to the query processing pipeline: (i) \emph{\Proxy{}}, a unified abstraction for stream operator and (ii) \emph{\run{}}, a system runtime that coordinates executions of all \proxies{}. \Proxy{} is a light-weight operator bridging two adjacent stream operators and decides ``how many'' records shall be forwarded to the next downstream operator vs. drained to the remote \server{} node for processing. Therefore, \proxy{} implements \datapart{} at \emph{operator level}. \run{} interacts with all \proxies{} within the \client{} node to coordinate their \datapart{} actions, enabling a refinement plan at \emph{query level}.

\ours{} modifies the query optimization pipeline to enable adding \proxy{} between adjacent stream operators. The optimized query is deployed onto \client{} and \server{} nodes. Figure~\ref{fig:jarvis_query} illustrates the query plan deployed on \client{} and \server{} for the running example query presented in Figure~\ref{fig:pipeline_tor}. \run{} deployed at each \client{} configures \proxies{} to execute a \datapart{} plan. \run{} continually probes the state of \proxies{} to observe their query state. If it detects changes to query resource conditions, a new \datapart{} plan is computed for the query. 
% Note that all partitioning decisions are made locally on each \client{} without relying on an external planner nor requiring coordination between \client{} and \server{}. 

\newcontent{
\subsection{Design considerations}
\label{sec:design-considerations}
\run{} is fully decentralized, i.e., each instance of the query on a \client{} has a dedicated runtime instance which functions independent of other query instances and \client{}s. Its interactions with \proxies{} are also local to the node, requiring no coordination with an external planner or the \server{}. This design avoids potential bottlenecks (e.g., from a central service performing joint optimization across queries and \client{}s~\cite{sonata}) to scaling the system when more \client{}s are considered. 

Existing backpressure mechanisms~\cite{flink-backpressure} enable detecting and mitigating over-subscription of node compute resources. However, they are challenging to apply to our target system (e.g., our focus on lossless monitoring means throttling source rate is not feasible as data loss can result due to \client{}s not being persistent). Section~\ref{sec:RelatedWork} provides more details. \Proxies{} enable an alternative mechanism to handle backpressure, by draining excess records to remote \server{} node. But in coordination with \run{}, it also provides two additional features: (1) enables implementing a \datapart{} plan to reduce network transfer costs, (2) enables quickly updating partitioning plan when resource conditions change. 
}

\subsection{Query Plan Generation}
\label{sec:query-plan-generation}
Monitoring queries may consist of sequence of operators; complex queries may join results of two different sub-queries~\cite{sonata}. Given the difference in compute capabilities and limitations in type of operations that can run on \client{} and \server{}, Query Optimizer generates custom query plans to deploy on the nodes. 

% \ours{} generates two separate physical plans: one for root \server{} and one for remaining \client{}/intermediate \server{} nodes. The details on physical plan generation are further described in Section~\ref{sec:query-plan-gen}.

\begin{figure}
  \centering
    \includegraphics[width=0.48\textwidth]{fig/jarvis}
    \caption{\ours{} rewrites query to incorporate \proxies{} and \run{}.
    Data path: routing path for incoming data; Control path: interaction between \proxies{} and \run{}.
    %\client{} side dataflow implementation of SQL query which involves filter and groupby operators on data stream coming from source. The control proxy uses the monitored backpressure at each operator queue to make routing decision. One route leads to the next dataflow on the \client{} and the other leads to uploading of data reaching the queue to the \server{}
    }
    \label{fig:jarvis_query}
    \vspace{-0.7cm}
\end{figure}

% We provide an overview of different design components within \ours{} and 
% \Paragraph{Query optimizer:} 

% We leverage common logical optimizations done by existing optimizers including constant folding, predicate pushdown, Boolean expression simplification, etc.
We reuse the query plan generation mechanism for existing streaming engines~\cite{calcite}. The input query is parsed to do syntactic checks and then logical optimizations (e.g., constant folding, predicate pushdown) are introduced to produce a logical plan. The optimized logical plan is used to generate a physical plan for deployment and execution. \ours{} additionally inserts a \proxy{} between each of the adjacent stream operators in the logical plan, for deployment to \client{} and intermediate \server{} nodes. 
% Multiple physical plans are then generated for the logical plan and execution cost of each plan is evaluated using a cost model. The best physical plan is picked for code generation and deployment.
\run{} is also deployed on \client{}s. Certain operations such as non-incremental updates cannot be supported in the \client{} and intermediate \server{}s. 
% since they perform incremental computation. 
Resource constraints further limit the operations that can be supported on \client{}s. \ours{} performs rule-based physical optimizations to account for such constraints. We describe below the rules to identify operations which \textit{cannot} execute on \client{}s: 

% To generate a physical plan, we need to account for \client{}s and intermediate \server{} nodes being limited in the type of operations that they can execute.  \ours{} does this by identifying operations that \textit{cannot} execute on \client{}s/intermediate \server{}s using rule-based physical optimization. 

\begin{myitemize}
\item \textit{[Rule 1]} Aggregation operations that are not incrementally updatable, such as exact quantiles. However, their approximate versions, such as approximate quantiles~\cite{aomg,prometheus-estimate-percentile}, can benefit from \ours{}. 
\item \textit{[Rule 2]} Downstream operators succeeding stateful operations that require aggregation across multiple \client{}s. 
\item \textit{[Rule 3]} Stateful joins across streams. Prior work~\cite{sonata} has also excluded such operations because they are expensive and may not reduce data that needs to be sent out of \client{}. 
\item \textit{[Rule 4]} Multiple physical operators for the same logical operator, which parallelize operator execution (e.g.~\cite{ds2}). \Client{}s have constrained compute budget; hence, benefits of exploiting operator parallelism are limited.
% \item Unlike works such as~\cite{ds2} which parallelize operators in query physical plan to improve performance, \ours{} does not parallelize operators because of limited compute resources on \client{}
\end{myitemize} 

\newcontent{\ours{} supports the extension of above rules via an user-provided configuration file.} All rules except the fourth rule apply also to intermediate \server{}s. As the latter are dedicated to run monitoring queries, hardware-level parallelism can be exploited to accelerate query operators. 
It may appear that the first rule limits queries that can leverage \ours{}. However,  a significant number of real-world queries use operators that support incremental updates. For example, Drizzle~\cite{drizzle} has reported 95\% of aggregation queries on a popular cloud-based data analytics platform consist of aggregates supporting incremental updates, such as sum and count. 

% It is possible to support such scaling because \ours{} introduces \proxy{} into the logical plan.

We note that after applying above rules, queries deployed on \client{}s typically consist of sequences of operators. Hereafter, while discussing query refinement on \client{}s, we restrict our discussion to operator sequence graphs. Nevertheless, our approach is extendable to handle graphs with split patterns that may execute on \client{}s---i.e., one operator output is an input to multiple downstream operators, and we leave this for future work.  

% Such a transformation of the query to construct a new computation pipeline enables performing data partitioning and query refinement in an efficient manner. 

\subsection{Dynamic Query Refinement}
\label{sec:dynamic-refinement}
After queries are deployed, a \datapart{} plan is implemented by \run{} by guiding each \proxy{} to select a portion $p$ (i.e., 0 $\leq p \leq$ 1) of incoming data to be inserted to the downstream queue and subsequently consumed by the downstream operator. Remaining data is drained over the network to be processed by the \server{} is routed to the \proxy{} associated with the same downstream operator. Hereafter, we refer to the $p$ value configured for each \proxy{} as its \emph{load factor}. 
% The above workflow applies to all \proxies{} that work independently.
% A \proxy{} in the \client{} node hooks the communication of two neighboring operators. 



% Guided by a query refinement algorithm (see Section~\ref{sec:dynamic-refinement}) which runs locally, \run{} decides $p$ values of individual \proxies{} to produce most network traffic reduction under given compute budget. 

%While \proxy{} do exist in both \client{} and \server{} nodes, for brevity,
%we henceforth use the term \proxy{} to mean one placed at \client{} node,
%unless specified otherwise.


%To initiate query refinement and steer its frequency, the data source emits
%strict monotonic event called watermark. An input stream to a monitoring
%query is an unbounded sequence of records produced in the data source node.
%Watermarks into records subsequently create ordered consecutive \emph{epochs}
%of records. \run{} initiates congestion control and refines the query
%execution plan upon receiving every epoch.

% \subsection{Rules For Query Plan Generation}
% \label{sec:query-plan-gen}

Unlike prior work that physically splits a query, our query partitioning scheme ``replicates'' query operators across the nodes. This approach simplifies scenarios that require switching to a new partitioning plan by locally updating \p{}s of each \proxy{}. \run{} orchestrates \p{}s through query refinement at an epoch granularity. During epoch processing, each \proxy{} monitors its downstream operator, and at the end of each epoch, it updates the state of the operator to one of three states: (i) \emph{Congested}: operator contains more than a predefined number of
pending records, experiencing backpressure; (ii) \emph{Idle}: operator
stays empty for longer than a predefined time duration; and (iii) \emph{Stable}:
operator is neither congested nor idle. \run{} collects state information
from all \proxies{} per epoch and classifies current \datapart{}
plan as \emph{non-stable} if all operators are idle or at least one operator
is congested. Upon identifying the query as non-stable, \run{} triggers adaptation to bring the query back to the stable state.
% An accurate data partitioning plan leads to the most network traffic reduction while keeping the query stable within the current compute budget. 
% However, computing this plan requires accounting for operator resource usage, data reduction rate and per-query resource budget that changes over time.
\begin{figure}
  \centering
    \includegraphics[width=0.48\textwidth]{fig/JarvisStateMachine.pdf}
    \caption{\run\ state machine.}
    \label{fig:jarvis_state_machine}
    \vspace{-0.7cm}
\end{figure}

Figure~\ref{fig:jarvis_state_machine} shows the interplay between \run{} and \proxies{} and the overall workflow with different operational phases:
% We explain below how \run{} transitions among the different operational phases:
%\run{} keeps a logical timestep to track the
%progress of epochs upon receiving refinement watermarks. The following
%explains how \ours{} transitions among the phases:

\begin{myitemize}

    \item \textbf{Startup: initialization.} All \p{} values are initialized to
    0 (the smallest value), so all stream records are processed by \server{}.

    \item \textbf{Probe: normal operation.} At the end of every epoch, \run{}
    executes \texttt{ProbeCP()} function to query all \proxies{} and
    determine their congestion states. It continues to do so until it
    identifies the computation pipeline as congested or idle. After that,
    the runtime enters \texttt{Profile} phase.

    \item \textbf{Profile: query plan diagnosis.} When the query is congested/idle, \ours{} obtains new estimates for the following during profiling phase: (1) compute cost of each operator by executing an operator at a time on the incoming epoch, (2) reduction in size of input stream by executing each operator, and (3) available compute budget for the query. These estimates are used to adapt load factors in the next \texttt{Adapt} phase.\footnote{Profiling estimates can still improve convergence time even if they do not exactly match the compute cost during normal operation (Section~\ref{sec:data-partitioning-problem}.)}.
    % Relay ratios are also estimated at each operator.
    % by our LP solver and thus improve convergence time to bring query back to stable state.

    \item \textbf{Adapt: load factor adaptation.} After profiling, \run{} executes an adaptation algorithm for computing a new \datapart{} plan. Initial \p{}s are first calculated using the profiling estimates and set for each \proxy{}. \run{} executes \texttt{ProbeCP()} to probe the query state and perform iterative fine-tuning if necessary, until the computation pipeline is back to stable state. At this point, it returns to \texttt{Probe} phase. %The adaptation algorithm is described in detail in Section~\ref{sec:data-partitioning-problem}
    % LP solver is first run to obtain
    
    % When the runtime enters adaptation phase from probing, it first executes $\texttt{calib   rate()}$ to obtain the latest data reduction ratios for each control proxy.

        % It does so by first executing $\texttt{calibrate()}$ to calibrate the query
        % for identifying subqueries/operators that result in data reduction
        % and then resetting the load factors to  $p_{min}$. It then updates
        % the control knobs for the next time step (which is denoted by $p_i
        % => p_{i+1}$ in Figure~\ref{fig:runtime-state-machine}).
\end{myitemize}

% If compute resource variability is small, it suffices for \run{} to start
% with the current partitioning configuration of operators and only fine-tune
% \p{} values to quickly converge to stable state. In this case, \run{} skips
% the \texttt{Profile} phase and does not run the LP solver. To detect
% variability, \run{} tracks the degree to which congestion state has changed
% in the current epoch, compared to previous epoch. It does so by measuring
% change in the number of records drained as well as change in idle duration
% for the query. If either change is within a certain level (10\% in our
% system, but configurable), then \run{} performs fine-tuning only.

%We use \texttt{ProbeCP()} to determine the congestion state of \proxies{},
%but the control system can result in oscillating behavior if the probing is
%sensitive to small changes in congestion state.

Small workload variation when in congested state or idle state can trigger a series of profile-adapt phases that put the control system in an oscillating behavior with small implications on the optimal load factors. To avoid this undesired behavior, each \proxy{} is configured with a threshold fraction of epoch records (\texttt{DrainedThres}) that can be drained by \proxies{} and tolerated by \texttt{ProbeCP()} without signaling congested state. Similarly, each \proxy{} is configured with a threshold fraction of epoch duration (\texttt{IdleThres}) that allows \proxies{} to stay idle and can be tolerated by \texttt{ProbeCP()} without signaling idle state. 

% Following that, we define \emph{\boundaryop{}} as an
% operator that is the target for fine-tuning. 

\begin{figure}
  \centering
    \includegraphics[width=0.4\textwidth]{fig/jarvis_parameters}
    \caption{Computation graph of M operators and parameters used by \ours{} for updating load factors in \proxies{}.}
    \label{fig:jarvis_parameters}
    \vspace{-0.4cm}
\end{figure}

Supporting multiple queries in \client{}s requires that a single \run{} instance is dedicated to a single individual query; each instance refines its query independently. When allocating the compute budget of \client{} node to the competing monitoring queries, \ours{} uses a popular fair resource allocation policy, such as non-weighted max-min fairness~\cite{minmax} without any loss in generality. Available budget per query is obtained by considering the number of queries and total compute available for the queries on \client{} node. %Consequently, \run{} instances do not need cooperation. 

% Stavros comment: This does not make any sense to me. Sharing compute resources across query operators is the essence of the paper. Why do we need to repeat ?

%Furthermore, operators within a query share compute resources, and we explain in the next section how \ours{} assigns processing load to each operator to minimize network data transfer without over/under-subscribing allocated resources. Note that although the illustration above is mainly focused on compute resource changes, our approach applies to a variety of variability sources such as input data generation rate.

\subsection{Computing \DataPart{} Plan}
\label{sec:data-partitioning-problem}
\run{} in its \texttt{Adapt} phase needs to compute a new \datapart{} plan to bring the query back to stable state. This is done by solving an optimization problem to compute initial \p{}s and then iteratively fine-tuning \p{}s if needed, to stabilize the query. %We now formalize the \datapart{} problem and discuss the fine-tuning algorithm. 

\subsubsection{Problem Definition}
\label{sec:problem-definition-opt}

\begin{table}
\begin{tabular}{ |p{0.3cm}|p{7.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Summary of variables used in the paper} \\
 \hline
 $M$ & Number of operators in the query\\
 $N$ & Total number of records injected into the query in an epoch\\
%  $b_i$ & $b_i \epsilon [0,M]$ to denote the index of boundary operator where the partitioning occurs for $i^{th}$ \client{}\\
%  $B$ & partition profile for the query with $b_i$ denoting boundary operator for $i^{th}$ \client{}\\
 $Op_{i}$ & $i^{th}$ operator in the query\\
 $r_{j}$ & Relay ratio of $Op_{j}$ i.e. fraction of input records relayed to the next operator $Op_{j+1}$ after they are consumed by $Op_{j}$\\
 $c_i$ & Compute cost of $Op_{i}$ for a single record\\
 $d_{i}$ & Number of records drained in an epoch, at the $i^{th}$ \proxy{}\\
 $C$ & Compute budget available to the query\\
 $p_{i}$ & $i^{th}$ \proxy{}'s load factor i.e. fraction of input records added to downstream queue and consumed by downstream operator\\
 $e_{i}$ & Effective load factor for $i^{th}$ \proxy{} i.e. product of load factors of sequence of upstream query operators until $Op_{i}$, in the transformed optimization problem\\

 \hline
\end{tabular}
\caption{\label{tab:notation}}
\vspace{-0.5cm}
\end{table}

Consider a computation pipeline as shown in
Figure~\ref{fig:jarvis_parameters} which contains $M$ operators. Table~\ref{tab:notation} summarizes the variables used. For each \proxy{}, guided by its \p{}, a record will be
either pushed to the downstream operator or drained. We want to minimize
the total number of drained records (i.e. $\sum_{i=1}^{M}d_i$) from \client{} given the compute budget $C$ available to the query. This yields the following optimization formulation: % for an epoch:
\begin{align*}
    \min_{p_{1},p_{2},...p_{M}}
    &\sum_{i=1}^{M}[\prod_{j=0}^{i-1}p_{j}r_{j}](1-p_{i}) \numberthis
    % &N(1-p_{1}(1-r_{1}(1-p_{2}...(1-r_{M-1}(1-p_{M}))..) \numberthis
    \label{eq:optimization-obj}
\end{align*}
subject to
\begin{align*}
    &\sum_{i=1}^{M}[\prod_{j=0}^{i-1}p_{j}r_{j}] p_{i}c_{i} \le C/N, \numberthis\\
    % &p_{1}N(c_{1}+p_{2}r_{1}(c_{2}+...p_{M}r_{M-1}c_{M})...) \le C\\
    &0 \le p_{i} \le 1,\ 0 \le r_{i} \le 1,\
    % 0 \le c_{i} \le 100/N\ \forall\ i\
    c_{i} \geq  0\ \forall\ i\
    \epsilon\ [1,M], p_{0}=1, r_{0}=1
    %&0 \le r_{i} \le 1\ \forall\ i\ \epsilon\ [1,M],\\
    %&0 \le c_{i} \le 100/N\ \forall\ i\ \epsilon\ [1,M]
    %\label{eq:optimization-constr}
    \vspace{-1cm}
\end{align*}
%where,
%\begin{align*}
%    &p_{i}\ \forall\ i\ \epsilon\ [1,M]\ \mathrm{are\ the\ optimization\ variables}\\
%    &p_{0}=1,r_{0}=1\\
%    &N,\ M,\ C,\ r_{i}\ \&\ c_{i} \forall\ i\ \epsilon\ [1,M] \mathrm{\ are\ constants}
%\end{align*}

\noindent 
$N$, $M$, and $C$ are fixed for an instance of the problem. 
% In summary, the objective function minimizes total size of drained data from each of the \proxies{} subject to the compute budget $C$ available to the query.

Unfortunately, there are two challenges in solving this optimization problem. First, it can be proved that Hessian matrix is not positive semi-definite even for the two-variable cases, resulting in a  computationally hard non-convex formulation~\cite{boyd-opt}. While it is possible to enumerate
all possible combinations of load factor values, doing so is expensive for online optimization. Second, the formulation assumes certain conditions, which may not always be satisfied in practice. For instance, to estimate $c_i$ accurately, each operator needs to be evaluated on a sufficient number of input records. As seen in Section~\ref{sec:background}, for grouping operation, $c_i$ is affected by the number of groups in input data which can change at runtime. Furthermore, relay ratio $r_i$ can vary non-linearly for grouping, as it is affected by grouping key distribution in the input.

%\begin{itemize}
%    \item Accurately estimating the execution cost per record of an
%        operator $c_i$ is hard. As we have seen in
%        Appendix~\ref{sec:characteristics}, such a cost depends on the
%        input data characteristics, which can change at runtime.
%        Furthermore, estimating the cost at runtime is complicated by (i)
%        non-linear behavior of computation cost with input data size, (ii)
%        performance interference in multi-query settings on \client{} node.
%    \item Relay ratio $r_i$ can vary non-linearly with the input data size.
%        In case of grouping operator for example, relay ratio is affected
%        by the grouping key distribution in input data. So depending on the
%        load factor of an operator, its $r_i$ values may change
%        non-linearly.
%    \item The total compute cost $C$ available for a query is not known.
%        Because it depends on the set of monitoring queries executing on
%        \client{} node which can change frequently \todo{Add citation} as
%        well as how underlying scheduler allocates resources to each query.
%\end{itemize}

\subsubsection{\algo{} Algorithm} We now describe how \ours{} deals with the \datapart{} problem. \ours{} employs our \emph{\algo{}}, a novel hybrid algorithm that combines two techniques: (i) a model-based technique which searches for near-optimal \p{}s based on the modeling assumptions of the \datapart{} problem defined in Equation~\ref{eq:optimization-obj}. %It overcomes the large amount of computation needed for estimating \p{}s during online adaptation; 
and (ii) a model-agnostic technique that monitors query execution using load factors obtained from step (i) and fine-tunes them if the query behavior deviates considerably from stable state---i.e., the available resources are either over/under-subscribed by the query.
% a model-agnostic technique that configures the system with obtained \p{}s from step (i) and monitors its query execution, and finally fine-tunes \p{}s when the query behavior deviates significantly from the model, overcoming  the observed query instability. 
For fast fine-tuning, step (ii) uses a heuristic inspired by first fit decreasing heuristic for bin packing problem~\cite{first-fit-bin-pack}, to prioritize \p{} updates of operators that contribute significantly to network data reduction.

\newcontent{To efficiently solve the optimization in Equation~\ref{eq:optimization-obj}, we consider if a transformation (i.e., change in optimization variables) exists to make the objective and constraint functions convex.}
\ifthenelse{\boolean{Extended}}{For example, we transformed the problem to a geometric program (GP)~\cite{gpsolver} for a small scale instance of the problem with just 2 optimization variables. When varying different parameters in the optimization, GP solver takes up to 7 seconds for solving the problem using CVXOPT solver~\cite{cvxopt} on a machine with four 2-GHz i7 CPUs. This is expensive for the fast convergence requirement of query refinement. To enable online optimization, we thus identified another simple transformation of the original problem that converts it into a linear program (LP).}
{\newcontent{We analyzed the performance of optimization solvers on problem formulations resulting from different transformations (details in~\cite{jarvis-extended}).} Based on our analysis, we settled on a transformation which yields a linear program(LP) to enable fast online optimization.}
The transformation is done by introducing a new optimization variable $e_i$ for the $i^{th}$ \proxy{} where $e_i=\prod_{j=0}^{i}p_j$. Then the optimization problem in Equation~\ref{eq:optimization-obj} can be rewritten as: 
\begin{align*}
    \min_{e_{1},e_{2},...e_{M}}
    &\sum_{i=1}^{M}[(\prod_{j=0}^{i-1}r_{j}).(e_{i-1}-e_{i})] \numberthis
    \label{eq:optimization-obj-linear} 
\end{align*}
subject to
\begin{align*}
    &\sum_{i=1}^{M}[(\prod_{j=0}^{i-1}r_{j}).e_i.c_i] \le C/N,\\
    % &p_{1}N(c_{1}+p_{2}r_{1}(c_{2}+...p_{M}r_{M-1}c_{M})...) \le C\\
    &0 \le e_{i} \le e_{i-1}\ \forall\ i\ \epsilon\ [1,M],\ e_{0} = 1
    %\label{eq:optimization-constr-linear}
\end{align*}
%where,
%\begin{align*}
%    &e_{i}\ \forall\ i\ \epsilon\ [1,M]\ \mathrm{are\ the\ optimization\ variables}, \\ 
%    &\&\ e_{0}=1
%\end{align*}
\noindent
Rest of the conditions on $N, M, C, c_i, r_i$ remain the same as in the original formulation. When a resource change occurs on \client{}, \p{}s need to change to stabilize the query. 

% stavros: cited this in fine-tuning strategy where we say that we update load factors obtained in the previou step (per LP solver)
%Fine-tuning can take a long time to converge if it starts with the current \p{}s, especially when large resource changes require \p{}s to change significantly. Instead, initializing \p{}s with the LP solver output enables faster convergence because the new cost estimates in LP reflect the resource change that occurred on \client{}.

A feasible solution provided by LP solver assumes that operator relay ratios/costs of operators are fixed and independent of load factors. However, if these parameters are unsteady or vary non-linearly, the solver provides \p{}s which would either over-subscribe or under-subscribe the compute budget, making the query execution unstable. To address the issue, \algo{} takes a post-LP solver step to further tune the \p{}s. In this step, \algo{} observes the congestion state of the query after it executes an epoch with current \p{}s of \proxies{} and updates them based on priorities of their downstream operators. An operator that has the \emph{lowest} data relay ratio is assigned the \emph{highest} priority, and \algo{} aims to increase its \p{} first when a query is in idle state. For a query in congested state, \p{} for the operator in the lowest priority will be decreased first. In this way, we can give more resources to operators that potentially bring about larger data reduction. All the information necessary for \algo{} is unknown beforehand, but can be readily obtained with profiling. Note that a high priority operator may have a high compute cost, but since our objective is to minimize the network transfer cost within the compute budget, we choose to find the smallest number of \p{} updates to fully utilize available compute.

% Note that while increasing load factors because the query is in idle state, the high priority operator is the one with lowest relay ratio, even if it has a large compute cost. This is because our objective is to minimize the network cost given a fixed compute budget, so we want to find the smallest number of \p{} updates to fully utilize the available budget and minimize network cost. A similar argument applies for a query in congested state reducing load factors. We validated this observation in a simulator that simulates the optimization problem defined earlier. 

\Paragraph{Fine-tuning strategy.} We update load factors obtained in the previous step (per LP solver) based on operator priorities, which are determined based on relay ratio of each operator. If a query is idle, we increase the load factor for the highest priority operator that is not fully executing yet---i.e., $p <1$. In contrast, if a query is congested, we reduce the load factor for the lowest priority operator that is still executing---i.e., $p > 0$. When updating \p{}s for an operator, we execute a binary search over discretized \p{} values of the operator to improve convergence time---i.e.,  from the current \p{} to the maximum value in
idle state or to the minimum value in congested state.

\section{Assumptions and limitations} \textcolor{blue}{Below we discuss the assumptions and limitations of \ours{}:
\begin{myitemize}
\item Our greedy approach may incur processing latency overhead. This overhead can be limited by configuring the epoch size for making partitioning decisions.
\item When \client{} resource conditions change (e.g. due to change in input stream characteristics), we assume stable workload characteristics during the time when \ours{} profiles and adapt to the new resource conditions. Our evaluation shows \ours{} can take up to 7 seconds for the query to stabilize during adaptation, which is less than 11\% of the time interval for resource changes to occur (i.e., in the order of minutes: Section~\ref{sec:motivation}).
\item Opportunities for sharing operators across multiple queries are not explored in this paper and left for future work. Operator sharing can significantly reduce compute usage costs in different scenarios, e.g., multiple queries sharing operator logic and computing query output over windows of increasing size (large windows can reuse output of smaller windows)~\cite{mqo,sbon}.
\end{myitemize}
}

==> archive/evaluation-v1.tex <==
\section{Evaluation}
\label{sec:evaluation}
We evaluate the effectiveness of \ours{} in improving the system throughput and in quickly adapting query partitioning plans to dynamic resource conditions at the~\client{}.
%\subsection{Experimental Setup}
\subsection{Methodology}
\label{sec:exp-methodology}
\Paragraph{Testbed setup.} For experiments in Section~\ref{sec:query-throughput-comparison},~\ref{sec:convergence-cost-eval} and~\ref{sec:scalability-analysis}, we deploy our \client{} on Amazon EC2
t2.micro nodes, each with one Intel Xeon E5-2676 core operating at 2.4GHz and 1 GB RAM running Ubuntu 16.04. For the experiment of multiple queries in Section~\ref{sec:multiple-nodes-eval}, we exercise 2 \client{} cores by deploying Amazon EC2 t2.medium node with two Intel Xeon E5-2686 cores operating at 2.4 GHz and 4 GB RAM, running Ubuntu 16.04. A \server{} instance is deployed on an Amazon EC2 m5a.16xlarge node with 64 AMD EPYC 7000 cores operating at 2.5GHz, with hyper-threading disabled, and 256 GB of memory running Ubuntu 16.04. \Client{} nodes are connected to \server{} with 12~Gbps Ethernet link. We use \emph{cpulimit}~\cite{cpulimit} to control the available compute budget for a query running on a \client{} node and \emph{wondershaper}~\cite{wondershaper} to shape the effective uplink bandwidth of a single \client{} node. 

%But, we restrict the upload rate on the \client{} node to 20.5 Mbps per
%query, we describe below how we arrive at this number.

%For each \client{} node, Apache MiNiFi runs a custom processor configured to
%execute a single concurrent task. For each \server{} node, Apache NiFi runs
%a custom processor configured to execute five concurrent
%tasks.

We conduct our experiments on two types of setups: (i) a single \client{}
node connected to a single \server{} node to evaluate performance of partitioning and adaptation strategies in \ours{}, and (ii) multiple \client{}s (up to 250 nodes) connected to a single \server{} node to evaluate \ours{} as we scale number of \client{}s. For each experiment, the first three minutes are used to warm up the system and the next five minutes are used to obtain performance results. 

\Paragraph{Performance metrics.}
We measure \textit{query processing throughput} in Mbps (megabit per second) with a latency bound of 5 seconds, \textit{epoch processing latency} in seconds, and \textit{convergence duration} in number of epochs after resource conditions change.   

% Note that \server{} can be multi-staged to deal with high fan-in traffic.
% Thus, in a real setup, there exist a number of intermediate \server{} nodes
% which are the workhorse of telemetry system. Each intermediate node manages a subset of
% \client{} nodes whose size is limited by its processing capacities for
% telemetry tasks associated with the \client{} nodes.

% and using a cluster of 1,000 \client{} nodes:
% Section~\ref{sec:scalability} discusses the cluster experimental results.
%connected to \server{} running on XX nodes.
 
%So in a real setup, there exist intermediate aggregation nodes which are
%medium sized (e.g., with capacities for each node equivalent to Amazon EC2
%t2.medium instance). Each node collects partial query results from a disjoint
%subset of \client{} nodes and sends either the final query results or any
%still unprocessed records to the stream processor, reducing as much inbound
%network traffic to the stream processor as possible. In doing so, each node
%simply runs a \ours{} instance. So the focus of our multi-\client{}/single
%\server{} node setup is to study the scalability in one level of aggregation
%hierarchy, which can be naturally extended to multiple levels given the
%design of \ours{}.

%Each \client{} node either replays trace records or generates synthetic
%records, and pushes them into a given computation pipeline in an open loop.
%The input rate is expressed as megabits per second (Mbps).

%We use the following testbeds/simulator to evaluate Jarvis at different
%scales:
%\begin{itemize}
%    \item Single \client{} testbed: One \client{} node
%        connected to a single \server{} instance for central
%        processing
%    \item Large scale testbed: 1,000 \client{} nodes connected to
%        100 \server{} instances for central processing
%    % \item Simulator: 250,000 \client{} nodes connected to 1000 \server{} instances
%\end{itemize}

\Paragraph{Workloads.} We use two datasets: (i)
\textbf{\pingmesh{}} dataset as described in Section~\ref{sec:background} and (ii) text-based logs \textbf{\dnnlog{}} which includes tenant name, job running time in milliseconds along with CPU and memory utilization for handling tenant-wise performance issues for jobs running in an analytics cluster. We run the following queries:

\begin{myitemize}
\item \textbf{\qone{}} (Listing~\ref{lst:motivating-query}) that runs on \pingmesh{} dataset, with the filter predicate delivering 14\% filter-out rate. 
\item \textbf{\qtwo{}} (Listing~\ref{lst:tor-level-count-probe}) that runs on \pingmesh{} dataset. It uses join operator to measure network latency aggregates for ToR-to-ToR pairs by joining the input stream with a table that maps server IP address to its ToR switch ID. 
\item \textbf{\dnnlog{}} (Listing~\ref{lst:dnnlog-query})  that runs on \dnnlog{} dataset. It parses unstructured logs to extract per-tenant latency and resource utilization. It then bucketizes the data to output histograms for tenant-wise job latencies and resource utilization.
\end{myitemize}

% \begin{figure*}[t]
% \begin{multicols}{3}
%     \includegraphics[width=\linewidth]{fig/pingmesh-plot-partitioning-thruput.pdf}\par\caption{\label{fig:pingmeshquery1-throughput}\qone{} throughput.}
%     \includegraphics[width=\linewidth]{fig/tor2tor-partitioning-thruput.pdf}\par\caption{\label{fig:pingmeshquery-tor-throughput}\qtwo{} throughput. Stream joined with table of size 500.}
%     \includegraphics[width=\linewidth]{fig/wordcount-plot-partitioning-thruput.pdf}\par\caption{\label{fig:wordcount-throughput}\dnnlog{} throughput.}
% \end{multicols}
% \vspace{-0.4cm}
% \end{figure*}

\begin{figure}
    \includegraphics[width=\linewidth]{fig/all-partitioning-thruput.pdf}\caption{(a) \qone{} throughput, (b) \qtwo{} throughput. Stream joined with table of size 500, (c) \dnnlog{} throughput.}
    \label{fig:all-throughput}
\vspace{-0.4cm}
\end{figure}

\begin{lstlisting}[caption={A temporal query for ToR-to-ToR latency probing. $m$ is a table to map server IP address to its ToR switch ID.}, label={lst:tor-level-count-probe}]
Stream
.Window(10_SECONDS).Filter(e => e.errorCode == 0)
.Join(m, e => e.srcIp, m => m.ipAddr, (e,m) => (e, srcTor=m.torId))
.Join(m, e => e.dstIp, m => m.ipAddr, (e,m) => (e, dstTor=m.torId))
.GroupApply((e.srcToR, e.dstToR))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
\end{lstlisting}

\begin{lstlisting}[caption={A text query for computing histogram data for per-tenant analytics job latency and resource utilization. JobStats is an object to store job related information.}, label={lst:dnnlog-query}]
patterns={"*tenant name*", "*job running time*","*cpu util*","*memory util*"}
Stream
.Window(10_SECONDS)
.map(l -> l.trim().toLowerCase())
.filter(l -> patterns.stream().anyMatch(s->l.contains(s)))
.map(j -> new JobStats(j.split('=')))
.map(j -> j.stat = width_bucket(j.stat, 0, 100, 10))
.groupapply(j.tenant_name,j.stat_name, j.stat)
.aggregate(c -> c.count())
\end{lstlisting}

\begin{myitemize}
\item \qone{}, described in Listing~\ref{lst:motivating-query}, running on \pingmesh{} dataset, with the filter predicate delivering 14\% filter-out rate. 
\item \qtwo{}, described in Listing~\ref{lst:tor-level-count-probe}, running on \pingmesh{} dataset. It uses join operator to measure network latency aggregates for ToR-to-ToR pairs by joining the input stream with a table that maps server IP address to its ToR switch ID. 
\item \dnnlog{}, described in Listing~\ref{lst:dnnlog-query},  running on \dnnlog{} dataset. It parses unstructured logs to extract per-tenant latency and resource utilization information. It then bucketizes the data to generate histograms for tenant-wise job latencies and resource utilization.
\end{myitemize}

% \begin{figure*}[t]
% \begin{multicols}{3}
%     \includegraphics[width=\linewidth]{fig/plot-pingmesh-convergence-v2-num.pdf}\par\caption{\label{fig:convergence-pingmesh}\qone{} convergence.}
%     \includegraphics[width=\linewidth]{fig/plot-pingmesh-torcountonly-jointable50-500-convergence-v2-num.pdf}\par\caption{\label{fig:convergence-pingmesh-tor} \qtwo{} convergence.}
%     \includegraphics[width=\linewidth]{fig/plot-wordcount-convergence-v2-num.pdf}\par\caption{\label{fig:convergence-wordcount} \dnnlog{} convergence.}
% \end{multicols}
% \vspace{-0.4cm}
% \end{figure*}

\begin{figure}
    \includegraphics[width=\linewidth]{fig/all-plot-convergence-v2-num.pdf}\caption{(a) \qone{} convergence, (b) \qtwo{} convergence. (c) \dnnlog{} convergence.}
    \label{fig:all-convergence}
\vspace{-0.4cm}
\end{figure}


For \pingmesh{}, we assume latency probing in a large-scale datacenter where more frequent probing occurs to include enough data for statistical significance. Specifically, guided by~\cite{pingmesh}, we set each server to probe 20K other servers at a time interval of 5 seconds. As a probe record is 86B, each server generates data approximately at 2.62 Mbps. For \dnnlog{}, guided by~\cite{chi} which reports text log data generated at 10s PB per day across 200K \client{} nodes in a production system, we set each server to generate 0.62 MBps (or 4.96 Mbps) of log data. For experimentation purpose, we scale up the data generation rate by 10x, i.e., 26.2 Mbps for \pingmesh{} and 49.6 Mbps for \dnnlog{} per \client{} node.

\Paragraph{Network configuration.} The number of \client{}s supported by a single \server{} node depends on the compute and network resources available on \server{}. Based on conversations with engineers at a large scale datacenter operator, we find that monitoring pipelines can typically have up to 250 \client{} nodes sending log data to a single \server{} node. And backed by estimates in~\cite{sonata}, we assume we have around 20 monitoring queries that concurrently run on each \client{}. We also assume that a \server{} node would have a network link of 10 Gbps~\cite{everflow}. For ease of experiment, we assume this bandwidth is fairly utilized across 250 nodes and 20 queries per node, allowing 2.048 Mbps effective bandwidth per query per \client{} node. We again scale up the obtained bandwidth by 10x to match with data rate scaling.

\Paragraph{Baseline systems.} For throughput, we compare \ours{} with the following systems: (i) \textbf{\allspconfig{}} that runs a query entirely on \server{} node (i.e., Gigascope~\cite{gigascope}), (ii) \textbf{\allsrcconfig{}} that runs a query entirely on \client{}, (iii) \textbf{\filtersrcconfig{}} that applies static operator-level partitioning and runs only filter operations on the \client{} node (i.e., Everflow~\cite{everflow}), (iv) \textbf{\bestopconfig{}} that applies dynamic operator-level partitioning and runs the best part of query obtained from a query planner on the \client{} node (i.e., Sonata~\cite{sonata}), and \newcontent{(v) \textbf{\coarsedp{}} does coarse-grained data partitioning (i.e., at query level) to split the input stream between \client{} and \server{} node, proportional to available compute on the nodes. For convergence time during adaptation, we compare \ours{} with: (i) \textbf{LP only} which runs \algo{} without fine-tuning (i.e., model-based approach in~\cite{heuristics-op-placement-dsps}) and (ii) \textbf{w/o LP-init} which runs \algo{} by initializing \p{}s to zero (i.e., model-agnostic approach in~\cite{heuristics-op-placement-dsps}).} %Sonata is the closest work to \ours{}. It does centralized, coarse-grained operator-level partitioning for network telemetry queries at runtime, by running an expensive integer linear program (ILP) solver for making partitioning decisions.   

\subsection{Comparing \ours{} with data synopses} 
\label{sec:sampling-vs-jarvis}
\begin{figure}
\centering     %%% not \center
\subfigure[]{\label{fig:b}\includegraphics[width=40mm]{fig/sampling_s2sprobe.pdf}}
\subfigure[]{\label{fig:a}\includegraphics[width=40mm]{fig/NetworkTransferPlot.pdf}}
\caption{\label{fig:sampling_s2sprobe} (a) Cumulative distribution function (CDF) of estimation error for server probe latency using sampling, (b) Network transfer costs due to sampling~\todo{clean up figures}..}
\vspace{-0.7cm}
\end{figure}

\newcontent{To investigate effectiveness of data synopses in reducing network transfer costs for our target scenarios, we focus on sampling and compare them with partitioning techniques in this section. Consider scenario 1 in Section~\ref{sec:background}. When the search service latency SLA is violated, it degrades user satisfaction and reduces revenues~\cite{web-search-predictive-parallel}. Developers need to quickly debug violations by correlating them with the alerts in scenario 1 to determine if the violation is due to a network issue~\cite{pingmesh}, so generating accurate alerts becomes critical. We analyze our \pingmesh{} trace to identify data indicating network issues on server nodes, resulting in high probe latencies. We then run the query in Listing~\ref{lst:motivating-query} using window-based sampling protocol in~\cite{continuous-sampling-streams}, to sample from a continuous stream of data in a distributed setting with multiple \client{}s. With different sampling rates, we plot the error in estimating range of probe latencies for
each server pair. Figure~\ref{fig:sampling_s2sprobe} shows the results.

Given the alert threshold of 5 ms used in scenario 1, we observe that with 0.6 and 0.8 sampling rates, we have 85-90\% of the errors within 1 ms. However, network transfer savings are not significant for these high rates (Figure~\ref{fig:sampling_s2sprobe}(b)). For lower sampling rates (i.e., 0.2 and 0.4), we get significant reductions in network transfer costs (10-32\% of input rate) but the reduction that can be obtained using partitioning in
\ours{} is comparable or better (i.e., 11.4-90\% of input rate reduction depending on available compute on \client{}). Critically, we note that 20-40\% of the error estimates exceed 1 ms, in the same order as 5 ms alert threshold. And 20\% of the error estimates exceed 5 ms for 0.2 sampling rate. The reason for the high errors is due to skewness in the probe latencies we observed on \client{}s over time, resulting in underestimation of the probe latency range. We further observe that for low sampling rates that result in network transfer savings (i.e., 0.2 and 0.4), between 10\%-38\% of the alerts that should be generated in scenario 1 (Section~\ref{sec:background}) are missed. The significant number of missed alerts makes it challenging for developers to quickly debug service failures. 

Given the challenges due to accuracy loss for telemetry tasks, similar to the works
in~\cite{sonata,helios,gandalf,omnimon}, our work focuses on optimizing server monitoring pipelines which require lossless and fully accurate query output. Thus, we process per-epoch
statistics for all monitoring traffic.}

\subsection{Query Throughput Analysis}
\label{sec:query-throughput-comparison}
%Accurate query partitioning would meet the data input rate by fully utilizing available compute resources on \client{} node, thereby
%minimizing network data transfer and improving query throughput. 
We use the single \client{} setup and vary it's available compute to evaluate query throughput for different partitioning strategies. \newcontent{In our setup, 64 \server{} cores are shared by up to 250 \client{}s (Section~\ref{sec:exp-methodology}). Thus, for \coarsedp{}, \server{} is assumed to have 25\% of a core per data source (i.e., 64 cores/250 \client{}s) available for query processing.}
% As compute may be shared with other queries, we perform a sensitivity analysis by varying the available compute between 0-100\% of a single core.
% We note that \ours{} incurs little overhead, consuming less than 1\% of a core while profiling operator states and making adaptation decisions.

\Paragraph{\qone{} query.} Figure~\ref{fig:all-throughput}(a) shows the results of query throughput on \qone{}. \newcontent{\ours{} outperforms other techniques in the 40-80\% CPU budget range, with throughput gains of 2.6x and 1.16x over \allsrcconfig{} and \coarsedp{} respectively at 60\% CPU, and 1.25x over \bestopconfig{} at 80\% CPU.} The query requires nearly 85\% CPU to execute entirely on \client{}. Thus, \allsrcconfig{} cannot meet the processing rate requirements at budgets lower than 80\% CPU. % so throughput declines drastically with low CPU budgets. 
Network bandwidth becomes a bottleneck for \filtersrcconfig{} as F operator is not effective in filtering out data. \bestopconfig{} executes F and G+R on \client{} only at 100\%. For lower CPU budgets, it hits compute bottleneck and runs only F at the source as its compute cost is just 13\%. 
% Note that the maximum benefit \ours{} can get over \bestopconfig{} is less than 1.28x because the input rate is 26.2 Mbps and network link is limited to 20.48 Mbps (i.e. 26.2/20.48=1.27).

% With 100\% CPU budget, \client{} node cannot fully process the G+R (grouping and reduction) operator due to its high cost.

%the compute demand of the
%query is higher due to the expensive G+R operator. But
\ours{} partially processes the input of the G+R operator within available compute to reduce network traffic. In comparison, \allspconfig{} is restricted by available network bandwidth, and thus its throughput does not change with available CPU. \newcontent{\coarsedp{} generates higher amounts of network traffic compared to \ours{} since its goal is to balance the compute load between \client{} and \server{} nodes.}

\Paragraph{\qtwo{} query.} Figure~\ref{fig:all-throughput}(b) shows the results of query throughput on \qtwo{}. This query requires more than a core to execute due to expensive J operator. Thus, \allsrcconfig{} cannot handle the input rate even at 100\% CPU, and its throughput declines drastically as CPU budget lowers further. \ours{} does \datapart{} to process the input partially on J operator, thereby reducing network traffic, outperforming other techniques in the 40-100\% CPU range. \ours{} performs 4.4x better than \allsrcconfig{} at 40\% CPU and 1.2x better than \bestopconfig{} \newcontent{and \coarsedp{}} between 60-100\% CPU range. Note that J operator is followed by a project on the fields srcToR, destToR and rtt, so output size of project is less than input size of J operator, leading to data reduction. Both \filtersrcconfig{} and \bestopconfig{} execute only F at the source while \bestopconfig{} cannot accommodate J operator even at 100\% CPU. \newcontent{\coarsedp{} relieves compute load on \client{} but the reduction is not sufficient for significant throughput gains.}

\Paragraph{\dnnlog{} query.} \dnnlog{} is relatively cheaper and uses 31\% CPU to process the input at 49.6 Mbps. Nonetheless, \ours{} does \datapart{} to reduce compute cost at 20\% CPU budget, as shown in Figure~\ref{fig:all-throughput}(c), outperforming \bestopconfig{} \newcontent{and \coarsedp{}} by 1.5x. \allsrcconfig{} shows lower throughput than \ours{} at 20\% CPU as it is resource constrained. \filtersrcconfig{} executes filtering on \client{}, but is bound by network cost due to low filter-out rate. On the contrary, \bestopconfig{} can perform the filter and map operators at the source, thus outperforming \filtersrcconfig{}. \allspconfig{} is always bound by the network, and hence \ours{} outperforms it by 2.3x in the 40-100\% CPU range. \newcontent{For low CPU budget of 20-40\%, \coarsedp{} transfers up to 45\% of the input over the network, which results in significant bottlenecks for a query like \dnnlog{} with large input size.}

\Paragraph{Summary.} Our results show \ours{} provides higher throughput (1.2-4.4x) in scenarios where compute resources are constrained on \client{}. The throughput gains are higher when query is compute- or network-bound.

% \subsection{Network traffic reduction}

% \subsection{Query Completion Time Comparisons}
% \begin{figure*}[t]
% \begin{multicols}{3}
%     \includegraphics[width=\linewidth]{fig/s2sprobe_80percentcpu_latencies_plot.pdf}\par\caption{\label{fig:pingmeshquery1-latency}\qone{} query completion time for 80\% CPU on \client{}}
%     \includegraphics[width=\linewidth]{fig/t2tprobe_100percentcpu_latencies_plot.pdf}\par\caption{\label{fig:pingmeshquery-tor-latency}\qtwo{} completion time for 100\% CPU on \client{}. I/P stream joined with table of size 500}
%     \includegraphics[width=\linewidth]{fig/dnnlog_20percentcpu_latencies_plot.pdf}\par\caption{\label{fig:wordcount-latency}\dnnlog{} query completion time for 20\% CPU on \client{}.}
% \end{multicols}
% \vspace{-0.8cm}
% \end{figure*}
% Figures~\ref{fig:pingmeshquery1-latency},~\ref{fig:pingmeshquery-tor-latency} and~\ref{fig:wordcount-latency} show the query completion times for~\qone{},~\qtwo{} and~\dnnlog{} queries evaluated. 

\subsection{Convergence Analysis}
\label{sec:convergence-cost-eval}
We evaluate how fast \ours{} adapts to changes in resource conditions on \client{} by measuring the convergence time in number of epochs. % available compute on \client{} as well as in query's compute demand by measuring convergence time for such changes. %Convergence time is measured in number of epochs on \client{} node as follows: vary available CPU at runtime for \qone{}, vary both available CPU and input join table size for \qtwo{}, and vary input rates for \dnnlog{}. 
We show that \ours{} converges in a few one-second epochs after resource change occurs. Note that Sonata~\cite{sonata} is a model-based approach and accurately solves an expensive optimization that takes several minutes to compute a new query plan. We now compare \ours{} against other approaches which have convergence time in order of seconds.

% \begin{figure}[t]
% \centering
% \subfigure[Without LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/pingmesh-conv-num-nolp-v2.pdf}}
% \subfigure[With LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/pingmesh-conv-num-withlp-v2.pdf}}
% % \subfigure[Join operator]{\includegraphics[width=1.6in]{fig/JoinOperatorProfileNew.png}}
% %\vspace{-0.1in}
% \caption{\label{fig:convergence-pingmesh}\qone{} convergence plot.} %\vspace{-0.2in}
% % \vspace{-1.277cm}
% \vspace{-0.4cm}
% \end{figure}

\Paragraph{\qone{} query.} Figure~\ref{fig:convergence-pingmesh} shows the results as we vary the available compute on the \client{} by starting with 10\% CPU, then switching to  90\% CPU in the $3^{rd}$ epoch, and finally reducing CPU down to 60\% of the CPU to cause congestion in the $18^{th}$ epoch.  Note that three epochs are required to detect that compute budget has changed to avoid triggering adaptation due to scheduling noise in the system.  

When compute budget changes at $3^{rd}$ epoch, \ours{} reduces the convergence time from six epochs in \modelagnostic{}, down to one epoch when employing initialization using LP solver. \newcontent{\modelbased{} also stabilizes the query using output of LP solver.} When CPU drops from 90\% to 60\%, the query reaches a stable state within two and four epochs for \ours{} and \modelagnostic{}, respectively. The additional epoch for \ours{} is required  because profiling within a one-second epoch is not sufficient for G+R to process all records, resulting in less accurate estimates for the cost of G+R. Inaccurate profiling also prevents \modelbased{} from stabilizing the query.

%In summary, we observe that \algo{} is effective in improving convergence time when a sudden increase or reduction in available resources is encountered. 

% \begin{figure*}[t]
% \centering
% \subfigure[Input rate scaled up by 10x.]{\includegraphics[width=1.8in]{fig/scale_10x_throughput.pdf}}
% \subfigure[Input rate scaled up by 5x.]{\includegraphics[width=1.8in]{fig/scale_5x_throughput.pdf}}
% \subfigure[Input rate with no scaling.]{\includegraphics[width=1.8in]{fig/scale_1x_throughput.pdf}}
% %\vspace{-0.1in}
% \caption{\label{fig:scalability-throughput} Throughput for multiple data source nodes at different input rates.} %\vspace{-0.2in}
% % \vspace{-1.277cm}
% \vspace{-0.4cm}
% \end{figure*}

\begin{figure}
    \includegraphics[width=\linewidth]{fig/all_scale_thruput.pdf}\caption{(a) Input rate scaled up by 10x, (b) Input rate scaled up by 5x, (c) Input rate with no scaling. Throughput for multiple data source nodes at different input rates.}
    \label{fig:scalability-throughput}
\vspace{-0.4cm}
\end{figure}

\Paragraph{\qtwo{} query.} Performance of a join-bound query is affected by the size of the static table. As shown in Figure~\ref{fig:convergence-pingmesh-tor}, we vary the available compute and the size of the static table by starting with 10\% CPU and a static table of size 50, then switching to 100\% CPU in the $3^{rd}$ epoch, and finally increasing the static table size by 10x to cause congestion.

Convergence duration is reduced from 11 epochs (in \modelagnostic{}) to 7 epochs in \ours{}, when the budget is increased to 100\%. The additional epochs for \ours{} after profiling is attributed to the fact that the expensive J operator cannot be executed on all records to get accurate profiling estimates. As a result, the downstream G+R operator is not profiled accurately. Thereafter, fine-tuning plays a critical role in stabilizing the query in \ours{}. When join table size increases, the compute cost of J operator increases leaving no resources for G+R to execute. It takes 5 and 3 epochs to converge \modelagnostic{} and \ours{}. \newcontent{Inaccurate profiling causes \modelbased{} to not converge in both cases  of change in resource conditions.}

%In summary, we observe that fine-tuning plays a critical role in stabilizing load factors when an expensive operator limits the accuracy of the profiling phase.

% \begin{figure}[t]
% \centering
% \subfigure[Without LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/pingmesh-torcountonly-jointable50-500-conv-num-nolp-v2.pdf}}
% \subfigure[With LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/pingmesh-torcountonly-jointable50-500-conv-num-withlp-v2.pdf}}
% % \subfigure[Join operator]{\includegraphics[width=1.6in]{fig/JoinOperatorProfileNew.png}}
% %\vspace{-0.1in}
% \caption{\label{fig:convergence-pingmesh-tor} \qtwo{} convergence plot.} %\vspace{-0.2in}
% % \vspace{-1.277cm}
% \vspace{-0.4cm}
% \end{figure}

% \begin{figure}[t]
% \centering
% \subfigure[Without LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/wordcount-conv-v2-num-nolp-v2.pdf}}
% \subfigure[With LP init]{\includegraphics[width=1.65in,height=1.3in]{fig/wordcount-conv-v2-num-withlp-v2.pdf}}
% % \subfigure[Join operator]{\includegraphics[width=1.6in]{fig/JoinOperatorProfileNew.png}}
% %\vspace{-0.1in}
% \caption{\label{fig:convergence-wordcount} \dnnlog{} convergence plot.} %\vspace{-0.2in}
% \vspace{-0.4cm}
% \end{figure}

\Paragraph{\dnnlog{} query.} We evaluate \ours{} while varying input rates and fixing compute budget to 25\% CPU. We start with an input rate of 49.6 Mbps causing congestion as the query requires 31\% CPU. We then reduce the rate by almost half, to 25 Mbps causing the query to idle. We finally increase the rate up to 80 Mbps. Figure~\ref{fig:convergence-wordcount} shows that when input rate drops to 25 Mbps in the $3^{rd}$ epoch, LP solver output enables \ours{} and \modelbased{} to converge immediately while it requires 3 epochs for \modelagnostic{} to converge. When the input rate is increased to 80 Mbps in the $14^{th}$ epoch, \newcontent{the query does not converge with \modelbased{}, takes 5 epochs with \modelagnostic{}, while it takes only 3 epochs with \ours{}.}

% We start with 10\% CPU on \client{} and then increase it to 90\%. We measure the convergence time and then bring the CPU down to 25\%. The lower 25\% CPU compared to \qone{} is to create congestion as this query is relatively cheaper. Figure~\ref{fig:convergence-wordcount}(a) shows at the $3^{rd}$ epoch, when available CPU increases to 90\%, \algo{} takes 3 epochs to converge without LP init. In Figure~\ref{fig:convergence-wordcount}(b), the query immediately converges using LP solver's load factors after a single profiling epoch. When the CPU is lowered to 25\% at $14^{th}$ epoch, the query takes 5 epochs to stabilize without LP init, and with LP init, it takes only 2 epochs to converge.

%Note that the query in this case entered $IDLE$ state instead of
%$CONGESTED$ after profiling, because LP solver under-estimated the load
%factors for the new resource conditions.

\ifthenelse{\boolean{Extended}}{
\Paragraph{Simulator-based analysis.} 
\begin{figure}
  \centering
    % \includegraphics[width=0.48\textwidth]{fig/MultiOpsConvTime.pdf}
    \includegraphics[width=0.3\textwidth]{fig/multiops-convtime-data.pdf}
    \caption{Convergence time in number of epochs as we increase number of query operators. 150K records per epoch.}
    \label{fig:convergence-multi-ops}
    \vspace{-0.4cm}
\end{figure}
We further analyze the potential benefit of LP solver in terms of convergence cost for \algo{}, as we increase the number of query operators. We simulate the query execution guided by the execution behavior captured by query refinement problem in Section~\ref{sec:problem-definition-opt}. By varying different parameters in the query refinement problem formulation, we obtain a range of possible convergence costs for each value of $M$ i.e. number of query operators. Figure~\ref{fig:convergence-multi-ops} shows that the convergence time can go up to 21 epochs in the worst case for 4 or more operators. The curve levels off at about 21 epochs because we fixed the input rate. Taking 21 epochs to converge is not fully satisfactory if the goal is to adapt to resource changes in the order of a few seconds. This analysis shows that using only fine-tuning in \algo{} with fixed \p{} initialization can incur a high convergence cost with larger $M$, indicating that LP solver is indispensable in \algo{} especially when a given query includes a number of operators.
}{
\Paragraph{Impact of number of operators.} As we increase number of query operators, we expect \modelagnostic{} which runs \algo{} without LP init, to take longer to converge. We analyze algorithm convergence via a simulator that performs an exhaustive search of different execution configurations with possible query resource needs and compute budgets, while measuring associated convergence cost for each configuration. We find that for a given input rate, convergence time can increase to as high as 21 epochs in the worst case, with four operators. Detailed analysis can be found in~\cite{jarvis-extended}. LP solver can be valuable part of design in improving convergence cost in such cases.
}

\Paragraph{Summary.} On one hand, \modelbased{} approach relying on LP solver to determine \p{} is quite effective in reducing convergence time if an accurate profiling of the operators can be obtained. On the other hand, fine-tuning is critical to stabilize the query if the profiling is not accurate. Previous model-based approaches~\cite{sonata} cannot fully rely on online profiling as they do not have a fine-tuning mechanism to stabilize the query. Our hybrid approach achieves convergence within a few epochs for various resource conditions.
% ~\todo{sonata does multi-query optimization and is expensive, \ours{} assumes fair resource allocation and does per-query optimization but with fine-grained partitioning. Sonata falls back to LP solver when run for single query, without fine-tuning}

%\subsection{Scaling the number of \client{} nodes}
%\subsection{Scaling \ours{} to more \client{}s}
\subsection{Multiple Data Source Nodes}
\label{sec:scalability-analysis}

We discuss the efficacy of \ours{} when multiple \client{}s are sending data to a single \server{} node. We compare \ours{} and \bestopconfig{}, i.e., the state-of-the-art in dynamic operator-level partitioning, on \qone{} query while varying the following dimensions: (i) number of \client{} nodes and (ii) input data rate per \client{} node. 

We start with the input rate of 26.2 Mbps for \pingmesh{}, which is scaled by 10x over the calculated rate for this 
dataset. On each \client{}, we set CPU to 55\% to ensure that \bestopconfig{} executes only the F operator while not fully utilizing the given CPU budget.
%\ours{} 
%adapts to enable \datapart{}---in the CPU budget, \bestopconfig{} executes the F operator only. 
Figure~\ref{fig:scalability-throughput}(a) shows the results as we increase number of \client{}s. In \bestopconfig{}, F operator does not reduce data significantly so the policy suffers from network bottleneck as soon as we increase the number of \client{}s. However, \ours{} scales up to 32 nodes without throughput degradation. Further scaling stops due to network bottleneck while peak compute usage on \server{} was at 24 cores. Beyond 32 nodes, we observe backpressure which causes epoch processing latency to grow, and number of \client{}s for which no data is being received on \server{} increases.

We now decrease input rate to 13.1 Mbps (5x scaling) on each \client{} and set available CPU to 30\%, to reflect the change in query compute demand from decreasing input rate. Figure~\ref{fig:scalability-throughput}(b) shows that \bestopconfig{} scales to 40 nodes after which it becomes network bottlenecked. \ours{} scales up to nearly 70 nodes, 75\% improvement in number of \client{}s supported over \bestopconfig{}. When we further reduce input rate to 2.62 Mbps in Figure~\ref{fig:scalability-throughput}(c) and allocate 5\% CPU to the query, \bestopconfig{} starts to degrade in throughput at 180 nodes while \ours{} is seen to scale even for 250 \client{}s, an 39\% improvement.

\Paragraph{Epoch processing latency.} \ours{} also improves epoch processing latency as a result of network traffic reduction. Based on the observed epoch latency distributions, we note for example, that \ours{} improves median latency of \bestopconfig{} by around 3.4x in the configuration with 5x scaling and 40 \client{}s, when both policies are able to handle the input data rate. Moreover, \bestopconfig{} exhibits 1.8 and 5.2 seconds for the median and max latency, respectively, which are much larger than 500 ms and 2 seconds for the two measures in \ours{}. For configurations where \bestopconfig{} could not keep up with input data after it hits network bottleneck, such as 5x scaling with 60 nodes, we see max latency of \ours{} to be within 5 seconds while \bestopconfig{} latency grows beyond 60 seconds.

\subsection{Multiple Queries on Data Source Node}
\label{sec:multiple-nodes-eval}

This experiment aims to investigate potential interference when we execute multiple queries with \ours{} on a single \client{} node.
%We execute multiple queries on a \client{} node with \ours{} and investigate interference. % for resources such as memory. 
For this purpose, we run multiple instances of \qone{} query while each instance is configured to use fixed amount of CPU resource.
%We replicate instances of \pingmesh{}'s \qone{} and 
Specifically, we measure \emph{aggregate} query throughput while fixing \p{}s for each query instance such that it utilizes 55\% CPU for input rate of 26.2 Mbps (i.e., 10x scaling).
%as we increase the number of queries on a single \client{}. Similar to Section~\ref{sec:scalability-analysis}, we restrict the total memory capacity to 1 GB, while fixing \p{}s so the query utilizes 55\% CPU for input rate of 26.2 Mbps (i.e., 10x scaled). 
Figure~\ref{fig:multiple-queries-eval} shows the results while varying the following dimensions: (1) input data rate per query and (2) number of cores on \client{}. 

% \begin{figure*}[t]
% \centering
% \subfigure[Input rate scaled up by 10x.]{\includegraphics[width=1.8in]{fig/10x_jarvis_multiqueries.pdf}}
% \subfigure[Input rate scaled up by 5x.]{\includegraphics[width=1.8in]{fig/5x_jarvis_multiqueries.pdf}}
% \subfigure[Input rate with no scaling.]{\includegraphics[width=1.8in]{fig/1x_jarvis_multiqueries.pdf}}
% %\vspace{-0.1in}
% \caption{\label{fig:multiple-queries-eval} Throughput for multiple queries on \client{}, at different input rates.} %\vspace{-0.2in}
% % \vspace{-1.277cm}
% \vspace{-0.4cm}
% \end{figure*}


\begin{figure}
    \includegraphics[width=\linewidth]{fig/all_scale_jarvis_multiqueries.pdf}\caption{(a) Input rate scaled up by 10x, (b) Input rate scaled up by 5x, (c) Input rate with no scaling. Throughput for multiple queries on \client{}, at different input rates.}
    \label{fig:multiple-queries-evalt}
\vspace{-0.4cm}
\end{figure}

We observe that there is no significant interference among query instances until the system is bottlenecked by compute budget.
Under system stress at 10x input scaling, single-core throughput saturates at 2 queries given per-query CPU cost. Two-core throughput does not increase beyond 3 queries, indicating saturation at 70 Mbps. At 5x scaling, per-query CPU cost drops to 30\% and \ours{} supports up to four and six queries on a single- and two-core setup, respectively. At no input scaling, \ours{} supports 15 queries and 25 queries with one and two cores, respectively.
%due to relatively low data rates on each \client{}. Queries are primarily bottlenecked by compute. 
%Furthermore, with query partitioning, as we add more queries, \ours{} can adapt to support more queries for a given compute budget.

%Even though resource interference is expected to increase when the system is stressed, \ours{} is able to handle up to 25 queries depending on system load, enabling it to support multi-query use cases in monitoring systems.   

% The plots for 5x scaling with 60 \client{}s and 10x scaling with 12 \client{} are used to show how the latencies continue to grow for \bestopconfig{} once we hit network bottleneck in the system. 

% dataset. On each \client{}, we set CPU to 60\% so \ours{}

%\begin{figure}[t]
%\centering
%\subfigure[5x scaling, 40 \client{} nodes]{\includegraphics[width=1.65in,height=1.45in]{fig/scale_cdf_latencies_5x_40nodes.pdf}}
%\subfigure[5x scaling, 60 \client{} nodes]{\includegraphics[width=1.65in,height=1.45in]{fig/scale_cdf_latencies_5x_60nodes.pdf}}
%\subfigure[10x scaling, 12 \client{} nodes]{\includegraphics[width=1.8in,height=1.3in]{fig/scale_cdf_latencies_10x_12nodes.pdf}}
%\vspace{-0.1in}
%\caption{\label{fig:scalability-latency-cdf} CDF of epoch processing latencies for different scaling configurations} %\vspace{-0.2in}
% \vspace{-1.277cm}
%\vspace{-0.3cm}
%\end{figure}

% \begin{figure}[t]
% \centering
% \subfigure[12 \client{} nodes]{\includegraphics[width=1.65in,height=1.3in]{fig/scale_Latencies_10x_12nodes.pdf}}
% \subfigure[20 \client{} nodes]{\includegraphics[width=1.65in,height=1.3in]{fig/scale_Latencies_10x_20nodes.pdf}}
% \subfigure[28 \client{} nodes]{\includegraphics[width=1.65in,height=1.3in]{fig/scale_Latencies_10x_28nodes.pdf}}
% %\vspace{-0.1in}
% \caption{\label{fig:scalability-latency-10x} Query completion time plots for input rates scaled by 10x} %\vspace{-0.2in}
% % \vspace{-1.277cm}
% \vspace{-0.65cm}
% \end{figure}

% \todo{Need to add section on localized adaptation}
% \todo{Do we need to handle global hot keys?}



% \Paragraph{Change in available CPU time}
% \begin{figure}
%   \centering
%     \includegraphics[width=0.5\textwidth]{fig/fig13.pdf}
%     \caption{Reaction time of Jarvis with changing available CPU time \todo{Change Y-axis to CPU available, and show effect of parameters like congestion/idle state thresholds. Keep graphs quantitative. }}
%     \label{fig:compute-adapt}
% \end{figure}
% Compute resource changes for a query can happen at different timescales. During normal resource usage on a node, it is reasonable to say that at smaller timescales, relatively small changes in CPU time occur, while at larger timescales the CPU time change can be large. So we evaluate Jarvis adaptivity under both these conditions.

% Figure~\ref{fig:compute-adapt} shows the reaction time for Jarvis when \client{}-side CPU changes from 40\% to 10\% available for the query at epoch 2, which is a large change. \ours{} is expected to reconfigure load factors for multiple operators, doing operator partitioning and then data partitioning. Thus is takes 4 epochs to converge after a resource change is detected. Detecting the resource change after it occurs, takes between one to two epochs.
% For small resource change from 40\% to 30\% which occurs at epoch 8, \ours{} adjusts the boundary operator's load factor, performing only data partitioning and stabilizing within 2 epochs after resource change detection.

% Focus on Jarvis and show its fast adaptation to the change of the available CPU resource. Show a graph with time progress at X-axis, which change the available CPU resource from 60\% to 80\% (small change) and then from 80\% to 20\% (large change). For the small change, Jarvis will just adjust the operator's probability ($p_e$). For the large change, Jarvis will reconfigure $p_e$ values for all operators.

% \subsection{Hot-key based data partitioning}
% \begin{figure}
%   \centering
%     \includegraphics[width=0.5\textwidth]{fig/hotkey.pdf}
%     \caption{Groupby operator throughput comparison across load factors, of random strategy with \ours{} which prioritizes hot key processing}
%     \label{fig:key-distr-adapt}
% \end{figure}
% Figure~\ref{fig:key-distr-adapt} shows the throughput benefits obtained by prioritizing hot key based processing over random strategy of choosing input records to process on \client{}. The benefit of hot-key based selection reduces as we increase the load factor value. This is expected because we choose all of the input records for processing at higher load values.

% We change key distributions in terms of 1) the number of keys and 2) the keys which are hot. 1) can be caused by zoom-in and zoom-out query execution similar to Sonata? 2) could be reconfiguration of mapping between \client{} nodes and intermediate node (the use case of intermediate node is explained below).
% Atul: (1) implies change in grouping key CPU cost. We already show adaptivity with CPU cost previously. So discarded that scenario here.

% \subsection{Scalability}
% \label{sec:scalability}

% We now use the large-scale testbed and simulator to demonstrate the scalability of Jarvis across a large number of \client{} nodes.
% \Paragraph{Throughput}
% \begin{figure}
%   \centering
%     \includegraphics[width=0.15\textwidth]{fig/Placeholder.png}
%     \caption{Throughput with increasing \client{} nodes}
%     \label{fig:scale-throughput}
% \end{figure}
% We compare the overall query throughput for Jarvis with \server{}-central, to evaluate how Jarvis scales with increasing number of \client{} nodes. Each \client{} node sends data at 3 MBps. Figure~\ref{fig:scale-throughput} shows the overall throughput as \client{} nodes are increased. We expect to see that in \server{}-central, a decline in throughput is observed while the scaling of intermediate aggregation servers with \client{} nodes enables Jarvis to keep up with aggregate source rate, at lower compute cost. This shows resource efficiency of Jarvis and low cost of operating Jarvis-based monitoring. This is due to efficient data reduction and network load balancing mechanism on the \server{} nodes.
% \Paragraph{Localized adaptation}
% Even at large scales, Jarvis is able to quickly adapt to dynamic conditions across one or more of the \client{} nodes. It doesn't rely on a global query partitioner and each \client{} node adapts independently, allowing Jarvis to scale in its adaptivity.
% To evaluate this, we change the available CPU resource (from 80\% to 20\%) for a subset of \client{} nodes (ranging from 80\% to 20\% of the \client{} nodes on large-scale testbed). We expect to see that partition adaptation occurs only for the subset of \client{} nodes where CPU resource changed, while other nodes do not perform any adaptation. Each node adapts its own partitioning without relying on any global scheduler.


% Figure~\ref{fig:local-adapt} shows this benefit by measuring average reaction time across \client{} nodes (on Y-axis) for different fractions of \client{} nodes in our large-scale testbed changing available CPU time from 80\% to 20\% (i.e. X-axis contains fractions of 20\%, 40\%, 60\% and 80\% of \client{} nodes). We observe that the average reaction time doesn't change as we increase the number of nodes in which resource availability changes.
% \Paragraph{Global hot key locality}
% \begin{figure}
%   \centering
%     \includegraphics[width=0.15\textwidth]{fig/Placeholder.png}
%     \caption{Jarvis global hot key locality}
%     \label{fig:global-hot-key}
% \end{figure}
% As we scale up the \client{} nodes, global hot key distributions can change depending on number of \client{} nodes from which records for a key are emitted (e.g. grouping based on error code in PingMesh). We compare the throughput for Jarvis with hot key locality enabled using hot key aggregators in \server{} vs. hot key locality disabled. We expect to see a significant gain in overall query throughput with hot key locality enabled.

% We change key distributions in terms of 2) the keys which are hot. 2) could be reconfiguration of mapping between \client{} nodes and intermediate node (the use case of intermediate node is explained below)

% \subsection{Overhead}
% \Paragraph{Runtime overhead on \client{}}
% In single-\client{} testbed, we evaluate the overhead of running Jarvis runtime alongside the query. To do so, we compare throughput of All-\server{} and Jarvis at the 0\% CPU time available on \client{}. We expect to see the throughput not changing much for Jarvis, compared to All-\server{}.

% \Paragraph{Repartitioning overhead}
% We compare the following: OP, which is solved by ILP focused on operator partitioning only, with Jarvis. We show how fast Jarvis provides a partitioning plan for a given available resource.
% Expected results: Jarvis takes much shorter time. Close to OP-ILP in terms of performance, but much faster in converging.

% \mj{end ----.}

% We also evaluate Jarvis on the following benchmarks:
% \textcolor{red}{[TODO]}\\
% The queries we execute are as follows: \\
% \textcolor{red}{[TODO]}\\



%\subsection{Data-driven Study}
% \todo{Rewrite to integrate with evaluation, currently just copy pasted from motivation section}
% For each execution plan, we present query performance in throughput measured in megabit per second (Mbps) and discuss potential causes if performance degradation is observed. We also investigate several operation-specific factors during
% study, such as filtering rate and data skewness across grouping keys. For this experiment, we use a data source node with 1~2.4~GHz core and 1~GB of memory to represent a small amount of resources assigned for monitoring, and a stream processor node with 4~2.4~GHz cores. For obtaining realistic source generation
% rates per \client{} node, we analyze a production
% trace, \textbf{\pingmesh{}}, for latency monitoring (see
% Section~\ref{sec:evaluation} for details). Based on this analysis, we set input stream rate at 27.2~Mbps (10x scaled up). Below demonstrates the network monitoring query we execute, and Figure~\ref{fig:pipeline_tor} shows how its pipeline is organized.

% \begin{lstlisting}[caption= {Stream query gathering server-level latency statistics for every 10-second fixed-size window},label={lst:pingmesh-query}]
% query = Stream
%   .Window(10_SECONDS)
%   .Filter(e => e.errorCode != 0)
%   .GroupApply(e.dstIP)
%   .Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
% \end{lstlisting}


% \begin{figure}[t]
% \centering
% \subfigure[All-SP]{\includegraphics[width=1.6in]{fig/all_sp}}
% \subfigure[All-Src]{\includegraphics[width=1.6in]{fig/all_src}}
% %\vspace{-0.1in}
% \caption{\label{fig:no-partition} Throughput achieved when query executes without partitioning. Network bandwidth is set to 15~Mbps in All-Src.}
% \end{figure}


% \subsubsection{Executing Query without Partitioning}

% We revisit classical query execution models without any partitioning. First,
% we consider executing the entire query in the stream processor (All-SP),
% where raw stream data must be sent by the data source over the network to be
% processed. For
% query in Listing~\ref{lst:pingmesh-query}, we initially set filtering to drop 85\% of records and
% grouping to handle 20K groups.

% Figure~\ref{fig:no-partition}(a) presents throughput achieved by All-SP when varying
% available network bandwidth between the single data source and the stream
% processor in the x-axis. Here, a lower bandwidth
% reflects network sharing occurred in the stream processor when it connects to
% more data source nodes. As the figure shows, when bandwidth is abundant
% (50~Mbps) for a data source node, no bottleneck is observed, with the throughput
% as high as the data
% generation rate. However, as the available network bandwidth decreases, the
% throughput decreases as well due to network gradually being a bottleneck. In
% general, a requirement for All-SP to operate with no performance degradation
% is that the stream processor be able to ingest incoming streams whose volume
% grows with the number of data source nodes. Obviously, this is too costly
% in datacenter-scale monitoring.

% Next, we examine a query plan executing the same query as above entirely on
% the data source node (All-Src) and sending out only the final output to the
% stream processor. As
% aforementioned, telemetry tasks commonly produce outputs with significant
% data reduction, so at first glance All-Src seems much more feasible than
% All-SP. However, it turns out that All-Src is effective only when there is
% ample CPU resource to use in the data source node, which is less likely
% as limited source-side resources are almost always shared by a number of
% queries (challenge 2 in Section~\ref{sec:challenges}),
% and as we cannot afford to isolate those queries on separate cores.
% We show throughput of All-Src as a function of
% source-side compute resource available for our query in
% Figure~\ref{fig:no-partition}(b).
% We restrict network bandwidth
% to be 15 Mbps so that the network becomes a bottleneck without proper network
% traffic reduction from the data source. If we run the entire query on full
% 1 CPU core for sending the query output only, as shown
% in Figure~\ref{fig:no-partition}(b), no performance degradation is observed
% thanks to considerably reduced network traffic.

% However, as we restrict CPU usage for
% the query, the throughput decreases accordingly due to backpressure building on
% the data source node, which indicates compute demand
% exceeds the available resource budget.

% \Paragraph{Lesson:} All-SP and All-Src work well if each telemetry task
% is provided with sufficient network and compute resources, respectively. But, once
% telemetry system starts operating on a high fan-in traffic and handles
% multiple telemetry tasks, a task would experience suboptimal
% performance.


% \subsubsection{Executing with Operator Partitioning Alone}
% \label{sec:OP_partitioning_only}

% Now, we apply an operator partitioning configuration wherein the data source
% node is in charge of executing only the first half of the query in
% Figure~\ref{fig:pipeline_tor} (Half-Src). So, for operations in
% Figure~\ref{fig:pipeline_tor}, the data source node executes window and
% filter operators, and offloads the remaining operators to the stream processor.
% From this operator partitioning, we see that the query throughput
% can reach close to the data generation rate for a wide range of CPU budget. In
% particular, unlike All-SP and All-Src, Half-Src does not exhibit a
% bottleneck in the use of 30\% CPU resource and 15~Mbps network bandwidth.

% A notable characteristic of the original query is that the filtering
% predicate is so effective that a large number of input records are eliminated
% from filtering. This makes all subsequent operations able to deal with
% computations and data transfers at low costs. Therefore, we test if performance
% is retained with less effective filtering predicates.
% When we invert the filtering predicate in the query into
% \texttt{e.errorCode == 0}, i.e. filtering to drop only 15\% of records,
% the throughput decreases
% markedly because backpressure starts to build in the pipeline.
% In this case, a plausible solution would be
% \emph{data partitioning}, which applies filtering on a subset of input
% records.


% When CPU resource remains after filtering, a natural question is if we can
% also execute grouping and reduction to alleviate the pressure on the network more.
% If available CPU resource is not sufficient to process the entire input
% stream for those operations, we should also process it partially with data
% partitioning.

% \Paragraph{Lesson:} Data partitioning is essential to better exploiting the limited compute resource, and to be effective it must consider operation-specific factors and how they contribute to data reduction.


==> archive/insight-v1.tex <==
\section{Problem Definition and Insights}
\label{sec:drawbacks}

\newcontent{In this paper, we investigate how to effectively utilize limited and dynamic compute resources available on \client{} nodes, by quickly partitioning query workloads between \client{} and \server{} nodes and reduce network transfer costs for supporting large scale server monitoring pipelines.}

Consider that a monitoring query can be represented as a DAG $G = (V,E)$. In
a DAG, the vertices V denote stream operations which transform their input
records and emit output records to downstream operation, and the edges $E$
denote dataflow dependencies between operations. Among prior approaches to
addressing query partitioning, the operator-level
partitioning~\cite{everflow,gigascope,jetstream} is one of the most widely
used approaches. Given a query DAG, an operator-level partitioning plan
identifies operations that can execute locally on each \client{} and those
that require remote execution on the \server{}. This requires a boundary
operator to be defined for each \client{} to indicate that all operators
prior to the boundary operator (including itself) in the topological order of
the DAG are executed on \client{} and those after the boundary operator are
executed remotely. In Figure~\ref{fig:pipeline_tor}, if F operator is
designated as a boundary operator, W and F operators would execute on the
\client{} to filter out unnecessary data inside the \client{}, effectively
reducing the amount of data transferred to the \server{}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/DataPartitionExplain.pdf}
%\vspace{-0.1in}
\caption{\label{fig:data-partition-explain} Coarse-grained operator-level vs. fine-grained data-level partitioning on \client{} with 80\% CPU budget. G+R requires 80\% CPU to process all output data from F operator.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}


% $b_i$
%To illustrate, consider a topologically sorted list of $M$ operators from the query graph $G$ following dataflow dependencies of the query.
%For instance, for a \client{} with 4 operators, if the boundary operator is 3
%then it implies that the first three operators execute on \client{} and the
%last operator executes remotely.
% $M=4$

%% Given fixed network and compute resources available on \server{}, we seek to maximize the number of \client{}s that can be served to execute a monitoring query in a timely manner. Thus,
%Subsequently, the optimization goal of query partitioning in the context of
%server monitoring ends up identifying the boundary operator for each
%\client{}, such that the processing load sent to \server{} is minimized while
%harnessing the given monitoring resources from the \client{}.
%%The optimization goal of query partitioning is to identify the boundary
%%operator for each \client{}, such that the processing load sent to \server{}
%%is minimized, subject to local computation not increasing overall processing
%%time of each data stream, compared to remote execution.

% This is a NP-hard problem and computationally difficult to solve: we present a formal definition and proof in~\cite{jarvis-extended}.


\textcolor{blue}{
We formally define the query partitioning problem. Let \textbf{b} represent the boundary operators for a given query, where $b_i$ denotes boundary operator for the $i^{th}$ \client{}. Our optimization problem is as follows:
\begin{align*}
    & \displaystyle \min_{\textbf{b}} \sum_{i=1}^{N_{d}}\sum_{j=1}^{M} c_j x_{ij}\\
    subject\ to,&\\
    & T_{local}(i,b_{i}) <= T_{remote}(i,b_{i})\ \forall b_{i}>0, i\epsilon[1,N_{d}]
\end{align*}
Here $x_{ij}$ indicates if boundary operator of $i^{th}$ \client{} is $j$, $c_j$ is the processing cost on \server{} due to partitioning the query on \client{} at $j^{th}$ operator, $T_{local}(i,b_{i})$ computes the local computation time cost for operators 1 to $b_{i}$ on the $i^{th}$ \client{} node and $T_{remote}(i,b_{i})$ denotes the network transmission time cost of intermediate data from $b_{i}^{th}$ operator to its parent stream processor node along with computation time cost of executing operators $b_{i}+1$ till $M$ on the parent node. We want to incentivize executing operators on \client{} so the partitioning costs are ordered as $c_1>c_2>,...>c_M$. Unfortunately, solving the partitioning problem is extremely challenging.
\begin{theorem}
Query partitioning problem to distribute query operators across \client{} and \server{} nodes, with the objective of maximizing the resource utilization of \client{} nodes without degrading query processing time, is NP-hard.
\end{theorem}
\begin{proof}
The key idea of the proof is that the generalized assignment problem~\cite{gap} can be reduced to a special case of our query partitioning problem in polynomial time. Therefore, if we have an algorithm that can minimize the number of operators sent to the \server{} without sacrificing query processing time, then we can also obtain optimal solution to GAP. Since GAP is NP-hard, our problem is also NP-hard. More details for the proof can be found in~\cite{jarvis-extended}.
\end{proof}
}
\newcontent{
Having established the NP-hardness of query partitioning, we note that in our monitoring system, each \client{} runs an instance of the query on its incoming input stream. Query partitioning involves determining the boundary operator for each query instance. Thus, we need to evaluate $M^{N_{d}}$ possible partitioning solutions, where $N_{d}$ is the number of \client{}s and $M$ is the number of operators per query instance. Given that resource conditions change in the order of minutes (Section~\ref{sec:motivation}), we need to quickly compute a new partitioning plan. Each \server{} node in our setup can receive data from up to 250 \client{}s so the exponential cost in \client{}s would not scale for the large number of \client{}s. Other techniques such as trading off accuracy for reducing network transfer costs using data summaries could be considered but their limitations are highlighted at the end of this section. Thus, to make query partitioning practical in large scale server monitoring pipelines, we investigate the effectiveness of a greedy and embarrassingly parallel partitioning heuristic, which reduces network traffic leaving each \client{}. We postulate that to effectively utilize the limited and dynamic compute on each \client{}, it is critical to make fine-grained, data-level partitioning decisions for query operators at runtime, which can be done using a query cost model-based partitioning approach that relies on online and fine-grained profiling of each operator's compute cost. However, accurate online profiling can be challenging due to limited compute available on \client{}. Thus, iteratively fine-tuning the output of query cost model-based approach, using a feedback-driven technique which is agnostic to the cost model, can significantly improve the performance of our adaptation. Our proposed heuristic is simple, computationally tractable and a reasonable first attempt at addressing the query partitioning problem in large scale server monitoring pipelines. Finally, we build a proof-of-concept system Jarvis, which implements the designed partitioning heuristic in a fully decentralized manner using novel system abstractions called \Proxy{} and \run{}. \ours{} is used to evaluate the practicality and effectiveness of our heuristic in scaling monitoring pipelines. Below, we discuss the insights to design the heuristic used by \ours{}. }

%We highlight the drawbacks of state-of-the-art approaches in addressing the operator-level partitioning problem as well as uncover insights for designing \ours{}.

%\Paragraph{Drawback 1: Coarse-grained partitioning can significantly
%under-subscribe \client{} node resources.} State-of-the-art monitoring systems~\cite{everflow,
%sonata, dshark} have explored coarse-grained partitioning strategies---i.e., either all records are processed by an operator or none.
\Paragraph{Data-level query partitioning.}
Operator-level query partitioning could be undesirable when attempting to run a computationally expensive operator like grouping within limited compute resources provided by \client{}, because it could over-subscribe available resources. However, the alternative is for the partitioning mechanism to leave the resource highly underutilized.
To highlight this issue concretely, we execute the query in
Figure~\ref{fig:pipeline_tor} using 80\% of single core operating at 2.4GHz, which reflects
compute constraints on \client{}. The upper part of Figure~\ref{fig:data-partition-explain}
shows the resulting resource usage statistics in detail among the operators.
Because F operator drops only a small portion of input records, it is not
possible to execute the expensive G+R operator entirely on \client{}. This leads to
under-utilization of the available compute resources and generation of network traffic as high as 22.5 Mbps, which is close to the query input rate.

On the contrary, extending the operator-level partitioning model to support \datapart{} could significantly improve the utilization of limited compute resources on \client{}.
This fine-grained \datapart{} allows an operator to process a fraction of its input records on \client{} and drain the rest for remote processing. With this approach, as shown in the lower part of Figure~\ref{fig:data-partition-explain}, the operator G+R in the query can process 83\% of its input, resulting in total network traffic of 9.4 Mbps. Note that this traffic amount is 2.4x lower than the traffic generated by the coarser-grained operator-level partitioning strategy.

%\noindent \underline{Insight 1:} \emph{Extending the operator-level partitioning model to support data-level partitioning significantly improves the utilization of limited compute available on \client{} nodes.}

\Paragraph{Fast and accurate adaptation enabled by combining cost model-based and model-agnostic techniques.}
% \Paragraph{Fast and effective adaptation mechanism.}
% Partitioning approaches need to keep up with highly dynamic resource conditions on \client{}s.
The requirement for frequent and dynamic query refinement due to high variability in resource conditions calls for a highly efficient refinement approach. In particular, given the aforementioned dynamics, query planners may need to compute and execute a new and effective partitioning plan in a timely manner, even in seconds.

%The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently the available compute per-query. Given these dynamics, query planners need to compute and execute a new partitioning plan in a timely manner, even in seconds.

While optimal partitioning can be achieved using a query cost model and a centralized planner to leverage global information about available resources~\cite{sonata,ds2,optimal-odp},  it is computationally expensive due to high algorithmic complexity (NP-hard~\cite{jarvis-extended}). A cost model-based heuristic is attractive if it can efficiently be solved to obtain a partitioning solution. However, the model may not accurately capture complex query behavior~\cite{model-free-control-drl}. Solely relying on a cost model may lead to inaccurate partitioning. A greedy and embarrassingly parallel heuristic utilizing a combination of cost model-based and model-agnostic techniques enables fast, accurate and fully decentralized query refinement on each \client{}.


% \Paragraph{Drawback 2: Without fast \& accurate adaptation, partitioning approaches cannot keep up with highly dynamic resource conditions on \client{}s.}
% The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently the available compute per-query. Given these dynamics, query planners need to compute and execute a new partitioning plan in a timely manner, even in seconds.

% While optimal partitioning can be achieved using a query cost model \& centralized planner to leverage global information about available resources~\cite{sonata,ds2,optimal-odp},  it is computationally expensive due to high algorithmic complexity (NP-hard~\cite{jarvis-extended}). Other cost model-based query planners have been explored in literature without considering partitioning under highly variable \client{} resource conditions~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (Section~\ref{sec:RelatedWork}).
% Optimizing for a cost model is attractive if it can be solved efficiently for a partitioning decision. However, the model may not accurately capture complex query behavior, in which case solely relying on it leads to inaccurate decisions~\cite{model-free-control-drl}.
% , potentially leading to inaccurate partitioning decisions.
% Furthermore, it may not be feasible to obtain accurate performance models at runtime.

% \noindent \underline{Insight 2:} \emph{A greedy \& embarrassingly parallel heuristic utilizing a combination of cost model-based \& model-agnostic techniques enables fast, accurate and fully decentralized query refinement on each \client{}.}

% Furthermore, a greedy approach which relies solely on optimizing for a cost model may output an incorrect partitioning decision as the model may not accurately capture complex query execution behavior~\cite{model-free-control-drl}.

% Prior work relies on centralized query planners that leverage global information about available resources to solve an expensive optimization function~\cite{sonata} and on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Optimal partitioning is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach for partitioning. Other centralized and decentralized query planners have also explored model-free and model-based approaches but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}).
%\ours{} investigates a greedy and embarrassingly parallel approach which uses hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}.
%dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs.
% \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}
% A greedy and embarrassingly parallel approach utilizing a hybrid performance model-based and model-agnostic technique can enable fast and fully decentralized query refinement on each \client{}, which is accurate, robust and scalable and automatic.

\newcontent{\Paragraph{Can data synposes reduce network traffic?} Data synopsis techniques, such as sampling, histograms, and
sketches~\cite{synopsis-berkeley}, are commonly used to enable scalable
stream analysis by trading off accuracy for
performance~\cite{continuous-sampling-streams, mergeable-summaries}. Despite
their effectiveness and practicality, losing output accuracy may be undesirable for telemetry tasks such as anomaly detection, in which anomalies are hard to predict before they occur~\cite{omnimon}. Data that corresponds to anomalies are typically infrequent, so the lossy output could lead to undetected anomalies and affect server reliability. And false alarms may also require developers to manually review alerts which quickly become a burden when dealing with complex and large scale systems~\cite{thread-alert-fatigue}. Furthermore, debugging scenarios for server misconfigurations and failures such as gray failures~\cite{gray-failure} benefit from having access to per-node statistics at fine-grained timescales, to enable localizing and repairing of problematic server nodes. In Section~\ref{sec:sampling-vs-jarvis}, we compare the effectiveness (i.e., accuracy and network transfer costs) of \ours{} and a state-of-the-art window-based sampling
protocol~\cite{continuous-sampling-streams} using the query in Listing~\ref{lst:motivating-query}. In particular, when network transfer costs between the two approaches are almost at par, sampling misses a number of anomalous data points, resulting in high errors in the final query result.
}

%\subsection{Can we use data synposes?}
%\label{sec:data-summaries}

% Pingmesh query uses threshold-based technique for alerts. Sampling is sensitive to skew and outliers, and requires knowledge of the underlying distribution of values to apply estimators like Horvitz-Thompson (HT)~\todo{cite}. HT cannot be applied to max and min. More recently, Condor~\cite{condor-approx-streams} proposed integrating data synopses into stream processing engines.
% Scenarios which benefit include:
% \begin{myitemize}
% \item Anomaly detection: do not worry about false alarms or undetected anomalies due to measurement error.
% \item performance diagnosis or gray failures?
% \end{myitemize}
% Three types of monitoring queries:
% \begin{myitemize}
% \item Queries processing raw data~\cite{helios,gandalf}.
% \item Queries that can use statistical summaries: Several monitoring pipelines utilize data summaries to reduce the data traffic going to \server{} for processing. Statistics work well if the raw data is well-behaved, i.e., it follows a certain distribution such as Gaussian~\cite{statistics-online-anomaly-detect}.  \todo{Can we show Pingmesh rtt's do not follow any well-known distributions over time? What about non-parametric statistical techniques? Can we compare Jarvis with a statistical technique and show as much data reduction without the burden of configuring parameters and/or introducing false positives/negatives?}.
% \item The summaries can be part of the monitoring query itself. E.g., histogram calculation to summarize the collected data is part of the monitoring query in \dnnlog{} query. Section~\ref{sec:evaluation} shows the benefits of using \ours{} to improve the performance of such queries.
% \end{myitemize}


==> archive/introduction-v1.tex <==
\section{Introduction}
\label{sec:Introduction}

%Datacenters run numerous important applications such as web services, machine
%learning (ML) pipelines, analytics services and database systems. Datacenter
%operators employ monitoring and analytics systems to detect, troubleshoot and
%recover from performance crises which disrupt normal service
%operation~\cite{fingerprint, pingmesh, autoscaling, netbouncer, m3,
%deepview}. To provide timely resolution, monitoring data is collected and
%analyzed in real time by a stream processing engine such as Apache
%Flink~\cite{flink} or Spark Streaming~\cite{sparkstreaming}. These systems
%require (i) transporting massive amounts of data from monitoring data source
%to the stream processor, (ii) processing complex analytics queries containing
%a number of dataflow operators (e.g., data grouping, aggregates, joins), and
%(iii) supporting low latency processing within seconds for queries having low
%time-to-detection requirements~\cite{chi,google-log-analysis}. With the
%continuous expansion of datacenters~\todo{require citation}, larger number of
%datacenter nodes need to be monitored and thus meeting the above requirements
%is becoming increasingly challenging for monitoring systems~\cite{helios}.

Today's large-scale datacenters use thousands of servers to host important services, such as web search, database systems, and machine learning (ML) pipelines, for millions of users. Operating these services with high availability requires that datacenter operators quickly detect performance and reliability issues, such as high network latency, disk failures, service outages from software bugs~\cite{fingerprint, pingmesh,netbouncer,deepview,slack-observability,autoscaling, m3}, and resolve these issues in a timely manner to restore normal service operation~ \cite{sonata,helios,google-log-analysis}. 

To deliver highly available services, datacenter operators deploy a dedicated monitoring system that analyzes real-time events collected across datacenter servers using a \server{}, as shown in Figure~\ref{fig:arch}. By processing the collected data, the \server{} further enables operators to visualize the behavior of the monitored system via dashboards and generate alerts upon observing issues impacting service availability. \emph{Monitoring data streams} are diverse, including service-level application logs and host-level metrics (e.g., network latency and CPU utilization) used to monitor the health of various system resources. Large-scale monitoring pipelines can generate up to 10s of PBs per day, processing data from hundreds of thousands of servers~\cite{chi, google-log-analysis}. Transferring such a high volume of data to remote \server{}s can cause network bottlenecks.  Moreover, the \server{} may require thousands of CPUs to keep up with such massive data streams while satisfying low time-to-detection requirements for reliability issues~\cite{helios}. If more data is processed at the \client{}, the amount of data transferred and processed by the stream processor can be significantly reduced.

 \begin{figure}
   \centering
     \includegraphics[width=0.48\textwidth]{fig/architecture}
     \caption{Overview of a datacenter monitoring system.}
     %. There are separate servers for stream processor that finalizes monitoring query executions and reports the results to dashboard.\atul{Highlight the part that our paper focuses on  }
     \label{fig:arch}
     \vspace{-0.4cm}
 \end{figure}

\Paragraph{Challenges.} 
%Additionally, processing them is prohibitively expensive as it may require 1000s of CPUs on the \server{} if the latter was to meet the low time-to-detection requirements~\cite{helios}. 
Not surprisingly, several monitoring pipelines have leveraged available compute resources on \client{}s (i.e. server nodes) to deploy a monitoring agent. Because available resources on the \client{} typically result from resource over-provisioning to handle peak resource demands~\cite{helios, uber-neris-motivation, nutanix-motivation, resource-overprovision1, resource-overprovision2}, 
often the monitoring agent is restricted to run a subset of query operations (e.g., aggregation, filtering) within a given compute budget to minimize interference with the hosted service. 
Prior work statically decides which operations to run on \client{}~\cite{everflow,gigascope,jetstream}.  However, there is \textit{variability} in  monitoring data across time and between \client{}s.  Thus static partitioning may be too conservative or, alternately, may affect query performance during periods of high peak resource demands by the agent's query operators~\cite{chi,helios}.
% e.g. apply only filter operations or compute aggregations at the source

%Monitoring agents can be statically configured by identifying query operators (e.g., filter, group-based aggregation) whose resource requirements fit within the compute budget on \client{}. However, static query partitioning can become sub-optimal due to \textit{variability in monitoring data across time and \client{}s}, which results in variable compute resource requirements of the agent's query operators~\cite{chi,helios}. 
In the network telemetry domain, Sonata~\cite{sonata} has proposed a query cost model-based optimization approach to distribute query execution across programmable switches and the \server{}. The query partitioning in Sonata, occurring at the operator level~\cite{everflow,gigascope,jetstream}, is dynamically adjusted by a central query planner running on \server{}. A query operator is deployed to the switch only if the switch's available compute resources are sufficient to process all of the incoming data of the operator.
Unfortunately, operator-level query partitioning is not effective in scenarios where available compute resources are highly constrained, such as \client{}s in monitoring systems. Furthermore, solving an expensive optimization using a centralized query planner is unsuitable for making frequent decisions in systems with \client{}s that exhibit fast changing resource conditions. 

\Paragraph{Our proposal.} We propose \ours{}, a monitoring system that targets large-scale systems generating \textit{high-volume data streams} with \textit{high variability across time and \client{}s}. \ours{} identifies independently for the query workload on each \client{}, a fine-grained \emph{\datapart{}} strategy by controlling the amount of data processed per query operator, namely \emph{load factor}. \ours{} can make frequent partitioning decisions by combining a model-based technique that quickly finds initial per-operator load factors with a model-agnostic technique that monitors query execution and fine-tunes the load factors if needed. Fine-grained data-level partitioning allows \ours{} to fully utilize the limited and dynamic compute resources over \client{}s while minimizing  network  data transfers. \ours{} is implemented in a fully decentralized manner, enabling it to scale to large number of \client{}s.

To achieve these goals, \ours{} introduces novel extensions to the pipeline of conventional query execution: the \emph{Control proxy} and the \emph{Jarvis runtime}. Control proxy is a light-weight routing logic---associated with a query operator---that given the current load factor decides ``how many'' incoming records should be forwarded to the associated query operator, realizing data-level partitioning per operator. In each \client{}, the local Jarvis runtime interacts with all the control proxies to identify their state (e.g., idle, congested, or stable) and  fine-tune the load factors of the control proxies. On observing state changes for the control proxies, Jarvis runtime refines its plan for the data-level partitioning to keep the query execution in each \client{} stable.

%\Paragraph{Evaluation.} 
We have built a fully functional proof-of-concept of \ours{}. Our evaluation with monitoring queries on host-level network latency metrics and application logs demonstrate that \ours{} enables a \server{} node to handle up to 75\% more \client{}s while improving query throughput by up to 4.4x over state-of-the-art partitioning strategies. \ours{} converges to a stable query configuration within seven seconds of a resource change occurring on \client{}.

\Paragraph{Contributions.} In summary, we make the following contributions: (1) we propose a fine-grained data-level partitioning mechanism with the goal of minimizing network data transfers while maximizing resource utilization on each \client{} node, (2) we design a fully decentralized query workload partitioning engine which quickly adapts its data-level partitioning strategy to dynamic resource conditions on each \client{} node while scaling to a large number of \client{}s, and (3) we experimentally evaluate our system with several monitoring queries and show its effectiveness.

==> archive/model.tex <==
\section{Models and Problem Definition}
\label{sec:models}
This paper investigates techniques to partition/distribute query operators between \client{} and \server{} nodes, to address the challenges with building large-scale server monitoring pipelines. In this section, we discuss models/assumptions and then define the query partitioning problem. 
\ifthenelse{\boolean{Extended}}{Table~\ref{tab:notation} provides a summary of the variables used in the rest of the paper.}
 
\Paragraph{Data and query models:} Monitoring data is an unbounded stream of
\emph{records}. In the stream, a single record is a
measurement or text log generated by the underlying host or application on
the server node. Each record has an associated timestamp which defines an event
time when the record was generated. The data stream also includes
\emph{watermark} records with strictly increasing timestamps.
A watermark with timestamp $w_{ts}$ guarantees no subsequent records will have a record time
earlier than $w_{ts}$. As a result, on observing watermarks, a single stream could be delimited into ordered consecutive \emph{epochs}
of records while promising time progresses. \ifthenelse{\boolean{Extended}}{An epoch may have records with timestamps greater than the epoch's end watermark due to out-of-order arrival.}

Each monitoring query is represented as a
directed acyclic graph (DAG) $G = (V,E)$. The vertices V in the DAG represent
stream operations such as
filter, grouping, reduction, etc, which transform their input records and emit output records to downstream operations, as shown in Figure~\ref{fig:pipeline_tor}. The edges $E$ denote dataflow dependencies
between operations. \ifthenelse{\boolean{Extended}}{An instance of the query $G$ deployed on a \client{}
$i$ is denoted by $G_{i}=(V_{i},E_{i})$.}

\Paragraph{Resource model:} Physical resources involved in the query execution can be seen as a
tree structure as shown in Figure~\ref{fig:arch-monitoring-scale}(b), where leaf
nodes represent the \client{}s that primarily run customer applications. In each leaf node, fixed amount of compute resources are allocated to facilitate monitoring queries. Such allocation can be done by provisioning a container
to isolate the resources (e.g. 1 core and 1 GB RAM) for
monitoring from foreground services. Each \client{} can send data to its parent \server{} node (i.e., intermediate node) and leverage its compute resources for query processing. The intermediate nodes eventually send data to root \server{} node which completes the query before outputting final result.

\Paragraph{Operator partitioning:} \ifthenelse{\boolean{Extended}}{Monitoring queries typically
consist of operations which filter out uninteresting records, aggregate
statistics, etc.~\cite{fingerprint,pingmesh, netbouncer, aomg}.} Given a query instance with $M$ operations, a partitioning plan identifies operations that can execute locally on each \client{} and those that require remote execution on it's parent node. To illustrate, consider a topologically sorted list of $M$
operators from the query graph $G$ following dataflow dependencies of the query. Due to underlying resource
topology, we can $partition$ the operators into two groups and split the query execution across the \client{} and other remote nodes. To this end, we can define a boundary operator $b_i$ for the $i^{th}$ \client{} to indicate operators prior to $b_i$ in the topological order are
executed on \client{} and those after $b_i$ are executed remotely.
For instance, for a \client{} $i$ with $M=4$ operators, $b_i=3$ means first 3
operators execute on \client{} and the last operator executes remotely.

\Paragraph{Refinement model:} When resource conditions change on a \client{} node, the query needs to be refined i.e. a new partitioning plan needs to be identified so that its compute needs meet available resource budget. To initiate refinement, \client{}s periodically inject \emph{refinement watermarks} into the stream (similar to~\cite{trill}) and they
delimit ordered consecutive \emph{refinement epochs} of records. Refinement watermarks are different from the traditional watermark described in data model. Epoch and watermark refer to refinement epoch and refinement watermark respectively, in the rest of the paper.

\ifthenelse{\boolean{Extended}}{
\begin{table*}[t]
\begin{tabular}{ |p{1.6cm}|p{15cm}|  }
 \hline
 \multicolumn{2}{|c|}{Common variables} \\
 \hline
 $M$ & Number of operators in the query\\
 $N$ & Total number of records injected into the query in an epoch\\
 \hline
 \multicolumn{2}{|c|}{Operator partitioning problem} \\
 \hline
 $N_d$ & Number of \client{}s\\
 $b_i$ & $b_i \epsilon [0,M]$ to denote the index of boundary operator where the partitioning occurs for $i^{th}$ \client{}\\
 $B$ & partition profile for the query with $b_i$ denoting boundary operator for $i^{th}$ \client{}\\
 $x_{ij}$ & indicates whether $b_i=j$\\
 $dr_{ij}$ & rate of data sent from \client{} to \server{} when $b_i=j$\\
 $T_{local}(i,b_{i})$ & computes local computation time for executing operators until $b_{i}$ on the $i^{th}$ \client{}\\
 $T_{remote}(i,b_{i})$ & computes network transmission time cost of intermediate output from $b_{i}^{th}$ operator to its parent node along with computation time cost of executing operators after $b_{i}$ on parent node\\
 \hline
 \multicolumn{2}{|c|}{Data partitioning problem} \\
 \hline
 $Op_{i}$ & $i^{th}$ operator in the query\\
 $r_{j}$ & relay ratio of $Op_{j}$ i.e. fraction of input records relayed to the next operator $Op_{j+1}$ after they are consumed by $Op_{j}$\\
 $c_i$ & compute cost of $Op_{i}$ for a single record\\
 $d_{i}$ & number of records drained in an epoch, at the $i^{th}$ \proxy{}\\
 $C$ & compute budget available to the query\\
 $p_{i}$ & $i^{th}$ \proxy{}'s load factor i.e. fraction of input records added to downstream queue and consumed by downstream operator\\
 $e_{i}$ & effective load factor for $i^{th}$ \proxy{} i.e. product of load factors of sequence of upstream query operators until $Op_{i}$, in the transformed optimization problem\\
%  \hline
%  \multicolumn{2}{|c|}{Input parameters} \\
%  \hline

%  \hline
%  \multicolumn{2}{|c|}{Resource Constraint} \\
%  \hline
%  \hline
%  \multicolumn{2}{|c|}{Output} \\
%  \hline
 \hline
\end{tabular}
\caption{\label{tab:notation}Summary of variables used in the paper}
\end{table*}
}{
\begin{table}
\begin{tabular}{ |p{0.3cm}|p{7.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Summary of variables used in the paper} \\
 \hline
 $M$ & Number of operators in the query\\
 $N$ & Total number of records injected into the query in an epoch\\
 $b_i$ & $b_i \epsilon [0,M]$ to denote the index of boundary operator where the partitioning occurs for $i^{th}$ \client{}\\
 $B$ & partition profile for the query with $b_i$ denoting boundary operator for $i^{th}$ \client{}\\
 $Op_{i}$ & $i^{th}$ operator in the query\\
 $r_{j}$ & relay ratio of $Op_{j}$ i.e. fraction of input records relayed to the next operator $Op_{j+1}$ after they are consumed by $Op_{j}$\\
 $c_i$ & compute cost of $Op_{i}$ for a single record\\
 $d_{i}$ & number of records drained in an epoch, at the $i^{th}$ \proxy{}\\
 $C$ & compute budget available to the query\\
 $p_{i}$ & $i^{th}$ \proxy{}'s load factor i.e. fraction of input records added to downstream queue and consumed by downstream operator\\
 $e_{i}$ & effective load factor for $i^{th}$ \proxy{} i.e. product of load factors of sequence of upstream query operators until $Op_{i}$, in the transformed optimization problem\\
%  \hline
%  \multicolumn{2}{|c|}{Input parameters} \\
%  \hline

%  \hline
%  \multicolumn{2}{|c|}{Resource Constraint} \\
%  \hline
%  \hline
%  \multicolumn{2}{|c|}{Output} \\
%  \hline
 \hline
\end{tabular}
\caption{\label{tab:notation}}
\vspace{-0.5cm}
\end{table}
}

\Paragraph{Problem definition:} 
\ifthenelse{\boolean{Extended}}{
We define the operator partitioning problem as follows (Table~\ref{tab:notation} describes the variables used):

\begin{align*}
    & \displaystyle \min_{\textbf{B}} \sum_{i=1}^{N_{d}}\sum_{j=1}^{M} dr_{ij} x_{ij}\\
    subject\ to,&\\
    & T_{local}(i,b_{i}) <= T_{remote}(i,b_{i})\ \forall b_{i}>0, i\epsilon[1,N_{d}]
\end{align*}

Network transfer and compute costs are incurred on \server{}, when data is sent from \client{} for remote processing. Our optimization goal is to
minimize the processing load sent to \server{} subject to the processing time not being delayed i.e. local computation not introducing additional delay compared to remote execution, in the processing of each data stream from being reflected in query output. We prove that the operator partitioning problem is NP-hard in Section~\ref{sec:appendix-optimal-partitioning}. This is because of finite resources available on \server{} which requires joint partitioning decision to be made across \client{}s.
}{
Given the network and compute resources available on \server{}, maximize  the number of \client{}s that can be served. Our optimization goal is to find a partition profile $\textbf{B}$ of boundary operators which minimizes processing load sent to \server{}, subject to local computation not introducing additional delay in the processing of each data stream, compared to remote execution. Formal definition and proof that the problem is NP-hard can be found elsewhere~\todo{cite}.} %In the extended version of the paper~\todo{cite}, we provide formal definition of the problem and prove that it is NP-hard. This is because of finite resources available on \server{} which requires joint partitioning decision to be made across \client{}s.}
% Compute resources on \server{} are used to process operators sent for remote execution after partitioning. Data transport also incurs network transfer cost. As we increase the number of \client{}s, the processing load from different \client{}s can result in network/compute bottleneck on \server{}, thus hurting query processing time.  When the remote resources are saturated, it is more beneficial for the \client{} to execute operators locally to avoid long processing time.

%  \todo{Note that the constraint for each \client{} will ensure that changes from each stream are reflected in final output without additional processing delay (e.g. incremental avg)}

% \begin{itemize}
%     \item Large number of edge nodes, relative to cloud
%     \item Per edge node resources for query processing less than cloud node
%     \item Cloud side nodes contain configurable aggregation servers
%     \item Single query involving groupby, filter, project, sort, percentile
%     \item Source rate is dynamic, with each edge node having different source rate
%     \item Problem Definition
% \end{itemize}

\section{Motivation for \ours{}}
\label{sec:drawbacks}

\Client{}s have limited compute, while query resource demands are highly
dynamic as explained in Section~\ref{sec:variabilities}. Given this, we
highlight the drawbacks of existing approaches in addressing the operator
partitioning problem and insights that \ours{} provides.

% Prior works have explored various techniques to address the operator partitioning problem to reduce network transfer costs and adapt to varying resource conditions at runtime.
% Since these operators result in data reduction, it would be ideal to run as much of the query on \client{}s as possible, to reduce network transfer costs.

% and refine the distributed execution to meet the query's resource demand under resource constraints on \client{} nodes

%However, this is unlikely because (i) as explained in
%Section~\ref{sec:variabilities}, resource demands for queries are highly
%dynamic and often surpass the available resources, (ii) multiple concurrent
%queries share the limited resources available in each \client{} node.
%Instead, an opportunity exists to partition query execution between \client{}
%and \server{} nodes, and refine the distributed execution to maintain the
%query's resource demand within the given resource budget. Now, we want to
%raise a question: ``do existing approaches apply well to datacenter
%monitoring scenarios''? We reveal two drawbacks as follows:

\Paragraph{(Drawback 1) Coarse-grained partitioning can significantly
undersubscribe \client{} node resources:} Existing works~\cite{everflow,
sonata, dshark} have explored partitioning strategies which are
coarse-grained, i.e., either all records are processed by an operator or
none. To examine its limitation, we execute the query in
Figure~\ref{fig:pipeline_tor} using 80\% of single core (2.4~GHz), to reflect
compute constraints on \client{}. Figure~\ref{fig:data-partition-explain}
shows that F operator drops only a small portion of input records, so we are
not able to execute the expensive G+R operator on \client{}. This leads to
under-subscription of the compute and generates network traffic as much as
22.5 Mbps.
% Because of this limitation, operator partitioning may not allow compute-expensive operators that bring huge data reduction (e.g., G+R operator in Figure~\ref{fig:pipeline_tor}) to run on the \client{}.

\begin{figure}[t]
\centering
%\subfigure[Filter operator]{\includegraphics[width=1.65in,height=1.3in]{fig/FilterProfileHighInpRate.pdf}}
\includegraphics[width=\linewidth]{fig/DataPartitionExplain.pdf}
%\vspace{-0.1in}
\caption{\label{fig:data-partition-explain} Coarse-grained operator vs. fine-grained data partitioning on \client{} with CPU budget of 80\%. G+R requires 80\% CPU to process all the output data from F operator.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

Data partitioning is fine-grained i.e. it enables an operator to process a
fraction of its input records on \client{} and drain the rest for remote
processing. In this case, G+R can process 83\% of its input 22.5 Mbps and greatly reduce it to result in a total of 9.4 Mbps (5.6+3.8 Mbps) leaving \client{} node. This is a
significant decrease over 22.5 Mbps in operator partitioning.
% , it would incur large compute cost to process most of input data (i.e. 22.5 Mbps).

% For the same input rate of 26.2 Mbps used in Section~\ref{sec:variabilities}, we observe that executing both F and G+R operators on \client{} oversubscribes compute budget (together they require over 100\% CPU). This is because

% %We obtain this data reduction because- F operator
% %outputs 23.39 Mbps (since it's filter-out rate is 86\%).
% Given budget of 80\% of a core on \client{}, F operator consumes 13\% CPU, so by allowing partial execution, G+R can use 67\% of the core idling time (i.e., 13\% for F + 67\% for partial execution of G+R) to process 83\% of the records received from F operator.
% % This allows G+R operator to compute aggregate latency distribution statistics. %\qts{} for a majority of data, i.e. 83\% of 22.5 Mbps or 18.7 Mbps.
% G+R operator reduces the input data size by 30\%, so it outputs the results at 5.6 Mbps. The remaining records %from F operator which were not processed by G+R gets drained to \server{} node at the rate of 3.8 Mbps. Thus, the total data sent out of \client{} becomes 9.4 Mbps.\\
\noindent \underline{Insight 1:} \emph{Extending the operator partitioning model to support data partitioning can significantly improve the utilization of limited compute available on \client{} nodes.}

% (i.e. 6.47 Mbps + 4.89 Mbps).
%(i.e. 6.47 Mbps processed data after applying G+R operator plus 4.89 Mbps %drained data after applying F operator).
%---when it comes to traffic
%aggregated across all \client{} nodes in datacenter, the effect of data
%partitioning is huge.


% The following summarizes our observations:
% \begin{myitemize}
% \item Executing the
%     entire pipeline on \client{} node is inadequate as it \emph{oversubscribes} the
%     compute budget---F operator
%     and G+R operator require 23\% and 92.8\% of the compute budget,
%     respectively, which is together over 100\%. G+R operator is unable to
%     fully execute since F operator just drops a
%     small portion (14\%) of erroneous probes.

% \item Operator partitioning that runs only F operator on \client{} node
% %and G+R operator on \server{} node
%     largely \emph{undersubscribes} the compute budget, with 77\% of the core idling.
%     It also generates the network traffic as much as 22.5 Mbps, a marginal reduction over the data input rate of 26.2~Mbps.
% \end{myitemize}
% MJ: we don't have time to integrate hot key stuff for now. But, will put it back once it's up and running at Jarvis.
% %When performing data partitioning, we observe an opportunity for higher
%reduction on network volume by primarily focusing on \emph{hot grouping
%keys}, which are keys occurring in a higher proportion of input records
%compared to cold grouping keys, as a result of data skewness~\cite{keyskew}.
%In Section~\ref{sec:data-partitioning-hot-keys}, we show evidence for
%existence of hot keys in real world traces and discuss in detail how hot key
%based data partitioning is done in \ours{}.
% and populate more records than colder grouping keys
%\emph{In summary, to better utilize resources allocated for monitoring
%workloads and to achieve effective network volume reduction, we need a
%mechanism to support hot key-based data partitioning across the execution of
%the entire query pipeline. }

\Paragraph{(Drawback 2) Slow adaptation cannot keep up with highly dynamic resource conditions on \client{}s:} The requirement for frequent and dynamic query refinement (as illustrated in Section~\ref{sec:variabilities}) is more prevalent in practice since \client{}s are shared by multiple in-flight queries which are initiated or terminated by engineers at runtime~\cite{m3}, changing the available compute per-query. Given these dynamics, query planners need to compute and realize (i.e. execute) a new refinement in a timely manner, even in seconds once requested.

% Previous works frame the query refinement problem as an optimization
In previous works, centralized planners leveraged global information about available resources to solve an expensive optimization function~\cite{sonata} and relied on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Doing so is computationally expensive (see Section~\ref{sec:models}). Other centralized and decentralized query planners have been explored but they do not consider the dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}). \ours{} investigates a greedy approach which is embarrassingly parallel and relies on a hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}. \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}

% Furthermore, such an approach causes monitoring system to suffer overheads, e.g., receiving/sending messages from/to all \client{} nodes, thus making query refinement an expensive process.
\noindent \underline{Insight 2:} \emph{A greedy and embarrassingly parallel approach can enable fast and fully decentralized query refinement on each \client{}, which is accurate, scalable and automatic.}
% This enables fast reaction to a lot of variations discussed in Section~\ref{sec:variabilities}
% In this paper, we propose \ours{} to provide two clear benefits over existing
% approaches. (i) \ours{} explores \emph{data partitioning} which executes part
% of the input stream on each operator. Data partitioning finds a good
% compute-communication tradeoff by partitioning data processed by costly
% operators and thus maximizing the utilization of compute resources in data
% source node. (ii) \ours{} makes fast, accurate, automatic query refinement
% decisions in a \emph{fully decentralized} manner. This enables fast reaction
% to a lot of variations discussed in Section~\ref{sec:variabilities}.

%Furthermore, previous works have explored scalability and availability %benefits of performing decentralized scheduling for query execution engines %~\cite{apollo,sparrow}.

% \ours{} proposes a fully decentralized and fine-grained query workload partitioning mechanism which enables fast adaptation of the partitioning plan on each \client{} node to dynamic resource conditions.

% and to increase overall latency in searching new partitioning plans for queries and responding to the nodes.

% \sout{However they are focused on batch processing applications. Recently, Drizzle\hbox{~\cite{drizzle}} argued for centralized scheduling in micro-batch streaming jobs due to scheduling dependencies across micro-batches of a single job. We are focused on the continuous operator streaming model\hbox{~\cite{timestream}}, with the primary objective of minimizing transfer of data to central stream processor.
% \\
% (Drawback 3) Accurate operator profiling is challenging: Accurate optimization parameters such as operator execution costs may not be available from online profiling, to feed into query planner. Sonata relies on historical traces as training data to determine resource cost for executing an operator on a switch but their estimates are conservative, based on total number of unique keys they expect for each stateful operation. In Jarvis, given the complex compute usage of query operators, such as compute varying between 50-350\% for G+R operator based on input size and output group count, accurate estimation of resource cost is challenging.
% }

% \subsection{Insights for Jarvis}
% \label{sec:insights}
% \Paragraph{How beneficial data partitioning is?}
% \Paragraph{Scaling to large number of \client{}s:}

%We now describe the focus of our optimization efforts for monitoring systems
%to scale to a large number of \client{}s.
%Figure~\ref{fig:arch-monitoring-scale} shows a monitoring pipeline wherein
%\server{} integrates several levels of computing nodes hierarchically. Each
%of the \client{}s communicates with a direct intermediate \server{} node at
%level $L_1$. The final output is generated at the root node. Each
%intermediate \server{} node has a maximum capacity for the monitoring data
%traffic it can process. Beyond this capacity, it hits network transfer and/or
%compute bottleneck at which point it cannot scale further. So as we increase
%the \client{}s, we would need to provision more intermediate \server{}s and
%possibly introduce additional levels in the topology.
%
%Query workload is distributed across the hierarchy of nodes in
%Figure~\ref{fig:arch-monitoring-scale} to progressively reduce network
%transfer size until we reach the root node. Consider a fixed topology for
%\server{}, monitoring data stream and a query whose workload is distributed
%across the \client{} and \server{} nodes. Let \textit{relay ratio} refer to
%fraction of input records at each node that are relayed to its parent node
%over the network, after being processed in that node. $NodeRelay_i$ is the
%maximum such relay ratio across the nodes in level $L_{i}$ where $H$ is the
%height of the tree, $i\epsilon[0,H]$ and $NodeRelay_i\epsilon[0,1]$. We note
%that the minimum number of \client{}s that can be supported by such a system
%$N_{data sources} \propto \frac{1}{\prod_{i=0}^{L_{H-1}} NodeRelay_{i}}$. A
%more detailed analysis and assumptions made to derive this relation are
%described in Section~\ref{sec:appendix}\todo{Link to tech report}. This
%relation describes the intuitive understanding that as we reduce size of data
%sent over the network at each level in the tree, the system scales better to
%handle traffic from more \client{}s. We use this insight to deploy \ours{} on
%each of the \client{}s and intermediate \server{}s and focus our optimization
%efforts on minimizing network traffic sent from multiple \client{}s to a
%single \server{} node.


==> archive/motivation.tex <==
\section{Challenges for Large-scale Server Monitoring}
\label{sec:challenges}
Given the input-dependent highly-varying resource usage characteristics of operators, we discuss the nature of monitoring data streams to understand their impact on query execution costs and associated challenges. 

\subsection{Illustrative Example}
\label{sec:motivating-query}

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{Pipeline of stream operations for motivating example query (detailed query in Listing~\ref{lst:motivating-query}).}
    \label{fig:pipeline_tor}
    \vspace{-0.4cm}
\end{figure}

We use a real-world query on Microsoft's \pingmesh{} trace as an illustrative example to highlight the challenges. In \pingmesh{}, servers in the datacenter probe each other to measure network latency for server pairs across the datacenter. A server sends a probe message, generating a 86B record, including timestamp (8B), source IP address (4B), source cluster ID (4B), destination IP address (4B), destination cluster ID (4B), round trip time (4B), and error code (4B). %The round trip time is in microseconds.

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}

\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}

This rich set of record fields allows exhaustive analyses, such as zoom-in/out
latency probes by grouping them across datacenter network hierarchy to identify issues at the cluster, ToR or spine switch and server level~\cite{tersecades, pingmesh}. Listing~\ref{lst:motivating-query} describes the implementation of the real-world \pingmesh{} query. The query is written in a declarative programming model used by popular stream engines, such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming}, which express a query using dataflow operations. Figure~\ref{fig:pipeline_tor} shows a pipeline of how data flows between operators for the query in Listing~\ref{lst:motivating-query}.

\subsection{Challenges}
Consider the traditional approach where the entire data from \pingmesh{} is aggregated into \emph{stream processor} to be analyzed. Assume that a datacenter has 200k servers. Each server may probe 20k other servers with a probing interval of 5 seconds ~\cite{pingmesh}. In such case, the data generation rate is estimated to be 512.6~Gbps due to the large-scale probing performed by 200K servers. Transferring such \textbf{high volumes of data} may result in network bottlenecks and incur high cost due to  provisioning high amount of compute resources on \server{}. 

\begin{figure}[t]
  \centering
    \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
    \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
    \label{fig:data-gen-rate}
    \vspace{-0.4cm}
\end{figure}

\textbf{High variability in the data} also results from changing data rates and their distribution across servers over time. In the \pingmesh{} system: 
\begin{myitemize}
\item A subset of servers probe a larger set of peers to cover a wider network range on behalf of other servers in the same ToR switch~\cite{pingmesh}. We measure data rates of network probe messages generated by individual \client{}s, illustrated in  Figure~\ref{fig:data-gen-rate}. The data rates are normalized to the highest one observed among \client{} nodes. Data generation rates exhibit high variability, with 58\% of nodes generating 50\% or lower of the highest data rate we observe.
\item When servers are being over-loaded, latency profiles become more variable~\cite{rubik, pegasus}. If a monitoring system runs a query to diagnose such network condition, it should quickly adapt the query to process a larger amount of network probes of high latency.
\end{myitemize}

Variability in data complicates resource usage characteristics of query operators during pipeline execution. Declarative operators in a pipeline execute in sequence as shown in Figure~\ref{fig:pipeline_tor}. Resource demand for an operator is affected by its incoming data rate after executing all preceding operators. For example, F operator leads to the first data volume reduction from the input stream (see filtering predicate in Listing~\ref{lst:motivating-query}). Since erroneous, insignificant records are not dominant, the operator happens to drop only a small fraction of records. A majority of records are then to be processed by G+R operator, increasing compute cost for the query. However, if we were to toggle the
filtering predicates to perform a zoom-in analysis on a small subset of erroneous data, there will be a high degree of data reduction in F operator, so G+R operator considerably lowers its resource usage.

\subsection{Summary}
While we focused on the \pingmesh{} example, we note that other real-world monitoring systems have observed similar monitoring data characteristics: (i) \textit{high volume}, logs collected from applications can generate up to 971 Gbps as per~\cite{chi}. Other systems~\cite{gandalf,m3} process up to tens of TB data per day or millions of events every second per monitoring task, straining compute, memory, and network capacities of the monitoring system; and (ii) \textit{high variability},  ingestion rates for log streams generated in production monitoring systems exhibit high variation~\cite{chi,helios}. 

Finally, we observe \Client{}s often generate monitoring data tightly associated with their targets to monitor (e.g., \# HW devices) and occurrences of anomalies (e.g., \# high-latency events for network/storage), which happen to be non-uniform across nodes. Resource requirements of queries on \client{} nodes are thus, \emph{different} and \emph{independent} of each other.
% To handle processing load from a large number of \client{} nodes, the \server{} may integrate several levels of computing nodes. 

Keeping up with high and unpredictable load of data, monitoring pipelines are over-provisioned with large amount of compute and memory resources, which are distributed across several nodes. This pressing issue suggests that achieving high efficiency and scalability is a key design challenge for modern large-scale server monitoring systems. 


%---(i) non-uniform data generation across \client{} nodes, (ii)
%non-uniform operator execution costs, (iii) XXX, and (iv) YYY \mj{can delete
%(i)-(iv) here}---



%\Paragraph{Data generation rates across \client{} nodes:} We first measure
%data generation rates for network latency monitoring over individual
%\client{}s, and show the results in Figure~\ref{fig:data-gen-rate}. The data
%rates are normalized to the highest one observed among \client{} nodes. Data
%generation rates exhibit high variability, especially with 58\% of nodes
%generating 50\% or lower of the highest data rate we observe.
%
%It is quite natural to have such variability in many cases as \client{} nodes
%generate monitoring data tightly associated with their targets to monitor
%(e.g., \# HW devices) and occurrences of anomalies (e.g., \# high-latency
%events for network/storage), which happen to be non-uniform across the nodes.
%In network latency monitoring, some servers probe a larger set of peers to
%cover a larger network range on behalf of other servers in the same ToR
%switch~\cite{pingmesh}. We also analyzed a publicly available production
%trace of deep neural network (DNN) training workload~\cite{philly} and
%observed a similar trend in variability of data generation rate. Not
%surprisingly, recent works have reported variability in data generation rates
%in other monitoring scenarios as well~\cite{chi,helios}. In summary, this
%analysis on data generation rates indicates that the resource requirements of
%\client{} nodes are \emph{different} and \emph{independent} of each other.


%We also analyzed a publicly available production trace of deep neural network
%(DNN) training workload~\cite{philly} and observed a similar trend in
%variability of data generation rate.



%Notice that in the presence of non-uniform data generation rates
%across \client{} nodes, we expect G+R and J operators to have more variable
%resource demands.

%Thus, query operators have complex resource usage characteristics, depending
%on the input data distribution at each operator.

% \begin{figure}[t]
%   \centering
%     \includegraphics[width=2.4in]{fig/FilterGroupbyProfile.pdf}
%     \caption{Profiling resource usage of query in Figure~\ref{fig:pipeline_tor}}
%     \label{fig:query-profile-op-pipeline}
% \end{figure}

==> archive/motivation_extended.tex <==
\section{Monitoring Workload Characteristics}
\label{sec:motivation_ext}

%Many telemetry queries require processing large raw data to produce a small
%number of aggregate statistics as performance indicators (e.g., average,
%count, top-k, and \qt{})~\cite{fingerprint, pingmesh, netbouncer, aomg},
%capturing root-cause signatures from logs of failed jobs~\cite{?, philly},
%etc. Therefore, to reduce network transfer costs, it would be ideal to always
%run, if not all, as much of the query on \client{} nodes, but the limitation
%is that datacenter operators assign only a small amount of HW resources
%(e.g., 1-2 cores) from individual \client{} nodes to cater to datacenter
%monitoring. As the resources are shared by multiple concurrent queries, not
%all in-flight queries can typically be pushed to the \client{}. Nonetheless,
%as done in recent work~\cite{sonata, dshark}, an opportunity still exists to
%partition query execution between \client{} and \server{} nodes, while
%maximizing partial query execution on \client{} nodes within the available
%compute budget.

%To avoid competing with foreground services, datacenter operators assign only
%a limited amount of HW resources from individual \client{} nodes for
%monitoring agents to pre-aggregate data and reduce network transfer costs. As
%the resources are shared by multiple in-flight monitoring queries limiting
%per-query resource budget, it is possible to partition a query, and push a
%subset of query computations close to \client{} as suggested
%in~\cite{everflow, sonata, dshark}. In this section, we first describe the
%motivating example for our work. We then discuss difficulties in estimating
%query computations which can execute at the \client{} and look at drawbacks
%of existing query partitioning solutions when used for datacenter monitoring.

Datacenter operators assign the monitoring system only a limited amount of HW
resources (e.g., only few cores) from individual \client{} nodes to promise
little interference with foreground services. The resources allowed per
monitoring query could be even more scarce as multiple queries with different
monitoring tasks could run on the system at the same time. Many prior works
take an approach to pre-process the query on limited resources by pushing a
subset of query computations close to \client{}, reducing data movements over
the network~\cite{everflow, sonata, dshark}. In this section, we discuss one
of our target scenarios in detail to reveal workload characteristics that
limit effectiveness of the existing approaches.

\subsection{Network Latency Monitoring Example}
\label{sec:motivating-query}

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{Pipeline of stream operations for motivating example query (detailed query in Listing~\ref{lst:motivating-query}).}
    \label{fig:pipeline_tor}
    \vspace{-0.4cm}
\end{figure}

We use a real-world trace on datacenter network latency monitoring,
\textit{Scenario 1}, collected from \pingmesh{} in Microsoft. In \pingmesh{},
servers in the datacenter probe each other to measure network latency for
server pairs across the datacenter. A server sending a probe message
generates a 86B record, including timestamp (8B), source IP address (4B),
source cluster ID (4B), destination IP address (4B), destination cluster ID
(4B), round trip time (4B), and error code (4B). The round trip time is in
microseconds.
%We refer to this dataset as \pingmesh{}.

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}

\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}

This rich set of record fields allows exhaustive analyses: e.g., zoom-in/out
latency probes by grouping them across datacenter network hierarchy to
identify issues at the cluster, ToR or spine switch and server
level~\cite{tersecades, pingmesh}. Here, we describe implementation of a real
query based on \pingmesh{} dataset in Listing~\ref{lst:motivating-query}. As can be
seen, we adopt a declarative programming model used by popular stream
engines such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming},
which express a query using dataflow operations.
Figure~\ref{fig:pipeline_tor} shows a pipeline of how data flows between
operators for the query in Listing~\ref{lst:motivating-query}.
%This query runs in production environment of an enterprise datacenter to
%perform fine-grained server-level latency analysis when diagnosing network
%latency issues.

% To facilitate effective monitoring, the observed results are visualized on a heatmap, as shown in Figure~\ref{fig:arch}.

% Our monitoring system supports a temporal query interface that allows programmers to easily express specific monitoring tasks over data stream of interest.
% We adopt a declarative programming model also used by popular stream engines such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming}, which express a query using dataflow operations such as filter, map, groupby, join, reduce over data stream. Listing~\ref{lst:motivating-query} shows the production query for network latency monitoring discussed in Section~\ref{sec:motivating-query}.

\subsection{Variabilities in the Wild}
\label{sec:variabilities}

Datacenter monitoring workloads exhibit variabilities in many aspects. We
describe four aspects that make precisely estimating resource requirements of
queries at scale highly complicated.
%---(i) non-uniform data generation across \client{} nodes, (ii)
%non-uniform operator execution costs, (iii) XXX, and (iv) YYY \mj{can delete
%(i)-(iv) here}---

\begin{figure}[t]
  \centering
    \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
    \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
    \label{fig:data-gen-rate}
    \vspace{-0.4cm}
\end{figure}

%\Paragraph{Data generation rates across \client{} nodes:} We first measure
%data generation rates for network latency monitoring over individual
%\client{}s, and show the results in Figure~\ref{fig:data-gen-rate}. The data
%rates are normalized to the highest one observed among \client{} nodes. Data
%generation rates exhibit high variability, especially with 58\% of nodes
%generating 50\% or lower of the highest data rate we observe.
%
%It is quite natural to have such variability in many cases as \client{} nodes
%generate monitoring data tightly associated with their targets to monitor
%(e.g., \# HW devices) and occurrences of anomalies (e.g., \# high-latency
%events for network/storage), which happen to be non-uniform across the nodes.
%In network latency monitoring, some servers probe a larger set of peers to
%cover a larger network range on behalf of other servers in the same ToR
%switch~\cite{pingmesh}. We also analyzed a publicly available production
%trace of deep neural network (DNN) training workload~\cite{philly} and
%observed a similar trend in variability of data generation rate. Not
%surprisingly, recent works have reported variability in data generation rates
%in other monitoring scenarios as well~\cite{chi,helios}. In summary, this
%analysis on data generation rates indicates that the resource requirements of
%\client{} nodes are \emph{different} and \emph{independent} of each other.

\Paragraph{Data generation rates across \client{} nodes:} \Client{} nodes
often generate monitoring data tightly associated with their targets to
monitor (e.g., \# HW devices) and occurrences of anomalies (e.g., \#
high-latency events for network/storage), which happen to be non-uniform
across the nodes. For example, in network latency monitoring, some servers
probe a larger set of peers to cover a larger network range on behalf of
other servers in the same ToR switch~\cite{pingmesh}.
%We also analyzed a publicly available production trace of deep neural network
%(DNN) training workload~\cite{philly} and observed a similar trend in
%variability of data generation rate.
More recent works have reported variability in data generation rates in a
variety of monitoring scenarios as well~\cite{chi,helios}. As a result, the
resource requirements of \client{} nodes would be \emph{different} and
\emph{independent} of each other.

To show the significance of such variability in \pingmesh{}, we measure data
rates of network probe messages generated by individual \client{}s, and show
the results in Figure~\ref{fig:data-gen-rate}. The data rates are normalized
to the highest one observed among \client{} nodes. Data generation rates
exhibit high variability, with 58\% of nodes generating 50\% or lower of the
highest data rate we observe.

\Paragraph{Quantitative analysis of resource usage across operators:} Popular declarative operators
used in monitoring queries include Filter(F), Grouping(G), Reduction(R),
Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. These
operators are computationally different and their costs are highly dynamic.
For example, Filter (stateless operator) drops uninteresting records by
applying the predicates on each record and typically operates at a low
computational cost. Grouping (stateful operator) organizes records by key
fields and hence requires key lookups and moving of records, making it an
expensive operator. Join (stateful operator) joins between an input stream
and a static table on \client{}\footnote{Due to limitations of \client{}-side
execution discussed in Section~\ref{sec:jarvis}, we do not consider other
complex join operators in \ours{}.}.

% The following summarizes key characteristics of popular operators:

% \begin{myitemize}
% % \item Project(P) operator extracts fields of interest from each record in the input stream
% % \item Map(M) takes an element from the input stream and outputs an element which is result of user-defined transformation.
% \item Filter(F) drops uninteresting records by applying filtering predicates on a set of record fields. It is a stateless operator, so typically operates at a low computational cost.

% \item Grouping(G) organizes records by key fields. In popular hash-based grouping, key lookups and moving of records needs to be done making it an expensive operator that dominates total query execution time~\cite{streamboxhbm}.
% \item Reduction(R) computes aggregate statistics incrementally, requiring only a few variables~\cite{trill}, e.g., sum and count to compute an average. If R aggregates on many records, it achieves enormous data reduction on the input stream.
% \item Join(J) operator combines record fields from one or more data sources within a time window, for those records satisfying a given join predicate. We focus on joins between input stream and a static table on \client{} nodes due to limitations of operators that can be executed on \client{} discussed in Section~\ref{sec:jarvis}.
% Other common operators include project and map operators which extract fields of interest from each input record and apply user-defined transformations on each record, respectively.

% % a join can occur between two streams or a stream and a static table. We focus on joins between input stream and a static table on \client{} nodes, due to limitations of executing operators on \client{} nodes discussed in Section~\ref{sec:jarvis}.
% \end{myitemize}

\begin{figure}[t]
\centering
%\subfigure[Filter operator]{\includegraphics[width=1.65in,height=1.3in]{fig/FilterProfileHighInpRate.pdf}}
\subfigure[G+R operator]{\includegraphics[width=1.65in,height=1.3in]{fig/GroupbyProfilePingmeshInpRate.pdf}}
\subfigure[Join operator]{\includegraphics[width=1.65in,height=1.3in]{fig/JoinOperatorProfileNew.pdf}}
%\vspace{-0.1in}
\caption{\label{fig:profile-op} Profiling of query operators.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

% This setup corresponds to running ten monitoring queries with equal sharing of the given single core budget and puts enough stress on the \server{} node.

%To observe how input data distribution causes operators' CPU utilization to
%vary, we profile F, G+R \footnote{Reduction commonly follows grouping to
%apply aggregation functions incrementally per group, so both are often
%combined.} and J operator using our trace on a \server{} node with 4 2.4~GHz
%cores. We configure data input rate to be 26.2~Mbps (10x scaled up) to ease
%our measurements (see \textbf{\pingmesh{}} in Section~\ref{sec:evaluation}
%for details). We then adjust different parameters that affect operator
%resource usage: (1) filtering predicate for F operator to obtain different
%filter-out rates (between 20-80\%), (2) output group counts for G+R operator
%reflecting a range from coarse-grained grouping (e.g., cluster level) to
%fine-grained grouping (e.g., server level) and (3) static table size for J
%operator which is joined with input stream reflecting query to look up ToR
%switch ID for each server IP address in \textbf{\pingmesh{}} dataset, to
%enable network latency analysis at the ToR level. We observed that for a
%range of filter-out rates, F operator requires 17-25\% CPU with low compute
%cost and variance. However, Figure~\ref{fig:profile-op} shows that when the
%number of groups and static table size changes for G+R and J operators
%respectively, CPU usage varies substantially between 50\%-350\%. Notice that
%in the presence of non-uniform data generation rates across \client{} nodes,
%we expect G+R and J operators to have more variable resource demands.

Next, we observe dynamic costs of operators by profiling F,
G+R\footnote{Reduction commonly follows grouping to apply aggregation
functions incrementally per group, so both are often combined.} and J
operator using our trace on a \server{} node with 4 2.4~GHz cores. We
configure data input rate to be 26.2~Mbps (10x scaled up) to ease our
measurements (see \textbf{\pingmesh{}} in Section~\ref{sec:evaluation} for
details). We then adjust several parameters that affect operator resource
usage: (i) filtering predicate for F operator to obtain different filter-out
rates (between 20-80\%), (ii) output group counts for G+R operator reflecting
a range of grouping granularity and (ii) the size of static table for J
operator which is joined with an input stream to add ToR switch IDes given server IP addresses to each record (for grouping by ToR IDes). We
observed that for a range of filter-out rates, F operator requires 17-25\%
CPU, i.e., low compute cost and variance. However, Figure~\ref{fig:profile-op}
shows that when the number of groups and the table size changes for G+R
and J operators respectively, CPU usage varies substantially between 50\%-350\%. 
%Notice that in the presence of non-uniform data generation rates
%across \client{} nodes, we expect G+R and J operators to have more variable
%resource demands.

%Thus, query operators have complex resource usage characteristics, depending
%on the input data distribution at each operator.

% \begin{figure}[t]
%   \centering
%     \includegraphics[width=2.4in]{fig/FilterGroupbyProfile.pdf}
%     \caption{Profiling resource usage of query in Figure~\ref{fig:pipeline_tor}}
%     \label{fig:query-profile-op-pipeline}
% \end{figure}

\Paragraph{Data reduction through a pipeline of operators:} Declarative
operators in a pipeline execute in sequence. Therefore, resource demand for
an operator in the pipeline is affected by the data incoming rate to the
operator out of executing all preceding operators. This further complicates
resource usage characteristics of pipeline execution while processing the
query on the input stream. For example, F operator leads to the first data
volume reduction from the input stream (see filtering predicate in
Listing~\ref{lst:motivating-query}). Since erroneous, insignificant records
are not dominant, the operator happens to drop only a small fraction of
records. A majority of records are then to be processed by G+R operator,
increasing compute cost for the query. However, if we were to toggle the
filtering predicates to perform a zoom-in analysis on a small subset of
erroneous data, there will be a high degree of data reduction in F operator,
so G+R operator considerably lowers its resource usage.

\Paragraph{Data distribution:} Large-scale server monitoring may see the data
with distribution shifting time-to-time. For example, when servers are being
over-loaded, latency profiles become more variable~\cite{rubik, pegasus}. If
a monitoring system runs a query to diagnose such network condition, it
should quickly adapt the query to process a larger amount of network probes
of high latency.





==> archive/related-extended-ver.tex <==
\balance
\section{Related Work}
\label{sec:RelatedWork}
%---------------BACKUP (DETAILED)-----------------------------
% Decentralized placement for streaming has been explored in~\cite{operator-tree-bokhari,decentral-tree-operator} but they consider limited query topologies such as single operators or trees. 
% ~\cite{decentral-scaling} have considered migrating operators based on CPU usage thresholds but their goal is to balance compute utilization in a cluster without considering query topologies or network traffic costs. 
% ~\cite{decentral-migration-cost} focuses on minimizing cost of migration across placement.~\cite{decentral-scaling} utilizes .

% ~\cite{} focus on minimizing network traffic across nodes without considering compute resource dynamics on each node. 
% But they apply to \server{}-side query optimizations for monitoring systems. 
% ~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral} consider placement techniques with the goal of reducing network usage and do not consider colocation of multiple queries on \client{} and resulting compute resource/query dynamics on \client{}

% DS2~\cite{ds2} makes operator scaling decisions by using an accurate performance model for the query using a centralized planner. Stela~\cite{stela} and Dhalion~\cite{dhalion} rely on observed processing rates to make operator scaling decisions. 
% Decentralized~\cite{self-adaptive-dsps-survey,multi-level-elasticity-dsps} and cost-model free strategies~\

% Similarly optimizations such as operator reordering~\cite{} can be applied during query compilation and operator resource allocation/scheduling~\cite{} can be used to make query allocation decisions on the~\client{}.

% based on thresholds and pre-defined rules respectively. 
% Decentralized scaling strategies have been proposed for large resource topologies within datacenters and geo-distributed settings~\cite{multi-level-elasticitity-wan,elasticity-heterogeneous}.
% ~\cite{model-free-scaling} utilizes a decentralized and cost model-free strategy to scale operators while

% Centralized~\cite{flink-scaling}
% Streaming systems such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming} are primarily targeted for \server{}-side workloads where resources are dedicated for analytics and typically consist of homogeneous compute nodes with different network topologies. 

% is a priority-based resource allocator for query processing.
% Above systems have typically been explored for  with a different network topology and/or do not consider processing data at the source, which requires adapting query execution to minimize network data transfer under limited and fast changing compute resources allocated to the query. 

% Performance models have been used in~\cite{ds2,stela}.

% \Paragraph{Streaming query planners} Streaming systems such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming} are primarily designed for \server{}-side workloads where resource nodes are dedicated to analytics. Several runtime optimizations have been explored including scaling in/out operators~\cite{heron,dhalion,storm,flink-scaling,ds2,stela}, operator reordering~\cite{eddies,teddies,reordering-interactive-queries,telegraphcq}, operator resource allocation and scheduling~\cite{cameo,adaptive-control-res-alloc}.  
% % is a priority-based resource allocator for query processing.
% Above systems have typically been explored for homogeneous compute nodes with a different network topology and/or do not consider processing data at the source, which requires adapting query execution to minimize network data transfer under limited and fast changing compute resources allocated to the query. 

% Performance models have been used in~\cite{ds2,stela}.

% Other centralized and decentralized query partitioning strategies have been have been explored for operator placement in stream processors, but they are: (1) either focused on batch processing and their techniques cannot be applied directly to continuous streaming queries~\cite{turbo,sparrow}, (2) consider limited operator topologies~\cite{decentral-tree-operator,operator-tree-bokhari}, (3) do not consider colocation of multiple queries on the same node and resulting compute resource/query dynamics on \client{}~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral}, or (4) consider different optimization goals~\cite{network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} such as scaling in/out of operator instances~\cite{self-adaptive-dsps-survey,multi-level-elasticitity-wan,multi-level-elasticity-dsps,elasticity-heterogeneous}, evaluates model-free~\cite{model-free-scaling} and model-based hybrid approaches for scaling~\cite{decentral-scaling}, CPU threshold based migration~\cite{decentral-scaling}, cost of migrating across placement decisions~\cite{decentral-migration-cost}.
%---------------BACKUP (DETAILED)-----------------------------

\Paragraph{Streaming query optimizations.} Runtime optimizations such as operator reordering~\cite{eddies,teddies,reordering-interactive-queries,telegraphcq} and resource allocation~\cite{cameo,adaptive-control-res-alloc} have been investigated for streaming systems which are complementary to our work. For operator placement, Turbo~\cite{turbo} and Sparrow~\cite{sparrow} have looked at decentralized scheduling for batch processing which do not directly apply to streaming data. 

% Several decentralized placement techniques for streaming ~\cite{network-aware-decentralized,decentral-placement-only-net,sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral} focus on reducing network usage between compute nodes and do not consider node compute constraints. 
% Similarly, cost model-based query planners have been explored for placement~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling}. These works do not consider partitioning under highly variable \client{} compute conditions. computes the cost of placement  explores centralized and decentralized algorithms which compute cost of operator placements in a topological order by considering subset of resource nodes for placement makes operator-level placement decisions with the goal to minimize network transfer costs between operators running on nodes in a distributed resource environment (e.g., analytics clusters in datacenters, sensor networks, WAN networks).
% ~\cite{rizou-multiop-placement} improves upon placement solutions of SBON by optimally solving a continuous version of the placement problem to map each operator to a virtual node in the cost metric space. It then uses a heuristic to map selected virtual nodes to the corresponding physical nodes which are discrete in the cost space.~\cite{subgraph-iso-zhu} uses subgraph isomorphism~\cite{subgraph-isomorphism} from graph theory to map application graphs to resource graphs and make placement decisions for query operators while considering network and compute constraints in the resource topology. ~\cite{utility-op-placement-decentral} provides a decentralized placement mechanism in which resource nodes are maintained in hierarchical manner, with nodes clustered based on their network delay, bandwidth, etc. Application nodes are recursively assigned to sub-graphs to make placement decisions. Placement is adapted efficiently by recomputing it only for the sub-graph in which resource conditions changed.
% ~\cite{decentral-migration-cost} considers the overhead of migrating operators when resource conditions change so a new placement decision needs to be computed and executed at runtime.
% ~\cite{operator-tree-bokhari} uses a dynamic programming based approach to efficiently determine an operator placement solution that minimizes the compute and communication costs between operators with restricted dependencies (i.e., query operators form a tree and not a generic graph). However, it is query cost model-based and uses coarse-grained operator partitioning.
% ~\cite{decentral-migration-cost}which satisfy a target performance objective (e.g., query latency, throughput).

% For comparing the greedy algorithm's convergence cost with \ours{}, there is unfortunately no separate treatment of the compute cost of operators. Basing on the network statistics profiled to obtain candidate placement solutions for reducing network communication cost, we could consider a corresponding compute cost constraint being checked using profiling information in a model-based constraint evaluation. This approach is represented by w/LP-init in Section~\ref{sec:convergence-cost-eval} in our evaluation to compare against \ours{}
\newcontent{\Paragraph{Stream operator placement.} Operator placement involves determining a mapping for each operator in the query graph, to the resource node on which it executes.~\cite{network-aware-decentralized} greedily traverses the query graph in post-order to make operator placement decisions and iteratively compute network transfer costs. To improve computed costs, centralized and decentralized placement algorithms are designed and made efficient using heuristics to reduce the number of resource nodes considered for placement.~\cite{decentral-placement-only-net} adopts a decentralized search strategy which executes an assignment of operators to resource nodes and uses the observed network costs to estimate the costs of other possible placement decisions in the search space. It is thus based on the profiled estimates of network transfer costs. SBON~\cite{sbon} minimizes  network usage  as  a  metric,  which  captures  the  network  bandwidth-delay product of the query. It considers a multi-query setting where operator outputs for co-located operators can be reused to save network transfer costs. Other works explore dynamic programming for placement~\cite{operator-tree-bokhari,utility-op-placement-decentral} and sub-graph isomorphism~\cite{subgraph-iso-zhu}. However, these works consider coarse-grained operator-level partitioning, which is compared against \ours{} in Section~\ref{sec:query-throughput-comparison}. Furthermore, they adopt query cost-model based approach which is compared to \ours{} in Section~\ref{sec:convergence-cost-eval}. Query cost model-agnostic approaches have also been explored for making placement decisions.~\cite{decentral-migration-cost}  collects runtime statistics as feedback to quantify query performance and iteratively improves a performance objective (e.g., query latency, bandwidth usage). ~\cite{decentral-tree-operator} greedily places nodes as close to the data source as possible to optimize query performance objectives. These techniques also perform coarse-grained operator-level partitioning and Section~\ref{sec:convergence-cost-eval} compares \ours{} with their cost-model agnostic approach.

\Paragraph{Parallel processing.} Previous works improved query performance by changing the parallelism degree of operators, so that the incoming data load can be split amongst multiple operator instances (i.e., data parallelism). These works are primarily focused on alleviating compute bottlenecks for the query operators. We now explain discuss these works.        
% For the query instance running on each \client{} in \ours{}, we can consider two instances (or replicas) of each query operator running on the \client{} and its parent \server{} node. And \ours{} determines how to split the input stream records between the two instances for each operator. 
% Previous works have handled dynamic input streams by changing number of operator instances deployed and thereby the compute resources allocated for each query operator at runtime. This enables data parallelism by splitting incoming records, to meet processing needs of streaming workloads. 
% Several works improve overall query performance by making operator-level scaling decisions.
Each query operator needs to be allocated resources to meet the compute needs of incoming data load. DS2~\cite{ds2} uses real-time performance traces to estimate the parallelism degree for all the query operators within a single scaling decision. Stela~\cite{per-op-stela} proposes a new metric that helps prioritize scaling of operators that have the greatest impact on overall query throughput. Other works in this domain~\cite{game-theory-scaling,decentral-scaling,nephele,model-predictive-control-scaling,per-op-icdcs-autoparallel,per-op-elastic-scale-ipdps,per-op-elastic-scale-tpds,per-op-elastic-iot-cloud,per-op-predictable-low-lat-iot,dhalion} also make operator-level scaling decisions to achieve query QoS objectives (e.g., throughput, resource utilization). Each operator instance is allocated a compute budget, and when incoming records cause congestion, operator scaling decisions are made. Applying these approaches to our setup requires considering the query operators replicated between the \client{} and its parent \server{} node. However, compute is not allocated at the operator level on the \client{} in our system. Instead compute allocation happens at the query level, which consists of multiple operators with different data reduction capabilities. Our optimization goal is thus different: incoming records need to be carefully apportioned across multiple co-located query operators within query level compute budget, by jointly tuning the compute load per-operator based on their data reduction capabilities. We still consider \coarsedp{} compared 

% Compute allocation is done at the operator level to eliminate processing bottlenecks. However, we need to solve a different problem in which we have a fixed compute budget on each \client{}. With \datapart{}, we are given the compute available to a query, and  (see operator priority in Section~\ref{sec:data-partitioning-problem}).
% These works do not investigate different strategies for splitting the input load across operator instances and their impact on overall query performance, which is required in \ours{} to minimize network transfer costs from each \client{}. 
Key-based load splitting strategies~\cite{key-splitting-pipeflow,key-splitting-graphcep,key-split-admission-control,key-split-debs-near-optimal,key-split-massive-scaleout,key-split-millwheel,key-split-s4,key-split-parallel-stateful-debs,key-split-vldb-holistic-view} dominate this space in which input key ranges are assigned to different stateful operator instances, such that each operator keeps the state of a distinct, non-overlapping key range. Integrating key-based load splitting into \ours{} can further reduce network transfer costs by minimizing number of output keys sent from the \client{}. We leave the investigation of key-based splitting in \ours{} for future work. Shuffle grouping~\cite{storm,heron,flink,aurora-cherniack,streamcloud,iot-dataflow-round-robin} is a load splitting technique in which data items are assigned to operator instances in a round robin manner. Partial key grouping~\cite{local-load-power-of-both-choices} combines the benefits of key-based and shuffle grouping to improve the load balancing of records for each key group. These works address a different problem of balancing the compute load across resource nodes. Doing so in our setup can cause network transfer costs to be incurred from \client{} even if it still has compute available to process the query and reduce data size. Other works improve query performance by assigning subsequences of records or windows, to operator instances based on the currently assigned compute load that is measured on the host node~\cite{local-load-sliding-window-harness,local-load-online-shuffle-grouping,local-load-elastic-ppq}. These approaches do not scale with large number of source nodes in our monitoring systems, because each \server{} node's compute is shared by multiple \client{}s (see Figure~\ref{fig:arch-monitoring-scale}). Compute load on \server{} node depends on jointly considering the splitting decisions on each \client{}, which is exponential in number of \client{}s.   
% Window or pane-based parallelization techniques split the input stream into subsequences of windows (with or without overlap across windows) and assign them to operator instances.
SkewTune~\cite{straggler-skewtune} and Google Dataflow~\cite{straggler-google-dataflow} employ work-stealing techniques for straggler mitigation while others~\cite{per-op-debs-window-cep,local-load-power-of-both-choices} use local estimates of compute load to detect a congested host node and re-route input records to a different operator instance in a greedy manner. However, in our setup we do not allocate resources at the operator level. On each \client{}, a fixed compute budget is allocated for a query consisting of multiple operators with different data reduction capabilities, and we need to coordinate the routing decisions across these operators to reduce network transfer costs within the available query-level compute budget. To facilitate comparison with \ours{}, we evaluate a variant of this mechanism adapted to our setup called \coarsedp{} in Section~\ref{sec:query-throughput-comparison}}. 
We discuss different backpressure mechanisms and their limitations for our target system: (1) \textit{Rate throttling at the source or dropping data~\cite{backpressure-spark-streaming,rxjava-backpressure}:} Our target system focuses on lossless monitoring and unlike systems like Kafka~\cite{apache-kafka}, we do not make assumptions about data persistence at the source so throttling it may result in data loss. (2) \textit{Operator queue resizing~\cite{flink-backpressure,rxjava-backpressure}:} Limited memory (e.g., 1 GB) on \client{}s restricts the benefits from dynamic sizing of operator queues, (3) \textit{Scaling compute resources~\cite{spark-dynamic-scaling-backpressure}:} They are similar to the operator scaling works discussed in this section.

% to avoid congestion by removing compute bottlenecks on the node hosting each operator instance.
% Such techniques manage the compute budget at the operator level, so they solve a different optimization from \datapart{} which manages compute allocated at the query level. Our queries have multiple operators with different data reduction capabilities, co-located on each \client{} with limited compute budget. \datapart{} reduces network traffic leaving the source node by jointly optimizing the compute load across these co-located operator instances, by tuning the compute load per-instance.\todo{discuss works on multiple ops?}}
% Our target system consists of heterogeneous compute nodes on each \client{}, requiring per-source query plan generation at large scale

\Paragraph{Near-data stream computations.} 
\textcolor{blue}{Previous works in the domain of in-situ analytics use programming paradigms like MapReduce to perform local query operations to process data on different nodes and then combine them using an aggregation operator to produce final output. iMR~\cite{imr}, lprof~\cite{lprof} and M3~\cite{m3-in-situ} apply MapReduce model to process server log streams on the source but they do not consider operator compute costs. Resource-aware techniques (DIRAQ~\cite{diraq}, FlexAnalytics~\cite{flexanalytics}, Logzip~\cite{logzip}) consider compute costs but focus only on indexing and data compression at the source. Redoop~\cite{redoop} performs coarse-grained query-level partitioning, while LambdaFlow~\cite{lambdaflow} and Scoop~\cite{scoop} push query operators to dedicated in-situ analytics servers statically, without considering dynamic resource conditions on source nodes. However, these works consider coarse-grained operator partitioning and do not investigate the effectiveness of fine-grained partitioning under highly constrained compute resources on \client{} nodes. Furthermore, they do not consider the challenges with performing fast adaptation of the partitioning plans to handle dynamic resource conditions, which scales to handle large number of \client{}s in server monitoring pipelines.}

State-of-the-art approaches in network telemetry domain which perform near-data computation are targeted towards analyzing network packets and are mostly based on operator-level partitioning. EverFlow~\cite{everflow} and dShark~\cite{dshark} apply light-weight operations on commodity network switches and computing nodes near data source, respectively. Gigascope~\cite{gigascope} classifies operators based on domain-specific knowledge and pushes low-cost operators close to data source. Sonata~\cite{sonata} utilizes an ILP solver to  optimize operator-level partitioning, but at the cost of latency as high as 20 minutes. These approaches neglect \datapart{} and/or are based on expensive centralized query refinement.

\textcolor{blue}{In-network stream processors~\cite{opt-replicate-place-sigmetrics,opt-placement-fog} find optimal operator replication and placement given heterogeneous resources. They solve an expensive optimization problem which is NP-hard. When applied to our monitoring system, each operator (on each data source) can be placed on \client{} or remote \server{} node. That means we need to evaluate at least $2^{M*N_{d}}$ solutions, where $N_{d}$ is the number of \client{}s and $M$ is the number of operators per query instance on each \client{}.  Note that when considering operator replication, this number would be even higher. Our problem requires a new partitioning plan within a few seconds, so the exponential cost in \client{}s would not scale for our setup with up to 250 \client{}s per \server{} node. \\
~\cite{wan-cep-network-opt} addresses the operator placement problem in geographically distributed sites. All the streaming data is collected at a single site for final aggregation and output. The work explores several algorithms and their effectiveness in finding assignment of operators to sites closer to the \client{} to minimize network transmission costs. However, except for the greedy heuristics, all their algorithms have exponential time complexity in maximum number of incoming edges to an operator in the query graph. In our setup, the operator with maximum number of incoming edges refers to the final merge operator in the query operator graph, which receives data from the queries running on each \client{}. Thus, even if we consider 2 sites (i.e., \client{} and \server{} node) for placement of each query operator, then we can have $2^{N_{d}}$ possible solutions to consider where $N_{d}$ is the number of \client{}s. Thus, they would not scale for the large number of \client{}s in \ours{}. The greedy algorithm and its variant on the other hand, consider coarse-grained operator-level partitioning (represented by Best-OP and compared in evaluation Section~\ref{sec:evaluation}). Furthermore, based on the profiled statistics (e.g., site-to-site network latency) the cost of each candidate placement solution is estimated. Such an approach based on the query cost model is compared with \ours{} in Section~\ref{sec:convergence-cost-eval}.~\cite{heuristics-op-placement-dsps} also investigates operator-level partitioning by using model-based and model-free heuristics. They are represented by Best-OP in our experiments (Section~\ref{sec:evaluation}) for throughput comparison and by model-based and model-agnostic approaches in Section~\ref{sec:convergence-cost-eval} for convergence cost evaluation.}
% Other collection systems such as~\cite{ganglia,azure} apply aggregation functions such as averaging or sampling over a coarse-grained time scale (e.g. 1 min) to mitigate network transfer costs. However, this leads to loss of information (e,g, missing low-density outliers during sampling), so is complementary to the lossless approach of \ours{}.
% planners which can be expensive. 

% Systems like~\cite{prometheus} use a pull based model to process metrics and rely on server side processing to analyze the metrics. 
% Some collection systems apply aggregation functions such as averaging~\cite{ganglia} or sampling~\cite{azure} on the data over a coarser-grained time scale (e.g., a min) to mitigate network effect. Typically, this is a pre-processing step before stream data is pushed into monitoring queries. The use of an aggregation in this way leads to loss of information (e,g, missing low-density outliers during sampling), so is complementary to the lossless approaches like \ours{}.

%There is also prior work on lossless data compression on stream
%data~\cite{tersecades}. This is primarily to accelerate in-memory stream
%processing and can be combined with \ours{}.

%\subsection{Reducing Network Traffic}
%
%\Paragraph{Lossy data reduction.} Some collection systems apply aggregation
%functions such as averaging~\cite{ganglia} or sampling~\cite{azure} on the
%data over a coarser-grained time scale (e.g., a min) to mitigate network
%effect. Typically, this is a pre-processing step that happens before stream
%data is pushed into monitoring queries. The use of an aggregation in this way
%leads to loss of information and so is not always desirable: e.g., sampling
%with a low sampling rate highly likely misses low-density outlier values
%representing abnormal behavior of the monitored system. Therefore, we limit
%our focus on approaches for lossless data reduction.
%
%\Paragraph{Lossless data reduction.} The state-of-the-art lossless approaches
%attempt to harness scarce resources in the devices located closer to the data
%source for the purpose of alleviating the pressure on network and stream
%processor resources. Their key mechanism is to partition a given monitoring
%query and offload a set of query operators to the source-side devices so that
%the stream processor does partial computations~\cite{everflow, sonata,
%dshark}. We call this approach \emph{query partitioning}. The query
%partitioning is effective in reducing not only the load on the stream
%processor but also the amount of data sent over the network.
%
%A naive way of query partitioning is to execute only filter operations on the
%target devices to prune the data. For instance, EverFlow~\cite{everflow} and
%dShark~\cite{everflow} apply filter operations on commodity network switches
%and nodes near data source, respectively. A more sophisticated way is to
%capitalize on a query placement optimizer that dynamically decides which
%operators to run on the target devices. For instance, SONATA~\cite{sonata}
%came up with an Integer Linear Program (ILP) solver that iteratively
%optimizes query partitioning so that network switches under resource
%constraints run a part of the query to minimize the amount of data sent out.
%While prior work mostly targets on analyzing network packets, the proposed
%concepts can be applied to our monitoring scenarios, where we ought to
%utilize datacenter server resources to perform partial computations.
%
%Also, there is prior work on lossless data compression on stream
%data~\cite{tersecades}. This is primarily to accelerate in-memory stream
%processing and thus is orthogonal to query partitioning.

%\Paragraph{Key partitioning on stream data:} Gigascope~\cite{gigascope}
%exploits subaggregate, which has similarities to our data partitioning
%on hot keys. For reduction on grouped data, both approaches apply aggregation
%functions to only partial groups under resource constraints
%and let machines with high capacities to complete the remaining reduction.
%However, %the two approaches are fundamentally different in that
%while Gigascope populates a fixed-size hash table with keys appearing first,
%we populate a table whose size is tunable based on a profiling of data,
%which can precisely identify keys with high density.

%There are also studies on enabling partial key grouping in typical
%distributed stream processing. Their optimizations are either for load
%balancing among many workers~\cite{pkg1, pkg2} or for low aggregation cost of
%partial key grouping results~\cite{keyskew}, and so do not share the same
%objective with ours.

\Paragraph{Stream computations on the edge.} EdgeWise~\cite{edgewise} is a streaming engine that incorporates a scheduler for congestion control to improve throughput and latency by prioritizing operators whose queues experience backpressure. \textcolor{blue}{Other works~\cite{droplet,costless} address the operator placement problem between edge and cloud resources for video analytics applications. However, they consider coarse-grained operator placement which do not leverage the benefits of fine-grained data-level partitioning on \client{} nodes with limited compute. They also do not consider the dynamic resource conditions and scale of \client{} nodes needed to be considered for placement in server monitoring pipelines.}  %Edgent~\cite{edgent} is an open-source engine and designed for data pre-processing. Both engines do not meet design requirements of \ours{}.

%efficient multi-threading on compute resource allocates threads to relieve
%congestion at the queueing experiencing maximum backpressure. So it decouples
%threads from operators. Does not do query/data partitioning.

\Paragraph{Wide-area streaming analytics.} 
% this paragraph does not add anything to wide-area analytics. just drop.
%Most of existing streaming engines have been developed for single machine~\cite{streambox, streamboxhbm, trill} or for distributed servers~\cite{sparkstreaming, timestream, heron, quill, streamscope, naiad, storm}, with their focus mainly on improving parallelism, responsiveness, scalability, programmability, and fault tolerance. Recently,
Novel streaming systems have been designed to operate efficiently on low-bandwidth networks, such as wide-area network (WAN). Sol~\cite{sol} introduces an early-binding
of analytics tasks to workers and dedicated communication tasks to improve
resource utilization over WAN. 
%Sol~\cite{sol} introduces an early-binding of tasks over high-latency
%networks (which addresses high-latency coordinations of task executions
%across workers) and dedicated communication tasks (which decouples
%communication from computation for a task and improves resource utilization).
AWStream~\cite{awstream} trades off accuracy for WAN bandwidth by controlling the sampling of data. MQO~\cite{mqo} provides a technique to share input/output data and operators across stream queries, saving WAN bandwidth. %While \ours{} aims at different design goals, future datacenter monitoring systems may need to consider the wisdom shared by these prior works.

% Sensor networks have explored query partitioning problems~\cite{sparksql,tag,tinydb,in-network-stream,semijoin-db,trackjoin}. However, these systems face different optimization problems because they typically involve lower traffic rates and involve special-purpose queries.

% Decentralized placement techniques such as~\cite{sbon} do not account for operator or compute resource dynamics. 

% WASP~\cite{wasp} relies on a central query planner and looks at optimizations such as scaling out operators. SpanEdge~\cite{spanedge} relies on programmers to inform of operations that need to be closer to the data source.



%The growing interest in stream data analytics has led to extensive research
%into building streaming engines for single machine~\cite{streambox,
%streamboxhbm, trill} and for distributed servers~\cite{sparkstreaming,
%timestream, heron, quill, streamscope, naiad, storm}, with their focus mainly
%on improving parallelism, responsiveness, scalability, programmability, and
%fault tolerance. As they are designed to run on high-capacity servers with
%high-bandwidth connectivity, they are best used in building stream processor
%in our monitoring system. In the related work, we focus our discussion mainly
%on query distribution methods across resource-constrained data source nodes.


==> archive/related-v1.tex <==
\balance
\section{Related Work}
\label{sec:RelatedWork}
%---------------BACKUP (DETAILED)-----------------------------
% Decentralized placement for streaming has been explored in~\cite{operator-tree-bokhari,decentral-tree-operator} but they consider limited query topologies such as single operators or trees. 
% ~\cite{decentral-scaling} have considered migrating operators based on CPU usage thresholds but their goal is to balance compute utilization in a cluster without considering query topologies or network traffic costs. 
% ~\cite{decentral-migration-cost} focuses on minimizing cost of migration across placement.~\cite{decentral-scaling} utilizes .

% ~\cite{} focus on minimizing network traffic across nodes without considering compute resource dynamics on each node. 
% But they apply to \server{}-side query optimizations for monitoring systems. 
% ~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral} consider placement techniques with the goal of reducing network usage and do not consider colocation of multiple queries on \client{} and resulting compute resource/query dynamics on \client{}

% DS2~\cite{ds2} makes operator scaling decisions by using an accurate performance model for the query using a centralized planner. Stela~\cite{stela} and Dhalion~\cite{dhalion} rely on observed processing rates to make operator scaling decisions. 
% Decentralized~\cite{self-adaptive-dsps-survey,multi-level-elasticity-dsps} and cost-model free strategies~\

% Similarly optimizations such as operator reordering~\cite{} can be applied during query compilation and operator resource allocation/scheduling~\cite{} can be used to make query allocation decisions on the~\client{}.

% based on thresholds and pre-defined rules respectively. 
% Decentralized scaling strategies have been proposed for large resource topologies within datacenters and geo-distributed settings~\cite{multi-level-elasticitity-wan,elasticity-heterogeneous}.
% ~\cite{model-free-scaling} utilizes a decentralized and cost model-free strategy to scale operators while

% Centralized~\cite{flink-scaling}
% Streaming systems such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming} are primarily targeted for \server{}-side workloads where resources are dedicated for analytics and typically consist of homogeneous compute nodes with different network topologies. 

% is a priority-based resource allocator for query processing.
% Above systems have typically been explored for  with a different network topology and/or do not consider processing data at the source, which requires adapting query execution to minimize network data transfer under limited and fast changing compute resources allocated to the query. 

% Performance models have been used in~\cite{ds2,stela}.

% \Paragraph{Streaming query planners} Streaming systems such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming} are primarily designed for \server{}-side workloads where resource nodes are dedicated to analytics. Several runtime optimizations have been explored including scaling in/out operators~\cite{heron,dhalion,storm,flink-scaling,ds2,stela}, operator reordering~\cite{eddies,teddies,reordering-interactive-queries,telegraphcq}, operator resource allocation and scheduling~\cite{cameo,adaptive-control-res-alloc}.  
% % is a priority-based resource allocator for query processing.
% Above systems have typically been explored for homogeneous compute nodes with a different network topology and/or do not consider processing data at the source, which requires adapting query execution to minimize network data transfer under limited and fast changing compute resources allocated to the query. 

% Performance models have been used in~\cite{ds2,stela}.

% Other centralized and decentralized query partitioning strategies have been have been explored for operator placement in stream processors, but they are: (1) either focused on batch processing and their techniques cannot be applied directly to continuous streaming queries~\cite{turbo,sparrow}, (2) consider limited operator topologies~\cite{decentral-tree-operator,operator-tree-bokhari}, (3) do not consider colocation of multiple queries on the same node and resulting compute resource/query dynamics on \client{}~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral}, or (4) consider different optimization goals~\cite{network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} such as scaling in/out of operator instances~\cite{self-adaptive-dsps-survey,multi-level-elasticitity-wan,multi-level-elasticity-dsps,elasticity-heterogeneous}, evaluates model-free~\cite{model-free-scaling} and model-based hybrid approaches for scaling~\cite{decentral-scaling}, CPU threshold based migration~\cite{decentral-scaling}, cost of migrating across placement decisions~\cite{decentral-migration-cost}.
%---------------BACKUP (DETAILED)-----------------------------

\Paragraph{Streaming query optimizations.} Runtime optimizations such as operator reordering~\cite{eddies,teddies,reordering-interactive-queries,telegraphcq} and resource allocation~\cite{cameo,adaptive-control-res-alloc} have been investigated for streaming systems which are complementary to our work. For operator placement, Turbo~\cite{turbo} and Sparrow~\cite{sparrow} have looked at decentralized scheduling for batch processing which do not directly apply to streaming data. 

% Several decentralized placement techniques for streaming ~\cite{network-aware-decentralized,decentral-placement-only-net,sbon,rizou-multiop-placement,subgraph-iso-zhu,utility-op-placement-decentral} focus on reducing network usage between compute nodes and do not consider node compute constraints. 
% Similarly, cost model-based query planners have been explored for placement~\cite{sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling}. These works do not consider partitioning under highly variable \client{} compute conditions. computes the cost of placement  explores centralized and decentralized algorithms which compute cost of operator placements in a topological order by considering subset of resource nodes for placement makes operator-level placement decisions with the goal to minimize network transfer costs between operators running on nodes in a distributed resource environment (e.g., analytics clusters in datacenters, sensor networks, WAN networks).
% ~\cite{rizou-multiop-placement} improves upon placement solutions of SBON by optimally solving a continuous version of the placement problem to map each operator to a virtual node in the cost metric space. It then uses a heuristic to map selected virtual nodes to the corresponding physical nodes which are discrete in the cost space.~\cite{subgraph-iso-zhu} uses subgraph isomorphism~\cite{subgraph-isomorphism} from graph theory to map application graphs to resource graphs and make placement decisions for query operators while considering network and compute constraints in the resource topology. ~\cite{utility-op-placement-decentral} provides a decentralized placement mechanism in which resource nodes are maintained in hierarchical manner, with nodes clustered based on their network delay, bandwidth, etc. Application nodes are recursively assigned to sub-graphs to make placement decisions. Placement is adapted efficiently by recomputing it only for the sub-graph in which resource conditions changed.
% ~\cite{decentral-migration-cost} considers the overhead of migrating operators when resource conditions change so a new placement decision needs to be computed and executed at runtime.
% ~\cite{operator-tree-bokhari} uses a dynamic programming based approach to efficiently determine an operator placement solution that minimizes the compute and communication costs between operators with restricted dependencies (i.e., query operators form a tree and not a generic graph). However, it is query cost model-based and uses coarse-grained operator partitioning.
% ~\cite{decentral-migration-cost}which satisfy a target performance objective (e.g., query latency, throughput).

% For comparing the greedy algorithm's convergence cost with \ours{}, there is unfortunately no separate treatment of the compute cost of operators. Basing on the network statistics profiled to obtain candidate placement solutions for reducing network communication cost, we could consider a corresponding compute cost constraint being checked using profiling information in a model-based constraint evaluation. This approach is represented by w/LP-init in Section~\ref{sec:convergence-cost-eval} in our evaluation to compare against \ours{}
\newcontent{\Paragraph{Stream operator placement.} Operator placement involves determining a mapping for each operator in the query graph, to the resource node on which it executes.~\cite{opt-replicate-place-sigmetrics,opt-placement-fog}~\todo{reviewer provided paper} finds the optimal operator placement given heterogeneous resources. They solve an expensive optimization problem which is NP-hard. When applied to our monitoring system, the operators per \client{} can be placed on \client{} or remote \server{} node. We need to evaluate at least $2^{M*N_{d}}$ solutions, where $N_{d}$ is the number of \client{}s and $M$ is the number of operators per query instance on each \client{}. Our target system with up to 250 \client{}s per \server{} node requires fast adaptation (Section~\ref{sec:motivation}), so the exponential placement cost would not scale with increasing \client{}s. \\
% Note that when considering operator replication, this number would be even higher.
% All the streaming data is collected at a single site for final aggregation and output. The work 
~\cite{wan-cep-network-opt}~\todo{reviewer provided paper} addresses operator placement in geographically distributed sites. They explore several heuristics to assign operators near the \client{} to minimize network transmission costs. However, except for the greedy heuristics, their algorithms have exponential time complexity in maximum number of incoming edges to an operator in the query graph. This is due to network transfer cost of each operator depending on the joint placement of all the operators with incoming edges to it. Applying their approach to our setup, query instances run on each \client{} node and their results are merged on \server{} side, whose network and compute resources are shared by all \client{}s.  
% the operator with maximum number of incoming edges refers to the final merge operator in the query operator graph, which receives data from the queries running on each \client{}.
Thus, if we consider 2 sites (i.e., \client{} and \server{} node) for placement of each query instance's operators, we have $O(2^{N_{d}})$ possible solutions to consider where $N_{d}$ is the number of \client{}s. Thus, they would not scale for the large number of \client{}s in \ours{}. Furthermore, all of their algorithms (including the greedy algorithm and its variants) consider coarse-grained operator-level partitioning. A query cost-model based approach is investigated in the paper in which site-to-site network latency and other profiled statistics are used to estimate cost of each possible placement solution.~\cite{heuristics-op-placement-dsps}~\todo{reviewer provided paper} also investigates coarse-grained operator-level partitioning by using model-based and model-free heuristics which are made efficient by reducing the number of resource nodes to consider for placement. Several other works in this space also consider coarse-grained operator-level placement (~\cite{network-aware-decentralized,decentral-tree-operator,decentral-placement-only-net,operator-tree-bokhari,utility-op-placement-decentral,sbon}). While some consider centralized placement algorithms~\cite{network-aware-decentralized}, others use decentralized approaches~\cite{decentral-placement-only-net} for making query cost model-based placement decisions.~\cite{decentral-tree-operator} uses rule-based heuristics (not based on any query cost model) to determine whether to execute an operator locally or send it to a node closer to \client{}. In summary, all of the above works consider coarse-grained operator-level placement which is compared against \ours{} (i.e., \bestopconfig{} in Section~\ref{sec:evaluation}). Model-based and model-agnostics approaches for convergence are evaluated in Section~\ref{sec:convergence-cost-eval}.

% ~\cite{network-aware-decentralized} and~\cite{decentral-tree-operator} focus on queries with operators in a tree structure.~\cite{network-aware-decentralized} traverses the query tree in post-order and considers placement of operators on different nodes to compute the resulting network transfer costs using a model-based approach. To make the search more efficient, centralized and decentralized placement algorithms are designed to investigate heuristics which reduce number of resource nodes to consider. In~\cite{decentral-tree-operator}, each resource node performs post-order traversal of operator tree and uses rule-based heuristics (not based on a query cost model) to determine whether to execute an operator locally or send it to a node closer to \client{}.~\cite{decentral-placement-only-net} executes an assignment of operators to resource nodes and reuses the observed network costs to estimate the cost of other possible placement decisions in the search space. It is a decentralized algorithm and based on profiled estimates of network transfer costs.
% ~\cite{decentral-migration-cost} collects runtime statistics as feedback to quantify query performance for each placement decision and iteratively improves query performance (e.g., latency, bandwidth usage) using a query cost-model agnostic approach.
% Other works explore dynamic programming for placement~\cite{operator-tree-bokhari,utility-op-placement-decentral} and optimizations in multi-query settings~\cite{sbon}. 
% However, all these works consider coarse-grained operator-level partitioning, which is compared against \ours{} in Section~\ref{sec:query-throughput-comparison}. Furthermore, query cost-model based and model-agnostic approaches are compared in Section~\ref{sec:convergence-cost-eval}.

%  the It greedily places nodes as close to the data source as possible to optimize query performance objectives.
% sub-graph isomorphism~\cite{subgraph-iso-zhu} 
% SBON~\cite{sbon} minimizes  network usage  as  a  metric,  which  captures  the  network  bandwidth-delay product of the query. It considers a multi-query setting where operator outputs for co-located operators can be reused to save network transfer costs.

\Paragraph{Parallel processing.}~\todo{reviewer suggested looking into more papers in this topic of operator replication, which includes scaling operators and load balancing across operator instances} Query performance can be improved by changing the parallelism degree of operators, so that incoming data load can be split amongst multiple operator instances (i.e., data parallelism). These works are primarily focused on alleviating query compute bottlenecks.  
% For the query instance running on each \client{} in \ours{}, we can consider two instances (or replicas) of each query operator running on the \client{} and its parent \server{} node. And \ours{} determines how to split the input stream records between the two instances for each operator. 
% Previous works have handled dynamic input streams by changing number of operator instances deployed and thereby the compute resources allocated for each query operator at runtime. This enables data parallelism by splitting incoming records, to meet processing needs of streaming workloads. 
% Several works improve overall query performance by making operator-level scaling decisions.
DS2~\cite{ds2} uses real-time performance traces to estimate the parallelism degree for all the query operators within a single scaling decision under ideal conditions. Stela~\cite{per-op-stela} proposes a new metric that helps prioritize scaling of operators that have the greatest impact on overall query throughput.

Other works in this domain~\cite{game-theory-scaling,decentral-scaling,nephele,model-predictive-control-scaling,per-op-icdcs-autoparallel,per-op-elastic-scale-ipdps,per-op-elastic-scale-tpds,per-op-elastic-iot-cloud,per-op-predictable-low-lat-iot,dhalion} also make operator-level scaling decisions to achieve query QoS objectives (e.g., throughput, resource utilization). Each operator instance is allocated a compute budget, and when incoming records cause congestion, operator scaling decisions are made. Applying these approaches to our setup requires considering the query operators replicated between the \client{} and its parent \server{} node. However, compute is not allocated at the operator level on the \client{} in our system. Instead compute allocation happens at the query level, which consists of multiple operators with different data reduction capabilities. Our optimization goal is thus different: incoming records need to be carefully apportioned across multiple co-located query operators within query level compute budget, by jointly tuning the compute load per-operator based on their data reduction capabilities. We still consider \coarsedp{} compared 

% Compute allocation is done at the operator level to eliminate processing bottlenecks. However, we need to solve a different problem in which we have a fixed compute budget on each \client{}. With \datapart{}, we are given the compute available to a query, and  (see operator priority in Section~\ref{sec:data-partitioning-problem}).
% These works do not investigate different strategies for splitting the input load across operator instances and their impact on overall query performance, which is required in \ours{} to minimize network transfer costs from each \client{}. 
Key-based load splitting strategies~\cite{key-splitting-pipeflow,key-splitting-graphcep,key-split-admission-control,key-split-debs-near-optimal,key-split-massive-scaleout,key-split-millwheel,key-split-s4,key-split-parallel-stateful-debs,key-split-vldb-holistic-view} dominate this space in which input key ranges are assigned to different stateful operator instances, such that each operator keeps the state of a distinct, non-overlapping key range. Integrating key-based load splitting into \ours{} can further reduce network transfer costs by minimizing number of output keys sent from the \client{}. We leave the investigation of key-based splitting in \ours{} for future work. Shuffle grouping~\cite{storm,heron,flink,aurora-cherniack,streamcloud,iot-dataflow-round-robin} is a load splitting technique in which data items are assigned to operator instances in a round robin manner. Partial key grouping~\cite{local-load-power-of-both-choices} combines the benefits of key-based and shuffle grouping to improve the load balancing of records for each key group. These works address a different problem of balancing the compute load across resource nodes. Doing so in our setup can cause network transfer costs to be incurred from \client{} even if it still has compute available to process the query and reduce data size. Other works improve query performance by assigning subsequences of records or windows, to operator instances based on the currently assigned compute load that is measured on the host node~\cite{local-load-sliding-window-harness,local-load-online-shuffle-grouping,local-load-elastic-ppq}. These approaches do not scale with large number of source nodes in our monitoring systems, because each \server{} node's compute is shared by multiple \client{}s (see Figure~\ref{fig:arch-monitoring-scale}). Compute load on \server{} node depends on jointly considering the splitting decisions on each \client{}, which is exponential in number of \client{}s.   
% Window or pane-based parallelization techniques split the input stream into subsequences of windows (with or without overlap across windows) and assign them to operator instances.
SkewTune~\cite{straggler-skewtune} and Google Dataflow~\cite{straggler-google-dataflow} employ work-stealing techniques for straggler mitigation while others~\cite{per-op-debs-window-cep,local-load-power-of-both-choices} use local estimates of compute load to detect a congested host node and re-route input records to a different operator instance in a greedy manner. However, in our setup we do not allocate resources at the operator level. On each \client{}, a fixed compute budget is allocated for a query consisting of multiple operators with different data reduction capabilities, and we need to coordinate the routing decisions across these operators to reduce network transfer costs within the available query-level compute budget. To facilitate comparison with \ours{}, we evaluate a variant of this mechanism adapted to our setup called \coarsedp{} in Section~\ref{sec:query-throughput-comparison}}. 
We discuss different backpressure mechanisms and their limitations for our target system: (1) \textit{Rate throttling at the source or dropping data~\cite{backpressure-spark-streaming,rxjava-backpressure}:} Our target system focuses on lossless monitoring and unlike systems like Kafka~\cite{apache-kafka}, we do not make assumptions about data persistence at the source so throttling it may result in data loss. (2) \textit{Operator queue resizing~\cite{flink-backpressure,rxjava-backpressure}:} Limited memory (e.g., 1 GB) on \client{}s restricts the benefits from dynamic sizing of operator queues, (3) \textit{Scaling compute resources~\cite{spark-dynamic-scaling-backpressure}:} They are similar to the operator scaling works discussed in this section.

% to avoid congestion by removing compute bottlenecks on the node hosting each operator instance.
% Such techniques manage the compute budget at the operator level, so they solve a different optimization from \datapart{} which manages compute allocated at the query level. Our queries have multiple operators with different data reduction capabilities, co-located on each \client{} with limited compute budget. \datapart{} reduces network traffic leaving the source node by jointly optimizing the compute load across these co-located operator instances, by tuning the compute load per-instance.\todo{discuss works on multiple ops?}}
% Our target system consists of heterogeneous compute nodes on each \client{}, requiring per-source query plan generation at large scale

\Paragraph{Near-data stream computations.} ~\todo{papers in this paragraph are on topic asked by reviewer}
\newcontent{Previous works in the domain of in-situ analytics use programming paradigms like MapReduce to perform local query operations to process data on different nodes and then combine them using an aggregation operator to produce final output. iMR~\cite{imr}, lprof~\cite{lprof} and M3~\cite{m3-in-situ} apply MapReduce model to process server log streams on the source but they do not consider operator compute costs. Resource-aware techniques (DIRAQ~\cite{diraq}, FlexAnalytics~\cite{flexanalytics}, Logzip~\cite{logzip}) consider compute costs but focus only on indexing and data compression at the source. Redoop~\cite{redoop} performs coarse-grained query-level partitioning, while LambdaFlow~\cite{lambdaflow} and Scoop~\cite{scoop} push query operators to dedicated in-situ analytics servers statically, without considering dynamic resource conditions on source nodes. However, these works consider coarse-grained operator partitioning and do not investigate the effectiveness of fine-grained partitioning under highly constrained compute resources on \client{} nodes. Furthermore, they do not consider the challenges with performing fast adaptation of the partitioning plans to handle dynamic resource conditions, which scales to handle large number of \client{}s in server monitoring pipelines.}

State-of-the-art approaches in network telemetry domain which perform near-data computation are targeted towards analyzing network packets and are mostly based on operator-level partitioning. EverFlow~\cite{everflow} and dShark~\cite{dshark} apply light-weight operations on commodity network switches and computing nodes near data source, respectively. Gigascope~\cite{gigascope} classifies operators based on domain-specific knowledge and pushes low-cost operators close to data source. Sonata~\cite{sonata} utilizes an ILP solver to  optimize operator-level partitioning, but at the cost of latency as high as 20 minutes. These approaches neglect \datapart{} and/or are based on expensive centralized query refinement.

% Other collection systems such as~\cite{ganglia,azure} apply aggregation functions such as averaging or sampling over a coarse-grained time scale (e.g. 1 min) to mitigate network transfer costs. However, this leads to loss of information (e,g, missing low-density outliers during sampling), so is complementary to the lossless approach of \ours{}.
% planners which can be expensive. 

% Systems like~\cite{prometheus} use a pull based model to process metrics and rely on server side processing to analyze the metrics. 
% Some collection systems apply aggregation functions such as averaging~\cite{ganglia} or sampling~\cite{azure} on the data over a coarser-grained time scale (e.g., a min) to mitigate network effect. Typically, this is a pre-processing step before stream data is pushed into monitoring queries. The use of an aggregation in this way leads to loss of information (e,g, missing low-density outliers during sampling), so is complementary to the lossless approaches like \ours{}.

%There is also prior work on lossless data compression on stream
%data~\cite{tersecades}. This is primarily to accelerate in-memory stream
%processing and can be combined with \ours{}.

%\subsection{Reducing Network Traffic}
%
%\Paragraph{Lossy data reduction.} Some collection systems apply aggregation
%functions such as averaging~\cite{ganglia} or sampling~\cite{azure} on the
%data over a coarser-grained time scale (e.g., a min) to mitigate network
%effect. Typically, this is a pre-processing step that happens before stream
%data is pushed into monitoring queries. The use of an aggregation in this way
%leads to loss of information and so is not always desirable: e.g., sampling
%with a low sampling rate highly likely misses low-density outlier values
%representing abnormal behavior of the monitored system. Therefore, we limit
%our focus on approaches for lossless data reduction.
%
%\Paragraph{Lossless data reduction.} The state-of-the-art lossless approaches
%attempt to harness scarce resources in the devices located closer to the data
%source for the purpose of alleviating the pressure on network and stream
%processor resources. Their key mechanism is to partition a given monitoring
%query and offload a set of query operators to the source-side devices so that
%the stream processor does partial computations~\cite{everflow, sonata,
%dshark}. We call this approach \emph{query partitioning}. The query
%partitioning is effective in reducing not only the load on the stream
%processor but also the amount of data sent over the network.
%
%A naive way of query partitioning is to execute only filter operations on the
%target devices to prune the data. For instance, EverFlow~\cite{everflow} and
%dShark~\cite{everflow} apply filter operations on commodity network switches
%and nodes near data source, respectively. A more sophisticated way is to
%capitalize on a query placement optimizer that dynamically decides which
%operators to run on the target devices. For instance, SONATA~\cite{sonata}
%came up with an Integer Linear Program (ILP) solver that iteratively
%optimizes query partitioning so that network switches under resource
%constraints run a part of the query to minimize the amount of data sent out.
%While prior work mostly targets on analyzing network packets, the proposed
%concepts can be applied to our monitoring scenarios, where we ought to
%utilize datacenter server resources to perform partial computations.
%
%Also, there is prior work on lossless data compression on stream
%data~\cite{tersecades}. This is primarily to accelerate in-memory stream
%processing and thus is orthogonal to query partitioning.

%\Paragraph{Key partitioning on stream data:} Gigascope~\cite{gigascope}
%exploits subaggregate, which has similarities to our data partitioning
%on hot keys. For reduction on grouped data, both approaches apply aggregation
%functions to only partial groups under resource constraints
%and let machines with high capacities to complete the remaining reduction.
%However, %the two approaches are fundamentally different in that
%while Gigascope populates a fixed-size hash table with keys appearing first,
%we populate a table whose size is tunable based on a profiling of data,
%which can precisely identify keys with high density.

%There are also studies on enabling partial key grouping in typical
%distributed stream processing. Their optimizations are either for load
%balancing among many workers~\cite{pkg1, pkg2} or for low aggregation cost of
%partial key grouping results~\cite{keyskew}, and so do not share the same
%objective with ours.

\Paragraph{Stream computations on the edge.} EdgeWise~\cite{edgewise} is a streaming engine that incorporates a scheduler for congestion control to improve throughput and latency by prioritizing operators whose queues experience backpressure. \textcolor{blue}{Other works~\cite{droplet,costless} address the operator placement problem between edge and cloud resources for video analytics applications. However, they consider coarse-grained operator placement which do not leverage the benefits of fine-grained data-level partitioning on \client{} nodes with limited compute. They also do not consider the dynamic resource conditions and scale of \client{} nodes needed to be considered for placement in server monitoring pipelines.}  %Edgent~\cite{edgent} is an open-source engine and designed for data pre-processing. Both engines do not meet design requirements of \ours{}.

%efficient multi-threading on compute resource allocates threads to relieve
%congestion at the queueing experiencing maximum backpressure. So it decouples
%threads from operators. Does not do query/data partitioning.

\Paragraph{Wide-area streaming analytics.} 
% this paragraph does not add anything to wide-area analytics. just drop.
%Most of existing streaming engines have been developed for single machine~\cite{streambox, streamboxhbm, trill} or for distributed servers~\cite{sparkstreaming, timestream, heron, quill, streamscope, naiad, storm}, with their focus mainly on improving parallelism, responsiveness, scalability, programmability, and fault tolerance. Recently,
Novel streaming systems have been designed to operate efficiently on low-bandwidth networks, such as wide-area network (WAN). Sol~\cite{sol} introduces an early-binding
of analytics tasks to workers and dedicated communication tasks to improve
resource utilization over WAN. 
%Sol~\cite{sol} introduces an early-binding of tasks over high-latency
%networks (which addresses high-latency coordinations of task executions
%across workers) and dedicated communication tasks (which decouples
%communication from computation for a task and improves resource utilization).
AWStream~\cite{awstream} trades off accuracy for WAN bandwidth by controlling the sampling of data. MQO~\cite{mqo} provides a technique to share input/output data and operators across stream queries, saving WAN bandwidth. %While \ours{} aims at different design goals, future datacenter monitoring systems may need to consider the wisdom shared by these prior works.

% Sensor networks have explored query partitioning problems~\cite{sparksql,tag,tinydb,in-network-stream,semijoin-db,trackjoin}. However, these systems face different optimization problems because they typically involve lower traffic rates and involve special-purpose queries.

% Decentralized placement techniques such as~\cite{sbon} do not account for operator or compute resource dynamics. 

% WASP~\cite{wasp} relies on a central query planner and looks at optimizations such as scaling out operators. SpanEdge~\cite{spanedge} relies on programmers to inform of operations that need to be closer to the data source.



%The growing interest in stream data analytics has led to extensive research
%into building streaming engines for single machine~\cite{streambox,
%streamboxhbm, trill} and for distributed servers~\cite{sparkstreaming,
%timestream, heron, quill, streamscope, naiad, storm}, with their focus mainly
%on improving parallelism, responsiveness, scalability, programmability, and
%fault tolerance. As they are designed to run on high-capacity servers with
%high-bandwidth connectivity, they are best used in building stream processor
%in our monitoring system. In the related work, we focus our discussion mainly
%on query distribution methods across resource-constrained data source nodes.


==> archive/related-v2.tex <==
\balance
\section{Related Work}
\label{sec:RelatedWork}

\Paragraph{In-situ analytics.} Works in this domain reduce data movement by executing operations such as map and reduce, locally on the \client{} nodes. iMR~\cite{imr} trades off accuracy for performance by sending data summaries from each \client{} node, which is compared with \ours{} in Section~\ref{sec:sampling-vs-jarvis}. Rule-based heuristics~\cite{lambdaflow,lprof,scoop} statically determine which operators to push down to \client{}, e.g., operators beyond first stateful operator cannot be pushed down. Compute demands of our query operators vary with changing resource conditions (Section~\ref{sec:motivation}), so such static partitioning quickly becomes sub-optimal in our system (Section~\ref{sec:evaluation}). Hadoop jobs adapted for streaming applications~\cite{m3,redoop} perform compute load balancing across map operator instances by splitting input load across them. Load balancing-based data parallelism is compared with \ours{} in Section~\ref{sec:query-throughput-comparison}. DIRAQ~\cite{diraq}, FlexAnalytics~\cite{flexanalytics}, and
Logzip~\cite{logzip} focus on indexing and data compression operators to execute at the \client{}. Dynamic resource allocation is enabled by frameworks like Spark using Mesos and YARN~\cite{spark-dynamic-scaling-backpressure} at the task level. For our setup, these works map to operator-level partitioning which is evaluated in Section~\ref{sec:query-throughput-comparison}. 
\todo{Need to remove this para after review}
\textcolor{red}{In-situ data analytics reduce data movement by executing query operations locally on the data distributed across nodes. iMR~\cite{imr}, lprof~\cite{lprof}, and M3~\cite{m3-in-situ} apply MapReduce
model to process server log streams on the \client{}, but do not consider
operator compute costs \mj{pursue offloading the entire query naively (i.e.,
AllSrc)?}. DIRAQ~\cite{diraq}, FlexAnalytics~\cite{flexanalytics}, and
Logzip~\cite{logzip} are compute cost-aware query partitioning techniques,
but focus only on indexing and data compression at the \client{}.
Redoop~\cite{redoop} performs coarse-grained input data partitioning at the query-level, while LambdaFlow~\cite{lambdaflow} and Scoop~\cite{scoop} offload query operators to in-situ analytics servers statically without considering dynamic resource conditions. Unlike \ours{}, none of these works investigate fine-grained data-level partitioning for stream query operators
under highly constrained compute resources on \client{} nodes. Furthermore,
they do not consider fast query refinement, which is indispensable for our
target monitoring scenarios.}

\Paragraph{Stream operator placement.} Operator placement determines how to
place operators in the DAG across computing nodes for efficient query
execution. Their approaches (to be discussed below) are all based on the
operator-level partitioning, so would be less effective than the data-level
partitioning when applied to over the \client{} and the \server{} nodes. With
regard to algorithmic costs, some prior work finds an optimal placement on
heterogeneous resources~\cite{opt-replicate-place-sigmetrics,
opt-placement-fog} which relies on solving an NP-hard optimization problem
(in the same complexity to Equation~\ref{eq:optimization-NP}). Hence, they
cannot be used for fast query refinement at scale, as discussed in
Section~\ref{sec:drawbacks}. Flouris et al. suggest several heuristics to
assign operators near \client{} to minimize network transmission costs under
geo-distributed sites~\cite{wan-cep-network-opt}. Among the proposed
algorithms, we observe that only the greedy heuristics exhibit
non-exponential time complexity---i.e., for two sites, the \client{} and the
\server{}, with $N_{d}$ \client{} nodes, other algorithms have $O(2^{N_{d}})$
possible solutions on how to place each query instance's operators.
Similarly, Nardelli et al. suggest several (independent) model-based and
model-free heuristics for operator
placement~\cite{heuristics-op-placement-dsps}, concluding that there is no
one-size-fits-all solution. A number of other works in this domain indeed
discuss the coarse-grained operator-level
placement~\cite{network-aware-decentralized, decentral-tree-operator,
decentral-placement-only-net, operator-tree-bokhari,
utility-op-placement-decentral, sbon}). Making algorithmic decisions on the
operator placement can be either
centralized~\cite{network-aware-decentralized} or
decentralized~\cite{decentral-placement-only-net} driven by query cost
model---rule-based heuristics can be used regardless. We show that combining
model-based and model-agnostics approaches in \ours{} outperforms using them
individually in Section~\ref{sec:convergence-cost-eval} (i.e., refining
queries faster and more effectively).


\Paragraph{Parallel query processing.} Much prior work improves query
performance by dynamically alleviating compute bottlenecks through operator
scaling on input data (i.e., data parallelism). DS2~\cite{ds2} can make a
scaling decision over all query operators at a time given the correct query
performance tracing result. Stela~\cite{per-op-stela} can prioritize scaling
of operators that have the greatest impact on overall query throughput.
Similarly, other works in this field all make scaling decisions at operator
level~\cite{game-theory-scaling, decentral-scaling,nephele,
model-predictive-control-scaling, per-op-icdcs-autoparallel,
per-op-elastic-scale-ipdps, per-op-elastic-scale-tpds,
per-op-elastic-iot-cloud, per-op-predictable-low-lat-iot, dhalion}. Applying
these approaches to our setup requires considering the query operators
replicated between each \client{} and its parent \server{} node. However,
compute resource allocation on the \client{} in our system happens at the
query level, which consists of multiple operators with different data
reduction capabilities. Our optimization goal is thus different: incoming
records need to be carefully apportioned across multiple co-located query
operators within a compute budget to reduce data transfer costs as much as
possible. \newcontent{Alternatively, one could consider increasing the
apportioned data load to operators which result in high data reduction,
thereby assigning higher fraction of the query compute to such operators. But
it amounts to \modelagnostic{} approach which is evaluated in
Section~\ref{sec:query-throughput-comparison}}.

Nonetheless, conventional key-based load splitting
strategies~\cite{key-splitting-pipeflow, key-splitting-graphcep,
key-split-admission-control, key-split-debs-near-optimal,
key-split-massive-scaleout, key-split-millwheel, key-split-s4,
key-split-parallel-stateful-debs, key-split-vldb-holistic-view} are
complementary to our work. These strategies assign input key ranges to
different stateful operator instances such that each instance keeps the state
of a distinct, non-overlapping key range. Integrating key-based load
splitting into \ours{} can further reduce network transfer costs by
minimizing number of output keys sent from the \client{}.

Recent studies investigate assigning subsequences of records or windows to
operator instances based on the currently assigned compute load that is
measured on the host node~\cite{local-load-sliding-window-harness,
local-load-online-shuffle-grouping, local-load-elastic-ppq}. These approaches
are not effective to apply on a large number of \client{} nodes in our
monitoring systems, because compute resources in each \server{} node are
shared by multiple \client{}s (see Figure~\ref{fig:arch-monitoring-scale}).
Compute load on \server{} node depends on jointly considering the splitting
decisions on each \client{}, which is exponential in number of \client{}s.
SkewTune~\cite{straggler-skewtune} and Google
Dataflow~\cite{straggler-google-dataflow} employ work-stealing techniques for
straggler mitigation while others~\cite{per-op-debs-window-cep,
local-load-power-of-both-choices} use local estimates of compute load to
detect a congested host node and re-route input records to a different
operator instance in a greedy manner. \newcontent{However, in our setup, each
\client{} has a fixed compute budget allocated for a query consisting of
multiple operators with different data reduction capabilities. Similar to the
discussion of scaling techniques above, we could consider re-routing input
records to \server{} node, for operators which do not result in high data
reduction. However, this again boils down to \modelagnostic{} which is
evaluated in Section~\ref{sec:convergence-cost-eval}.}


\newcontent{\sout{However, in our setup we do not
allocate resources at the operator level. On each \client{}, a fixed compute
budget is allocated for a query consisting of multiple operators with
different data reduction capabilities, and we need to coordinate the routing
decisions across these operators to reduce network transfer costs within the
available query-level compute budget.}} \mj{discuss backpressure in the
Jarvis system section briefly.}

%To facilitate comparison with \ours{}, we evaluate a variant of this
%mechanism adapted to our setup called \coarsedp{} in
%Section~\ref{sec:query-throughput-comparison}. We discuss different
%backpressure mechanisms and their limitations for our target system: (1)
%\textit{Rate throttling at the source or dropping
%data~\cite{backpressure-spark-streaming,rxjava-backpressure}:} Our target
%system focuses on lossless monitoring and unlike systems like
%Kafka~\cite{apache-kafka}, we do not make assumptions about data persistence
%at the source so throttling it may result in data loss. (2) \textit{Operator
%queue resizing~\cite{flink-backpressure,rxjava-backpressure}:} Limited memory
%(e.g., 1 GB) on \client{}s restricts the benefits from dynamic sizing of
%operator queues, (3) \textit{Scaling compute
%resources~\cite{spark-dynamic-scaling-backpressure}:} They are similar to the
%operator scaling works discussed in this section.


%State-of-the-art approaches in network telemetry domain which perform
%near-data computation are targeted towards analyzing network packets and are
%mostly based on operator-level partitioning. EverFlow~\cite{everflow} and
%dShark~\cite{dshark} apply light-weight operations on commodity network
%switches and computing nodes near data source, respectively.
%Gigascope~\cite{gigascope} classifies operators based on domain-specific
%knowledge and pushes low-cost operators close to data source.
%Sonata~\cite{sonata} utilizes an ILP solver to  optimize operator-level
%partitioning, but at the cost of latency as high as 20 minutes. These
%approaches neglect \datapart{} and/or are based on expensive centralized
%query refinement.


\Paragraph{Stream computations on the edge.} EdgeWise~\cite{edgewise} is a
streaming engine improves throughput and latency by prioritizing query
operators who experience backpressure within the edge. Droplet~\cite{droplet}
and Costless~\cite{costless} address the operator placement problem between
edge and cloud resources for video analytics applications. They neither
leverage the benefits of the data-level partitioning nor respond to dynamic
resource conditions on the edge, whereas we do both in this work.


%\Paragraph{Wide-area streaming analytics.} Novel streaming systems have been
%designed to operate efficiently on low-bandwidth networks, such as wide-area
%network (WAN). Sol~\cite{sol} introduces an early-binding of analytics tasks
%to workers and dedicated communication tasks to improve resource utilization
%over WAN. AWStream~\cite{awstream} trades off accuracy for WAN bandwidth by
%controlling the sampling of data. MQO~\cite{mqo} provides a technique to
%share input/output data and operators across stream queries, saving WAN
%bandwidth.


%\Paragraph{Streaming query optimizations.} Runtime optimizations such as
%operator
%reordering~\cite{eddies,teddies,reordering-interactive-queries,telegraphcq}
%and resource allocation~\cite{cameo,adaptive-control-res-alloc} have been
%investigated for streaming systems which are complementary to our work. For
%operator placement, Turbo~\cite{turbo} and Sparrow~\cite{sparrow} have looked
%at decentralized scheduling for batch processing which do not directly apply
%to streaming data.


==> archive/solution.tex <==
% %\section{Jarvis}
% \section{QUERY CONGESTION CONTROL}
% \label{sec:jarvis}

% %Given a limited resource budget for executing monitoring queries on each
% %\client{} node, \ours{} comes up with an execution plan for each query
% %that could maximize network traffic reduction while greatly mitigating
% %resource costs needed for the stream processor to complete the query. \ours{}
% %enables both query partitioning and data partitioning, i.e., \emph{hybrid
% %partitioning}, and it is non-trivial to accomplish this in a timely manner in
% %datacenter scale while facing the following dynamics: (i) varying telemetry
% %data generation rates across \client{} nodes and (ii) varying amount of
% %resources available per query \mj{make it clear somewhere; we do not schedule
% %resources among queries in a node; OS does that}. We have to promptly refine
% %query plans upon identifying such dynamics. However, doing so through a
% %centralized query planner is not scaling in datacenter scale, as explained in
% %Section~\ref{sec:new-requirements}. \mj{mostly redundant. will cleanup.}

% A central contribution of our work is to meet both network traffic reduction and scalable query refinement at a time so as to withstand a high fan-in traffic to the stream processor. This is enabled by letting each query independently reconfigure its execution for both operator and data partitioning without consulting any centralized query planner. As described earlier, we introduce extensions to the pipeline of stream operators: (i) \proxy{}, a unified abstraction for stream operator and (ii) \run{}, a system runtime that coordinates executions of all \proxies{}. \Proxy{} is a light-weight operator bridging two adjacent stream operators and decides ``how much'' and ``which'' records it needs to forward to the next downstream operator. Therefore, \proxy{} implements data partitioning and reduction on hot keys at stream operator level. \run{} interacts with all \proxies{} within the \client{} node to coordinate their actions, enabling a desired partitioning plan at query level. \run{} refines the execution plan for its query without consulting any external planner, so it is able to quickly adapt to system dynamics. 


% %To facilitate
% %these new components, an original monitoring query is rewritten when 
% %deployed onto datacenter.

% %\begin{itemize}
% %    \item Per-query available resources are variable.
% %    \item Source rate is dynamic, with each \client{} node having different source rate
% %    \item Difficult to statically condfigure execution plan across \client{} nodes and the query processor.
% %\end{itemize}

% \begin{figure}
%   \centering
%     \includegraphics[width=0.48\textwidth]{fig/jarvis}
%     \caption{How \ours{} rewrites a query to incorporate \proxies{} and \run{}.
%     Data path: routing path for incoming data; Control path: interaction between \proxies{} and \run{}.
%     %\client{} side dataflow implementation of SQL query which involves filter and groupby operators on data stream coming from source. The control proxy uses the monitored backpressure at each operator queue to make routing decision. One route leads to the next dataflow on the \client{} and the other leads to uploading of data reaching the queue to the \server{}
%     }
%     \label{fig:jarvis_query}
% \end{figure}

% Figure~\ref{fig:jarvis_query} shows how \proxies{} and \run{} are structured in a computation pipeline (or graph) of the query in 
% Figure~\ref{fig:pipeline_tor}. During deployment, \ours{} rewrites the query to wire a \proxy{} with the input queue of each stream operator. Rather than physically splitting a given query
% as done in the past, \ours{} instead replicates it across the \client{}
% and \server{} nodes. A \proxy{} in the \client{} node hooks the
% communication of two neighboring operators. Guided by \run{}, it
% selects a portion $p$ of incoming data to be put in the downstream queue and subsequently consumed by the downstream operator. The \proxy{}
% drains the remaining data over the network to be processed by the
% \server{}, and the data is routed to the \proxy{} associated with 
% the same downstream operator in \server{}. For brevity, we henceforth use the term \proxy{} to mean one placed at \client{} node, unless specified
% otherwise.

% The challenge is to decide $p$ values across \proxies{} correctly. If $p$
% values are too large, we end up processing too many records that will lead to congestion and backpressure in the query dataflow, thus impacting performance; if $p$ values are too small, we end up draining too much data that will leave compute resources idle and bottleneck on network. We develop an efficient algorithm to carefully select appropriate $p$ values across \proxies{} based on dynamic resource usage states, avoiding oversubscription or undersubscription of compute resources.


% %Control Proxy does only two things. First, it collects statistics that
% %enable- \textit{backpressure detection} when the query oversubscribes given
% %resources, and \textit{hot key detection} so that grouping and reduction
% %occur only for hot keys if key skewness exists. Note that hot key detection
% %is only enabled at Control Proxy before grouping. Second, it can be
% %configured to drain records over the network if the node is about to
% %oversubscribe resources. Jarvis runtime helps coordinate the actions of
% %multiple control proxies, in order to maximize data reduction using available
% %compute resources.


% %\subsection{Congestion Control}
% \subsection{Reducing Network Traffic}
% \label{sec:reducing_traffic}

% %\Paragraph{Defining operator and query states.}
% In this section, we formalize the operator and data partitioning problem for monitoring queries on \client{} nodes. An input stream to a monitoring query is an unbounded sequence of records produced by the data source node.
% %Each record consists of an event timestamp
% %and an arbitrary number of attribute keys (\emph{fields}).
% The data source injects watermarks into record streams to guarantee time
% progress, i.e., no subsequent records will have an event timestamp earlier
% than the watermark's timestamp. Watermarks subsequently create ordered
% consecutive \emph{epochs} of records. \ours{} initiates congestion control
% and refines the query execution plan upon receiving every epoch.

% During epoch processing, a \proxy{} collects statistics for its downstream
% queue, and at the end of the epoch, it defines its downstream operator to be one of three states: (i) \emph{Congested}: the queue contains more than a predefined number of pending records, experiencing backpressure. (ii)
% \emph{Idle}: the queue stays empty for longer than a predefined time
% duration. (iii) \emph{Stable}: the queue is neither congested nor empty.
% Based on queue states, \run{} determines that a query is congested if at
% least one \proxy{} is congested and idle if all \proxies{} are idle.
% Otherwise, the query is in stable state, which is preferred.

% \Paragraph{Problem definition.} Each \Proxy{} $i$ has an associated parameter $p_i$, which we refer to as \emph{\p{}}. It is the probability of pushing incoming records down to the next operator for execution in the
% node, i.e., $0 \le p_i \le 1$, thus enabling data partitioning. Note that
% \proxy{} can behave as operator partitioning by having $p_i$ only alter
% between 0 and 1. Subsequently, with the probability $1-p_i$, \proxy{}
% $i$ must drain the incoming records to the remote \server{}.

% Once the current epoch is finished, each \proxy{} cleans up the downstream
% queue by draining any remaining records in the queue to the \server{} 
% and defines the congestion state of the downstream operator. 
% Then, if the query is identified as either congested or idle based on aggregating operator states informed by \proxies{}, we refine \p{}s. Since the compute budget on a \client{} node is a shared resource, \proxies{} cannot update their own \p{}s independently. \run{} instead jointly configures \p{}s for the next epoch. Therefore, refining the execution plan of a query is subject to how we configure its \p{}s. The ideal \p{} values will lead to the most network traffic reduction while keeping the query stable on the current compute budget. \todo{Address issue that the same argument could hold for multiple queries and that we need to update load factors across queries in lockstep?}

% %The goal of \ours{} is to search for the best \emph{\sub{}} to execute on the
% %\client{} node via hybrid partitioning that keeps the query stable. A
% %\sub{} is organized as a continuous subsequence of operators in a computation
% %graph and must reduce data volume from input streams to be \emph{valid}.

% %\subsubsection{Optimization Objective}

% \begin{figure}
%   \centering
%     \includegraphics[width=0.4\textwidth]{fig/jarvis_parameters}
%     \caption{Computation graph with M operators and parameters used by \ours{} for updating load factors in \proxies{}.}
%     \label{fig:jarvis_parameters}
% \end{figure}

% \Paragraph{Optimization.}
% \mj{This optimization part needs to be neat and shorted. BTW, to develop equations, can we formally define a virtual overlay op which consists of a single or multiple physical ops and which lead to data reduction?}
% To simplify our discussion on optimizing for network traffic reduction, we assume that a query operator always results in data reduction for the output stream as compared to the input stream. Note that such a condition might not hold for operators such as Join, in which output stream can be larger in size compared to input. If Join is the final operator in the query, we don't consider it in our optimization. But if there are downstream operators such as Filter that effectively reduces the data stream size, then we combine the minimal number of downstream operators (Join and Filter in above case) and represent it as a single operator in our optimization that effectively reduces data size. \lowpri{How is optimization and subsequent analysis affected if the only constraint is relay ratio $r \geq 0$ so there is no upper bound?}

% \todo{Extend the optimization to more general DAGs} Consider a computation graph as shown in Figure~\ref{fig:jarvis_parameters}, where it contains $M$ operators $\{Op_i : 1 \le i \le M\}$. 
% %, with $op_i$ in the graph relaying a fraction
% %$r_i$ of input records to the next operator after execution.
% For each \proxy{}, guided by its \p{}, a record will be either pushed to the downstream operator or drained. As a result, minimizing the drained network traffic from \client{} with compute budget on a single core $C$ yields optimization of variables $p_{1}+p_{2},...,p_{M}$, where $p_{i}$ is the load factor for each \proxy{} $i$ subject to $C$. This turns into the following optimization formulation for an epoch:

% %\begin{align*}
% %     \min_{p_{1},p_{2},...p_{M}} &N_{1}+N_{2}...N_{M}\\
% %     subject to,\\
% %     &Compute\: budget\: constraints
% %\end{align*}
% %
% %More specifically, the above can be rewritten as
% %\begin{align*}
% %    \min_{p_{1},p_{2},...p_{M}} &N(1-p_{1}(1-r_{1}(1-p_{2}...(1-r_{M-1}(1-p_{M}))..) \numberthis \label{eq:optimization} \\
% %    subject to,\\
% %    &p_{1}N(c_{1}+p_{2}r_{1}(c_{2}+...p_{M}r_{M-1}c_{M})...) \le C
% %    \label{eq:optimization-constr}
% %\end{align*}

% % \begin{align*}
% % &\argmin_{p_{1},p_{2},..,p_{M}} d_1+d_2+,...,+d_M \numberthis \label{eq:netopt}\\
% % &d_1 = N - Np_1\\
% % &d_i = (1-d_{i-1}) - (i-d_{i-1})p_i~~~~~~~~2 \leq i \leq M \nonumber
% % \end{align*}
% % subject to
% % \begin{align*}
% % &Np_{1}(c_{1}+r_{1}p_{2}(c_{2}+...r_{M-1}p_{M}c_{M})) \le C \numberthis \label{eq:netconst}\nonumber
% % \end{align*}

% \begin{align*}
%     \min_{p_{1},p_{2},...p_{M}}
%     &N\sum_{i=1}^{M}[\prod_{j=0}^{i-1}p_{j}r_{j}](1-p_{i}) \numberthis
%     % &N(1-p_{1}(1-r_{1}(1-p_{2}...(1-r_{M-1}(1-p_{M}))..) \numberthis
%     \label{eq:optimization-obj} 
% \end{align*}
% subject to,
% \begin{align*}
%     &N\sum_{i=1}^{M}[\prod_{j=0}^{i-1}p_{j}r_{j}] p_{i}c_{i} \le C,\\
%     % &p_{1}N(c_{1}+p_{2}r_{1}(c_{2}+...p_{M}r_{M-1}c_{M})...) \le C\\
%     &0 \le p_{i} \le 1\ \forall\ i\ \epsilon\ [1,M],\\
%     &0 \le r_{i} \le 1\ \forall\ i\ \epsilon\ [1,M],\\
%     &0 \le c_{i} \le 100/N\ \forall\ i\ \epsilon\ [1,M]\\ \numberthis
%     \label{eq:optimization-constr}
% \end{align*}
% where,
% \begin{align*}
%     &p_{i}\ \forall\ i\ \epsilon\ [1,M]\ \mathrm{are\ the\ optimization\ variables}\\
%     &p_{0}=1,r_{0}=1\\
%     &N,\ M,\ C,\ r_{i}\ \&\ c_{i} \forall\ i\ \epsilon\ [1,M] \mathrm{\ are\ constants\ for\ a\ problem\ instance}
% \end{align*}

% \noindent Note that $r_{i}$ is relay ratio of operator $i$ i.e. fraction of input records relayed to the next operator $op_{i+1}$ after they are consumed by $op_i$. $c_{i}$ is the compute cost of $op_i$ for a single record, given total $N$ records injected into the query in an epoch. So the objective function minimizes the total data size of drained data from each of the \proxies{}, subject to the compute budget available on \client{} node. 
% %The optimization
% %objective is to minimize the total size of data that needs to be drained to %\server{} across $M$ operators within compute budget $C$.

% % The objective and constraints contain multilinear terms, and in the general case, multilinear programming is known to be NP-hard~\cite{multilinear-complexity}. 

% We show in Appendix~\ref{sec:characteristics} that this original formulation for the optimization problem is non-convex and thus computationally hard. Furthermore, we made certain assumptions in our problem formulation which may not be true in practice. Following are the additional challenges in solving the congestion control problem:

% \begin{itemize}
%     \item Accurately estimating the execution cost per record of an operator $c_i$ is hard. As we have seen in Appendix~\ref{sec:characteristics}, such a cost depends on the input data characteristics, which can change at runtime. Furthermore, estimating the cost at runtime is complicated by (i) non-linear behavior of computation cost with input data size, (ii) performance interference in multi-query settings on \client{} node.
%     \item Relay ratio $r_i$ can vary non-linearly with the input data size. In case of grouping operator for example, relay ratio is affected by the grouping key distribution in input data. So depending on the load factor of an operator, its $r_i$ values may change non-linearly. 
%     \item The total compute cost $C$ available for a query is not known. Because it depends on the set of monitoring queries executing on \client{} node which can change frequently \todo{Add citation} as well as how underlying scheduler allocates resources to each query.
% \end{itemize}
% % In general it contains multilinear terms and hence is non-convex and computationally hard~\cite{multilinear-complexity}. With $M=2$, we observe that the bilinear terms in Equation~\ref{eq:netopt} and~\ref{eq:netconst} can be written in quadratic form. Hence, this optimization results in a quadratic objective with quadratic constraints. This is known to be NP-Hard in general case. 
% % Further, dynamic resource conditions mean available compute resources per query are unknown beforehand so the constraint is a blackbox:
% % \begin{itemize}
%     % \item The cost for individual operators changes based on the number of records processed by the operator i.e. $p_{i}$ and is possibly non-linear
%     % \item Cost for individual operators estimated by the observed execution time of an epoch isn't accurate because changing the $p_{i}$ values may change the observed execution time. 
%     % \item Total cost $C$ for a single query may not be available. \atul{What happens with multiple queries? Because in that case, we assume 1-2 cores and 1 GB memory}
% % \end{itemize} 

% In the rest of this section, we describe the system and algorithmic details of how \ours{} addresses the network traffic reduction problem in \client{} nodes.  
% % \atul{Show that for convergence check, determining if the currConstraint-targetConstraint<constrTolerance is a sufficient condition, because of prioritizing operator updates based on r-values}

% \subsection{Jarvis Design}
% We first focus on how the \run{} and \proxies{} coordinate together to enable query adaptation at runtime to reduce network traffic. Details of our algorithm called \algo{} which is used to search for proper \p{} values and quickly end up with an execution plan for a query that provides great network traffic reduction is described in Section~\ref{sec:adaptation-algo}. 

% \begin{figure}
%   \centering
%     \includegraphics[width=0.48\textwidth]{fig/JarvisStateMachine.png}
%     \caption{\run state machine. \todo{Redraw figure to make it look better}}
%     \label{fig:jarvis_state_machine}
% \end{figure}


% \subsubsection{Runtime Adaptation}
% \label{sec:runtime-adaptation}

% %\Paragraph{Adapting \p{}s.}
% % to enable congestion control on \client{}.
% %\Run{} periodically adjusts the \p{}s to relieve congestion or increase data
% %processing rates on \client{} within compute budget.
% Figure~\ref{fig:jarvis_state_machine} shows the overall workflow of \p{} orchestration and the various phases that \run{} goes through. \run{} keeps a logical timestep to track the progress of epochs. When records for the epoch at timestep $j$ are all processed, the timestep advances to $j+1$. If \run{} detects that \p{}s need to be refined due to the query being either congested or idle, it triggers an adaptation phase wherein the new query resource characteristics are profiled in one epoch, and then an adaptation algorithm (Section~\ref{sec:adaptation-algo}) kicks in to either increase or decrease \p{} to bring query back to stable state. The following explains how \run{} transitions among operational phases:

% \begin{myitemize}
%     \item \textbf{Startup: initial phase.} All \p{} values are initialized to zero, so all stream records are sent out to \server{} \mj{not doing so anymore right?, Atul: this is for when we start the system for the first time. So I would think load factors need to be set to some value so we just start in cloud-only configuration.}.

%     \item \textbf{Probe: normal operation.} At the end of every epoch, \run{} executes \texttt{ProbeCP()} function to query all the \proxies{} and determine their congestion states. It continues to do so until it identifies the computation pipeline to be congested or idle. At this point, the runtime enters \texttt{Profile} phase.

%     \item \textbf{Profile: enter adaptation phase.} Given the query was congested/idle, \ours{} needs to obtain estimates of the new query resource characteristics such as compute cost of each operator and their \reduc{}s \mj{the only case?, Atul: writing out the case was unnecessary, removed}. To facilitate profiling, we assume fair compute resource allocation made by underlying scheduler, amongst the monitoring queries. This helps us determine the compute budget available per query, based on the number of queries and total compute available for the queries on \client{} node. \mj{scheduler at the server would already perform resource splitting based on shares of queries. Are you suggesting another scheduling here?, Atul: No, I rewrote the sentence so hopefully its clearer.}. Note that the profiling estimates need not exactly match the compute cost during normal operation, but are instead used to better initialize \p{} values and thus improve convergence time to bring query back to stable state (details in Section~\ref{sec:algo-convergence-optimization}). \mj{we do this profiling always?, Atul: Yes, every time a major resource change occurs, we profile the operators. } 
    
%     \item \textbf{Adapt: query refinement by updating \p{}s.} \run{} iteratively updates load factors until the computation pipeline is back to stable state, in which case it returns to \texttt{Probe} phase. Details of which load factors to change and by how
%     much are discussed in detail in Section~\ref{sec:adaptation-algo}.
%     Upon entering into \texttt{Adapt} phase after \texttt{Probe} phase, when we update load factors, query operators could be in the middle of processing records from different epochs. In this case, \run{} cannot accurately observe the effect of load factor updates immediately in the next timestep. So, it waits for a new epoch to be processed once the load factors are updated, and then executes \texttt{ProbeCP()} to probe the query congestion state. Consequently, during \texttt{Adapt} phase, only a single epoch is executed at a time by all the operators in the computation graph (i.e., no pipelining of epochs across operators).

%     % When the runtime enters adaptation phase from probing, it first executes $\texttt{calibrate()}$ to obtain the latest data reduction ratios for each control proxy.

%         % It does so by first executing $\texttt{calibrate()}$ to calibrate the query
%         % for identifying subqueries/operators that result in data reduction
%         % and then resetting the load factors to  $p_{min}$. It then updates
%         % the control knobs for the next time step (which is denoted by $p_i
%         % => p_{i+1}$ in Figure~\ref{fig:runtime-state-machine}).
% \end{myitemize}

% %We use \texttt{ProbeCP()} to determine the congestion state of \proxies{},
% %but the control system can result in oscillating behavior if the probing is
% %sensitive to small changes in congestion state. 
% The control system can result in oscillating behavior if the probing is sensitive to small changes in the congestion state. Therefore, as stated in Section~\ref{sec:reducing_traffic}, each \proxy{} is configured with a threshold fraction of epoch records (\texttt{DrainedThres}) that can be drained by the \proxies{} and tolerated by \texttt{ProbeCP()} without signaling congested state. Similarly, each \proxy{} is configured with a threshold fraction of epoch duration (\texttt{IdleThres}) that allows the \proxies{} to stay idle and can be tolerated by \texttt{ProbeCP()} without signaling idle state. 
% \todo{Talk about draining algorithm at each control proxy and how it preserves streaming semantics}

% We now describe the \algo{} algorithm to address the challenges mentioned in solving the optimization problem we formulated in Equation~\ref{eq:optimization-obj} \mj{which ones? Atul: clarified. }. We also discuss the optimizations we have done for it to work well in practice.

% \subsubsection{\algo{} Algorithm}
% \label{sec:adaptation-algo}
% To design the algorithm for adaptation, we return to the optimization problem in Equation~\ref{eq:optimization-obj}. Note that when we increase \p{} values, it would increase the compute cost in Equation~\ref{eq:optimization-constr} while simultaneously decreasing the objective function, because more data is being processed on \client{} node. Furthermore, since \p{} for first operator $p_1$ appears to affect all the terms in both objective and compute cost functions, changing it might appear to result in largest change in compute cost and associated decrease in objective function. \mj{does not flow well. how the largest increase in compute for p1 leads to the use of our naive approach? Atul: tried to change language a bit, but not spending time on it since it might be better to completely remove this as you mention in your later comment} With this basic observation, we devised a simple heuristic called \oldalgo{}, to update $p_1$ first \mj{you may decrease, Atul: fixed}, using a fixed step size (say $\Delta p = 0.1$) to fully utilize the available compute budget yet not exceed it. Then update $p_2$, and then $p_3$ and so on. We analyzed the effectiveness of this approach using a simulator. \mj{How about starting 4.2.2. by emphasizing "the order in which p values change matters", then say we will show evidence using a simulator exploring computation graphs. BTW, instead of focusing on naive stepwise-adapt here, can we just evaluate combinations present in Table 1 and say optimal orderings differ across them? And explain why using figure 8?}


% % For M=2 operators, it can be rewritten as:
% % \begin{align*}
% %     f_o(p_1,p_2) = N ( 1 - p_1 ( 1 - r_1 ( 1 - p_2)))
% % \end{align*}
% \todo{Figure out how to move parts of this analysis to evaluation section or appendix.}
% \Paragraph{Limitations of \oldalgo{}.} We simulated the behavior of \oldalgo{} by varying parameters of the optimization problem and then evaluating its effectiveness in reaching the optimal solution of \p{} values for each problem instance. In particular, for the M=2 operator case, we generate data at the rate of 150,000 records/s (equivalent to 27.2 Mbps) at the source (numbers derived from analysis of \pingmesh{} data). And then we discretize range of values that parameters like $c_{1}, c_{2}, r_{1}$ and $C$ can take, based on their range constraints in Equation~\ref{eq:optimization-constr}. We then sweep through the possible values of these parameters to create each optimization problem instance.


% \begin{table}[h!]
% \centering
% \begin{tabular}{ |p{1cm}|p{1cm}|p{1cm}|p{2cm}|  }
%  \hline
%  $c_1$ & $c_2$ & $r_1$ & \oldalgo{} effective?\\
%  \hline\hline
%   High & High & High & No\\
%   High & High & Low & Yes\\
%   High & Low & High & No\\
%   High & Low & Low & Yes\\
%   Low & High & High & No\\
%   Low & High & Low & Yes\\
%   Low & Low & High & No\\
%   Low & Low & Low & Yes\\
%  \hline
%  \end{tabular}
%  \caption{Effectiveness of \oldalgo{} for 2 operators}
%  \label{tab:simulator-analysis}
% \end{table}

% Table~\ref{tab:simulator-analysis} shows whether \oldalgo{} is effective or not i.e. does increasing $p_1$ first and then $p_2$ bring us closer to the optimal solution, or does increasing $p_2$ first and then $p_1$ work better. High and Low indicate the boundary values for $c_1, c_2$ and $r_1$ within their ranges. So for example, High for $r_1$ indicates a value of 0.9 while Low indicates 0.1. Similarly $c_1, c_2$ have their High and Low values computed based on the input records $N$. 

% \begin{figure}[t]
% \centering
% \subfigure[r1 is low]{\includegraphics[width=1.65in,height=1.2in]{fig/ObjVsConstr_r1low_c1high_c2mid.pdf}}
% \subfigure[r1 is high]{\includegraphics[width=1.65in,height=1.2in]{fig/ObjVsConstr_r1high_c1_high_c2low.pdf}}
% \caption{\label{fig:ObjectiveVsConstraint} \todo{Enlarge figures} Objective vs Constraint for different $r_{1}$ values in the case of 2 operators. Arrows indicate direction in which p1 or p2 increase. E.g, in first graph, each cluster of points corresponds to a fixed p1 value. Points in the cluster correspond to increasing p2 value}
% \end{figure}

% \oldalgo{} is effective only when $r_1$ is low. If $r_1$ is high, then increasing $p_2$ first and then $p_1$ brings us closer to the optimal solution. This also becomes apparent when we observe the graph of objective function plotted against compute cost as shown in Figure~\ref{fig:ObjectiveVsConstraint}. In the case of $r_1$ being low, it shows that for a given value of total compute budget $C$, increasing $p_1$ and then $p_2$ is effective in minimizing the network cost. However, when $r_1$ is high, it is more effective to maximize $p_2$ first, and then increase $p_1$ to meet compute budget. 

% Based on above insight, we show the following result for ordering the updates of \p{} values for $M$ operators: 
% \todo{Would a proof be interesting? We might simply be able to show the ordering based on r values is optimal, using gradients of objective/constraint functions }

% \Paragraph{Prioritizing operators.} \mj{seems we highly require an algorithm pseudo-code.}
% We propose \algo{}, which improves upon \oldalgo{}, by estimating the desired \p{}s of \proxies{} and updates those \p{}s based on priorities of the downstream operators. We prioritize maximizing \p{} values of operators that have lower \reduc{}s first. This is also intuitive as such operators provide significant data reduction \mj{do not?, Atul: fixed} and are thus high utility operators for network traffic reduction. 

% So briefly, if a query is congested, we need to reduce load factor of operators starting with the lowest priority operator that is currently executing, i.e., \p{} $0 < p \le 1$. If a query is idle, we need to increase the load factor for the highest priority operator that is not fully executing yet, \p{} $0 \le p < 1$. Following that, we define \emph{\boundaryop{}} as an operator that is the target for adaptation at each timestep. As we order operators before query execution based on prioritization rules, a \boundaryop{} would always have \p{} $p$ between 0 and 1. While operators that are higher priority than \boundaryop{} would have $p=1$ and lower priority operators would have $p=0$. \run{} needs to identify the \boundaryop{} for each query at each timestep in \texttt{Adapt} phase, and then update its load factor by step size $\Delta p$ based on the congestion state.

% % Note that reordering operators here doesn't imply changing their ordering in the query physical plan. Though doing so is complementary to our solution. 

% Furthermore, as illustrated in Appendix~\ref{sec:characteristics}, grouping/reduction and join operators are computationally expensive (also discussed in~\cite{streamboxhbm}). So their \reduc{} values are critical in determining their \p{} values and consequently whether they are executed on \client{} node or not. Interestingly, if \reduc{} of computationally cheap operator like Filter is high, its \p{} updates would have low priority. As for Join operators, it is preferred to run on \client{} in case of joining with a static table, as commonly done in datacenter telemetry tasks~\cite{tersecades}. Since their \reduc{} can be greater than 1, we execute them on \client{} node only if they are followed by a filter or grouping operation that will effectively result in data size decrease. Otherwise, they are delegated for execution on \server{} node.

% % \ours{} takes into account the cost effectiveness of each stream operation for achieving data reduction. Briefly, \ours{} prioritizes inexpensive operators with potential of high data reduction. 
% % Driven by the characteristics of stream operations illustrated in Appendix~\ref{sec:characteristics}, we come up with a few prioritization rules among operations: (i) filtering and projection are stateless and inexpensive, so run on \client{} with high priority; (ii) grouping and reduction are less prioritized as they typically dominate total query execution time~\cite{streamboxhbm}; and (iii) joining is preferred to run on \client{} in case of joining with table, as commonly done in datacenter telemetry tasks~\cite{tersecades}. To facilitate these rules, we first organize a computation graph such that ``\emph{operators with the highest priority appear first in the graph}''. 

% \subsubsection{\algo{} Analysis}
% \label{sec:algo-analysis}

% \mj{certainly not a right place to show lots of numbers. not good to mix methods and numbers fine-grained, in general. we move this detail to either eval while we can clearly present intuitions why good initialization is needed.}
% We now look at the accuracy and convergence time for \algo{} using our simulator. 
% \begin{figure}
%   \centering
%     \includegraphics[width=0.48\textwidth]{fig/AccuracyVsConvergence-2operators.pdf}
%     \caption{Accuracy vs convergence time in number of epochs. Y-axis shows the additional records drained from \client{} due to \algo{}, compared to optimal solution. Input number of records is 150000}
%     \label{fig:acc-convergence-2-operators}
% \end{figure}

% \Paragraph{Accuracy vs. convergence cost.} To quantify accuracy of \algo{}, we analyze further the M=2 operator case. We fix $c_1, c_2$ and $r_1$ parameters in the optimization, and sweep through the possible values of total compute budget $C$ in Equation~\ref{eq:optimization-constr}. For each value of $C$, we determine the optimal network transfer cost via brute force search and compare it with the network transfer cost that \algo{} converges to, to determine the absolute error in the cost determined by \algo{} compared to optimal. Figure~\ref{fig:acc-convergence-2-operators} shows the results. As can be seen, for 2 operators, \algo{} performs well. It has a loss in accuracy (in terms of additional records drained per epoch) of about 10000 records, which is ~6.7\% of input record count, within 4 epochs. We discuss optimizations to \algo{} in Section~\ref{sec:algo-convergence-optimization}, that helped achieve good convergence time. 

% \begin{figure}
%   \centering
%     \includegraphics[width=0.48\textwidth]{fig/MultiOpsConvTime.pdf}
%     \caption{Convergence time in number of epochs as we increase number of query operators. Input number of records is 150000. \todo{Replot graph if it is confusing}}
%     \label{fig:convergence-multi-ops}
% \end{figure}

% \Paragraph{Scaling to multiple operators.} We now increase $M$, the number of operators in the query. We fix the accuracy of \algo{} this time, and sweep through the space of total compute budget values $C$ between 0 and 100. For each value of $C$ we determine the number of iterations it took \algo{} to converge. Figure~\ref{fig:convergence-multi-ops} shows that the convergence time can go up to 15 epochs for 4 or more operators. The stabilizing at ~15 epochs is because we fixed the range of values $C$ can take. 15 epochs is high for us because one of the requirements for \ours{} is to adapt quickly to resource changes that can happen in the order of a few (<10) seconds. So we discuss in the next section, this and some other optimizations to improve convergence time of \algo{}.

% %Recall that we allow operators in high priority to appear early in a
% %computation graph. This makes it easy for \algo{} to update \p{}s of
% %\proxies{} based on priories of their downstream operators during
% %\texttt{Adapt} phase.
% %For instance, for a graph with two \Proxies{} such as one in
% %Figure~\ref{fig:jarvis_query}, \algo{} attempts to maximize \p{} for the
% %first \Proxy{} wired with filtering. Then, if there is any available compute
% %budget left, \algo{} increases \p{} for the second \Proxy{} wired with
% %grouping.


% %So if data had been partitioned at an operator and its load factor can still
% %be increased or decreased, it becomes the \boundaryop{} for the current
% %timestep. Otherwise, if we are doing operator partitioning and a query is
% %congested, we need to reduce load factor of operators starting with lowest
% %priority operator that is currently executing. If a query is idle however
% %during operator partitioning, we need to increase the load factor for the
% %highest priority operator that is not currently executing yet.

% %Load factors are updated based on the congestion state of \proxies{}.
% %We define a step size for each load factor to be updated as $\Delta p$.
% %So when there is congestion, we decrease the load factor for the
% %\boundaryop{} in the query by $\Delta p$. If \Run{} detected the query to be
% %idle, it increases the load factor for the \boundaryop{} in the query by
% %$\Delta p$.

% \subsubsection{Optimizing Convergence Cost of \algo{}}
% \label{sec:algo-convergence-optimization}
% We discuss optimizations we introduced in designing \algo{} to improve its convergence cost. 
% \Paragraph{1. Initializing load factors.} As discussed in Section~\ref{sec:algo-analysis}, \algo{} suffers with higher convergence cost for 4 or more operators. A primary reason for this is that when we enter \texttt{Adapt} phase, we always re-initialize each \p{} value to the same minimum (i.e. 0.05) for all operators. This means when the optimal \p{} values are much higher, then it takes a large number of iterations to converge. 

% In order to get better initialization values for \p{}s, we devise a hybrid approach that combines the model-free \algo{} for updating \p{} values, with a model-based solution that solves the optimization problem in Equation~\ref{eq:optimization-obj} and helps more accurately initialize \p{}s. We earlier described the non-convex nature of the objective function. However, there does exist a simple reformulation of the original problem in which the optimization variables can be solved as a linear program (LP), as described below:\\
% Let $e_i=\prod_{j=0}^{i}p_j$ be the effective load factor of cumulative sequence of operators until $op_i$. Then the objective function in Equation~\ref{eq:optimization-obj} and constraints in Equation~\ref{eq:optimization-constr} can be rewritten as: 
% \begin{align*}
%     \min_{e_{1},e_{2},...e_{M}}
%     &N\sum_{i=1}^{M}[(\prod_{j=0}^{i-1}r_{j}).(e_{i-1}-e_{i})] \numberthis
%     \label{eq:optimization-obj-linear} 
% \end{align*}
% subject to,
% \begin{align*}
%     &N\sum_{i=1}^{M}[(\prod_{j=0}^{i-1}r_{j}).e_i.c_i] \le C,\\
%     % &p_{1}N(c_{1}+p_{2}r_{1}(c_{2}+...p_{M}r_{M-1}c_{M})...) \le C\\
%     &0 \le e_{i} \le e_{i-1}\ \forall\ i\ \epsilon\ [1,M]
%     \label{eq:optimization-constr-linear}
% \end{align*}
% where,
% \begin{align*}
%     &e_{i}\ \forall\ i\ \epsilon\ [1,M]\ \mathrm{are\ the\ optimization\ variables}, \\ 
%     &\&\ e_{0}=1
% \end{align*}
% The rest of the conditions on $N, M, C, c_i, r_i$ remain the same as in the original formulation. To solve the problem using existing LP solvers, we need the per-operator compute cost $c_i$ and \reduc{} $r_i$. We also need the available compute budget $C$. For doing so, we leverage the runtime estimates we collected for query operators in \texttt{Profiling} phase and set $C$ to the compute cap imposed on the query during \texttt{Profile} phase. We then solve the LP using these estimates, and use them as initial \p{} values when \ours{} enters \texttt{Adapt} phase. Even though the problem formulation doesn't capture the non-linearity for compute cost and \reduc{} with input data size, we see in Section~\ref{sec:evaluation} that the linear approximation still helps \ours{} converge quickly in practice. 

% \Paragraph{2. Binary search in partitioning configuration space.}
% \mj{Binary search partitioning: we need this? no binary search anymore, and combining it with LP is not intuitive. And, naive way does not work well, we already explained. just move some good explanations forward. Atul: based on our discussion, kept this part but made it small}
% A naive approach for adaptation in \texttt{Adapt} phase would be to incrementally update \p{} of the current \boundaryop{} using a fixed step size (say $\Delta p = 0.1$). However, this approach would result in linear number of steps to converge. To improve convergence time, \run{} executes a binary search over the \p{} values of \boundaryop{}, at each timestep. It enables \run{} to quickly set \p{} of each operator so that its execution cost on \client{} meets available compute budget. 
% scr
% % %It is impractical for adaptation at short timescales, which is a requirement for \ours{}.
% % \todo{Reconsider if below can still be done with the current algo version? If not, remove}
% % We can improve the %performance of this approach by prioritizing
% % convergence times by scanning operators in a priority order that can run with full capacity using $\Delta p=1.0$ first (i.e., operator partitioning), and then by making the best use of any remaining compute resource budget on
% % the \boundaryop{} using $\Delta p=0.1$ (i.e., data partitioning). While this strategy yields a considerable improvement over the naive approach, it takes linear time for identifying the correct operator and data partitioning, and thus could be expensive for a large computation graph. 

% % We modify the operator partitioning-first strategy described earlier, by doing a binary search instead of a linear search in the space of operator and data partitioning configurations. So for operator partitioning, \run{} first executes a binary search over operators, and then when it settles on the maximal number of operators that can be executed on \client{} without
% % exceeding compute budget, it then explores the load factor values for the
% % next high priority operator using binary search to exploit any remaining
% % compute resource. 

% %operator partitioning first, and then perform data partitioning on the
% %\boundaryop{} to avail any remaining compute resource budget. To achieve
% %this, a dynamic load factor update step strategy can be used, wherein
% %operator partitioning is done first using $\Delta p=1.0$. Then, data
% %partitioning is done to use spare compute budget by setting $\Delta p=0.1$.
% %Even with this improved strategy, for a large computation graph, it takes
% %linear time for identifying the correct operator partitioning. Further, with
% %$\Delta p=0.1$, data partitioning can still take up to ten timesteps to
% %explore all the possible configurations for load factor between 0 and 1.


% % \subsubsection{Optimizations to improve convergence time}


% % In the adaptation phase, increasing the processing load on \client{} by
% % $\Delta p$, one load factor at a time, can result in prohibitively large
% % convergence times. So we have the following optimizations to improve the
% % duration for convergence: \label{sec:optimization-convergence-time}


% %For data partitioning actions, we have seen $\Delta p =
% %0.1$ to work well in our evaluation.

% %Control proxies provide the following four interfaces to \run{} to enable
% %binary search-based query partitioning:
% %\begin{myitemize}
% %    \item $\texttt{IncreaseOpLoad()}$: This action performs binary search
% %        to increase the maximal number of operators that can be executed on
% %        \client{} without exceeding compute budget. It performs operator
% %        partitioning and is used in adaptation phase when the
% %        query is in empty state.
% %    \item $\texttt{IncreaseDataLoad()}$: When the query is in idle state and
% %    $\texttt{increaseOpLoad()}$ cannot increase the number of operators further
% %    without causing congestion, this action increases the load
% %        factor for the \boundaryop{} to maximize processing on
% %        \client{}. This performs data partitioning.
% %    \item $\texttt{DecreaseOpLoad()}$: This action performs binary search to
% %    reduce the number of operators executed on \client{}, so as to avoid
% %    congestion. It performs operator partitioning and is used in adaptation phase
% %    when the query is in congested state
% %    \item $\texttt{DecreaseDataLoad()}$: When the query is congested and
% %    $\texttt{decreaseOpLoad()}$ cannot decrease the number of operators further
% %     without causing query to be in idle state, this  action decreases the load
% %     factor for the \boundaryop{} to reduce processing on \client{}. This
% %     performs data partitioning.
% %\end{myitemize}

% \Paragraph{3. Fast adaptation for small resource changes.}
% %Upon entering \texttt{Adapt} phase from \texttt{Probe}, as described earlier,
% %we incur a cost from waiting for existing epochs to complete processing.
% %Then,
% If the change in available resources is small, it suffices for \run{} to
% start with the current partitioning configuration of operators and only
% explore \p{} vlaues on the \boundaryop{} to quickly converge to stable
% state. In this case, \run{} skips the \texttt{Profile} phase when congestion state of query changes. It also doesn't run the LP solver. But if available resource changes are large, \run{} reruns full adaptation by first profiling operators, then running the LP solver and lastly executing \algo{}.
% % prioritizing operator partitioning and
% % then data partitioning from the boundary operator. 

% %\atul{Remove the part to reset load factors}
% %So to make adaptation decisions based on resource changes and thus improve
% %convergence time,
% %To detect small resource changes, we define threshold configuration parameter
% %for change in the epoch records drained $\Delta EpochRecordsDrained_{thres}$
% %and threshold parameter for change in the fraction of epoch duration that the
% %query is idle $\Delta EpochFractionIdle_{thres}$.
% To detect small resource changes, \ours{} tracks the degree to which
% congestion state has changed in the current epoch, compared to previous
% epoch. It does so by measuring change in the number of records drained and
% change in idle duration for the query. If either level is within configured
% thresholds,
% %So if the congestion state change is within these threshold values,
% then the load factor for only the \boundaryop{} is adjusted by executing binary search in the range above current \p{} if the query is idle, or below the current \p{} if it is congested. 
% % reset to execute binary search on the operator with $\Delta p = 0.1$.


% \revmarker{}
% %$\texttt{increaseDataLoad()}$ or $\texttt{decreaseDataLoad()}$ actions
% %depending on whether query is congested or idle. Otherwise, full adaptation
% %involving operator and data partitioning is triggered.

% % \Paragraph{Empirical analysis on optimization objective v.s. \algo{}.} We
% % wrote a simulator to sweep through the space of parameters in the
% % optimization and identified configurations in which \emph{Stepwise-Adapt}
% % would not provide optimal solution. We show the results for the specific case
% % of 2 operators in the query dataflow in Table~\ref{tab:opt-analysis}. It
% % shows the results with $c_1$ being the CPU cost for processing per byte of
% % data for operator 1, $c_2$ the CPU cost for processing per byte of data for
% % operator 2 and $r_1$ the data reduction ratio for operator 1. $c_1$ and $c_2$
% % being high means that the CPU costs simulated are $\geq 90\%$ while low
% % indicates the costs are $\leq 10\%$. While $r_1$ being high indicates the
% % data reduction ratios simulated are $\geq 0.9$ while low indicates $\leq 0.1$

% % \begin{table}[h!]
% % \centering
% % \begin{tabular}{ |p{1cm}|p{1cm}|p{1cm}|p{2cm}|  }
% %  \hline
% %  $c_1$ & $c_2$ & $r_1$ & Stepwise-Adapt works?\\
% %  \hline\hline
% %   High & High & High & No\\
% %   High & High & Low & Yes\\
% %   High & Low & High & No\\
% %   High & Low & Low & Yes\\
% %   Low & High & High & Yes\\
% %   Low & High & Low & Yes\\
% %   Low & Low & High & No\\
% %   Low & Low & Low & Yes\\
% %  \hline
% %  \end{tabular}
% %  \caption{Optimization analysis for 2 operators}
% %  \label{tab:opt-analysis}
% % \end{table}

% % We can see that in majority of the cases, \emph{Stepwise-Adapt} works to
% % identify the optimal load factors for operators. There are three cases
% % however where the "No" indicates we have a data partitioning configuration in
% % which $p_1 < p_2$ converges to an optimal solution. This behavior is observed
% % when $c_1 > c_2$ and $r_1$ is close to 1. We refer to such operators as
% % \emph{low-utility operators} because they have a high compute cost while
% % having a low data reduction ratio. So the takeaways from our analysis are:
% % (1) \emph{Stepwise-Adapt} works in majority of cases, (2) increase load
% % factor for compute-cheap operators, especially if they enable high data
% % reduction, (3) identify low-utility operators with high compute cost but low
% % data reduction, and reduce the load factor on such operators.

% %\begin{figure}
% %  \centering
% %    \includegraphics[width=0.5\textwidth]{fig/ExampleControlProxy.png}
% %    \caption{Query dataflow graph with 3 operators}
% %    \label{fig:controlproxy-gen-example}
% %\end{figure}


% \subsubsection{Coordinating Multiple Queries within a Node.}
% \label{sec:query-coordination}

% \mj{We should move this part earlier and clarify how compute budget is decided, given multiple queries. Then say our current focus (within one query).}
% A single \run{} instance is dedicated to a single query, and each runtime
% updates load factors independently for a query. Therefore, 
% when there are multiple queries running on a data source node,
% the queries may never 
% stabilize without a proper coordination. In allocating the entire compute budget to the competing queries, our system currently relies on a popular 
% fair resource allocation policy, i.e., (non-weighted) max-min 
% fairness~\cite{minmax}. Future work includes integrating a more sophisticated resource allocator that improves network transfer reduction across concurrent queries. 
% %takes into account various types of telemetry workloads.
% \todo{Remember to discuss Sonata potentially needing to support thousands of monitoring queries concurrently}

% %\subsection{Data Partitioning on Hot Keys}
% %\label{sec:data-partitioning-hot-keys}
% %
% %\begin{figure}
% %  \centering
% %    \includegraphics[width=2.5in]{fig/data_skew}
% %    \caption{CDF of ToR-pair group sizes. Groups are ranked and appear as quantiles in x-axis for confidentiality.}
% %    \label{fig:data_skew}
% %\end{figure}
% %
% %To show evidence for existence of hot keys in real-world workloads, we calculate group sizes when grouping happens on ToR-to-ToR pair for records in \pingmesh{} trace. Figure~\ref{fig:data_skew} shows the cumulative distribution of the group sizes, with groups ranked by size in the x-axis. Some groups are large: the largest 5\% of groups account for 24.0\% of the total records. This skewness is not surprising: the network monitoring system probes servers between ToRs
% %requiring high connectivity and low latency more extensively. Applying reduction on the records of hot keys is more effective as it maintains a smaller hash table with fewer keys (in case of hash-based grouping~\cite{streamboxhbm}), leading to lower costs for key lookups and subsequent network transfers. \emph{Data skewness} on hot keys, i.e., keys with many
% %records~\cite{keyskew}, is in fact a very natural property for other telemetry scenarios too. For instance, in GPU-based DNN cluster~\cite{philly}, we found a number of servers are equipped with 8 GPUs. When we monitor HW counters, GPU metrics in these
% %servers will bring out 8x more records than other system-wise metrics such as host memory usage. Hence, in the face of data skewness, we would run reduction operations for records in hot keys first during data partitioning.
% %
% %%When a grouping operation exists in a query (as shown in
% %%Figure~\ref{fig:edge-controller}), the nature of data distribution across the
% %%grouping keys allows us to prioritize processing of certain groups over
% %%others. Specifically, if the distribution is skewed such that a higher
% %%fraction of incoming records corresponds to a small group of keys, then we
% %%refer to them as hot keys. We prioritize the processing of hot keys for each
% %%grouping operator on the \client{}, as performing reduce operation on
% %%these keys enables larger data reduction benefits over processing of cold
% %%keys on the \client{}.
% %
% %%Depending on the skewed distribution of keys in the input stream to a
% %%grouping operator on a data source node, we can define a set of hot keys.
% %%For example, if service telemetry from an application running on an
% %%\client{} node indicates anomalous behavior, then the records on that
% %%particular node would be skewed towards the corresponding error code (i.e.
% %%error code can be a non-zero value such as 2). Other nodes may be in normal
% %%operation mode, with the error code of 0 being the hot key.
% %If there is a considerable skewness on data distribution across keys, we
% %prioritize the processing of hot keys for each grouping operator.
% %The reason is that
% %reduction, a typical operation following grouping, on these keys
% %maintains a smaller state over reduction on cold keys: e.g., for each
% %group, reduction using an average aggregator can be computed incrementally on
% %stream records by keeping two variables, sum and count~\cite{trill}.
% %This hot key-based reduction brings out a smaller state that must be transferred
% %over the network to stream processor, providing a smaller network transfer cost.
% %
% %Hot keys are distinct across data source nodes, so detected and leveraged
% %independently for each node. \ours{} does hot key-based partitioning
% %using the steps described below:
% %% \mj{shorten based on the final implementation}
% %
% %% There are two types of hot keys:
% %% \begin{itemize}
% %%     \item Local hot keys: Depending on the query, data on each \client{} operator can have its own set of hot and cold keys. For example, if service telemetry from an application running on an \client{} node indicates anomalous behavior, then the records on that particular node would be skewed towards the corresponding error code.
% %%     \item Global hot keys: The distribution of keys for grouping done on the \server{} side can be skewed as observed over records sent from multiple \client{} nodes. Note that the global view of hot keys on \server{} side, may not always be consistent with local view of hot keys on \client{} nodes.
% %% \end{itemize}
% %% We focus on detecting local hot keys in this section.
% %
% %\Paragraph{1. Profiling for key distribution.} We first need to obtain the data
% %distribution of keys to identify hot keys in the input stream. So we obtain a
% %sample of the telemetry data collected across \client{} nodes and
% %analyze the dataset offline. We calculate the occurrence count for each
% %unique key. We also obtain a total count of records seen in each epoch. This
% %is used to compute occurrence probability or frequency distribution for each
% %key in an epoch. To avoid transient effects in individual epochs we would
% %like to collect key statistics across a large number of epochs. However, we
% %also want to avoid collecting stale statistics from older epochs in the
% %dataset. So we maintain above statistics averaged over the most recent $n$
% %epochs (e.g. $n=10$).
% %
% %Key distributions can change over time. To keep our statistics updated
% %without additional runtime overhead, we adopt a simple policy to sample the
% %telemetry data periodically at large enough time intervals (e.g., every 1000
% %epochs). And then rerun our profiling analysis to obtain updated key
% %distribution statistics.
% %
% %% These statistics are updated for each newly arrived record per \client{} node.
% %% To avoid unexpected transient effects in individual epochs, we maintain above statistics averaged over the recent K epochs. (e.g. K=5).
% %%The counts are weighted in exponentially decreasing manner
% %%going back in time. So recent windows are weighted higher than older ones.
% %%When a record arrives at a control proxy, the likelihood of sending the
% %%record to the operator is proportional to occurrence probability of the key
% %%in that record. \atulH{Include the technique to update load factor for
% %%groupby operator, which accounts for the hot keys}
% %% \textcolor{red}{TODO: update section so we do expensive local hot key detection only when it becomes inconsistent with global hot key view}
% %
% %\Paragraph{2. Identifying hot keys.} Given $N_i$ (number of incoming records)
% %and $p_i$ (load factor corresponding to the grouping) for an operator $i$,
% %the number of records to process by a grouping operation is decided. Since
% %$N_i$ and $p_i$ change every epoch, the number of keys that can be processed
% %by the operator can also vary. However, it is expensive to store and manage
% %statistics for each key and apply data partitioning on a per-key basis. So
% %instead, we sort the grouping keys based on their frequency of occurrence and
% %categorize the top $K$\% of the keys (e.g. K=10) as hot keys. Each
% %\client{} node only maintains a list of these hot keys.
% %
% %% if we individualize each key and operate data partitioning on per-key basis, the cost related to managing will be very high. So, we group keys into a few categories and process records for hottest group first..
% %
% %\Paragraph{3. Applying data partitioning on hot keys.} For each incoming record
% %to grouping operation on \client{} node, we need to determine if the
% %grouping key is a hot key or not. Since the number of hot keys can be large,
% %maintaining them on each \client{} can be expensive. So we use Bloom
% %filters~\cite{bloom-filters}, which are compact, probabilistic data
% %structures that support membership testing by maintaining a fix-sized bitmap,
% %with a tunable small false positive rate and zero false negative rate.
% %\todo{Write about the configured parameters for bloom filter}
% %At runtime,
% %given $N_i$, $p_i$ for operator $i$ and the estimated number of records per
% %hot key in an epoch, we determine the hot keys to execute on \client{}.
% %If we estimate that cold keys can also be processed within the available
% %compute budget on \client{}, it is done with probability $p_i$.
% %
% %% Note that we use data partitioning on hot keys when we observe skewness and show in Section~\ref{sec:evaluation} that the benefit from hot key-based data partitioning offsets the overhead of checking membership for every record.
% %
% %\Paragraph{Hot keys in the wild.}
% %Note that there are largely two types of groupings observed in monitoring
% %queries. i) grouping based on fields that represent configurations for
% %datacenter system components (e.g., network switches or GPUs). Key
% %distribution can change infrequently for such keys as they are affected only
% %when there is a major update in the datacenter architecture, ii) grouping
% %based on fields that represent measurement data (errorcode, network latency).
% %Key distribution can change relatively more frequently for such keys
% %depending on the target monitoring scenario. For instance, if we groupby
% %observed latencies over ranges of values, data distribution is mostly stable
% %because datacenter networks function well most of the time, with high
% %concentration on low latency values. On the other hand, if we groupby
% %errorcode, the records on a particular faulty node could be skewed towards
% %the corresponding error code. Other nodes may be in normal operation mode,
% %with the error code of that mode being the hot key. With the simple profiling
% %policy described above, it's possible we may have outdated hot key
% %information between profiling intervals for frequently changing key
% %distributions. We still reduce the amount of records to transfer to stream
% %processor in this case however, so benefits of data partitioning hold.
% %
% %Note that other works such as~\cite{sonata} also provide the ability to do partial processing of data on query operators deployed on network switches. But their technique of key refinement is limited to certain types of keys (that are hierarchical in nature) and complementary to our hot key based partitioning.
% %
% %\todo{How are the hot keys different from SONATA key refinement and other key
% %distribution related topics like partial key grouping? Also how do we include
% %hot key detection in optimization formulation?}{}



==> backup/PaperBackup.tex <==
% % \documentclass[conference]{IEEEtran}
% % \IEEEoverridecommandlockouts
% % % The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
% % \usepackage{cite}
% % \usepackage{amsmath,amssymb,amsfonts}
% % \usepackage{algorithmic}
% % \usepackage{graphicx}
% % \usepackage{textcomp}
% % \usepackage{xcolor}
% % \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
% %     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
% % \begin{document}

% % \title{Jarvis: Large-scale Server Monitoring with\\ Adaptive Near-Data Processing*\\
% % {\footnotesize \textsuperscript{*}Note: Sub-titles are not captured in Xplore and
% % should not be used}
% % % \thanks{Identify applicable funding agency here. If none, delete this.}
% % }

% % \author{\IEEEauthorblockN{1\textsuperscript{st} Atul Sandur}
% % \IEEEauthorblockA{\textit{Computer Science department} \\
% % \textit{University of Illinois at Urbana-Champaign)}\\
% % sandur2@illinois.edu}
% % \and
% % \IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
% % \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% % \textit{name of organization (of Aff.)}\\
% % City, Country \\
% % email address or ORCID}
% % \and
% % \IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
% % \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% % \textit{name of organization (of Aff.)}\\
% % City, Country \\
% % email address or ORCID}
% % \and
% % \IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
% % \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% % \textit{name of organization (of Aff.)}\\
% % City, Country \\
% % email address or ORCID}
% % \and
% % \IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
% % \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% % \textit{name of organization (of Aff.)}\\
% % City, Country \\
% % email address or ORCID}
% % \and
% % \IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
% % \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% % \textit{name of organization (of Aff.)}\\
% % City, Country \\
% % email address or ORCID}
% % }


% % VLDB template version of 2020-08-03 enhances the ACM template, version 1.7.0:
% % https://www.acm.org/publications/proceedings-template
% % The ACM Latex guide provides further information about the ACM template

% \documentclass[sigconf, nonacm]{acmart}
% \input{header}
% % \linespread{0.95}

% %% The following content must be adapted for the final version
% % paper-specific
% \newcommand\vldbdoi{XX.XX/XXX.XX}
% \newcommand\vldbpages{XXX-XXX}
% % issue-specific
% \newcommand\vldbvolume{14}
% \newcommand\vldbissue{1}
% \newcommand\vldbyear{2020}
% % should be fine as it is
% \newcommand\vldbauthors{\authors}
% \newcommand\vldbtitle{\shorttitle}
% % leave empty if no availability url should be set
% \newcommand\vldbavailabilityurl{URL_TO_YOUR_ARTIFACTS}
% % whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
% \newcommand\vldbpagestyle{plain}

% \begin{document}
% %-------------------------------------------------------------------------------

% %don't want date printed
% \date{}

% % make title bold and 14 pt font (Latex default is non-bold, 16 pt)
% \title{Jarvis: Large-scale Server Monitoring with\\ Adaptive Near-Data Processing}

% %%
% %% The "author" command and its associated commands are used to define the authors and their affiliations.
% \author[1]{Atul Sandur}
% \affiliation{%
%   \institution{UIUC}
%   %\city{Champaign}
%   %\state{Illinois}
%   %\country{USA}
% }
% \email{sandur2@illinois.edu}

% \author[2]{ChanHo Park}
% \affiliation{%
%   \institution{UNIST}
%   %\city{Ulsan}
%   %\country{South Korea}
% }
% \email{pch8286@unist.ac.kr}

% \author[3]{Stavros Volos}
% \affiliation{%
%   \institution{Microsoft Research}
%   %\city{Cambridge}
%   %\country{United Kingdom}
% }
% \email{svolos@microsoft.com}

% \author[4]{Gul Agha}
% \affiliation{%
%   \institution{UIUC}
%   %\city{Champaign}
%   %\state{Illinois}
%   %\country{USA}
% }
% \email{agha@illinois.edu}

% \author[5]{Myeongjae Jeon}
% \affiliation{%
%   \institution{UNIST}
%   %\city{Ulsan}
%   %\country{South Korea}
% }
% \email{mjjeon@unist.ac.kr}

% %-------------------------------------------------------------------------------
% \input{abstract}
% \maketitle
% %%% do not modify the following VLDB block %%
% %%% VLDB block start %%%
% \pagestyle{\vldbpagestyle}
% \begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
% \vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
% \href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
% \endgroup
% \begingroup
% \renewcommand\thefootnote{}\footnote{\noindent
% This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
% \raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
% ISSN 2150-8097. \\
% \href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
% }\addtocounter{footnote}{-1}\endgroup
% %%% VLDB block end %%%

% %%% do not modify the following VLDB block %%
% %%% VLDB block start %%%
% \ifdefempty{\vldbavailabilityurl}{}{
% \vspace{.3cm}
% \begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
% The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
% \endgroup
% }
% %%% VLDB block end %%%
% % \balance
% \input{introduction}
% \input{background}
% \input{motivation}
% \input{design}
% \input{implementation}
% \input{evaluation}
% \input{related}
% \input{conclusion}
% \input{appendices}

% % %--------
% % \section*{Availability}
% % %-------------------------------------------------------------------------------

% % USENIX program committees give extra points to submissions that are backed by artifacts that are publicly available. If you made your code or data available, it's worth mentioning this fact in a dedicated section.

% % %-------------------------------------------------------------------------------
% \bibliographystyle{ACM-Reference-Format}
% % \bibliography{\jobname}
% \bibliography{references}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{document}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  LocalWords:  endnotes includegraphics fread ptr nobj noindent
% %%  LocalWords:  pdflatex acks


==> backup/background_motivation_backup.tex <==
\section{Background \& Motivation}
%\vspace{-0.15cm}
In this section, we describe the monitoring system targeted by our work. We showcase challenges in building efficient large-scale monitoring systems and uncover insights for designing such systems by characterizing the resource usage of query operators for a real-world enterprise workload.

\subsection{Monitoring System}
Although numerous useful scenarios correspond to large-scale server monitoring~\cite{helios,deepview,fingerprint}, here we describe two scenarios that guide the design of \ours{}:

\begin{myitemize}
\item \textit{Scenario 1:} Network team deploys Pingmesh~\cite{pingmesh} agents on datacenter nodes to collect  latency data between server pairs. An internal web search team uses Pingmesh to monitor network health of their latency-sensitive service and generate an alert if median probe latency of nodes hosting their service exceeds a threshold as determined by the search service SLA.
 
\item \textit{Scenario 2:} A log processing system, Helios~\cite{helios}, enables live debugging of storage analytics services such as Cosmos~\cite{cosmos}. A bug in cluster resource manager leads to service resources being under-provisioned. To temporarily mitigate performance degradation, several TBs of log streams~\cite{helios} are processed quickly to identify impacted tenants. Their latency and CPU/memory utilization data are queried to predict resource needs and make scaling decisions.
\end{myitemize}

Processing in these scenarios requires a diverse set of operations. The first scenario requires processing of periodically generated metrics composed of structured numerical data; queries consist of common operators specific to numerical data, such as filtering and aggregation. On the contrary, the second scenario requires processing of aperiodically generated logs composed of unstructured strings; queries consist of string processing operators, such as parsing, splitting, and search. 

%Moreover, resource usage for these operators is diverse, varies significantly, and  depends on the operator logic and the input data. We consider a common set of operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. 
Moreover, these operators are computationally different and their costs are highly dynamic depending on the input data. In this paper, we mainly consider a common set of operators, including  Filter(F), Grouping(G), Reduction(R), Join(J), Project(P) and Map(M)~\cite{streamboxhbm,trill,flink}. Filter (stateless operator) drops uninteresting records by applying the predicates on each record and typically requires little amount of compute resource. Grouping (stateful operator) organizes records by key fields, and hence requires key lookups in hash tables. Join (stateful operator) joins an input stream with a static table on \client{}, which typically requires building a hash table over the static table followed by key lookups for the input stream.%\footnote{Due to limitations in \client{}-side execution discussed in Section~\ref{sec:jarvis}, we do not consider other complex join operators.} 
Both grouping and join operators can be quite expensive due to the irregular compute patterns of hash table lookups. Their cost highly depends on the hash table size, which depends on the group count and the static table size, respectively. Map operator performs user-defined transformations on the input (e.g., parsing and splitting text logs) and its cost depends on the transformation logic. We present a quantitative analysis of resource usage characteristics of these operators in~\todo{cite}. 

\Paragraph{Illustrative example.} For the remaining section, we consider a real-world query on Microsoft's \pingmesh{} trace to highlight challenges in designing large-scale monitoring systems. \pingmesh{} measures network latency for server pairs across the datacenter, by requiring that each server send probe messages to its peer servers in the datacenter. Each probe message generates a 86B record that includes timestamp (8B), source IP address (4B), source cluster ID (4B), destination IP address (4B), destination cluster ID (4B), round trip time in microseconds (us) (4B), and error code (4B). %The round trip time is in microseconds.

\begin{figure}[t]
  \centering
    \includegraphics[width=3.3in]{fig/pipeline_tor}
    \caption{DAG of stream operations for the query in Listing~\ref{lst:motivating-query}.}
    \label{fig:pipeline_tor}
    \vspace{-0.4cm}
\end{figure}

This rich set of record fields allows exhaustive analyses, such as zoom-in/out latency probes by grouping them across datacenter network hierarchy to identify cluster-, ToR-, spine switch-, and server-level issues  ~\cite{tersecades, pingmesh}. Listing~\ref{lst:motivating-query} describes the implementation of a real-world \pingmesh{} query. The query is written in a declarative programming model used by popular stream engines, such as Flink~\cite{flink} and Spark Streaming~\cite{sparkstreaming}, which express a query using dataflow operations. 

\lstset{
	%language=C++,
	%basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	xleftmargin=1.0ex,
	framexleftmargin=1.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:correct-spi,
	%belowskip=-1.0 \baselineskip
	}


\begin{lstlisting}[caption={A temporal query for server-to-server latency probing in every 10-second fixed-size window.}, label={lst:motivating-query}]
/* 1. create a pipeline of operators */
query = Stream
.Window(10_SECONDS)
.Filter(e => e.errorCode == 0)
.GroupApply((e.srcIp, e.dstIp))
.Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
/* 2. Execute the pipeline */
Runner r( /* config info */ );
r.run(query);
\end{lstlisting}


Each monitoring query can be represented as a directed acyclic graph (DAG) $G = (V,E)$. In a DAG, the vertices V denote stream operations which transform their input records and emit output records to downstream operation, and the edges $E$ denote dataflow dependencies between operations. Subsequently, in Figure~\ref{fig:pipeline_tor}, we show a simple DAG of how data flows between operations for the query in Listing~\ref{lst:motivating-query}.


\subsection{A Case for Adaptive Partitioning in Query Engines}
\Paragraph{Hierarchical Query Engines.} Physical resources involved in the query execution can be seen as a tree structure as shown in Figure~\ref{fig:arch-monitoring-scale}(b), where leaf nodes represent the \client{}s. In each leaf node, fixed amount of compute resources are allocated to facilitate monitoring queries. Such allocation can be done by provisioning a container to isolate the monitoring resources (e.g. 1 core and 1 GB RAM) from foreground services. Each \client{} can send data to its parent \server{} node (i.e., intermediate node) and leverage its compute resources for query processing. The intermediate nodes send data to the root \server{} node which completes the query before outputting final result.

\Paragraph{Query Partitioning.} Real-world monitoring scenarios exhibit \textit{high volume}. Logs collected from applications can generate up to 971 Gbps~\cite{chi}. Other systems~\cite{gandalf,m3} process up to tens of TB data per day or millions of events every second per monitoring task, straining compute, memory, and network capacities of the monitoring system. We corroborate these findings by quantifying the volume of data transferred over the network in the \pingmesh{} scenario. Assuming that a datacenter consists of 200K servers and each server probes 20K other servers with a probing interval of 5 seconds ~\cite{pingmesh}, the data generation rate is estimated to be 512.6~Gbps. Transferring such high volumes of data may result in network bottlenecks and incur high deployment cost in the \server{}.  

Query partitioning can alleviate network bottlenecks and reduce deployment cost by leveraging available compute resources at \client{} to offload a subset of the query's execution. Given a query instance with $M$ operations, a partitioning plan identifies operations that can execute locally on each \client{} and those that require remote execution on the \server{}. We define a boundary operator $b_i$ for the $i^{th}$ \client{} to indicate that operators prior to $b_i$ in the topological order are executed on \client{} and those after $b_i$ are executed remotely. To illustrate, consider a topologically sorted list of $M$ operators from the query graph $G$ following dataflow dependencies of the query. For a \client{} $i$ with $M=4$ operators, $b_i=3$ implies that the first three operators execute on \client{} and the last operator executes remotely.

\Paragraph{Adaptive Query Partitioning.} Resource conditions can change dramatically across \client{}s and time due to high variability in the generation of monitoring data \cite{chi,helios} affecting the effectiveness of a query partitioning plan.

In our running example, we observe that data source nodes generate highly variable data rates and distributions:
\begin{myitemize}
\item A subset of servers probes a larger set of peers to cover a wider network range on behalf of other servers in the same ToR switch~\cite{pingmesh}. We measure data rates of network probe messages generated by individual \client{}s, illustrated in  Figure~\ref{fig:data-gen-rate}. The data rates are normalized to the highest one observed among \client{} nodes. Data generation rates exhibit high variability, with 58\% of nodes generating 50\% or lower of the highest data rate we observe.
\item When a subset of servers are being over-loaded, latency profiles become more variable~\cite{rubik, pegasus}, and hence each data source node will generate a unique data footprint, which is quite different than the average data source node, which does not encounter any abnormality.
\end{myitemize}

Variability in data complicates resource usage characteristics of query operators during pipeline execution. Declarative operators in a pipeline execute in sequence as shown in Figure~\ref{fig:pipeline_tor}. Resource demand for an operator is affected by its incoming data rate after executing all preceding operators. In our example, F operator leads to the first data volume reduction from the input stream. Since erroneous, insignificant records are not dominant, the operator happens to drop only a small fraction of records. A majority of records are then to be processed by G+R operator, increasing compute cost for the query. However, if we were to toggle the filtering predicates to perform a zoom-in analysis on a small subset of erroneous data, there would be a high degree of data reduction in F operator, thereby lowering resource usage of the G+R operator.

When resource conditions change on a \client{} node, a new partitioning plan needs to be identified so that its compute demands meet available resource budget. To initiate refinement, \client{}s periodically inject \emph{refinement watermarks} into the stream (similar to~\cite{trill}) and they
delimit ordered consecutive \emph{refinement epochs} of records. Refinement watermarks are different from the traditional watermark described in data model. Epoch and watermark refer to refinement epoch and refinement watermark respectively, in the rest of the paper.

\Paragraph{Problem Definition.} Given the network and compute resources available on \server{}, we seek to maximize  the number of \client{}s that can be served. Our optimization goal is to find a partition profile $\textbf{B}$ of boundary operators which minimizes processing load sent to \server{}, subject to local computation not introducing additional delay in the processing of each data stream, compared to remote execution. Formal definition and proof that the problem is NP-hard can be found elsewhere~\todo{cite}.

\begin{figure}[t]
  \centering
    \includegraphics[width=2.4in]{fig/pingmesh_data_rate}
    \caption{Non-uniform data generation rates across \client{} nodes in real network latency monitoring trace.}
    \label{fig:data-gen-rate}
    \vspace{-0.4cm}
\end{figure}

\subsection{Insights for Fast Adaptive Query Partitioning}

We highlight the drawbacks of state-of-the-art approaches in addressing the operator partitioning problem as well as uncover insights for designing \ours{}.

\Paragraph{Drawback 1: Coarse-grained partitioning can significantly
under-subscribe \client{} node resources.} State-of-the-art monitoring systems~\cite{everflow,
sonata, dshark} have explored coarse-grained partitioning strategies---i.e., either all records are processed by an operator or none. To highlight their limitation, we execute the query in
Figure~\ref{fig:pipeline_tor} using 80\% of single core operating at 2.4GHz, to reflect
compute constraints on \client{}. Figure~\ref{fig:data-partition-explain}
shows that because F operator drops only a small portion of input records, it is not
possible to execute the expensive G+R operator on \client{}. This leads to
under-utilization of the available compute resources and generation of network traffic as high as
22.5 Mbps. 

\begin{figure}[t]
\centering

\includegraphics[width=\linewidth]{fig/DataPartitionExplain.pdf}
%\vspace{-0.1in}
\caption{\label{fig:data-partition-explain} Coarse-grained operator vs. fine-grained data partitioning on \client{} with CPU budget of 80\%. G+R requires 80\% CPU to process all the output data from F operator.} %\vspace{-0.2in}
\vspace{-0.4cm}
\end{figure}

On the contrary, fine-grained data-level partitioning allows an operator to process a fraction of its input records on \client{} and drain the rest for remote processing. In our example, G+R can process 83\% of its input 22.5 Mbps, resulting in total network traffic of 9.4 Mbps, which is 2.4x lower than the traffic generated by the coarse-grained partitioning strategy.

\noindent \underline{Insight 1:} \emph{Extending the operator partitioning model to support data-level partitioning significantly improves the utilization of limited compute available on \client{} nodes.}

\Paragraph{Drawback 2: Without fast adaptation, partitioning approaches cannot keep up with highly dynamic resource conditions on \client{}s}
% \Paragraph{Drawback 2: Highly dynamic resource conditions on \client{}s require fast adaptation.} 
The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently per-query available compute resources. Given these dynamics, query planners need to compute and execute a new query partitioning plan in a timely manner, even in seconds.

Optimal partitioning is possible using query performance models and a centralized query planner that leverages global information about available resources but it is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach to partitioning. Heuristics have been investigated 

Prior work relies on centralized query planners that leverage global information about available resources to solve an expensive optimization function~\cite{sonata} and on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Optimal partitioning is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach for partitioning. Other centralized and decentralized query planners have also explored model-free and model-based approaches but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}). %\ours{} investigates a greedy and embarrassingly parallel approach which uses hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}. 
%dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs. 
% \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}

\noindent \underline{Insight 2:} \emph{A greedy and embarrassingly parallel approach which utilizes hybrid performance model-based and model-agnostic techniques can enable fast and fully decentralized query refinement on each \client{}, which is accurate, scalable and automatic.}

\todo{how does greedy help accelerating the decision making? isn't the hybrid nature of the algorith that allows for quick adaptation? this insight does not come across when reading the drawback.}



\Paragraph{Drawback 2: Without fast adaptation, partitioning approaches cannot keep up with highly dynamic resource conditions on \client{}s}
% \Paragraph{Drawback 2: Highly dynamic resource conditions on \client{}s require fast adaptation.} 
The requirement for frequent and dynamic query refinement due to high variability in data generation is more prevalent in practice as \client{}s are shared by multiple in-flight queries. These queries are initiated or terminated by engineers at runtime~\cite{m3}, changing frequently per-query available compute resources. Given these dynamics, query planners need to compute and execute a new query partitioning plan in a timely manner, even in seconds.

Optimal partitioning is possible using a query performance model and a centralized query planner that leverages global information about available resources~\cite{sonata,ds2,optimal-odp} but it is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate a greedy and embarrassingly parallel approach to partitioning. Other performance model-based approaches have been investigated but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}). 

\noindent \underline{Insight 2:} \emph{A greedy and embarrassingly parallel approach utilizing a hybrid performance model-based and model-agnostic technique can enable fast and fully decentralized query refinement on each \client{}, which is accurate, scalable and automatic.}

\todo{how does greedy help accelerating the decision making? isn't the hybrid nature of the algorith that allows for quick adaptation? this insight does not come across when reading the drawback.}

% Prior work relies on centralized query planners that leverage global information about available resources to solve an expensive optimization function~\cite{sonata} and on accurate query performance models~\cite{ds2,optimal-odp} to make optimal partitioning decisions. Optimal partitioning is NP-hard as discussed in Section~\ref{sec:motivation}. We investigate greedy and embarrassingly parallel approach for partitioning. Other centralized and decentralized query planners have also explored model-free and model-based approaches but they do not consider query partitioning under highly variable resource conditions on \client{}s~\cite{turbo,sparrow,sbon,rizou-multiop-placement,subgraph-iso-zhu,decentral-migration-cost,decentral-tree-operator,operator-tree-bokhari,network-aware-decentralized,decentral-migration-cost,decentral-scaling,decentral-placement-only-net} (details in Section~\ref{sec:RelatedWork}). 
%\ours{} investigates a greedy and embarrassingly parallel approach which uses hybrid combination of query performance model-based and model-agnostic techniques to partition queries on each \client{}. 
%dynamics resulting from co-located monitoring queries on \client{}s with high variability in available compute and query resource needs. 
% \ifthenelse{\boolean{Extended}}{It is fully transparent to the user with low cost of migrating to a new refinement.}

A greedy and embarrassingly parallel approach utilizing a hybrid performance model-based and model-agnostic technique can enable fast and fully decentralized query refinement on each \client{}, which is accurate, robust and scalable and automatic.

==> backup/evaluation_bak.tex <==
% \section{EVALUATION}
% \label{sec:evaluation}

% In this section, we evaluate \ours{} with other competing strategies
% using a variety of workloads and queries. 

% % We summarize key results as follows:

% % \begin{myitem}
% %     \item There is no other strategy that achieves better performance than \
% %     \ours{} over a wide range of compute resource constraints.

% %     \item \ours{} outperforms the best operator partitioning strategy. It improves query throughput by XX--XX\% and reduces network transfer by XX--XX\%.

% %     \item \ours{} converges into the stable state in 2--4 epochs
% %     without relying on a centralized query planner.

% %     % \item \ours{} adds a small overhead, degrading query throughput by only
% %     % XX\%.
% % \end{myitem}

% %\begin{myitemize}
% %    \item Given fixed resource conditions on the \client{} node and input data to query operators, does congestion control in Jarvis identify a feasible operator/data partitioning configuration that minimizes network data transfer?
% %    \item Is the convergence time for congestion control reasonably small, when query runtime conditions change- (1) resource availability on the \client{} node and (2) input data to query operators?
% %    \item What is the overhead of Jarvis runtime on the \client{} node?
% %    \item Does Jarvis scale well with increasing number of \client{} nodes?
% %    \item Does Jarvis load balancing minimize compute resource cost on the \server{} side, for input streams with skewed distribution of grouping keys?
% %    % \item $[OPTIONAL]$ What is the overhead of hot key detection (on the \client{} and \server{} side)?
% %\end{myitemize}


% \subsection{Experimental Setup}

% \Paragraph{Machine and cluster setup.} We deploy our \client{}
% instances on Amazon EC2 t2.micro nodes, each with 1~2.40GHz Intel Xeon E5-2676
% core and 1~GB of memory running Ubuntu 16.04. Stream processor
% instances are deployed on Amazon EC2 t2.xlarge nodes, each with 4~2.30GHz
% Intel Xeon E5-2686 cores and 16~GB of memory running Ubuntu 16.04 as well.
% %\client{} nodes are connected to
% %\server{} on a 1~Gbps network bandwidth ethernet link.
% For each \client{} node, Apache MiNiFi runs a custom processor configured to
% execute a single concurrent task. For each \server{} node, Apache NiFi runs
% a custom processor configured to execute five concurrent
% tasks. We use \emph{cpulimit} tool~\cite{cpulimit} to control the available
% compute budget for a query running on a \client{} node and
% \emph{wondershaper}~\cite{wondershaper} to shape the effective bandwidth
% between a single \client{} and the \server{}. \todo{Cloud node has 40 Gbps NIC, based on~\cite{everflow}} 

% We conduct our experiments using a single \client{} node connected to
% a single \server{}.
% % and using a cluster of 1,000 \client{} nodes:
% % Section~\ref{sec:scalability} discusses the cluster experimental results.
% %connected to \server{} running on XX nodes. 
% Each \client{} node
% either replays trace records or generates synthetic records, and pushes
% them into a given computation pipeline in an open loop. The input rate is 
% expressed as megabits per second (Mbps).

% %We use the following testbeds/simulator to evaluate Jarvis at different
% %scales:
% %\begin{itemize}
% %    \item Single \client{} testbed: One \client{} node
% %        connected to a single \server{} instance for central
% %        processing
% %    \item Large scale testbed: 1,000 \client{} nodes connected to
% %        100 \server{} instances for central processing 
% %    % \item Simulator: 250,000 \client{} nodes connected to 1000 \server{} instances
% %\end{itemize}

% \Paragraph{Workload.} We use \textbf{\pingmesh{}} dataset which 
% includes network 
% latency in microseconds (us), with each entry measuring round-trip time (RTT) 
% between any two servers in a large-scale datacenter. We analyzed this dataset to 
% obtain a realistic input data rate on each~\client{} node. As 
% per~\cite{pingmesh}, a server can probe up to 5000 other datacenter servers to 
% obtain 
% latency measurements. With a time interval of 10 seconds per probing and a 
% record size of 86 bytes, we obtain 336 Kbps of input data generated by each source
% agent. 
% However, input data rate depends on the size of the datacenter, and
% a large datacenter today would probe more servers more frequently to include 
% enough data for statistical significance.
% Therefore, we increase the number of target servers to probe by 4x, 
% and get 20,000 servers probed by each source agent.
% And with a time interval of 5 seconds per probing, we obtain approximately 
% 2.72~Mbps input data rate per source agent. Note that these are reasonable 
% estimates for datacenters today. 
% %Large datacenters can comprise of up to 250,000 
% %machines and to monitor and debug complex network problems at scale, higher ping 
% %rates would only provide better coverage for accurate and timely detection of 
% %network faults. 
% Finally, for experimentation purpose, we scale up the input data rate 
% by 10x, giving us an average source rate of 27.2 Mbps per \client{} node, 
% and appropriately scale up CPU budget per query and network bandwidth
% per \client{} node.

% As described in Section~\ref{sec:OP_partitioning_only}, to highlight the benefits 
% of fine-grained partitioning for telemetry systems, we focus on the query 
% described in Listing~\ref{lst:pingmesh-query} for our \pingmesh{} trace, with the 
% filter predicate delivering 15\% filter-out rate
% (i.e., \texttt{e.errorCode == 0}).
% % (ii) \textbf{\philly{}} dataset
% % includes DNN training job scheduler logs and HW utilization logs for DNN GPU
% % cluster. 
% In addition, to show the efficacy of \ours{} over a wide spectrum,
% we generate a synthetic dataset. 
% %Table~\ref{} presents queries used in evaluations along with a summary for query run on each dataset.\atul{remove?}

% %\Paragraph{Data and queries: } We use the following real world datasets to
% %evaluate Jarvis:
% %\begin{itemize}
% %    \item PingMesh dataset includes network latency in microseconds, with
% %        each entry measuring round-trip-time (RTT) between any two servers
% %        in a Microsoft datacenter. \client{} node  \atulH{TODO:
% %        Briefly describe data analysis we did on PingMesh that helped us
% %        pick 3.3 MBps as a reasonable data source generation rate per edge
% %        node}
% %    \item Philly dataset
% %    % \item \atul{NYC Taxis dataset [OPTIONAL Maybe consider if we need another dataset?]} comprised of routes from 10, 000 taxis and limousines in New York in 2017. Each vehicle is equipped with GPS tracking to record data for each route, including: passenger number, charged amount, tip amount, payment type, pickup/dropoff location, etc. In total, each record captures 18 metrics
% %\end{itemize}
% %\atul{Describe queries and add other benchmarks. Note: Rather than having
% %more datasets, have more queries.}

% \Paragraph{Baselines for comparisons.} We compare \ours{} with the following
% baselines: (i) \textbf{\allspconfig{}} runs a query entirely on the
% \server{} node. (ii) \textbf{\allsrcconfig{}} runs a query entirely on
% the \client{} node (i.e., Gigascope~\cite{gigascope}). (iii)
% \textbf{\filtersrcconfig{}} applies static operator partitioning and runs
% only filter operations on the \client{} node
% (i.e., Everflow~\cite{everflow}). (iv) \textbf{\bestopconfig{}} applies 
% dynamic operator partitioning and runs the best part of query obtained from a
% query planner on the \client{} node (i.e., Sonata~\cite{sonata}).

% %\begin{myitemize}
% %    \item \textbf{\allspconfig{}} runs a query entirely on the \server{} node.
% %
% %    \item \textbf{\allsrcconfig{}} runs a query entirely on the \client{} node
% %    (Gigascope~\cite{gigascope}).
% %
% %    \item \textbf{\filtersrcconfig{}} applies static operator partitioning and
% %    runs only filter operations on the \client{} node (Everflow~\cite{everflow}).
% %
% %    \item \textbf{\bestopconfig{}} applies dynamic operator partitioning and
% %    runs the bests part of query obtained from a query planner on the \client{}
% %    node (Sonata~\cite{sonata}).
% %\end{myitemize}

% %For the Jarvis load balancer, we compare it with \server{}-central,
% %which refers to a configuration of 100 t2.xlarge nodes in the large-scale
% %testbed, to run any pending query processing as in~\cite{SparkSQL}.

% \Paragraph{Metrics.} Our performance metric of query execution is the average
% throughput measured in megabit per second (Mbps): we use the same expression
% as that in the input data rate to make it easy to pinpoint the performance
% degradation issue. We also present the amount of network transfer to
% qualitatively compare \ours{} with other query partitioning methods.

% \subsection{Data-driven Study}
% \todo{Rewrite to integrate with evaluation, currently just copy pasted from motivation section}
% For each execution plan, we present query performance in throughput measured in megabit per second (Mbps) and discuss potential causes if performance degradation is observed. We also investigate several operation-specific factors during 
% study, such as filtering rate and data skewness across grouping keys. For this experiment, we use a data source node with 1~2.4~GHz core and 1~GB of memory to represent a small amount of resources assigned for monitoring, and a stream processor node with 4~2.4~GHz cores. For obtaining realistic source generation 
% rates per \client{} node, we analyze a production 
% trace, \textbf{\pingmesh{}}, for latency monitoring (see 
% Section~\ref{sec:evaluation} for details). Based on this analysis, we set input stream rate at 27.2~Mbps (10x scaled up). Below demonstrates the network monitoring query we execute, and Figure~\ref{fig:pipeline_tor} shows how its pipeline is organized.

% \begin{lstlisting}[caption= {Stream query gathering server-level latency statistics for every 10-second fixed-size window},label={lst:pingmesh-query}]
% query = Stream
%   .Window(10_SECONDS)
%   .Filter(e => e.errorCode != 0)
%   .GroupApply(e.dstIP)
%   .Aggregate(c => c.avg(rtt) && c.max(rtt) && c.min(rtt))
% \end{lstlisting}


% \begin{figure}[t]
% \centering
% \subfigure[All-SP]{\includegraphics[width=1.6in]{fig/all_sp}}
% \subfigure[All-Src]{\includegraphics[width=1.6in]{fig/all_src}}
% %\vspace{-0.1in}
% \caption{\label{fig:no-partition} Throughput achieved when query executes without partitioning. Network bandwidth is set to 15~Mbps in All-Src.}
% \end{figure}


% \subsubsection{Executing Query without Partitioning}

% We revisit classical query execution models without any partitioning. First,
% we consider executing the entire query in the stream processor (All-SP),
% where raw stream data must be sent by the data source over the network to be 
% processed. For
% query in Listing~\ref{lst:pingmesh-query}, we initially set filtering to drop 85\% of records and
% grouping to handle 20K groups.

% Figure~\ref{fig:no-partition}(a) presents throughput achieved by All-SP when varying
% available network bandwidth between the single data source and the stream
% processor in the x-axis. Here, a lower bandwidth
% reflects network sharing occurred in the stream processor when it connects to
% more data source nodes. As the figure shows, when bandwidth is abundant
% (50~Mbps) for a data source node, no bottleneck is observed, with the throughput 
% as high as the data
% generation rate. However, as the available network bandwidth decreases, the
% throughput decreases as well due to network gradually being a bottleneck. In
% general, a requirement for All-SP to operate with no performance degradation
% is that the stream processor be able to ingest incoming streams whose volume
% grows with the number of data source nodes. Obviously, this is too costly
% in datacenter-scale monitoring. 

% Next, we examine a query plan executing the same query as above entirely on
% the data source node (All-Src) and sending out only the final output to the 
% stream processor. As
% aforementioned, telemetry tasks commonly produce outputs with significant
% data reduction, so at first glance All-Src seems much more feasible than
% All-SP. However, it turns out that All-Src is effective only when there is
% ample CPU resource to use in the data source node, which is less likely
% as limited source-side resources are almost always shared by a number of
% queries (challenge 2 in Section~\ref{sec:challenges}),
% and as we cannot afford to isolate those queries on separate cores.
% We show throughput of All-Src as a function of
% source-side compute resource available for our query in 
% Figure~\ref{fig:no-partition}(b).
% We restrict network bandwidth
% to be 15 Mbps so that the network becomes a bottleneck without proper network
% traffic reduction from the data source. If we run the entire query on full
% 1 CPU core for sending the query output only, as shown 
% in Figure~\ref{fig:no-partition}(b), no performance degradation is observed
% thanks to considerably reduced network traffic.

% However, as we restrict CPU usage for
% the query, the throughput decreases accordingly due to backpressure building on 
% the data source node, which indicates compute demand
% exceeds the available resource budget.

% \Paragraph{Lesson:} All-SP and All-Src work well if each telemetry task
% is provided with sufficient network and compute resources, respectively. But, once
% telemetry system starts operating on a high fan-in traffic and handles
% multiple telemetry tasks, a task would experience suboptimal
% performance.


% \subsubsection{Executing with Operator Partitioning Alone}
% \label{sec:OP_partitioning_only}

% Now, we apply an operator partitioning configuration wherein the data source
% node is in charge of executing only the first half of the query in
% Figure~\ref{fig:pipeline_tor} (Half-Src). So, for operations in
% Figure~\ref{fig:pipeline_tor}, the data source node executes window and
% filter operators, and offloads the remaining operators to the stream processor. 
% From this operator partitioning, we see that the query throughput
% can reach close to the data generation rate for a wide range of CPU budget. In
% particular, unlike All-SP and All-Src, Half-Src does not exhibit a
% bottleneck in the use of 30\% CPU resource and 15~Mbps network bandwidth. 

% A notable characteristic of the original query is that the filtering
% predicate is so effective that a large number of input records are eliminated
% from filtering. This makes all subsequent operations able to deal with
% computations and data transfers at low costs. Therefore, we test if performance 
% is retained with less effective filtering predicates.
% When we invert the filtering predicate in the query into
% \texttt{e.errorCode == 0}, i.e. filtering to drop only 15\% of records,
% the throughput decreases
% markedly because backpressure starts to build in the pipeline. 
% In this case, a plausible solution would be
% \emph{data partitioning}, which applies filtering on a subset of input
% records.


% When CPU resource remains after filtering, a natural question is if we can
% also execute grouping and reduction to alleviate the pressure on the network more.
% If available CPU resource is not sufficient to process the entire input
% stream for those operations, we should also process it partially with data
% partitioning. 

% \Paragraph{Lesson:} Data partitioning is essential to better exploiting the limited compute resource, and to be effective it must consider operation-specific factors and how they contribute to data reduction.


% \subsection{Partitioning Accuracy on the Data Source}
% An accurate query partitioning configuration would be able to meet the data input 
% rate by fully utilizing available compute resources on \client{} node, 
% thereby minimizing network data transfer and improving query throughput.\\
% % \Paragraph{Throughput}

% We use our single client/server setup, and generate streaming data at 27.2 Mbps as
% explained in previous section. We also set the egress network bandwidth at 15 Mbps
% per query on \client{} node. Note that this rate is reasonably scaled based 
% on our discussions with engineers at a large-scale datacenter operator. They
% mentioned anywhere between 10-100 queries can be running on each \client{} 
% node. If we then assume a 150 Gbps link available in aggregate on the \server{} side, it can be processing data from a reasonably sized cluster (e.g. 100,000 \client{} nodes). This leaves each \client{} node to have 1.5 Mbps of upload rate. We then scale number up by 10x for purpose of experimentation. Compute capacity on each \client{} node is shared by other queries and services, so available compute capacity can range anywhere between  10-100\% CPU depending on other operations running in the shared environment. 

% \begin{figure}
%     % \centering
%     % \begin{minipage}{.25\textwidth}
%     %   \centering
%     %   \includegraphics[width=.25\linewidth]{fig/Placeholder.png}
%     %   \caption{Network data reduction vs. Available CPU time}
%     %   \label{fig:accuracy-data-reduction}
%     % \end{minipage}%
%     % \begin{minipage}{.25\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{fig/PartitionAccuracy1.pdf}
%       \caption{Throughput achieved when query executed with different partitioning strategies. Network bandwidth of \client{} node set to 15 Mbps}
%       \label{fig:accuracy-throughput}
%     % \end{minipage}
% \end{figure}

% Figure~\ref{fig:accuracy-throughput} shows the results of query throughput achieved by different policies, for variable amounts of compute available on the \client{} node.
% Due to limited network bandwidth, All-SP cannot outperform Jarvis even when low compute capacity of 20\% is available on \client{}. Jarvis is able to extract the limited data reduction benefits that the limited CPU provides, to obtain marginal improvement in throughput. At 100\% CPU, Jarvis is able to meet the throughput benefits obtained by All-Src. At its peak, Jarvis is able to provide ~20\% improvement in throughput over existing policies at the 60\% CPU range. Note that this is the throughput gain for a single query. 

% The throughput benefits offered by Half-Src become stabilized when the network becomes a bottleneck for the filtered data on \client{}, while All-Src is able to exploit the additional compute to perform grouping operation on \client{}. For lower compute
% capacity on the \client{}, we observe running group by aggregation entirely on the
% \client{} is too costly. Best-OP decides to move group by aggregation to \server{},
% leaving CPU capacity idling on \client{}. Jarvis is able to exploit this
% compute capacity by exploring fine-grained data partitioning for group by aggregation. 
% % Note
% % that worst case latency per record in the input stream is the size of an epoch.

% % We see that All-\server{} outperforms at the
% % 0\% CPU on \client{} in terms of throughput. All-\client{} outperforms
% % at the 100\%. Overall, OP is better than Filter-\client{} when both
% % All-\server{} and All-\client{} do not perform well.  

% % Compare competing policies for the fixed amount of compute resource.
% % Compute resource is fixed for each measurement, but we compare the policies over different amounts.
% % X-axis has 0\%, 20\%, 40\%, 60\%, 80\%, 100\% CPU resource available. Y-axis shows the throughput that can be achieved within a latency bound.
% % Expected results: All-\server{} outperforms at the 0\%. All-\client{} outperforms at the 100\%. Overall, OP is better than Filter-\client{} when both All-\server{} and All-\client{} do not perform well. There will be points where running GroupByAggr entirely on the \client{} is too costly (and not doing so leaves CPU idling). Jarvis will be good at there. We can also reveal the overhead of Jarvis runtime on the \client{} node by comparing All-\server{} and Jarvis at the 0\%.



% % \Paragraph{Grouping key distribution}
% % Jarvis identifies hot keys on the local node and exploits skewness in the key distribution to provide significant data reductions and associated throughput improvement. Figure~\ref{fig:accuracy-key-distr} compares the data reduction gains for Jarvis and OP, with increasing skewness of a key. We have compute constraint on \client{} node so groupby can only process 60\% of 100000 records in an epoch. We have 40000 unique keys in an epoch. Initially the hot key occurs in 10\% of the epoch. The remaining records equally distributed across other keys. As the fraction of records corresponding to the hot key increases, we expect Jarvis to reduce the data until a single key appears across all records in an epoch. We expect data reduction obtained by OP however, is random and cannot take advantage of key skewness. 


% % \begin{figure}  
% %   \centering
% %     \includegraphics[width=0.15\textwidth]{fig/HotKeyMatPlotlib.pdf}
% %     \caption{Jarvis optimizing grouping based on hot keys}
% %     \label{fig:accuracy-key-distr}
% % \end{figure}

% % \Paragraph{5.2. Degree of key skewness}

% % We change the degree of hot keys from high skewness to no skewness. Jarvis is effective in achieving data reduction by being aware of high skewness and the existence of hot keys. However, when there's no data skewness, Jarvis will do a good job from exploiting data partitioning.
% % \atul{Should we show this for global hot keys?}


% % \Paragraph{2. Data reduction}
% % Repeat 1 and show the amount of data reduction in Y-axis.

% \todo{What about OP with key refinement?}
% \subsection{Runtime adaptation on the \client{}}
% We now evaluate the convergence time for Jarvis congestion control, when changes occur in compute resource availability on \client{} nodes. 
% \Paragraph{Change in available CPU time}
% \begin{figure}  
%   \centering
%     \includegraphics[width=0.5\textwidth]{fig/fig13.pdf}
%     \caption{Reaction time of Jarvis with changing available CPU time \todo{Change Y-axis to CPU available, and show effect of parameters like congestion/idle state thresholds. Keep graphs quantitative. }}
%     \label{fig:compute-adapt}
% \end{figure}
% Compute resource changes for a query can happen at different timescales. During normal resource usage on a node, it is reasonable to say that at smaller timescales, relatively small changes in CPU time occur, while at larger timescales the CPU time change can be large. So we evaluate Jarvis adaptivity under both these conditions. 

% Figure~\ref{fig:compute-adapt} shows the reaction time for Jarvis when \client{}-side CPU changes from 40\% to 10\% available for the query at epoch 2, which is a large change. \ours{} is expected to reconfigure load factors for multiple operators, doing operator partitioning and then data partitioning. Thus is takes 4 epochs to converge after a resource change is detected. Detecting the resource change after it occurs, takes between one to two epochs. 
% For small resource change from 40\% to 30\% which occurs at epoch 8, \ours{} adjusts the boundary operator's load factor, performing only data partitioning and stabilizing within 2 epochs after resource change detection.

% % Focus on Jarvis and show its fast adaptation to the change of the available CPU resource. Show a graph with time progress at X-axis, which change the available CPU resource from 60\% to 80\% (small change) and then from 80\% to 20\% (large change). For the small change, Jarvis will just adjust the operator's probability ($p_e$). For the large change, Jarvis will reconfigure $p_e$ values for all operators.

% \subsection{Hot-key based data partitioning}
% \begin{figure}  
%   \centering
%     \includegraphics[width=0.5\textwidth]{fig/hotkey.pdf}
%     \caption{Groupby operator throughput comparison across load factors, of random strategy with \ours{} which prioritizes hot key processing}
%     \label{fig:key-distr-adapt}
% \end{figure}
% Figure~\ref{fig:key-distr-adapt} shows the throughput benefits obtained by prioritizing hot key based processing over random strategy of choosing input records to process on \client{}. The benefit of hot-key based selection reduces as we increase the load factor value. This is expected because we choose all of the input records for processing at higher load values. 

% % We change key distributions in terms of 1) the number of keys and 2) the keys which are hot. 1) can be caused by zoom-in and zoom-out query execution similar to Sonata? 2) could be reconfiguration of mapping between \client{} nodes and intermediate node (the use case of intermediate node is explained below).
% % Atul: (1) implies change in grouping key CPU cost. We already show adaptivity with CPU cost previously. So discarded that scenario here.  

% % \subsection{Scalability}
% % \label{sec:scalability}

% % We now use the large-scale testbed and simulator to demonstrate the scalability of Jarvis across a large number of \client{} nodes. 
% % \Paragraph{Throughput}
% % \begin{figure}  
% %   \centering
% %     \includegraphics[width=0.15\textwidth]{fig/Placeholder.png}
% %     \caption{Throughput with increasing \client{} nodes}
% %     \label{fig:scale-throughput}
% % \end{figure}
% % We compare the overall query throughput for Jarvis with \server{}-central, to evaluate how Jarvis scales with increasing number of \client{} nodes. Each \client{} node sends data at 3 MBps. Figure~\ref{fig:scale-throughput} shows the overall throughput as \client{} nodes are increased. We expect to see that in \server{}-central, a decline in throughput is observed while the scaling of intermediate aggregation servers with \client{} nodes enables Jarvis to keep up with aggregate source rate, at lower compute cost. This shows resource efficiency of Jarvis and low cost of operating Jarvis-based monitoring. This is due to efficient data reduction and network load balancing mechanism on the \server{} nodes. 
% % \Paragraph{Localized adaptation}
% % Even at large scales, Jarvis is able to quickly adapt to dynamic conditions across one or more of the \client{} nodes. It doesn't rely on a global query partitioner and each \client{} node adapts independently, allowing Jarvis to scale in its adaptivity. 
% % To evaluate this, we change the available CPU resource (from 80\% to 20\%) for a subset of \client{} nodes (ranging from 80\% to 20\% of the \client{} nodes on large-scale testbed). We expect to see that partition adaptation occurs only for the subset of \client{} nodes where CPU resource changed, while other nodes do not perform any adaptation. Each node adapts its own partitioning without relying on any global scheduler. 
% \todo{Need to add section on localized adaptation}

% % Figure~\ref{fig:local-adapt} shows this benefit by measuring average reaction time across \client{} nodes (on Y-axis) for different fractions of \client{} nodes in our large-scale testbed changing available CPU time from 80\% to 20\% (i.e. X-axis contains fractions of 20\%, 40\%, 60\% and 80\% of \client{} nodes). We observe that the average reaction time doesn't change as we increase the number of nodes in which resource availability changes. 
% % \Paragraph{Global hot key locality}
% % \begin{figure}  
% %   \centering
% %     \includegraphics[width=0.15\textwidth]{fig/Placeholder.png}
% %     \caption{Jarvis global hot key locality}
% %     \label{fig:global-hot-key}
% % \end{figure}
% % As we scale up the \client{} nodes, global hot key distributions can change depending on number of \client{} nodes from which records for a key are emitted (e.g. grouping based on error code in PingMesh). We compare the throughput for Jarvis with hot key locality enabled using hot key aggregators in \server{} vs. hot key locality disabled. We expect to see a significant gain in overall query throughput with hot key locality enabled.
% \todo{Do we need to handle global hot keys?}

% % We change key distributions in terms of 2) the keys which are hot. 2) could be reconfiguration of mapping between \client{} nodes and intermediate node (the use case of intermediate node is explained below)

% % \subsection{Overhead}
% % \Paragraph{Runtime overhead on \client{}}
% % In single-\client{} testbed, we evaluate the overhead of running Jarvis runtime alongside the query. To do so, we compare throughput of All-\server{} and Jarvis at the 0\% CPU time available on \client{}. We expect to see the throughput not changing much for Jarvis, compared to All-\server{}. 

% % \Paragraph{Repartitioning overhead}
% % We compare the following: OP, which is solved by ILP focused on operator partitioning only, with Jarvis. We show how fast Jarvis provides a partitioning plan for a given available resource.
% % Expected results: Jarvis takes much shorter time. Close to OP-ILP in terms of performance, but much faster in converging.

% % \mj{end ----.}

% % We also evaluate Jarvis on the following benchmarks: 
% % \textcolor{red}{[TODO]}\\
% % The queries we execute are as follows: \\
% % \textcolor{red}{[TODO]}\\


==> sections/_abstract.tex <==
\renewcommand\abstractname{Abstract}
\begin{abstract}

Rapid detection and mitigation of performance and reliability issues is paramount for  
large-scale online services. 
For real-time detection of these issues,
datacenter operators exploit a \server{} and analyze HW/SW data streams collected from servers hosting the service, referred to as \client{} nodes.
However, operating the \server{} for low detection
latency in the datacenter is challenging as it requires the network transfer of massive telemetry data
and a large amount of compute resources to avoid stream analytics being a bottleneck.

%Stream monitoring systems, employed for real-time 
%detection of such issues, are resource-intensive as they rely on a \server{}---consuming 
%up to thousands of servers---to analyze massive amounts of telemetry data received from servers hosting the service, referred to as \client{} nodes.

We propose \ours{}, a stream monitoring system which employs near-data processing and partitions queries for execution across \client{} nodes and the \server{}. Jarvis addresses two major issues of state-of-the-art monitoring systems.
Unlike conventional coarse-grained operator-level partitioning schemes,
\ours{} processes a subset of the input records on each operator through 
fine-grained \datapart{}, enabling resource-intensive operators to
execute on resource-constrained data source nodes. %In doing so, \ours{} 
%reduces the amount of data transferred to the stream processor over the network as 
%well as the number of servers employed by the stream processor. 
Unlike time-consuming centralized query planners, by exploiting a novel decentralized partitioning algorithm 
%thanks to its decentralized 
% makes fast and fully decentralized near-data query refinement decisions guided by a hybrid approach that combines model-based and model-free heuristics
%nature and its novel hybrid %partitioning algorithm 
that combines model-based and 
model-free heuristics, \ours{} enables quick adaptation to dynamic resource conditions on 
each data source independently. Our evaluation of \ours{} on a diverse set of monitoring 
workloads suggests that \ours{} converges to a stable query partition within a few 
seconds of a dynamic resource change on the \client{}, and handles up to 75\% more data 
source nodes while improving throughput in resource-constrained scenarios by 1.2-4.4$\times$ when compared to state-of-the-art partitioning strategies.


%-------------------------------------------------------------------------------
%Server monitoring pipelines are key to deploying highly available
%datacenter services. Telemetry data is collected from across the stack,
%transferred to a stream processor, and analyzed to quickly detect and
%understand failures, so they can be resolved to restore normal service
%operation. Unfortunately, scaling such an architecture to support large
%number of servers is challenging as it suffers from the network transfer of
%massive volumes of monitoring data while query analysis requires a large
%amount of compute resources.
%
%We propose Jarvis, a monitoring system that pushes queries near the data
%source by partitioning a query across data source and stream processor.
%Jarvis addresses two major issues of state-of-the-art monitoring systems.
%Unlike conventional coarse-grained operator-level partitioning schemes,
%Jarvis employs fine-grained \datapart{} to process only a part of the input
%on each operator, thereby enabling resource-intensive operators to execute
%under resource constraints. Unlike time-consuming and fully centralized
%query planners, Jarvis makes fast and fully decentralized near-data query
%refinement decisions, thereby enabling quick adaptation to dynamic resource
%conditions on each data source. Our evaluation of \ours{} on a diverse set
%of monitoring queries and data suggests that Jarvis converges to a stable
%query partition within a few seconds of a resource change occurring on data
%source, and handles up to 75\% more data source nodes while improving
%throughput in resource-constrained scenarios by 1.2-4.4x when compared to
%state-of-the-art partitioning strategies.

\end{abstract}

\begin{IEEEkeywords}
analytics, stream processing, server monitoring, near-data, edge analytics, query partitioning, query refinement
\end{IEEEkeywords}


==> sections/appendices.tex <==
\begin{appendices}
\section{Compute cost of optimal query partitioning}
\label{sec:appendix-optimal-partitioning}
Consider the hierarchical architecture of resource nodes in Figure~\ref{fig:arch-monitoring-scale} where each node in the tree topology can communicate with its parent node. A query with $M$ operators are to be executed on monitoring stream being generated on \client{}s. Each \client{} has a query instance which can be represented as a computational pipeline of operators as vertices and edges denoting dataflow dependencies. On the \server{} side, a fixed number of compute nodes are provisioned for processing the query on data from all \client{}s. Each \client{} needs to identify operators which need to be executed locally vs. those that require remote execution on parent node. Due to dataflow dependencies, we can $partition$ the query graph at $M+1$ possible locations in the graph i.e. a partition splits the operators into two sets. Operators before the partition point are executed on \client{} and those after the partition are executed remotely. As an example, for a \client{} $i$ with $M=4$ operators, $p_i \epsilon [0,M]$ represents the operator where partition occurs. So $p_i=3$ means first 3 operators execute on \client{} and the last operator executes remotely.  

Compute resources on \server{} are used to process operators sent for remote execution after partitioning. Data transport also incurs a network overhead cost. Our goal is to parallelize query processing between compute resources on \client{} and \server{} nodes, while minimizing the utilization of finite compute and network resources on \server{}. As we increase the number of \client{}s, processing load increases on the system. And the processing load from different \client{}s can result in network/compute bottleneck on \server{}, hurting query processing time. Thus, we cannot independently partition operators for each \client{}, instead joint partitioning decision needs to be made across \client{}s. When the remote resources are saturated, it is more beneficial for the \client{} to execute operators locally to avoid long processing time. 

Let \textbf{p} denote the partitioning profile for a query, where $p_i$ denotes query partition point for $i^{th}$ \client{}. We now define the following query partitioning problem as follows:
\begin{align*}
    & \displaystyle \min_{\textbf{p}} \sum_{i=1}^{N_{d}}\sum_{j=1}^{M} c_j x_{ij}\\
    subject\ to,&\\
    & T_{local}(i,p_{i}) <= T_{remote}(i,p_{i})\ \forall p_{i}>0, i\epsilon[1,N_{d}]
\end{align*}
Here $x_{ij}$ indicates if partition point of $i^{th}$ \client{} is $j$, $c_j$ is the processing cost on \server{} due to partitioning the query on \client{} at $j^{th}$ operator, $T_{local}(i,p_{i})$ computes the local computation time cost for operators 1 to $p_{i}$ on the $i^{th}$ \client{} node and $T_{remote}(i,p_{i})$ denotes the network transmission time cost of intermediate data from $p_{i}^{th}$ operator to its parent node along with computation time cost of executing operators $p_{i}+1$ till $M$ on the parent node. We want to incentivize executing operators on \client{} so the partitioning costs are ordered as $c_1>c_2>,...>c_M$.

Unfortunately, solving the partitioning problem is extremely challenging.  
\begin{theorem}
Query partitioning problem to distribute query operators across \client{} and \server{} nodes, with the objective of maximizing the resource utilization of \client{} nodes without degrading query processing time, is NP-hard. 
\end{theorem}
\begin{proof}
% Following is the definition for NP-hard problem for maximum cardinality bin packing~\cite{max-cardinality-bin-packing,central-placement-hard}: we are given $N$ items with sizes $p_i$ for $i \epsilon [1,N]$, and $M$ bins of capacity $C$, and the objective is to assign maximum number of items to the fixed number of bins without violating capacity constraint. It can be stated as below:

We introduce the generalized assignment problem (GAP)~\cite{gap} which finds a minimum cost assignment of $n$ items to $m$ bins such that each item is assigned to precisely one bin subject to capacity restrictions on the bin. Following is the definition:
\begin{align*}
    &min\ \sum_{i=1}^{m}\sum_{j=1}^{n} c_{ij} x_{ij}\\
    subject\ to,&\\
    &\sum_{i=1}^{m} x_{ij} = 1, j\epsilon\{1,...,n\},\\
    &\sum_{j=1}^{n} w_{ij} x_{ij} \le b_i, i\epsilon\{1,...,m\},\\
    &x_{ij} \epsilon {0,1}, i\epsilon\{1,...,m\}, j\epsilon\{1,...,n\}\\
\end{align*}
where $c_{ij}$ is the cost associated with assigning item $j$ to bin $i$, $w_{ij}$ the claim on the capacity of bin $i$ by item $j$ if it is assigned to bin $i$, $b_i$ the capacity of bin $i$ and $x_{ij}$ a 0-1 variable indicating whether item $j$ is assigned to bin $i$ ($x_{ij}=1$) or not ($x_{ij}=0$). This problem is known to be NP-hard~\cite{gap}.


% \begin{align*}
%     &min\ \sum_{i=1}^{N}\sum_{j=1}^{M} x_{ij}\\
%     subject\ to,&\\
%     &\sum_{i=1}^{N} w_{i}x_{ij} \le C\ \forall\ j\epsilon[1,M],\\
%     &\sum_{j=1}^{M} x_{ij} \le 1\ \forall\ i\epsilon[1,N],\\
%     &x_{ij} \epsilon {0,1}\ \forall\ i\epsilon[1,N], j\epsilon[1,M]\\
% \end{align*}
% This problem is known to be NP-hard~\cite{max-cardinality-bin-packing}. 
A \client{} $n$ can execute operators remotely with partitioning $p_{n}$ while improving query processing time, if and only if resource usage on \server{} due to remaining \client{}s is below a threshold data rate $D_{n}$ i.e. $\displaystyle \sum_{i\epsilon [1,N]\setminus\{n\}:p_i=p_n} d_i(p_i) < D_{n}$. Here, $d_i(p_i)$ is a function that provides rate of data leaving \client{} $i$ given the partitioning $p_i$ and $D_n$ is the threshold data rate for all the remaining nodes with partitioning $p_n$ so that \client{} $n$ with $p_n$ has enough resources to execute operators remotely. We use the data rate as a measure for the network and compute overhead on the \server{}. Based on this, we transform generalized assignment problem to a special case of our problem of configuring minimum number of \client{}s to execute operators remotely. We can regard the items and bins in GAP as the \client{} nodes and possible partitioning values i.e. possible values in \textbf{p} in our problem, respectively. Then the weight of an item $n$ assigned to bin $m$ is $w_{mn}=d_n(p_n)$ where $m=p_n$, capacity constraint of each bin $b_m=D_{n} + d_n(p_n)$ and cost of each assignment $c_{mn}=c_{p_n}$. Here, $c_{n1}>...>c_{nM}$. By this, we can ensure that as long as \client{} $n$ on its assigned partition $p_n$ is able to improve processing time compared to executing the query locally, total size of items assigned to bin $p_n$ will not violate capacity constraint $b_{p_n}$. This is because $\displaystyle \sum_{i\epsilon [1,N]\setminus\{n\}:p_i=p_n} d_i(p_i) < D_{n}$ which implies $\sum_{j=1}^{n} w_{nj} x_{nj}=\displaystyle \sum_{i\epsilon [1,N]\setminus\{n\}:p_i=p_n} d_i(p_i) + d_n(p_n) < b_{p_n}$.

Therefore, if we have an algorithm that can minimize the number of operators sent to the \server{} without sacrificing processing time, then we can also obtain optimal solution to GAP. Since GAP is NP-hard, our problem is also NP-hard. 
\end{proof}

The key idea of the proof is that GAP can be reduced to a special case of our query partitioning problem. We note that previous works have also established the hardness of optimal query partitioning in other related domains~\cite{central-placement-hard,placement-scheduling-in-mec-arch}. In this paper, we investigate a greedy heuristic approach which is embarrassingly parallel, for making partitioning decisions. We enable the potential latency overhead resulting from our greedy solution to be bound by an upper limit, by configuring the processing duration or epoch for making partitioning decisions. Our approach is implemented in a fully decentralized manner to ensure high scalability of our partitioning system. 

% \begin{definition}[Remote friendly]
% Given a query with partitioning profile \textbf{p} where $p_i$ denotes query partition point for $i^{th}$ data source, partitioning $p_i$ for \client{} $i$ which uses remote resources (i.e. $p_i>0$) is beneficial as it does not affect the 
% \end{definition}

% Each query operator on a \client{} node can be running on \client{}, or any of the $H$ parent nodes going back to the root node. Our goal for placement is to reduce network data transfer between each node and its parent in the resource tree. We can do this by executing query operators close to \client{} which reduce the output data size. But we have a finite budget on each resource node. So we need to execute query operators within available budget on each node going up the tree


% Consider the hierarchical architecture of resource nodes in Figure~\ref{fig:arch-monitoring-scale} where each node in the tree topology can communicate with its parent node. A query set of $N_q$ queries are to be executed on data streams being generated on \client{}s. with $M$ operators running on each \client{} node's data stream. Query operators need to be placed between \client{} and its parent \server{} nodes, with the goal to minimize network transfer cost between nodes. Each query operator on a \client{} node can be running on \client{}, or any of the $H$ parent nodes going back to the root node. Our goal for placement is to reduce network data transfer between each node and its parent in the resource tree. We can do this by executing query operators close to \client{} which reduce the output data size. But we have a finite budget on each resource node. So we need to execute query operators within available budget on each node going up the tree.

% \begin{theorem}
% Optimal query planning to distribute query operators across resource nodes in hierarchical monitoring pipelines shown in Figure~\ref{fig:arch-monitoring-scale} with the objective of minimizing network transfer costs between nodes, is NP-hard. 
% \end{theorem}
% \begin{proof}

% Let's represent the query graph of each of $N_d$ \client{}s $G_i=(V_i,E_i) \forall i \epsilon [1,N_d]$. We then have a union of all the disjoint operator graphs as $G=(V,E)$ where $V=\bigcup\limits_{i=1}^{N_d} V_{i}$ and $E=\bigcup\limits_{i=1}^{N_d} E_{i}$. Let's denote $D={d_i | i \epsilon {0,|V|}, d_i \ge 0}$, where $d_i$ denotes output data size of query operator $i$ upon processing an epoch. Let $X=\{x_{ih} | x_{ih} \epsilon \{0,1\},\\ i \epsilon [0,|V|], h \epsilon [0,H]\}$ where $x_{ih}$ indicates if query operator $i$ is boundary operator on a node at height $h$ in the resource tree i.e. whether it is the final operator on the node sending output over network to its parent node. Let $Y=\{y_{ih} | x_{ih} \epsilon \{0,1\}, i \epsilon [0,|V|], h \epsilon [0,H]\}$ where $y_{ih}$ indicates if query operator $i$ is placed on a node at height $h$ in the resource tree. We consider the following optimization problem to solve for placement:
% \begin{align*}
%     & \displaystyle \min_{X} \sum_{j=0}^{H}\sum_{i=0}^{|V|} x_{ij} c_{ij}\\
%     subject\ to,&\\
%     &\sum_{i=0}^{|V|} x_{ij} w_{ij} \le C_{j} \forall j \epsilon [0,H]
% \end{align*}


% $u_{ij}=d_i+c_{ij}$ is the combination of data network transfer cost and utilization cost to the bin $j$. This is the utilization penalty for using up the network and compute resources. MR-GAP allows both compute and network resource cost to be bounded. Note that in order to ensure dataflow dependencies are not violated, we need to check each feasible solution to ensure it is not violating the dependencies. And that is quadratic in number of operators. Or the dataflow dependencies are not violated, if the   

% %https://www.cs.cmu.edu/~xia/resources/Documents/grandl_sigcomm14.pdf
% %https://www.sciencedirect.com/science/article/pii/S1383762120302174?dgcid=rss_sd_all


% Cost $c_{ij}$ is proportional to the value of $j$. The optimization is incentivizing the execution of operators closer to data source, within the available compute budget. $w_{ij}$ is used to model the compute cost of executing an operator $i$ at a given tree height $j$, modeling the different capacities of nodes provisioned at the different tree heights.  



% For our problem, we want to minimize the network transfer and thereby provisioned compute cost for processing data on \server{}s. This can be done by maximizing utilization of compute resources available closer to data source. However, resources at each level are limited. And the execution of a query operator at a given tree height depends on resource needs of operator $o_{i} \epsilon V$ and is executed on its parent level only if $\sum\nolimits_{j \epsilon V\textbackslash \{o_{i}\}} x_{jl} w_{jl} > T_l$ for a given level $l$. On \client{}s, joint placement needs to be done for all the queries on each node. For intermediate \server{}s, joint placement needs to be done for operators from multiple \client{}s in lower level. Based on this, we can transform the generalized assignment problem to our query planning problem as follows. We can regard jobs and agents in generalized assignment as query operators and levels in our problem, respectively. Then the cost of each job $i$ placed on layer $j$ can be given as $c_{ij}=w_{ij}$ and the capacity of nodes in layer $l$ as $C_{l}=T_{l}+w_{il}$. By this we can ensure that as long as operator at level $l$ is within a threshold given all the other operators executing at that level, it will not violate the capacity threshold $C_{l}$. This is because $\sum\nolimits_{j \epsilon V\textbackslash \{o_{i}\}} x_{jl} w_{jl} <= T_l$ which implies that $\sum_{j=1}^{n} w_{ij}x_{ij}=\sum\nolimits_{j \epsilon V\textbackslash \{o_{i}\}} x_{jl} w_{jl} + w_{il} \le C_{l}$. 


% There are dataflow dependencies between query operators. So the number of placements to consider is ${M+H-1 \choose H-1}$. This is because each configuration of operators distributed across resource nodes can be represented by a sequence of resource nodes and operators placed adjacent to each other. And number of placements involves choosing $H-1$ positions for resource nodes from a total of $M+H-1$ positions. 


    
% We now consider a graph $G=(V,E)$ where $V$ represents the items to be added to bins in the well known bin packing problem~\cite{binpacking} and $E$ represents the dataflow dependencies between items, enforcing the precedence constraints for placing them into bins in order of increasing bin cardinality. Following is the formal definition of variable size bin packing problem with precedence constraints~\cite{variable-bin-packing,bin-packing-precedence}: 
% \begin{align*}
%     &min\ \sum_{i=1}^{m} f_i y_i\\
%     subject\ to,&\\
%     &\sum_{j=1}^{n} w_jx_{ij} \le C_{i}y_{i}, i\epsilon[1,m],\\
%     &\sum_{i=1}^{m} x_{ij} = 1, j\epsilon[1,n],\\
%     &x_{ij} \le \sum_{h=1}^{i-1}x_{hj}, i\epsilon[1,m], (j,k) \epsilon E\\
%     &y_{i} \epsilon {0,1}, i\epsilon[1,m]\\
%     &x_{ij} \epsilon {0,1}, i\epsilon[1,m], j\epsilon[1,n]\\
% \end{align*}
% Bin-packing with precedence constraints is NP-hard so the variable bin sizes also is NP-hard, since identical bin sizes is a special case of the variable bin size version. To map the bin packing to our placement problem, we consider each resource node in the resource graph to be a bin. The resource nodes are numbered starting from the nodes at the lowest height i.e. leaf nodes. Then we assign incremental counts to each node encountered as we traverse up the tree. And each operator is an item. Each operator has its own compute cost, and it is mapped to a resource node. A feasible mapping is one which does not violate the  
% represented by $f_p(M,H)$ where $f_p$ is number of possible placements and is a function of number of query operators and height of the tree. For a single \client{}, following recursive definition is used to compute $f_p$:
% \begin{align*}
%     & f_p(M,H)=\sum_{i=0}^M f_p(i,H-1) \\
%     & with\ base\ case f_p(0,j)=1 \forall j \geq 0 \\
%     & and\ f_p(j,1)=1 \forall j \geq 0
% \end{align*}
% \end{proof}

% For $N_d$ data sources, $f_p(N_d,M,H)=f_p(1,M,H)^d$ to perform an exhaustive search of all possible placement combinations across \client{}s. Note that given the hierarchical structure, one may not need to do an exhaustive search as different sub-trees in the hierarchy of \server{} nodes are independent of other sub-trees. Thus, we can reduce the search space by

\begin{comment}
\section{Query refinement problem}
\todo{show that the hessian matrix is not positive semi-definite}\\
Proof for original optimization problem with objective in Equation~\ref{eq:optimization-obj} being non-convex:
Consider the objective function for 2 operators i.e. set M=2 to analyze the  behavior of objective. The function becomes:
\begin{align*}
    f_o(p_1,p_2) = N(1 - p_1 + p_1*r_1 - p_1*r_1*p_2)
\end{align*}
The function is continuous and differentiable in the feasible region. So its Hessian matrix is given by:
\todo{For multiple queries, can we show that running StepWiseAdapt independently on each query would still converge across all queries?}

\end{comment}
% \section{Characteristics of Stream Operators}
% \label{sec:characteristics}

% We describe the key characteristics of a few important
% stream operations from the perspective of resource usage and data volume
% reduction as follows:

% \Paragraph{Filtering} is stateless computation that applies filtering predicates
% on a set of fields in the
% input stream to drop uninterested records. It
% does not maintain any state internally, so typically operates in low
% computational cost. It leads to volume reduction from the input stream
% depending on how values of the fields are distributed and how effective
% filtering predicates are on the distribution of the values. Data reduction
% could be enormous if it intends to pinpoints outliers from the input records.

% \Paragraph{Grouping} is a stateful operation that organizes records by key
% fields. In hash-based grouping, which is a
% dominant scheme, records are grouped in a hash table such that the records in
% a group share the same key. It keeps invoking key lookups and moving records,
% making it inefficient if there are a large number of groups maintained in the
% hash table.
% In many pipelines, grouping dominates total execution time~\cite{streamboxhbm}.

% \Paragraph{Reduction} summarizes records by using aggregation functions such
% as averaging, min/max, count, quantiles, etc. It can be computed incrementally
% with a small memory footprint~\cite{trill}, e.g., incrementally computing
% the average requires two variables, sum and count.
% Due to the small memory usage, reduction can effectively reduce
% data volume. Reduction commonly follows grouping to perform
% aggregation functions per group. For groups with many records,
% data reduction ratio is enormous, e.g., computing the average of 1K records results in 99.8\% data reduction.

% \Paragraph{Resource usage characteristics of operators:} To profile query
% operators, we run our experiments on a single \client{} node with 1~2.4~GHz
% core and 1~GB of memory to represent a small amount of resources assigned for
% monitoring. For obtaining realistic source generation rates per \client{}
% node, we analyze a production trace, \textbf{\pingmesh{}}, for latency
% monitoring (see Section~\ref{sec:evaluation} for details). Based on this
% analysis, we set input stream rate at 27.2~Mbps (10x scaled up). We
% synthesized different input data streams and queries involving Filter and
% Groupby operators, to vary the number of groups output by Groupby operator
% and filter-out rates of Filter operator.

% \begin{figure}[t]
% \centering
% \subfigure[Groupby operator]{\includegraphics[width=1.6in]{fig/GroupbyOperatorProfileNew.png}} \label{fig:groupby-profile}
% \subfigure[Join operator]{\includegraphics[width=1.6in]{fig/JoinOperatorProfileNew.png}} \label{fig:filter-and-groupby-profile}
% %\vspace{-0.1in}
% \caption{\label{fig:query-op-profiling} Profiling of query operators}
%  %when discarding low-order digits.}
% %\vspace{-0.2in}
% \end{figure}

% We noted that executing just the Filter operator on \client{} node resulted
% in only up to XX\% of compute time used by the operator. It indicated that
% for a range of filter-out rates, Filter operation is computationally cheap.
% Figure~\ref{fig:query-op-profiling} shows the results of profiling for
% queries involving groupby operator. Figure~\ref{fig:query-op-profiling}(a)
% shows the result of executing just the Groupby operator for different number
% of output groups. It shows that grouping and reduction are highly sensitive
% to the number of output groups and can require anywhere between XX\% to YY\%
% of a core for aggregating the data. We then combined filter predicate with
% groupby operation, as shown in the query in Figure~\ref{fig:pipeline_tor}.
% Figure~\ref{fig:query-op-profiling}(b) shows that resources for grouping
% depends on the input data size, and consequently on the filter-out rate of
% preceding Filter operator. High filter-out rate significantly reduces the
% cost of grouping to XX\%. Thus, depending on the filter-out rate of Filter
% operator, we can accommodate the grouping operation on \client{} nodes. Thus,
% query operators have complex resource usage characteristics, depending on the
% input data distribution at each operator. \todo{Include discussion on join
% operator}

\end{appendices}

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\Paragraph{Scaling to more \client{}s.} \ours{} optimizes a core building block, composed of a single \server{} node and a number of \client{}s as high as 250. As the number of \client{}s increases, \ours{} replicates the core building block, resulting in a set of intermediate \server{} nodes; each node aggregates results obtained from its \client{} nodes. A root node computes the final query result by aggregating results obtained from  intermediate \server{} nodes. As there is no communication between building blocks, the system can scale better with improved scaling of the core building block and availability of upstream network bandwidth between intermediate nodes and the root node. 
% the system's ability to scale is mainly impacted by how well the core building block scales and the available upstream network bandwidth between intermediate nodes and the root node. 

% the system's ability to scale is mainly impacted by the ability of the core building block to scale the scalability is mainly impacted by the scalability of the core building block and the available upstream network bandwidth between intermediate nodes and the root node. %The system can be further optimized by designing each intermediate node to process incoming data to minimize upstream network traffic.

% Stavros: the par. below does not add anything. the key for scalability is that core building blocks do not talk to each other. The system scales similar to how a web search cluster scale.
%Note that as we scale number of \client{} nodes, larger network bandwidth is required to communicate with each \server{} node. Hence, the increased processing in \client{}s reduces network bandwidth required to communicate with the \server{} as well as reduce its computational resource use. \todo{include analysis}

\Paragraph{Fault tolerance.} We are currently extending Jarvis to support fault tolerance. When \client{} fails, no further data is generated from that node. Intermediate state accumulated by the \client{} for the current window can be periodically checkpointed by re-using the drain path from \proxies{}. We are investigating how Flink's mechanism to draw consistent snapshots while guaranteeing exactly-once semantics~\cite{flink-exactly-once1} (and its use in supporting rescaling of stateful operators~\cite{flink-exactly-once}), can be adapted to \ours{}. The \server{} node then identifies \client{} failures (using heartbeats), uses the latest checkpoint for the node, and processes the remaining data for the current window. When the \server{} node fails, its processing state can be checkpointed using existing fault recovery techniques~\cite{seep} so that a new node can restart processing from the last checkpoint. An external data store may need to be updated by \server{} so that \client{}s can read its last successful checkpoint. \Client{}s can then replay records as they contain the upstream query operators. Our setup consists of operators on \server{} nodes which receive multiple input streams from \client{}s. Taking snapshots using the Flink approach requires aligning the snapshot barriers across the \client{}s to guarantee exactly-once semantics. This introduces processing latencies. Exploring mechanisms to address this issue and scale fault tolerance mechanisms for \ours{} consisting of large number of \client{}s is an interesting direction of future work.
% We are looking at this and other design approaches as interesting directions for Jarvis. 
% We are also investigating Flink’s approach to checkpointing and support rescaling of stateful operators with exactly-once guarantees~\cite{flink-exactly-once}. To reassign operator state when rescaling, Flink decomposes operator state into a list of state partitions. State reassignment to the rescaled operators now involve splitting and merging partition lists. 

%An instance of the data store is required only at the level of core building block. %We are also investigating techniques used by previous works such as~\cite{helios} which provide fault tolerance when performing indexing on \client{} nodes.
%  introduces coordination overhead 
% \Paragraph{Internet-of-things (IoT) analytics.} The techniques investigated in \ours{} can be applied to IoT scenarios where billions of devices can sense, communicate, compute and potentially actuate. IoT scenarios exhibit similar constraints as the ones assumed in our work, mainly network bandwidth (e..g, WAN) and limited compute and power resources.

%It will be challenging for traditional stream processing approaches to handle data streams coming from these devices (i.e. \client{}s). Apart from compute cost of query planning, the need for transporting data over wide-area networks can also introduce significant network overhead for coordination~\cite{sol}. Thus, \ours{} agents can be deployed on each \client{} to summarize data on-the-fly and reduce network traffic, enabling complex query processing in a timely manner. It also opens up new challenges for operating \ours{} under resource constrained environments including power. 

% We have provided an analysis of query optimization strategies for a single query. This work in isolation, stands to benefit existing monitoring pipelines wherein the analysis can be used to optimize high-priority/high-scale queries. Most production environments however, have thousands of queries running concurrently, and we are currently extending Jarvis to optimize resource usage globally, across multiple queries on data streams collected from the edge.
